Effortless Data Exploration with zenvisage: An Expressive and Interactive Visual Analytics System

Data visualization is by far the most commonly used mechanism to explore data, especially by novice data analysts and data scientists. And yet, current visual analytics tools are rather limited in their ability to guide data scientists to interesting or desired visualizations: the process of visual data exploration remains cumbersome and time-consuming. We propose zenvisage, a platform for effortlessly visualizing interesting patterns, trends, or insights from large datasets. We describe zenvisage's general purpose visual query language, ZQL ("zee-quel") for specifying the desired visual trend, pattern, or insight - ZQL draws from use-cases in a variety of domains, including biology, mechanical engineering, climate science, and commerce. We formalize the expressiveness of ZQL via a visual exploration algebra, and demonstrate that ZQL is at least as expressive as that algebra. While analysts are free to use ZQL directly, we also expose ZQL via a visual specification interface that we describe in this paper. We then describe our architecture and optimizations, preliminary experiments in supporting and optimizing for ZQL queries in our initial zenvisage prototype, and a user study to evaluate whether data scientists are able to effectively use zenvisage for real applications.

==> challenges.tex <==
%!TEX root=zenvisageql.tex

\section{Future Directions}
\label{sec:challenges}

\subsection{Backend challenges}
\label{subsec:backendchallenges}


\subsection{Frontend specification challenges}
\label{subsec:frontendchallenges}


\subsection{Algorithmic challenges}
\label{subsec:algorithmicchallenges}

==> cover.tex <==
%!TEX root=zenvisageql.tex


\section*{Summary for Revised Paper ``Effortless Data Exploration with zenvisage: An Expressive and Interactive Visual Analytics System''}

We thank the reviewers and meta-reviewer for their insightful 
and very detailed feedback, 
and for giving a chance to address these comments---we have taken this feedback to 
heart in preparing an {\em almost entire
rewrite} of the present paper---{\bf \em each and every section was substantially modified; 
new sophisticated optimized \zq engine,
\fuse,
(using speculation,
parallel, and query combining) along with cache-aware optimization
techniques (and an {\sc NP-Hardness} proof) were developed; 
an extensive performance evaluation on multiple datasets and parameters was added
and a new Upwork user survey was conducted. }
The major changes to each section of the paper include:
\begin{enumerate}
\item {\em A complete rewrite and repositioning of the introduction.}
We rewrote most of the introduction to (i) position our system correctly
as a system that facilitates the search for desired patterns as opposed to a
visualization recommendation system; (ii) describe how \zv solves
some of the articulated problems alluded to in the examples; and (iii) 
describe the challenges in building \zv.

\item {\em A complete rewrite of the query language section.}
To improve readability and make
the paper more self-contained, we rewrote this section to have fewer references
to the technical report. We removed the list of initial examples,
and made this section read less like a user manual, with more intuition 
built in. We also added more details on the task processors (now called
processes),
and clearly defined the interfaces of our exploration functions.
At the same time, we trimmed the description of features that were
not essential to grasp the core contributions of \zq.
% \alkim{Opened up task processors, and made them seem less like a black box,
% both in language section and execution section. Also better defined our
% exploration functions so the interface is more clear}

\item {\em Full-fledged modeling and optimization, 
hardness proof, intelligent optimization schemes, and 
complete rewrite of the query execution section.}
To extend and articulate clearly the novelty of the query optimizer,
we added 
a thorough system modeling and exploration of solution alternatives.
We extended our previous naive graph-based optimization 
technique to a sophisticated technique, called \fuse, reliant on speculation,
caching, and
query combination---a particularly tricky aspect
was that query combination led to non-monotonically increasing gains, so
determining the optimal set of combinations was non-trivial.
%was trading off
%query combination and batching,
%and optimization across task processors (now called processors).
% \alkim{To be fair, our speculation scheme is not really intelligent... we just
% speculation everything. But we do do both batching AND query combining, and the
% decisions for when to combine/batch are based on our complex algorithms that we
% talk aboutl ater.}
We additionally proved that the problem of identifying the optimal set of
combinations 
is {\sc NP-Hard}
and developed an approach to solve the problem. 
In our revision, we now also
spend a lot of room articulating clearly how a \zq query gets
translated, with detailed descriptions of processors and functions $T$ and $D$.
Overall, this section has been entirely rewritten and enhanced.


\item {\em Reimplementation of the \zq Engine.}
  One of the main concerns of the reviewers was the large execution times of \zq
  queries. To address this point, in addition to the optimizations
  mentioned before, we reimplemented the \zq engine to use the much faster
  array-based indexing (as opposed to hash-based indexing) 
  which provided a 50$\times$ speedup in processing time
  (and explained the poor performance earlier). 
  We also showed in the experimental section that if we swap out
  PostgreSQL for a column-store
  database with a large in-memory cache, we can reach interactive response
  times for large datasets.


\item {\em Completely redone performance experiments and rewritten experimental
section.}
We completely redid the performance experiments to better
focus on parameters and aspects that the reviewers suggested.
Specifically, we compared the performance of our query optimizer 
against three algorithms (we had just one baseline in prior work), 
including one which leverages
the standard multi-query optimization within traditional 
database systems---our algorithm performs much better than this baseline.
We compared the algorithms on a range of real-world and 
synthetic datasets, varying parameters,
including the complexity of the queries and the number of
visualizations processed. We also report 
the breakdown of
runtime
%our algorithm
across retrieving visualizations
and processing them. 

\item {\em Entirely new analyst interview section, and 
extensive rewrites to user study section.}
To enable us to judge whether the tasks used in the previous user study
capture the typical tasks used in practice, 
we conducted an entirely new set of user interviews of analysts from Upwork, 
focused on the data exploration tasks from a comprehensive list 
provided by Amar et al.~\cite{amar2005low}. 
Additionally, we rewrote most of the user study section to clearly articulate
the proposed benefits of \zv and focus on 
the utility of \zv and \zq relative to other tools,
as opposed to general usability aspects. 
We specifically revamped and expanded the portion of the study
that compares \zv to other database and data mining tools, along with 
participant quotes and code examples. 


\item {\em Trimmed down system architecture section.}
Since reviewers felt that the paper was busy enough as it is,
so
we have considerably trimmed the system architecture 
%section---especially
%the front-end technologies,
section---only leaving what is absolutely
necessary to support the user study.%, and the experimental sections.

\item {\em Modified related work section.}
We edited this section to emphasize technical differences
as opposed to philosophical differences between \zv and other
systems.
%(these differences were also summarized in the introduction). 
%We briefly also mentioned these differences in the
%introduction.
Also mirroring the positioning of \zv in the introduction,
we focused on comparing with systems that support similar
searches for desired patterns, as opposed to recommendation systems.
For comparison with raw relational databases and \sql,
%Within the related work section, for the relational databases
%comparison,
we additionally added a short experiment to illustrate
how \sql is unsuitable for expressing \zq queries.

\item {\em Removed the \vzalg section.}
Since the \vzalg section could be removed without affecting
the readability or impact of other sections---especially
now that the optimization section has been expanded---we
decided to remove this section entirely, and link to it
via the technical report.


%\tar{Since multiple reviewers were concerned about the timings of task-processors, we may want to highlight we reimplemented the task-processors using arrays and used cache-based optimizations to gain upto 50X speedup in processing, making task-processors 
%take tiny fraction of the overall execution time}
\end{enumerate}
In addition, we have addressed all the questions raised by the reviewers, as detailed below. 
We begin with the meta-review questions and then address the questions raised by individual reviewers. 



\subsection*{Metareview}

\com{1. Rework the structure of the paper so that it is comprehensible, including removing many of the references to the technical report. Remove (at least) the UI description and save it for another paper/demo.}

Based on this comment, we have tried to rewrite most of the paper to make it self-contained.
We removed the entirety of \vzalg to make room for the other content---while interesting,
this didn't take away from and was not a prerequisite for the other contributions of the paper. 
The \vzalg can be found in the technical report.
We have additionally trimmed most of the system architecture and 
front-end description (Section~\ref{sec:architecture})
in order to make more room for the other content. 
We have substantially revised all sections in making it more intuitive and self-contained:
In Section~\ref{sec:querylanguage}, we have modified the description to
read less like a user manual and more like a paper, like the reviewers suggest.
The key concepts are conveyed along with intuition, and the entire description is self-contained.
In Section~\ref{subsec:query_execution}, which has been completely revamped with 
new optimizations, we have spent a lot of time with the basic translation and
each of the optimizations in order to convey the key intuitions---in the past this section
had a lot of references to the technical report even for basic notions.
Even for the other sections, we have tried to opt for having the sections self-contained,
with minimal references to the technical report.

\com{2. Improve the related work comparison}

We have completely revamped the related work comparison, 
focusing primarily on differences
in functionality as opposed to differences in the UI,
with details in the related work section.
We now spend an entire column of text on comparing against visual analytics tools,
relational databases, data mining and statistics tools, and programming libraries.
In addition, we have expanded our description of the user study
to talk about these other tools (in addition to the visual analytics baselines).

In short, for relational databases, we talk about how relational databases
are not able to support certain types of processing;
and even for the small subset of \zq that relational databases can support---we provide
a \sql translation for one such query---it requires complex constructs 
not supported and optimized for in many relational databases.
In addition, we show through one experiment in the related work section that
%We show through one experim
\zq along with our cache-aware \fuse optimization
%Our \zq along with \fuse \tar{and cache-optimized in memory processing}
gives up to 10$\times$ better performance than this \sql query.
%(we've added one experiment in the related work section).
For most other queries, even we, the authors, were unable to write the query.
Most user study participants who knew \sql said that they would not use \sql
for \zq-like queries.

%didn't suggest it as an option
%when asked if they had tools that could replace \zv. 

Then, for data mining and statistics tools, we describe how 
they do not support any expressive querying for patterns or
optimization across such queries. In essence, these tools support built-in machine learning
or statistics algorithms, and only support changes in the parameters used to invoke 
these algorithms. 

Last, we describe how visual analytics tools generate one visualization at a time, 
while \zv is a query language over collections of visualizations. This increased capabilities
also leads to additional challenges in optimization.


\com{3. The user study needs to be at the very least rewritten, and probably redone, to find a good baseline to compare to and to describe what claims it is validating.}
%\agpyell{this isn't great}
To address these concerns, we reanalyzed collected data 
and rewrote large parts of the user study section; and we conducted 
an additional set of 7 analyst interviews recruited via Upwork. 

In particular, Reviewer 1 and 2 raised concerns about the design of the user study, 
and the task selection.
To remedy this, we conducted a survey with active data analysts
to augment the decisions behind our task selection.
We recruited them via Upwork, an online freelancing platform,
and probed them on the types of tasks they perform on a day-to-day basis.
We used a taxonomy of exploration tasks prescribed
by Amar et al.~\cite{amar2005low} to categorize these tasks.
We then cross-referenced this list with the actions completed in the tasks for the user
study to examine the breadth of activities the user study tasks covered.
We demonstrated how the selected user study tasks encompass most of the task
used in data exploration; however, we acknowledge that \zv does not offer
improvements for certain exploration tasks, and we explicitly state this in the
user study section.
%\tar{above paragraph looks much better now}

We then substantially rewrote the user study section to focus primarily on the comparison
with visual analytics tools, and other data analytics tools. 
We have also clarified the claims made by this user study and made the findings and contributions more precise.
%The user survey can be found in Section~\label{sec:interviews},
%while the new user study can be found in Section~\label{sec:userstudy}


\com{4. Improve the description of the novelty of the approach. In particular, the authors must provide a more detailed description of the execution engine that convinces the reviewers that this paper makes sufficient contributions... In particular, ...
(a) the idea of introducing processors and filter visualization is not explored in detail, and no optimizations are provided: these are implemented as black-box functions over visualizations, and no special optimization technique is described; in fact, based on the experiments some of them seem to require quite a long time to be executed;
(b) the translation of zenvisage queries into SQL is based on a shallow form of batching, and again does not look very insightful.}

We would like to emphasize that the primary contribution of the paper is not the query execution engine, but
in fact the \zq query language and the overall vision of the system. 
The auxiliary contributions include the query execution, the \vzalg and completeness proof, and the interface aspects. 
However, we took the reviewer's comments to heart to pursue a ``deep-dive'' exploration of the query execution part,
adding a host of new optimization techniques---employing speculation, query
combination, and cache-aware execution---touching both the optimization of the visualization retrieval as well as the processing of visualizations. 
We prove that the optimization problem for finding the optimal query
combination is {\sc NP-Hard},
and identify an effective solution---called \fuse.
As it turns out, vanilla parallelism, a simple form of multi-query optimization adopted by traditional relational databases
performs much more poorly than \fuse.
%We additionally add two other baselines to demonstrate the benefits of our optimization.

To address the other concerns: 
(a) We now fully explore optimizations that affect both the processing and the
retrieval of visualization data. 
The overall execution of \zq queries is now interactive with moderately sized
%datasetss
%Both the processing and generation is now interactive time on moderately sized
datasets---on large datasets,
we simply have no way of getting interactive time without approximation. In fact,
we show that our optimization schemes now overall lead to runtimes which are
virtually the same as the time it takes to run 
{\em a single group-by query} on the dataset.
This means that the bottleneck is not \zq, but in fact is the basic cost of scanning the entire dataset.
To test this further, we tested our optimized solution on our largest datasets in Vertica, and
we found that the techniques once again led to interactive times.
Thus, the bottleneck is not our code, but is in fact the basic database system bottleneck.
Note that even when the solution is NOT interactive---perhaps because the database is large---it is still
valuable, because it automates a lot of manual work of generating individual visualizations
and perusing them. 
(b) Indeed, in our previous version, the translation was rather shallow. 
In this version, we have shown that the optimal translation of \zq into \sql
%optimally for a simpler setting
%(when all the group-bys are distinct)
is itself {\sc NP-Hard}. We have developed a new
technique, called \fuse which finds a close approximation to the optimal
solution using a metric called $EFGV$.%trading off combining and batching that optimizes a new metric called $EFGV$. 



% \alkim{We do get interactive times when either dataset is small
%   enough or if we use in-memory database as our analytics systems (such as
%   Tableau do). However, there is no way to get interactive times if there is
%   too much data, other than to do sampling/estimation. Also, it should be
%   stressed that even if the system is not interactive, it provides a lot of use
%   because it automates a lot of the work being done manually right now (0 man
% hours).}


\subsection*{Reviewer 1}
\com{5. Organization - the paper tries to squeeze too much content within the page limit of the submission. As a result, many of the sections feel rather superficial and somehow rushed on. ... In this respect, this submission does not look sufficiently self-contained.}

See response to MetaReview point 1. 

\com{6. Contributions - The main intuition is to introduce processors to compare and filter visualizations. This is an interesting idea, and it is indeed an advancement wrt other visual analytics tools. However, this extension is not particularly deep from the technical viewpoint: the authors essentially introduce a number of black-box functions to process visualizations -- but besides this they do not offer significant insights related to the execution of the functions over visualizations. In fact, it can be seen from the experiments that on complex data, processing visualizations in main memory may take a significant time, and it is unclear how this would be compatible with the expectations of users in terms of response times. Other technical contributions in the paper are related to the translation of zenvisage queries into SQL queries, and their execution. These optimizations, however, amount to a rather straigtforward batch execution strategy, and essentially rely on the DBMS to do most of the actual optimization work.}

See response to MetaReview point 4.

\com{7. The language - the language is very expressive ... this raises a concern about the overall usability of the language, in two directions. First, the language itself does not look easy to use. Second, I think it is easy to write zenvisage scripts that take considerable time to be executed.}

%\tar{maybe we should add that we provide more details on the syntax/structure of process column, and participants' could understand it pretty easily. Moreover, we help users with drop-down menus to build the  process column.}

From our user study, we found that not only are users able to learn how to write
effective, correct \zq in a short amount of time (a 15 minute tutorial),
all of them were able to answer the tasks, i.e., formulate the \zq queries, 
within two minutes, and with over 95\% accuracy.
(In contrast, the users ended up having very poor accuracy of 70\% when they used 
a vanilla visualization tool AND took longer.)
This means that users are indeed able to understand and use \zq effectively. 
We have considerably expanded our user study section to clarify such issues.
Regarding the second point --- indeed, it is possible to write \zq scripts
that take a long time to be executed, however, that is a problem with any
declarative query language. That said, one benefit of our new optimization algorithm \fuse 
is that it can analyze a query and provide an estimate of the time, preventing 
users from running queries that take a long while to be executed.
%We have added a note about this to the paper \agp{we should.}



\com{8. Experimental Evaluation - experimental results do not look particularly convincing.... In terms of scalability, the study of the query optimization techniques simply that... batching queries improves performance. With respect to the performance of the task processors, the paper does not really discusses any optimizations ... and, as mentioned above, times may increase significantly when the number of groups increase. The user study also looks somehow flawed: it is completely unclear what is the baseline .... I can see that the problem of identifying the baseline in this case is tricky, since there is no system capable of performing a form of processing of visualizations that is similar to the one of zenvisage, but it is known that user studies, even more than other quantitative studies, are very sensitive to design choices like this.}

Our new experimental results are much more exhaustive and study sophisticated
optimizations 
that go beyond simple batching.
%In particular, we evaluate four algorithms. 
In fact, We provide experimental evidence that our \fuse optimization
does not take much longer than simply running a group-by query on the entire dataset---a powerful result,
indicating that we are able to extract as much mileage as possible from the database.
In addition, please see response to MetaReviewer's point 4.

Regarding the user study, indeed, finding a good baseline for \zv is tricky.
However, we have now revamped the user study to first justify the set of tasks and baselines we compare against
via user survey,
and further presented the comparison with visual analytics tools, followed by other analytics tools.
Our visual analytics tool baseline is modeled in such a way such that it replicates
the look and feel of \zv, while providing functionality similar to the likes of Tableau or Spotfire.
In addition, please see response to MetaReviewer's point 3.

% We have rewritten the user study section to better articulate the results and design decisions behind the user study. Finding a good baseline for \zv is indeed tricky. We now explicitly compare \zv with existing visual analytical tools and analytical tools to demonstrate the benefits of \zv, and reference the taxonomy of low-level analytical tasks by Amar et al. \cite{amar2005low} to clearly describe the tasks where \zv excels over existing tools (identifying correlations, anomalies, and clustering similar attributes). We do acknowledge that \zv does not offer improvements over certain tasks and explicitly state this fact in the user study section.



% \com{
% 1. I believe the paper would greatly benefit from splitting the presentation of the language and the study of its formal properties, from the discussion of the technical aspects related to the architecture and optimizations. Separating the content in two different papers would give proper space to both treatments, and improve the overall readability.}

% \com{
% 2. with respect to the language, I suggest that the authors concentrate on the discussion of how such an expressive and ambitious language can be made practical for users, especially the ones without a strong technical background. It would be interesting, for example, to discuss how the syntax can be restricted to improve the usability, or techniques to estimate the execution time of scripts in advance, in order to warn the users about possible slowdowns.
% }

% \com{
% 3. as far as the technical development is concerned, I think the authors may want to investigate more the implementation of the task processors (as opposed to the SQL optimization algorithm, that looks quite straightforward). In fact, designing optimized implementations of the very expressive processors allowed within the language seems an interesting challenge.
% }


\smallskip
\noindent
We have also addressed the other typographical errors identified by the reviewer.
%\agp{we should...}

\subsection*{Reviewer 2}


\com{9. Introduction and Motivation: The introduction is a bit confusing 
regarding the main contribution of the paper.... I believe that the contribution of this paper 
is the query visualization language that allows the user to declaratively express 
the desired visualizations, and the authors need to clearly say that 
avoiding the visualization recommendation hints.}

We agree. We have eliminated any mention of the visualization recommendation notion,
and focus on the fact that \zq is a language that supports querying over visualizations. 
We have completely rewritten the introduction and the related work sections 
to emphasize these notions. 


\com{10. Contribution and Positioning to Other Works/tools: databases that have query languages, data mining tools, and visual analytics tools. The paper makes comparisons to all three but these comparisons are more at the level of "user-friendliness".  What is needed is also a comparison at the level of expressivity and functionality.
}

See response to MetaReview point 2.


\com{11. Paper structure:
The paper organization is rather unorthodox and confusing. 
(i) Section 2 starts with examples of the Query Language using a table syntax and then explains the table syntax. I think we could skip the examples or move them after explaining the syntax. ... It would be best to focus on a few that ... are also representative of the query capabilities
(ii) Then Section 3 is query execution followed by the system architecture followed by experiments and finally followed by the relational algebra. why not finishing with the query language, then presenting an overview of the system, then explaining the particular components of the system around query execution...? 
}
We agree with the reviewer: we have made significant changes to the organization and presentation.
(i) We have completely rewritten Section~\ref{sec:querylanguage} 
and eliminated the early examples
and focused on the intuition behind the key language functionalities
with a minimal number of examples.
(ii) We have eliminated the algebra from the main body of the paper---the rest of the paper
did not depend on this. Since we significantly shortened the architecture section---focused 
primarily on describing a screenshot---we believe it is
best placed before the user study, where it is most relevant. The query execution section 
is self-contained, and does not require any concepts from the architecture section. 
Also see response to MetaReview point 1 for overall organizational changes. 


\com{12. Query Language:
\begin{inparaenum}[(i)]
\item The paper should add a summary of the capabilities and limitations of the language. 
\item How are joins expressed in ZQL? How are they mapped to SQL? 
\item ZQL queries can be supported in Java through the Java client library. Why would one use ZQL in Java vs any visualization language (e.g. D3) coupled with SQL (assuming that he is already programming in Java?
\item The Constraints and Viz sections are quite short. What type of operations does it support? It supports filtering but does it support any functions over column values, such as taking the average of a column or concatenating strings or adding values, etc, before filtering them? What type of processing on the values can be done before they mapped, what type of functions are supported, e.g. take the log of X values?
\item Please discuss how the (process) functions cover the breadth and diversity of visual analytics tasks. What kind of variants of these functions can the user define?
\item Section 2 provides one view of the language while section 7 describes the relational algebra behind it. First of all, everything about the language should be in one place. Second, section 7 is confusing because ... the two sections seem disconnected to large degree.
\end{inparaenum}
}

We thank the reviewer for the suggestions. 
Overall, we have rewritten most of  
the query language section, taking the reviewer's comments into account.
Specifically, we have eliminated the upfront examples, and focused instead
on the key concepts, and the examples to illustrate them. 
We have tried to be as formal and careful about describing features of the language,
while also providing intuition about the utility.
Specifically, the process column discussion has expanded, 
and we have added a detailed discussion on capabilities and limitations.

We answer point-by-point below:
\begin{inparaenum}[(i)]
\item We agree. We have added a detailed discussion on capabilities and limitations 
in Section~\ref{subsec:cap-lim}.
We have articulated how \zq's primary contribution is as a 
query language over collections of visualizations---composing, filtering, sorting,
and comparing visualizations iteratively.
On the other hand \zq is not appropriate for any sort of data modification
or data transformation, among other functionalities that \sql can support,
such as recursion and nesting.
\item We have added a short line about how joins are supported to the paper.
%\agpyell{Add.}
\item This is already addressed in the related work comparison---see response to MetaReview point 2.
In short, \sql is very cumbersome to near impossible to use, and inefficient for the queries \zq is good at.
The benefit of the {\tt Java} library is that some users may want to develop domain specific 
visualization tools that compile down to \zq queries issued via {\tt Java}. 
\item We have folded the Constraints column into the discussion of the Z column, and we are 
now spending more time clearly explaining the capabilities of these columns.
In short, while the Viz column does support certain fixed types of aggregations
and binning, it doesn't support arbitrary functions.
Further, none of the other columns support data transformations. This is
one of the main limitations of \zq as it stands, and is described in Section~\ref{subsec:cap-lim}.
%\agpyell{alkim check}
\item We have simplified the presentation of the process functions as well, and we
now clarify the various ways the process functions can be used, and
how it can be extended.
%\agpyell{alkim check}
\item We have removed Section 7 (former \vzalg discussion) from the main body of the paper,
reducing this concern. In the technical report, we have tried to be more consistent when
rewriting the section.
\end{inparaenum}


\com{13. Query Execution: The translation is described very briefly making it hard to understand the mechanism ... furthermore, how are the Viz, X, Y parts translated to? Obviously, they are not translated to SQL, are they? Provide an example of a ZQL and its translation ... use this example to illustrate the optimizations of Section 3.2 too. The language supports three simple functions ... How are these functions translated into the executable SQL code?
}

(also raised by Reviewer 3)

We thank the reviewers for the excellent suggestions. 
We agree that our previous query execution section described the translation and optimization strategies
in an excessively terse manner.
To remedy this (and also because we now have a host of additional optimizations),
we have rewritten the query execution and optimization section (Section~\ref{subsec:query_execution}) in its entirety.
For the query execution, we have added 
a clear step-by-step description of the entire translation process. 
This includes the mapping for all of the columns except Process, which are mapped
I%\agpyell{alkim check Viz}
to portions of the \sql queries, and for the processes. We have also considerably
clarified the presentation of the processes in Section~\ref{sec:querylanguage}).
We also made sure that the same examples were used for the optimization
discussion.

%, to this section by using the same example for the optimization discussion, 
%which was covered in our response to MetaReview point 4. 


\com{14. System:
\begin{inparaenum}[(i)]
\item Figures 3 and 4 are almost invisible ... 
\item  The front-end description does not add much... 
\item I would first show the system and then focus on its main components.
\item Section 3 needs to clearly refer to the main system components of Figure 2 (maybe as separate subsections). 
\end{inparaenum}
}
Responses below:
\begin{inparaenum}[(i)]
\item While it is still hard to read the font of the screenshot, 
we have now added a large font overlay --- only this text is meant to be read.
We have eliminated one of the two figures.
\item We have eliminated most of the description of the front-end and only kept the essential parts.
\item We now show the system screenshot as the first step.
\item We have eliminated the system components diagram (Figure 2), and kept
  Section 3 self-contained.
The architecture section is now a short section primarily focused on what is needed to understand
the user study and the experimental evaluation.
\end{inparaenum}

\com{15. Experiments:
I have hard time understanding the effect of optimizations ... 
I think a more comprehensive study would be more helpful and insightful. 
For example, show performance based on the number of visualizations, ....
}

We thank the reviewer for this suggestion --- based on the suggestion 
we have thoroughly revamped the experimental section by conducting performance
evaluation studies on varying all of the parameters the reviewer suggests,
among others. The results can be found in Section~\ref{sec:experiments}.

\com{16. Experiments: For the user study, the authors prepared the tasks ... Were they tasks better suited for ZenVisage? ... It would be fairer ... if the tasks were actually diverse and the study would show where the current system excels and where not. In fact, one could organize two-level study. first, a variety of analytics tasks are chosen. The second level could focus on specific tasks (for which Zenvisage is appropriate) and show how well it performs.
}

We agree with the reviewer's point --- it's not clear if the 
tasks are indeed diverse enough, and we really appreciated
the suggestion of performing a two-stage study 
where we first identify a variety of analytics tasks
and test their relevance, and then focus on specific tasks
for \zv. 
We have done precisely that. 

Please see response to MetaReview point 3. 

% We conducted an additional user interview with data analysts to augment the decisions behind our task selection. We probed the different type of tasks analysts work on during their daily activities, and we reference the taxonomy of low-level analytical tasks described by Amar et al. \cite{amar2005low} to categorize the tasks. We cross-referenced the low-level task list with the actions completed by the user study participants to examine the breath of activities our tasks covered. We rewrote the user study section to more accurately describe where \zv excels over existing tools (identifying correlations, anomalies, and clustering similar attributes) and where \zv does not offer improvements.



%\com{Too much breadth and many dependencies to the technical report. Needs focus.}



\subsection*{Reviewer 3}
\com{17. ...the proposed ZQL language is quite like breaking the visual analytics task step by step and describing each step through a sub-query, which could also be described using SQL sub-query. How much user effort could be reduced by using ZQL? ...
}

See response to MetaReview point 2.


% The reviewer brings up an important question: can \sql replace \zq in functionality? 
% As it turns out, the answer is yes for 
% certain types of \zq queries, but not all queries. 
% We now provide a \sql translation for a \zq query in Table~\agp{xxx} in our
% paper---this translation assumes 
% that the distance function $D$ is Euclidean.
% For any other distance functions, 
% we are not aware of any way of issuing a \sql
% query to replace \zq. 
% Furthermore, there are other types of processors 
% which similarly cannot be replaced
% directly with \sql.
% However, the more problematic aspect is that the \sql query thus written is
% fairly complicated and hard to understand and debug;
% it also necessarily involves some complex \sql constructs,
% that are not supported universally across all database systems,
% and are poorly optimized. 
% Our user study participants, for example, despite knowing and using \sql,
% did not think \sql is an appropriate language to issue these types of requests.
% We have added a detailed description to the related work section to describe
% the comparison of \zq with \sql. 
% We have additionally added experiments that demonstrate that the
% \sql queries of this type take a very long time to be executed (in Section~\agp{xxx})



\com{18. ...the query execution section presents the translation approach and optimization strategies too briefly. More algorithmic details and examples would be good for the readers.}

See response to Reviewer 2 point 13.


\com{...zenvisage aims to provide an interactive visual analytics system, but the overall performance takes tens of seconds as shown in Figure 6, it is a bit too long for interactive analytics. For the user, they only care about the overall performance, I am wondering what the major part of the time consumed in the system.}

We thank the reviewer for the suggestion 
--- we now have a breakdown in the paper for the time consumed by our
optimization algorithms.
Furthermore, we reimplemented the \zq engine to use a much faster array-based
index (as opposed to a hash-based index, which along with our optimizations, provided us with a 50$\times$
speedup in processing.
%each step of \fuse, our new optimization algorithm.
%\tar{we may want to highlight we reimplemented the task-processors using arrays and used cache-based optimizations to gain upto 50X speedup in processing, making task-processors 
%take tiny fraction of the overall execution time}
In short, our algorithm is only non-interactive for practical queries when the time it takes
to run a single group-by query on the dataset (essentially the cost of a single
scan) is non-interactive. 
%Essentially, the time for \fuse is a small multiple of the time to take a run single group-by query.
We describe in detail the changes to the optimization, and the explanation for how we investigated
where the bottlenecks to interactivity are --- along with an additional experiment on Vertica --- in the response to the MetaReview point 4.



% In our previous version, we were using relatively naive optimization schemes, as a result of which the overall
% performance took tens of seconds---after developing additional optimization techniques, capturing 
% combination, speculation, batching, and caching, practical queries on real datasets now take orders of XXX\agp{xxx} seconds. 
% Also to address the issue raised by the reviewer, we have added an experimental breakdown
% in Figure~\ref{xxx}\agp{xxx} that displays where the time is being spent in the system.
% In short, we find that the bulk of the time is spent in the \sql queries that are issued,
% as opposed to the task processing. \agp{xxx}.
% Note however, we are fundamentally limited by the size of the dataset---if a 
% single sequential scan takes \agp{xxx} seconds, then it is impossible for us to 
% achieve better times than that, without adding on additional
% optimizations such as sampling and precomputation. 
% We plan to explore these additional optimizations
% in future work. 
% We have additionally added an experiment to demonstrate that as well---in Figure~\agp{x}, we show
% that our optimizations lead to a moderate complexity \zq query taking not more
% than \agp{xx}x of the time taken for a single group-by query on the entire dataset
% on PostgreSQL.



==> docs copy/abstract.tex <==
%!TEX root=zenvisageql.tex

\begin{abstract}
Data visualization is by far the most commonly used mechanism to explore
and extract insights from datasets, especially by novice data scientists.
And yet, current visual analytics tools are rather limited in their ability
to operate on collections of 
visualizations---by composing, filtering, comparing, and sorting them---to
find those that depict desired trends or patterns. 
The process of visual data exploration remains a 
tedious process of {\em trial-and-error}.
We propose \zv, a visual analytics platform for effortlessly finding desired visual patterns 
from large datasets. We introduce \zv's general purpose visual exploration language, \zq 
("zee-quel") for specifying the desired visual patterns, drawing from use-cases in a variety of domains, including biology, mechanical engineering, climate science,
and commerce. 
We formalize the expressiveness of
\zq via a \vzalg---an algebra on collections of visualizations---and 
demonstrate that \zq is as expressive as that algebra. 
\zv exposes an interactive front-end 
that supports the issuing 
of \zq queries, and also supports 
interactions that are ``short-cuts'' to certain
commonly used \zq queries.
To execute these queries, 
\zv uses a novel \zq graph-based query optimizer that leverages a suite of 
optimizations tailored to the goal of processing collections of visualizations
in certain pre-defined ways. 
Lastly, a user survey and study demonstrates that
data scientists are able to effectively use \zv to 
eliminate error-prone and tedious exploration
and directly identify desired visualizations.
\end{abstract} 


==> docs copy/architecture-new.tex <==
%!TEX root=zenvisageql.tex
\vspace{-2pt}
\section{{\Large \zv} System Description}
\label{sec:architecture}
\vspace{-2pt}

\noindent We now give a brief description of the \zv system.
%describe the architecture of \zv,
%also depicted in Figure~\ref{fig:arch}.


%\begin{figure}
%\centering
%\includegraphics[width=0.9\columnwidth]{figs/arch.pdf}
%\vspace{-10pt}
%\caption{System architecture}
%\label{fig:arch}
%\vspace{-5pt}
%\end{figure}


\begin{figure}
\vspace{-10pt}
\centering
        \includegraphics[width=7cm]{figs/barchart_v2_new}
    \vspace{-5pt}
        \caption{\zv basic functionalities}
        \label{fig:querytable}
\vspace{-20pt}
    
\end{figure}


\paragraph{Front-end.}
The \zv front-end is designed as a 
lightweight web-based client application.
It provides a GUI to compose \zq queries, 
and displays the resulting visualizations
using Vega-lite~\cite{wongvoyager2015}. 
A screenshot of \zv in action is shown in Figure~\ref{fig:querytable}.
A list of attributes, divided into qualitative and quantitative, is provided on
the left; a table to enter \zq queries, with auto-completion, 
is on top, and the resulting
visualizations are rendered at the bottom.
Users also have the option of hiding the \zq specification table and
instead using a simpler drop-down menu-based interface complemented by a
sketching canvas.
The sketching canvas allows users to draw their desired trend that can then be
used to search for similar trends. The menu-based interface makes it easy for
users to perform some of the more common visual exploration queries, such as
searching for representative or outlier visualizations. Furthermore, the user
may drag-and-drop visualizations from the results onto the sketching canvas,
enabling further interaction with the results.

\paragraph{Back-end.}
The \zv front-end issues \zq queries to the back-end over a {\sf REST}
protocol. The back-end (written in {\tt node.js}) receives the queries and
forwards them to the \zq engine (written in {\tt Java}), which is
responsible for parsing, compiling, and optimizing the queries as in Section~\ref{subsec:query_execution}. \sql queries issued by the \zq
engine are submitted to one of our back-end databases (which
currently include PostgreSQL and Vertica), and the resultant visualization data
is returned back to the front-end encoded in {\tt JSON}.


==> docs copy/challenges.tex <==
%!TEX root=zenvisageql.tex

\section{Future Directions}
\label{sec:challenges}

\subsection{Backend challenges}
\label{subsec:backendchallenges}


\subsection{Frontend specification challenges}
\label{subsec:frontendchallenges}


\subsection{Algorithmic challenges}
\label{subsec:algorithmicchallenges}

==> docs copy/conclusion.tex <==
%!TEX root=zenvisageql.tex
\vspace{-5pt}
\section{Conclusion}
\label{subsec:conclusion}
\vspace{-2pt}
We propose \zv, a visual analytics tool for effortlessly identifying desired
visual patterns from large datasets.
We described the formal syntax of the query language \zq, motivated by many
real-world use-cases, and demonstrated that \zq is \vzalg-complete\papertext{ (See~\cite{techreport})}.
\zv enables users
to effectively and accurately perform visual exploration tasks, 
as shown by our user study, and complements other tools.
In addition, we show that our
optimizations for \zq execution lead to considerable improvements over
leveraging the parallelism inherent in databases.
Our work is a promising first step towards substantially simplifying
and improving the process of interactive data exploration
for novice and expert analysts alike.
%We then described three simple optimizations for translating
%\zq queries into \sql queries, and demonstrated
%how these optimizations lead to several orders of 
%performance improvement on real and synthetic datasets. \new{Finally, we presented a user study that demonstrated the usability and effectiveness of \zv.} 

% In this paper, we propose a data exploration system for an effortless specification and visualisation of interesting patterns, trends and insights from large datastets. We developed a novel visual query specification language \zq for users to specify their desired trend and patterns. We presented a detailed formalisation of \zq and showed the robustness and usefulness of the language through a number of real world examples from a variety of domains. We discuss some simple optimisations on \zq which minimizes the number of \sql queries that we need to execute on the underyling database. We also described the system architecure of \zv and implemented an initial prototype. It consists of two components: front-end and backend. Front-end provides an intuitive graphical interface to compose ZQL queries and to visualise of results of the queries. We talk about the components of interface to show how effectively it can be used by both novice and expert users. Back end implements \zq engine and task processor for execution of \zq queries. Finally, we provide our preliminary experiments on query optimisations and the performance of common exploration queires on our system. \tar{Future work}



==> docs copy/cover.tex <==
%!TEX root=zenvisageql.tex


\section*{Summary for Revised Paper ``Effortless Data Exploration with zenvisage: An Expressive and Interactive Visual Analytics System''}

We thank the reviewers and meta-reviewer for their insightful 
and very detailed feedback, 
and for giving a chance to address these comments---we have taken this feedback to 
heart in preparing an {\em almost entire
rewrite} of the present paper---{\bf \em each and every section was substantially modified; 
new sophisticated optimized \zq engine,
\fuse,
(using speculation,
parallel, and query combining) along with cache-aware optimization
techniques (and an {\sc NP-Hardness} proof) were developed; 
an extensive performance evaluation on multiple datasets and parameters was added
and a new Upwork user survey was conducted. }
The major changes to each section of the paper include:
\begin{enumerate}
\item {\em A complete rewrite and repositioning of the introduction.}
We rewrote most of the introduction to (i) position our system correctly
as a system that facilitates the search for desired patterns as opposed to a
visualization recommendation system; (ii) describe how \zv solves
some of the articulated problems alluded to in the examples; and (iii) 
describe the challenges in building \zv.

\item {\em A complete rewrite of the query language section.}
To improve readability and make
the paper more self-contained, we rewrote this section to have fewer references
to the technical report. We removed the list of initial examples,
and made this section read less like a user manual, with more intuition 
built in. We also added more details on the task processors (now called
processes),
and clearly defined the interfaces of our exploration functions.
At the same time, we trimmed the description of features that were
not essential to grasp the core contributions of \zq.
% \alkim{Opened up task processors, and made them seem less like a black box,
% both in language section and execution section. Also better defined our
% exploration functions so the interface is more clear}

\item {\em Full-fledged modeling and optimization, 
hardness proof, intelligent optimization schemes, and 
complete rewrite of the query execution section.}
To extend and articulate clearly the novelty of the query optimizer,
we added 
a thorough system modeling and exploration of solution alternatives.
We extended our previous naive graph-based optimization 
technique to a sophisticated technique, called \fuse, reliant on speculation,
caching, and
query combination---a particularly tricky aspect
was that query combination led to non-monotonically increasing gains, so
determining the optimal set of combinations was non-trivial.
%was trading off
%query combination and batching,
%and optimization across task processors (now called processors).
% \alkim{To be fair, our speculation scheme is not really intelligent... we just
% speculation everything. But we do do both batching AND query combining, and the
% decisions for when to combine/batch are based on our complex algorithms that we
% talk aboutl ater.}
We additionally proved that the problem of identifying the optimal set of
combinations 
is {\sc NP-Hard}
and developed an approach to solve the problem. 
In our revision, we now also
spend a lot of room articulating clearly how a \zq query gets
translated, with detailed descriptions of processors and functions $T$ and $D$.
Overall, this section has been entirely rewritten and enhanced.


\item {\em Reimplementation of the \zq Engine.}
  One of the main concerns of the reviewers was the large execution times of \zq
  queries. To address this point, in addition to the optimizations
  mentioned before, we reimplemented the \zq engine to use the much faster
  array-based indexing (as opposed to hash-based indexing) 
  which provided a 50$\times$ speedup in processing time
  (and explained the poor performance earlier). 
  We also showed in the experimental section that if we swap out
  PostgreSQL for a column-store
  database with a large in-memory cache, we can reach interactive response
  times for large datasets.


\item {\em Completely redone performance experiments and rewritten experimental
section.}
We completely redid the performance experiments to better
focus on parameters and aspects that the reviewers suggested.
Specifically, we compared the performance of our query optimizer 
against three algorithms (we had just one baseline in prior work), 
including one which leverages
the standard multi-query optimization within traditional 
database systems---our algorithm performs much better than this baseline.
We compared the algorithms on a range of real-world and 
synthetic datasets, varying parameters,
including the complexity of the queries and the number of
visualizations processed. We also report 
the breakdown of
runtime
%our algorithm
across retrieving visualizations
and processing them. 

\item {\em Entirely new analyst interview section, and 
extensive rewrites to user study section.}
To enable us to judge whether the tasks used in the previous user study
capture the typical tasks used in practice, 
we conducted an entirely new set of user interviews of analysts from Upwork, 
focused on the data exploration tasks from a comprehensive list 
provided by Amar et al.~\cite{amar2005low}. 
Additionally, we rewrote most of the user study section to clearly articulate
the proposed benefits of \zv and focus on 
the utility of \zv and \zq relative to other tools,
as opposed to general usability aspects. 
We specifically revamped and expanded the portion of the study
that compares \zv to other database and data mining tools, along with 
participant quotes and code examples. 


\item {\em Trimmed down system architecture section.}
Since reviewers felt that the paper was busy enough as it is,
so
we have considerably trimmed the system architecture 
%section---especially
%the front-end technologies,
section---only leaving what is absolutely
necessary to support the user study.%, and the experimental sections.

\item {\em Modified related work section.}
We edited this section to emphasize technical differences
as opposed to philosophical differences between \zv and other
systems.
%(these differences were also summarized in the introduction). 
%We briefly also mentioned these differences in the
%introduction.
Also mirroring the positioning of \zv in the introduction,
we focused on comparing with systems that support similar
searches for desired patterns, as opposed to recommendation systems.
For comparison with raw relational databases and \sql,
%Within the related work section, for the relational databases
%comparison,
we additionally added a short experiment to illustrate
how \sql is unsuitable for expressing \zq queries.

\item {\em Removed the \vzalg section.}
Since the \vzalg section could be removed without affecting
the readability or impact of other sections---especially
now that the optimization section has been expanded---we
decided to remove this section entirely, and link to it
via the technical report.


%\tar{Since multiple reviewers were concerned about the timings of task-processors, we may want to highlight we reimplemented the task-processors using arrays and used cache-based optimizations to gain upto 50X speedup in processing, making task-processors 
%take tiny fraction of the overall execution time}
\end{enumerate}
In addition, we have addressed all the questions raised by the reviewers, as detailed below. 
We begin with the meta-review questions and then address the questions raised by individual reviewers. 



\subsection*{Metareview}

\com{1. Rework the structure of the paper so that it is comprehensible, including removing many of the references to the technical report. Remove (at least) the UI description and save it for another paper/demo.}

Based on this comment, we have tried to rewrite most of the paper to make it self-contained.
We removed the entirety of \vzalg to make room for the other content---while interesting,
this didn't take away from and was not a prerequisite for the other contributions of the paper. 
The \vzalg can be found in the technical report.
We have additionally trimmed most of the system architecture and 
front-end description (Section~\ref{sec:architecture})
in order to make more room for the other content. 
We have substantially revised all sections in making it more intuitive and self-contained:
In Section~\ref{sec:querylanguage}, we have modified the description to
read less like a user manual and more like a paper, like the reviewers suggest.
The key concepts are conveyed along with intuition, and the entire description is self-contained.
In Section~\ref{subsec:query_execution}, which has been completely revamped with 
new optimizations, we have spent a lot of time with the basic translation and
each of the optimizations in order to convey the key intuitions---in the past this section
had a lot of references to the technical report even for basic notions.
Even for the other sections, we have tried to opt for having the sections self-contained,
with minimal references to the technical report.

\com{2. Improve the related work comparison}

We have completely revamped the related work comparison, 
focusing primarily on differences
in functionality as opposed to differences in the UI,
with details in the related work section.
We now spend an entire column of text on comparing against visual analytics tools,
relational databases, data mining and statistics tools, and programming libraries.
In addition, we have expanded our description of the user study
to talk about these other tools (in addition to the visual analytics baselines).

In short, for relational databases, we talk about how relational databases
are not able to support certain types of processing;
and even for the small subset of \zq that relational databases can support---we provide
a \sql translation for one such query---it requires complex constructs 
not supported and optimized for in many relational databases.
In addition, we show through one experiment in the related work section that
%We show through one experim
\zq along with our cache-aware \fuse optimization
%Our \zq along with \fuse \tar{and cache-optimized in memory processing}
gives up to 10$\times$ better performance than this \sql query.
%(we've added one experiment in the related work section).
For most other queries, even we, the authors, were unable to write the query.
Most user study participants who knew \sql said that they would not use \sql
for \zq-like queries.

%didn't suggest it as an option
%when asked if they had tools that could replace \zv. 

Then, for data mining and statistics tools, we describe how 
they do not support any expressive querying for patterns or
optimization across such queries. In essence, these tools support built-in machine learning
or statistics algorithms, and only support changes in the parameters used to invoke 
these algorithms. 

Last, we describe how visual analytics tools generate one visualization at a time, 
while \zv is a query language over collections of visualizations. This increased capabilities
also leads to additional challenges in optimization.


\com{3. The user study needs to be at the very least rewritten, and probably redone, to find a good baseline to compare to and to describe what claims it is validating.}
%\agpyell{this isn't great}
To address these concerns, we reanalyzed collected data 
and rewrote large parts of the user study section; and we conducted 
an additional set of 7 analyst interviews recruited via Upwork. 

In particular, Reviewer 1 and 2 raised concerns about the design of the user study, 
and the task selection.
To remedy this, we conducted a survey with active data analysts
to augment the decisions behind our task selection.
We recruited them via Upwork, an online freelancing platform,
and probed them on the types of tasks they perform on a day-to-day basis.
We used a taxonomy of exploration tasks prescribed
by Amar et al.~\cite{amar2005low} to categorize these tasks.
We then cross-referenced this list with the actions completed in the tasks for the user
study to examine the breadth of activities the user study tasks covered.
We demonstrated how the selected user study tasks encompass most of the task
used in data exploration; however, we acknowledge that \zv does not offer
improvements for certain exploration tasks, and we explicitly state this in the
user study section.
%\tar{above paragraph looks much better now}

We then substantially rewrote the user study section to focus primarily on the comparison
with visual analytics tools, and other data analytics tools. 
We have also clarified the claims made by this user study and made the findings and contributions more precise.
%The user survey can be found in Section~\label{sec:interviews},
%while the new user study can be found in Section~\label{sec:userstudy}


\com{4. Improve the description of the novelty of the approach. In particular, the authors must provide a more detailed description of the execution engine that convinces the reviewers that this paper makes sufficient contributions... In particular, ...
(a) the idea of introducing processors and filter visualization is not explored in detail, and no optimizations are provided: these are implemented as black-box functions over visualizations, and no special optimization technique is described; in fact, based on the experiments some of them seem to require quite a long time to be executed;
(b) the translation of zenvisage queries into SQL is based on a shallow form of batching, and again does not look very insightful.}

We would like to emphasize that the primary contribution of the paper is not the query execution engine, but
in fact the \zq query language and the overall vision of the system. 
The auxiliary contributions include the query execution, the \vzalg and completeness proof, and the interface aspects. 
However, we took the reviewer's comments to heart to pursue a ``deep-dive'' exploration of the query execution part,
adding a host of new optimization techniques---employing speculation, query
combination, and cache-aware execution---touching both the optimization of the visualization retrieval as well as the processing of visualizations. 
We prove that the optimization problem for finding the optimal query
combination is {\sc NP-Hard},
and identify an effective solution---called \fuse.
As it turns out, vanilla parallelism, a simple form of multi-query optimization adopted by traditional relational databases
performs much more poorly than \fuse.
%We additionally add two other baselines to demonstrate the benefits of our optimization.

To address the other concerns: 
(a) We now fully explore optimizations that affect both the processing and the
retrieval of visualization data. 
The overall execution of \zq queries is now interactive with moderately sized
%datasetss
%Both the processing and generation is now interactive time on moderately sized
datasets---on large datasets,
we simply have no way of getting interactive time without approximation. In fact,
we show that our optimization schemes now overall lead to runtimes which are
virtually the same as the time it takes to run 
{\em a single group-by query} on the dataset.
This means that the bottleneck is not \zq, but in fact is the basic cost of scanning the entire dataset.
To test this further, we tested our optimized solution on our largest datasets in Vertica, and
we found that the techniques once again led to interactive times.
Thus, the bottleneck is not our code, but is in fact the basic database system bottleneck.
Note that even when the solution is NOT interactive---perhaps because the database is large---it is still
valuable, because it automates a lot of manual work of generating individual visualizations
and perusing them. 
(b) Indeed, in our previous version, the translation was rather shallow. 
In this version, we have shown that the optimal translation of \zq into \sql
%optimally for a simpler setting
%(when all the group-bys are distinct)
is itself {\sc NP-Hard}. We have developed a new
technique, called \fuse which finds a close approximation to the optimal
solution using a metric called $EFGV$.%trading off combining and batching that optimizes a new metric called $EFGV$. 



% \alkim{We do get interactive times when either dataset is small
%   enough or if we use in-memory database as our analytics systems (such as
%   Tableau do). However, there is no way to get interactive times if there is
%   too much data, other than to do sampling/estimation. Also, it should be
%   stressed that even if the system is not interactive, it provides a lot of use
%   because it automates a lot of the work being done manually right now (0 man
% hours).}


\subsection*{Reviewer 1}
\com{5. Organization - the paper tries to squeeze too much content within the page limit of the submission. As a result, many of the sections feel rather superficial and somehow rushed on. ... In this respect, this submission does not look sufficiently self-contained.}

See response to MetaReview point 1. 

\com{6. Contributions - The main intuition is to introduce processors to compare and filter visualizations. This is an interesting idea, and it is indeed an advancement wrt other visual analytics tools. However, this extension is not particularly deep from the technical viewpoint: the authors essentially introduce a number of black-box functions to process visualizations -- but besides this they do not offer significant insights related to the execution of the functions over visualizations. In fact, it can be seen from the experiments that on complex data, processing visualizations in main memory may take a significant time, and it is unclear how this would be compatible with the expectations of users in terms of response times. Other technical contributions in the paper are related to the translation of zenvisage queries into SQL queries, and their execution. These optimizations, however, amount to a rather straigtforward batch execution strategy, and essentially rely on the DBMS to do most of the actual optimization work.}

See response to MetaReview point 4.

\com{7. The language - the language is very expressive ... this raises a concern about the overall usability of the language, in two directions. First, the language itself does not look easy to use. Second, I think it is easy to write zenvisage scripts that take considerable time to be executed.}

%\tar{maybe we should add that we provide more details on the syntax/structure of process column, and participants' could understand it pretty easily. Moreover, we help users with drop-down menus to build the  process column.}

From our user study, we found that not only are users able to learn how to write
effective, correct \zq in a short amount of time (a 15 minute tutorial),
all of them were able to answer the tasks, i.e., formulate the \zq queries, 
within two minutes, and with over 95\% accuracy.
(In contrast, the users ended up having very poor accuracy of 70\% when they used 
a vanilla visualization tool AND took longer.)
This means that users are indeed able to understand and use \zq effectively. 
We have considerably expanded our user study section to clarify such issues.
Regarding the second point --- indeed, it is possible to write \zq scripts
that take a long time to be executed, however, that is a problem with any
declarative query language. That said, one benefit of our new optimization algorithm \fuse 
is that it can analyze a query and provide an estimate of the time, preventing 
users from running queries that take a long while to be executed.
%We have added a note about this to the paper \agp{we should.}



\com{8. Experimental Evaluation - experimental results do not look particularly convincing.... In terms of scalability, the study of the query optimization techniques simply that... batching queries improves performance. With respect to the performance of the task processors, the paper does not really discusses any optimizations ... and, as mentioned above, times may increase significantly when the number of groups increase. The user study also looks somehow flawed: it is completely unclear what is the baseline .... I can see that the problem of identifying the baseline in this case is tricky, since there is no system capable of performing a form of processing of visualizations that is similar to the one of zenvisage, but it is known that user studies, even more than other quantitative studies, are very sensitive to design choices like this.}

Our new experimental results are much more exhaustive and study sophisticated
optimizations 
that go beyond simple batching.
%In particular, we evaluate four algorithms. 
In fact, We provide experimental evidence that our \fuse optimization
does not take much longer than simply running a group-by query on the entire dataset---a powerful result,
indicating that we are able to extract as much mileage as possible from the database.
In addition, please see response to MetaReviewer's point 4.

Regarding the user study, indeed, finding a good baseline for \zv is tricky.
However, we have now revamped the user study to first justify the set of tasks and baselines we compare against
via user survey,
and further presented the comparison with visual analytics tools, followed by other analytics tools.
Our visual analytics tool baseline is modeled in such a way such that it replicates
the look and feel of \zv, while providing functionality similar to the likes of Tableau or Spotfire.
In addition, please see response to MetaReviewer's point 3.

% We have rewritten the user study section to better articulate the results and design decisions behind the user study. Finding a good baseline for \zv is indeed tricky. We now explicitly compare \zv with existing visual analytical tools and analytical tools to demonstrate the benefits of \zv, and reference the taxonomy of low-level analytical tasks by Amar et al. \cite{amar2005low} to clearly describe the tasks where \zv excels over existing tools (identifying correlations, anomalies, and clustering similar attributes). We do acknowledge that \zv does not offer improvements over certain tasks and explicitly state this fact in the user study section.



% \com{
% 1. I believe the paper would greatly benefit from splitting the presentation of the language and the study of its formal properties, from the discussion of the technical aspects related to the architecture and optimizations. Separating the content in two different papers would give proper space to both treatments, and improve the overall readability.}

% \com{
% 2. with respect to the language, I suggest that the authors concentrate on the discussion of how such an expressive and ambitious language can be made practical for users, especially the ones without a strong technical background. It would be interesting, for example, to discuss how the syntax can be restricted to improve the usability, or techniques to estimate the execution time of scripts in advance, in order to warn the users about possible slowdowns.
% }

% \com{
% 3. as far as the technical development is concerned, I think the authors may want to investigate more the implementation of the task processors (as opposed to the SQL optimization algorithm, that looks quite straightforward). In fact, designing optimized implementations of the very expressive processors allowed within the language seems an interesting challenge.
% }


\smallskip
\noindent
We have also addressed the other typographical errors identified by the reviewer.
%\agp{we should...}

\subsection*{Reviewer 2}


\com{9. Introduction and Motivation: The introduction is a bit confusing 
regarding the main contribution of the paper.... I believe that the contribution of this paper 
is the query visualization language that allows the user to declaratively express 
the desired visualizations, and the authors need to clearly say that 
avoiding the visualization recommendation hints.}

We agree. We have eliminated any mention of the visualization recommendation notion,
and focus on the fact that \zq is a language that supports querying over visualizations. 
We have completely rewritten the introduction and the related work sections 
to emphasize these notions. 


\com{10. Contribution and Positioning to Other Works/tools: databases that have query languages, data mining tools, and visual analytics tools. The paper makes comparisons to all three but these comparisons are more at the level of "user-friendliness".  What is needed is also a comparison at the level of expressivity and functionality.
}

See response to MetaReview point 2.


\com{11. Paper structure:
The paper organization is rather unorthodox and confusing. 
(i) Section 2 starts with examples of the Query Language using a table syntax and then explains the table syntax. I think we could skip the examples or move them after explaining the syntax. ... It would be best to focus on a few that ... are also representative of the query capabilities
(ii) Then Section 3 is query execution followed by the system architecture followed by experiments and finally followed by the relational algebra. why not finishing with the query language, then presenting an overview of the system, then explaining the particular components of the system around query execution...? 
}
We agree with the reviewer: we have made significant changes to the organization and presentation.
(i) We have completely rewritten Section~\ref{sec:querylanguage} 
and eliminated the early examples
and focused on the intuition behind the key language functionalities
with a minimal number of examples.
(ii) We have eliminated the algebra from the main body of the paper---the rest of the paper
did not depend on this. Since we significantly shortened the architecture section---focused 
primarily on describing a screenshot---we believe it is
best placed before the user study, where it is most relevant. The query execution section 
is self-contained, and does not require any concepts from the architecture section. 
Also see response to MetaReview point 1 for overall organizational changes. 


\com{12. Query Language:
\begin{inparaenum}[(i)]
\item The paper should add a summary of the capabilities and limitations of the language. 
\item How are joins expressed in ZQL? How are they mapped to SQL? 
\item ZQL queries can be supported in Java through the Java client library. Why would one use ZQL in Java vs any visualization language (e.g. D3) coupled with SQL (assuming that he is already programming in Java?
\item The Constraints and Viz sections are quite short. What type of operations does it support? It supports filtering but does it support any functions over column values, such as taking the average of a column or concatenating strings or adding values, etc, before filtering them? What type of processing on the values can be done before they mapped, what type of functions are supported, e.g. take the log of X values?
\item Please discuss how the (process) functions cover the breadth and diversity of visual analytics tasks. What kind of variants of these functions can the user define?
\item Section 2 provides one view of the language while section 7 describes the relational algebra behind it. First of all, everything about the language should be in one place. Second, section 7 is confusing because ... the two sections seem disconnected to large degree.
\end{inparaenum}
}

We thank the reviewer for the suggestions. 
Overall, we have rewritten most of  
the query language section, taking the reviewer's comments into account.
Specifically, we have eliminated the upfront examples, and focused instead
on the key concepts, and the examples to illustrate them. 
We have tried to be as formal and careful about describing features of the language,
while also providing intuition about the utility.
Specifically, the process column discussion has expanded, 
and we have added a detailed discussion on capabilities and limitations.

We answer point-by-point below:
\begin{inparaenum}[(i)]
\item We agree. We have added a detailed discussion on capabilities and limitations 
in Section~\ref{subsec:cap-lim}.
We have articulated how \zq's primary contribution is as a 
query language over collections of visualizations---composing, filtering, sorting,
and comparing visualizations iteratively.
On the other hand \zq is not appropriate for any sort of data modification
or data transformation, among other functionalities that \sql can support,
such as recursion and nesting.
\item We have added a short line about how joins are supported to the paper.
%\agpyell{Add.}
\item This is already addressed in the related work comparison---see response to MetaReview point 2.
In short, \sql is very cumbersome to near impossible to use, and inefficient for the queries \zq is good at.
The benefit of the {\tt Java} library is that some users may want to develop domain specific 
visualization tools that compile down to \zq queries issued via {\tt Java}. 
\item We have folded the Constraints column into the discussion of the Z column, and we are 
now spending more time clearly explaining the capabilities of these columns.
In short, while the Viz column does support certain fixed types of aggregations
and binning, it doesn't support arbitrary functions.
Further, none of the other columns support data transformations. This is
one of the main limitations of \zq as it stands, and is described in Section~\ref{subsec:cap-lim}.
%\agpyell{alkim check}
\item We have simplified the presentation of the process functions as well, and we
now clarify the various ways the process functions can be used, and
how it can be extended.
%\agpyell{alkim check}
\item We have removed Section 7 (former \vzalg discussion) from the main body of the paper,
reducing this concern. In the technical report, we have tried to be more consistent when
rewriting the section.
\end{inparaenum}


\com{13. Query Execution: The translation is described very briefly making it hard to understand the mechanism ... furthermore, how are the Viz, X, Y parts translated to? Obviously, they are not translated to SQL, are they? Provide an example of a ZQL and its translation ... use this example to illustrate the optimizations of Section 3.2 too. The language supports three simple functions ... How are these functions translated into the executable SQL code?
}

(also raised by Reviewer 3)

We thank the reviewers for the excellent suggestions. 
We agree that our previous query execution section described the translation and optimization strategies
in an excessively terse manner.
To remedy this (and also because we now have a host of additional optimizations),
we have rewritten the query execution and optimization section (Section~\ref{subsec:query_execution}) in its entirety.
For the query execution, we have added 
a clear step-by-step description of the entire translation process. 
This includes the mapping for all of the columns except Process, which are mapped
I%\agpyell{alkim check Viz}
to portions of the \sql queries, and for the processes. We have also considerably
clarified the presentation of the processes in Section~\ref{sec:querylanguage}).
We also made sure that the same examples were used for the optimization
discussion.

%, to this section by using the same example for the optimization discussion, 
%which was covered in our response to MetaReview point 4. 


\com{14. System:
\begin{inparaenum}[(i)]
\item Figures 3 and 4 are almost invisible ... 
\item  The front-end description does not add much... 
\item I would first show the system and then focus on its main components.
\item Section 3 needs to clearly refer to the main system components of Figure 2 (maybe as separate subsections). 
\end{inparaenum}
}
Responses below:
\begin{inparaenum}[(i)]
\item While it is still hard to read the font of the screenshot, 
we have now added a large font overlay --- only this text is meant to be read.
We have eliminated one of the two figures.
\item We have eliminated most of the description of the front-end and only kept the essential parts.
\item We now show the system screenshot as the first step.
\item We have eliminated the system components diagram (Figure 2), and kept
  Section 3 self-contained.
The architecture section is now a short section primarily focused on what is needed to understand
the user study and the experimental evaluation.
\end{inparaenum}

\com{15. Experiments:
I have hard time understanding the effect of optimizations ... 
I think a more comprehensive study would be more helpful and insightful. 
For example, show performance based on the number of visualizations, ....
}

We thank the reviewer for this suggestion --- based on the suggestion 
we have thoroughly revamped the experimental section by conducting performance
evaluation studies on varying all of the parameters the reviewer suggests,
among others. The results can be found in Section~\ref{sec:experiments}.

\com{16. Experiments: For the user study, the authors prepared the tasks ... Were they tasks better suited for ZenVisage? ... It would be fairer ... if the tasks were actually diverse and the study would show where the current system excels and where not. In fact, one could organize two-level study. first, a variety of analytics tasks are chosen. The second level could focus on specific tasks (for which Zenvisage is appropriate) and show how well it performs.
}

We agree with the reviewer's point --- it's not clear if the 
tasks are indeed diverse enough, and we really appreciated
the suggestion of performing a two-stage study 
where we first identify a variety of analytics tasks
and test their relevance, and then focus on specific tasks
for \zv. 
We have done precisely that. 

Please see response to MetaReview point 3. 

% We conducted an additional user interview with data analysts to augment the decisions behind our task selection. We probed the different type of tasks analysts work on during their daily activities, and we reference the taxonomy of low-level analytical tasks described by Amar et al. \cite{amar2005low} to categorize the tasks. We cross-referenced the low-level task list with the actions completed by the user study participants to examine the breath of activities our tasks covered. We rewrote the user study section to more accurately describe where \zv excels over existing tools (identifying correlations, anomalies, and clustering similar attributes) and where \zv does not offer improvements.



%\com{Too much breadth and many dependencies to the technical report. Needs focus.}



\subsection*{Reviewer 3}
\com{17. ...the proposed ZQL language is quite like breaking the visual analytics task step by step and describing each step through a sub-query, which could also be described using SQL sub-query. How much user effort could be reduced by using ZQL? ...
}

See response to MetaReview point 2.


% The reviewer brings up an important question: can \sql replace \zq in functionality? 
% As it turns out, the answer is yes for 
% certain types of \zq queries, but not all queries. 
% We now provide a \sql translation for a \zq query in Table~\agp{xxx} in our
% paper---this translation assumes 
% that the distance function $D$ is Euclidean.
% For any other distance functions, 
% we are not aware of any way of issuing a \sql
% query to replace \zq. 
% Furthermore, there are other types of processors 
% which similarly cannot be replaced
% directly with \sql.
% However, the more problematic aspect is that the \sql query thus written is
% fairly complicated and hard to understand and debug;
% it also necessarily involves some complex \sql constructs,
% that are not supported universally across all database systems,
% and are poorly optimized. 
% Our user study participants, for example, despite knowing and using \sql,
% did not think \sql is an appropriate language to issue these types of requests.
% We have added a detailed description to the related work section to describe
% the comparison of \zq with \sql. 
% We have additionally added experiments that demonstrate that the
% \sql queries of this type take a very long time to be executed (in Section~\agp{xxx})



\com{18. ...the query execution section presents the translation approach and optimization strategies too briefly. More algorithmic details and examples would be good for the readers.}

See response to Reviewer 2 point 13.


\com{...zenvisage aims to provide an interactive visual analytics system, but the overall performance takes tens of seconds as shown in Figure 6, it is a bit too long for interactive analytics. For the user, they only care about the overall performance, I am wondering what the major part of the time consumed in the system.}

We thank the reviewer for the suggestion 
--- we now have a breakdown in the paper for the time consumed by our
optimization algorithms.
Furthermore, we reimplemented the \zq engine to use a much faster array-based
index (as opposed to a hash-based index, which along with our optimizations, provided us with a 50$\times$
speedup in processing.
%each step of \fuse, our new optimization algorithm.
%\tar{we may want to highlight we reimplemented the task-processors using arrays and used cache-based optimizations to gain upto 50X speedup in processing, making task-processors 
%take tiny fraction of the overall execution time}
In short, our algorithm is only non-interactive for practical queries when the time it takes
to run a single group-by query on the dataset (essentially the cost of a single
scan) is non-interactive. 
%Essentially, the time for \fuse is a small multiple of the time to take a run single group-by query.
We describe in detail the changes to the optimization, and the explanation for how we investigated
where the bottlenecks to interactivity are --- along with an additional experiment on Vertica --- in the response to the MetaReview point 4.



% In our previous version, we were using relatively naive optimization schemes, as a result of which the overall
% performance took tens of seconds---after developing additional optimization techniques, capturing 
% combination, speculation, batching, and caching, practical queries on real datasets now take orders of XXX\agp{xxx} seconds. 
% Also to address the issue raised by the reviewer, we have added an experimental breakdown
% in Figure~\ref{xxx}\agp{xxx} that displays where the time is being spent in the system.
% In short, we find that the bulk of the time is spent in the \sql queries that are issued,
% as opposed to the task processing. \agp{xxx}.
% Note however, we are fundamentally limited by the size of the dataset---if a 
% single sequential scan takes \agp{xxx} seconds, then it is impossible for us to 
% achieve better times than that, without adding on additional
% optimizations such as sampling and precomputation. 
% We plan to explore these additional optimizations
% in future work. 
% We have additionally added an experiment to demonstrate that as well---in Figure~\agp{x}, we show
% that our optimizations lead to a moderate complexity \zq query taking not more
% than \agp{xx}x of the time taken for a single group-by query on the entire dataset
% on PostgreSQL.



==> docs copy/experiments-new.tex <==
%!TEX root=zenvisageql.tex

\vspace{-4pt}
\section{Experimental Study}
\label{sec:experiments}
\vspace{0pt}

In this section, we evaluate the runtime performance of the \zq engine.
We present the runtimes for executing both synthetic and realistic \zq queries
and show that we gain speedups of up to 3$\times$
with the optimizations from Section~\ref{subsec:query_execution}.
We also varied the characteristics of a synthetic \zq query to observe
their impact on our optimizations. Finally, we show that disk I/O
was a major bottleneck for the \zq engine, and if we switched our back-end
database to a column-oriented database and cache the dataset in memory, we
can
achieve interactive run times for datasets as large as 1.5GB.

%In this section, we evaluate the impact of the query optimizations (described in Section~\ref{subsec:query_execution}) on
%both synthetic and real datasets. We show the impact of following parameters on query optimizations:
%number of visualizations, complexity of \zq queries, complexity of task 
%processors, and the size of the datasets. Orthogonal to our query optimization evaluation, 
%we explain that disk IO is the major bottleneck is making zenvisage interactive as the size 
%of dataseset increases, and show that \zv is capable of providing interactive response times 
%on vertica database when allocated with a large memory for it to cache all rows.  

\paragraph{Setup.}
All experiments were conducted on a 64-bit Linux server
with 8 3.40GHz Intel Xeon E3-1240 4-core processors and 8GB of
1600 MHz DDR3 main memory. We used 
PostgreSQL with working memory size set to 512 MB and shared buffer
size set to 256MB for the majority of the experiments; the last set of 
experiments demonstrating interactive run times additionally 
used Vertica Community Edition with a
working memory size of 7.5GB.

\techreport{
\paragraph{PostgreSQL Modeling.}
For modeling the performance
on issuing multiple parallel queries with varying number of group by values, 
we varied the 
number of parallel queries issued (\#Q) from 1 to 100,
and the group by values per query (\#V) from 10 to 100000, 
and recorded the response times (T).
We observed that the time taken for a batch of queries was 
practically linearly dependent 
to both the number of queries as 
well as the group by values. 
Fitting a linear equation by performing 
multiple regression over the observed data, 
we derived the following cost-model,
$$ T(ms)= 908\times(\#Q) + 1.22\times\frac{(\#V)}{100} + 1635$$
As per the above model, adding a thread leads to the same rise in response time as increasing the number 
of group by values by 75000 over the existing threads in the batch. In other words, it is better to merge queries 
with small number of group by values. Moreover, since there is a fixed cost (1635 ms) associated with
every batch of queries, we tried to minimize the number of batches by packing as many queries as possible 
within the memory constraints.
}




\paragraph{Optimizations.} The four versions of the \zq engine we use are:
\begingroup
\plitemsep=.2em
\pltopsep=.2em
\begin{inparaenum}[(i)]
\item \noopt: The basic translation from Section~\ref{subsec:query_execution}.
\item \para: Concurrent \sql queries for independent nodes from Section~\ref{sec:para}.
\item \spec: Speculating and pre-emptively issuing \sql queries from Section~\ref{sec:spec}.
\item \fuse: Query combination with speculation from Section~\ref{sec:comb}. %\emph{Final version.}
\end{inparaenum}
\endgroup
\noindent In our experiments, we consider \noopt and the MQO-dependent \para to be our
baselines, while \spec and \fuse were considered to be completely novel optimizations.
For certain experiments later on, we also evaluate the performance of the caching optimizations 
from Section~\ref{sec:cache} on \fuse.
 
\begin{table*}
\vspace{-5pt}
\small
%  \vspace{0pt}
%\scriptsize
  \scalebox{0.90}{
%  \begin{adjustbox}{center}
    \begin{tabular}{|C{1pt}|L{220pt}|C{33pt}|C{33pt}|C{30pt}|C{30pt}|C{30pt}|C{40pt}|C{48pt}|}
      \hline
      & Query Description & \# \cnode[s] & \# \pnode[s] & \# $T$ & \# $D$ & \#
      Visualizations & \# \sql Queries: \noopt & \# \sql Queries: \fuse \\
      \hline
      1 & Plot the related visualizations for airports which have a correlation
      between arrival delay and traveled distances for flights arriving there.
     % 
     % average delays and traveled distances for flights going to
     % airports which have a correlation between arrival delay and traveled
     % distance for flights arriving at that airport.
      & 6 & 3 & 670 & 93,000 & 18,642 & 6 & 1 \\ \hline
      2 & Plot the delays for carriers whose delays have gone up at airports
      whose average delays have gone down over the years.
      & 5 & 4 & 1,000 & 0 & 11,608 & 4 & 1 \\ \hline
      3 & Plot the delays for the outlier years, outlier airports, and outlier
      carriers with respect to delays.
      & 12 & 3 & 0 & 94,025 & 4,358 & 8 & 2 \\ \hline
    \end{tabular}
%  \end{adjustbox}
}
%
%\begin{tabular}{|p{1cm}|p{10cm}|p{2cm}|p{2cm}|p{2cm}|}      \hline
%      \# & Query & \#taskprocessors & \# sql queries (avg groupby vals) before smartfuse & \# sql queries (avg groupby vals) after smartfuse \\ \hline	
%       1 & find all destination airports where the increase in average arrival delays over the years is correlated with increase in the distance travelled by fights arriving there, and not because of the increase in flights' departure delays. For these airports, plot average arrival delays, departure delays and distance by flights arriving there over the years.   & 3 (T, D and T) & 6 (3.2k)	& 1 (24k) \\ \hline																			
%       2 & find pairs of origin and destination airports between which the departure and arrival delays of flights have decreased over the years, for these pairs of airports find all flight carriers that show the opposite behaviour, i.e, their delays have gone up over the years, and plot their delays over years.  & 4 (T, T, T and T) & 4 (3k)	& 1 (38k) \\ \hline	
%       3 & a multi-step drill down query where we first find 5 years where the  average delay patterns were most different, over those five years find the top 5 airports with most different average delay patterns, and finally find the carriers that show most different average delay patterns with destination as these airports over the 5 years. We plot the average arrival delays over the months as well as destination airports for these flights over the 5 years  & 3 (D, D and D) & 8 (300) &  2 (32k) \\ \hline		
%				     	
%\end{tabular}
   \vspace{-5pt}
   \caption{Realistic queries for the airline dataset with the \# of
   \cnode[s], \# of \pnode[s], \# of $T$ functions calculated, \# of $D$ functions
 calculated, \# of visualizations explored, \# of \sql queries issued with
 \noopt, and \# of \sql queries issued with \fuse per query.}
  \label{tab:realworldqueries}
  \vspace{-15pt}
\end{table*}

\noindent
%\textbf{Modeling} \tar{Will wait for Alkim to finish optimization section, we just need to say what values we set for constants, do we also need to talk how we did the modeling?}


%For the first two experiments, we load the data in postgresql without any indexing.
\begin{figure}[!h]
\vspace{-10pt}
\begin{center}
  \begin{subfigure}[c]{0.48\columnwidth}
    \includegraphics[width=\textwidth]{figs/optreal20m.pdf}
  \end{subfigure}
  \begin{subfigure}[c]{0.48\columnwidth}
    \includegraphics[width=\textwidth]{figs/chain.pdf}
  \end{subfigure}
\end{center}
\vspace{-20pt}
\caption{Runtimes for queries on real dataset (left) and single chain synthetic query (right)}
\vspace{-8pt}
\label{fig:optrealnviz}
\end{figure}



\begin{figure}[!h]
\vspace{-5pt}
\begin{center}
\includegraphics[width=0.48\columnwidth]{figs/optsynparamviz.pdf}
%\includegraphics[width=0.48\columnwidth]{figs/optsynparamtp.pdf}
\includegraphics[width=0.48\columnwidth]{figs/optsynparamnodes.pdf}
\end{center}
\vspace{-20pt}
\caption{Effect of number of  visualizations (left) and length
of the chain (right) on the overall runtimes.}
\vspace{-15pt}
\label{fig:optsynviz}
\end{figure}

\vspace{2pt}
\subsection{Realistic Queries}
\vspace{-3pt}

For our realistic queries, we used 20M rows of a real 1.5GB airline
dataset~\cite{airlinedata} which contained the details of flights within the
USA from 1987-2008, with 11 attributes. On
this dataset, we performed 3 realistic \zq queries inspired by the case
studies in our introduction. Descriptions of the queries can be found in Table~\ref{tab:realworldqueries}.

Figure~\ref{fig:optrealnviz} (left) depicts the runtime performance of the
three realistic \zq queries, for each of the optimizations. 
For all queries, each level of optimization provided a substantial speedup
in execution time compared to the previous level.
{\em Simply by going from \noopt to \para, we saw a 45\% reduction in runtime. From
\para to \spec and \spec to \fuse, we saw 15-20\% reductions in
runtime}.
A large reason for why the optimizations were so effective was because \zq
runtimes are heavily dominated by the execution time of the issued \sql
queries. In fact, we found that for these three queries, 94-98\% of the overall
runtime could be contributed to the \sql execution time. We can see from
Table~\ref{tab:realworldqueries}, \fuse always managed to lower the number of
\sql queries to 1 or 2 after our optimizations, thereby heavily impacting the
overall runtime performance of these queries.

\vspace{-2pt}
\subsection{Varying Characteristics of {\large \zq} Queries}
\vspace{-2pt}

We were interested in evaluating the efficacy of our optimizations with respect
to four different characteristics of a \zq query:
\begin{inparaenum}[(i)]
\item the number of visualizations to explore,
\item the complexity of the \zq query,
\item the level of interconnectivity within the \zq query, and
\item the complexity of the processes.
\end{inparaenum} 
To control for all variables except these characteristics, we used a synthetic
chain-based \zq query to conduct these experiments. Every row of the
chain-based \zq query specified a collection of visualizations based on the
results of the process from the previous row, and every process was applied on
the collection of visualizations from the same row. Therefore, when we created
the query plan for this \zq query, it had the chain-like structure depicted by
Figure~\ref{fig:optrealnviz} (right).
Using the chain-based \zq query, we could then
\begin{inparaenum}[(i)]
\item vary the number of visualizations explored,
\item use the length of the chain as a measure of complexity,
\item introduce additional independent chains to decrease
  interconnectivity, and
\item increase the number of loops in a \pnode[] to control the complexity of
  processes.
\end{inparaenum}

\smallskip
\noindent To study these characteristics, we used a 
synthetic dataset with 10M rows and 15 
attributes (10 dimensional and 5 measure) 
with cardinalities of dimensional attributes varying from 10 to 10,000. 
By default, we set the input number of visualizations per chain to be 100,
with 10 values for the X attribute, 
number of \cnode[s] per chain as 5, the process as $T$ (with a single for loop)
 with a selectivity of .50, and  number of chains as 1.

\paragraph{Impact of number of visualizations.} 
Figure \ref{fig:optsynviz} (left) shows the performance of \noopt, \spec, and
\fuse on our chain-based \zq query as we increased the number of visualizations
that the query operated on. The number of visualizations was increased by
specifying larger collections of Z column values in the first \cnode[]. We
chose to omit \para here since 
it performs identically to \noopt.
With the increase in visualizations, the overall response time increased for
all versions
because the amount of processing per \sql query increased. \fuse showed better
performance than \spec up to
10k visualizations due to reduction in the total number of \sql queries issued.
However, at 10k visualization, we reached the threshold of the number of unique
group-by values per combined query (100k for PostgreSQL), so it was less optimal
to merge queries. At that point, \fuse behaved similarly to \spec.

\begin{figure}[!h]
\vspace{-10pt}
\begin{center}
%\includegraphics[width=0.48\columnwidth]{figs/optsynparamnodes.pdf}
\includegraphics[width=0.48\columnwidth]{figs/optsynparamchains.pdf}
\includegraphics[width=0.48\columnwidth]{figs/optsynparamtp.pdf}
\end{center}
\vspace{-15pt}
\caption{Effect of number of independent chains (left) and the number of loops
in a \pnode[] (right) on the overall runtimes.}
\vspace{-10pt}
\label{fig:opt_syn_nodes}
\end{figure}



\paragraph{Impact of the length of the chain.}
We varied the length of the chain in the query plan (or the number of rows in
the \zq query) to simulate a change in the complexity of the \zq query and
plotted the results in Figure~\ref{fig:optsynviz} (right). As the number of
nodes in the query plan grew, the overall runtimes for the different
optimizations also grew. However, while the runtimes for both \noopt and \spec
grew at least linearly, the runtime for \fuse grew sublinearly due to its query
combining optimization. While the runtime for \noopt was much greater than for \spec,
since the overall runtime is linearly dependent on the number of
\sql queries run in parallel, we see a linear growth for \spec.

\paragraph{Impact of the number of chains.}
We increased the number of independent chains from 1 to 5 to observe the effect
on runtimes of our optimizations; the results are presented in
Figure~\ref{fig:opt_syn_nodes} (left). While \noopt grew linearly as expected, all
\para, \spec, and \fuse were close to constant with respect to the number of
independent chains. We found that while the overall runtime for concurrent \sql
queries did grow linearly with the number of \sql queries issued, they grew much
slower compared to issuing those queries sequentially, thus leading to an
almost flat line in comparison to \noopt. 

\paragraph{Impact of process complexity.}
We increased the complexity of processes by increasing the number of loops in
the first \pnode[] from 1 to 2. For the single loop, the \pnode[] filtered
based on a positive trend via $T$, while for the double loop, the \pnode[] found
the outlier visualizations.
Then, we varied the number of visualizations to
see how that affected the overall runtimes. Figure~\ref{fig:opt_syn_nodes}
(right) shows the results. For this experiment, we compared regular \fuse with
cache-aware \fuse to see how much of a cache-aware execution made.
We observed that there was not much difference
between cache-aware \fuse and regular \fuse below 5k visualizations when all
data could fit in cache.
After 5k visualizations, not all the visualizations could be
fit into the cache the same time, and thus the cache-aware execution of the
\pnode[] had
an improvement of 30-50\% as the number of visualizations increased from 5k to
25k. However, this improvement, while substantial, is only a minor change in 
the overall runtime. 
% However, this improvement was only in the execution of the process, and
% since \sql queries still heavily dominated,  it was a minor change
% in the overall runtime.


 
%For our experiments, we used the following datasets and queries:
%\begin{inparaenum}[(i)]
%\item We used a synthetic dataset with 10M rows and 15 attributes (10 dimensional and 5 measure) with cardinalities of dimensional attributes varying from 10 to 10000. 
%For evaluationg the impact of different parameters, we created a synthetic \zq query consisting one or more chains of visual component and process nodes \tar{should we add a diagram, or say it looks similar to Figure 2 when set to have two chains?}.
%Each chain starts with a collection of visualizations, on which further filtering or transformations are applied by the subsequent nodes in the chain. By default, we set the input number of visualizations per chain to be 100, number of visual component nodes per chain to be 5, task processor to be T (consisting of a single for loop) with selectivity of .50, and  number of chains to be 1. Each visualization consists of 10 X groups. 
%%For depicting the impact of the number of visualizations, we varied the input number of visualizations from 1 to 10k, for complexity of \zq queries, we varied the number of visual component nodes in a chain from 1 to 5 as well as varied the number of chains from 1 to 5, and for complexity of task processors, we showed the performance of task-processors with 1 and 2 loops over varying number of visualizations.
%
%\item A real airline dataset~\cite{airlinedata} with different number of rows: 2M,20M, and 120M. We used 20M as the default number of rows. \tar{why? need to think of a good reason saying 20M reflects the standard dataset size}. We use three 3 realistic queries as depicted in Table ~\ref{tab:realworldqueries}. 
%\later{
%\begin{inparaenum}[(i)]
%\item Query 1: find all destination airports where the increase in average arrival delays over the years is correlated with increase in the distance travelled by fights arriving there, and not because of the increase in flights' departure delays. For these airports, plot average arrival delays, departure delays and distance by flights arriving there over the years. This query has 5 visual component nodes
%\item Query 2: find pairs of origin and destination airports between which the departure and arrival delays of flights have decreased over the years, for these pairs of airports find all flight carriers that show the opposite behaviour, i.e, their delays have gone up over the years, and plot their delays over years.
%\item Query 3: a multi-step drill down query where we first find 5 years where the  average delay patterns were most different, over those five years find the top 5 airports with most different average delay patterns, and finally find the carriers that show most different average delay patterns with destination as these airports over the 5 years. We plot the average arrival delays over the months as well as destination airports for these flights over the 5 years. 
%\end{inparaenum}
%}

%\end{inparaenum}

\vspace{-2pt}
\subsection{Interactivity}
\vspace{-2pt}

The previous figures showed that the overall execution times of \zq queries took
several seconds, even with \fuse, thus perhaps indicating
\zq is not fit for interactive use with large datasets.
However, 
we found that this was primarily due
to the disk-based I/O bottleneck of \sql queries. In
Figure~\ref{fig:optrowcolumstores} (left), we show the \fuse runtimes of the
3 realistic queries from before on varying size subsets of the airline dataset,
with the time that it takes to do a single group-by scan of the dataset. As we
can see, the runtimes of the queries and scan time are \emph{virtually the
same}, indicating that \fuse comes very close to the optimal I/O runtime
(i.e., a ``fundamental limit'' for the system). 

To further test our hypothesis, we ran our \zq engine with Vertica with a large
working memory size to cache the data in memory to avoid expensive disk I/O. The
results, presented in Figure~\ref{fig:optrowcolumstores} (right), showed that
there was a 50$\times$ speedup in using Vertica over PostgreSQL with these
settings. Even with a large dataset of 1.5GB, we were able to achieve
sub-second response times for many queries. Furthermore, for the dataset
with 120M records (11GB, so only 70\% could be cached), we were able to
reduce the overall response times from 100s of seconds to less than 10 seconds.
Thus, once again, \zv returned results in a small multiple of the time 
it took to execute a single group-by query.
\noindent
Overall, \fuse is interactive on moderate sized datasets on PostgreSQL, or on 
large datasets that can be cached in memory and operated on using a columnar database---which 
is standard practice adopted by visual analytics tools~\cite{tableau-inmem}. 
Improving on interactivity is impossible due to fundamental limits to the system;
in the future, we plan to explore returning approximate answers using samples,
since even reading the entire dataset is prohibitively slow. 


% \alkim{For providing
%   interactivity, existing visual analytics tools either cache all the data
%   inmemory, or make use of large inmemory databases for avoiding expensive disk
%   ios, which are orthogonal to the query optimization technique we propose in
% this paper. This is a good sentence, we should have it somewhere.}

% Finally, note that even with a disk-based PostgreSQL and non-interactive
% response times, \zv is still an overall very useful system, since it automates
% the search for patterns. This drastically reduces number of man hours required
% to find visual insights in a dataset, and it is not unreasonable to think that
% a visual analyst would issue many \zq queries and perform some other task while
% waiting for the results.


%A real airline dataset~\cite{airlinedata} with different number of rows: 2M,20M, and 120M. We used 20M as the default number of rows. \tar{why? need to think of a good reason saying 20M reflects the standard dataset size}. We use three 3 realistic queries as depicted in Table ~\ref{tab:realworldqueries}. 
%\alkim{It's still useful even though not interactive cuz it removes manual
%labor}
%results of query optimizations. For demonstrating interativity of our system, we used Vertica with a 
%large memory size of 7.5GB, (and thus having all rows in memory for 20M flight dataset, and having 
%70\% of the rows in memory for 120M large dataset). 



%\noindent
%\textbf{Effect of Query Optimizations}
%Figure \ref{fig:optrealnviz} (left) depicts the improvement in performance for three \zq queries on the real airline 
%dataset due to query optimizations discussed in Section ~\ref{subsec:query_execution}.
%By running multiple queries in parallel (see parallel vs no-opt), we observe speed-ups upto 50\% in the overall time.
%Further increasing the number of parallel queries by speculating results in improvement in the response time (see speculate).
%As depicted in Table\ref{tab:realworldqueries}, smartfuse merges multiple threads that process small number of group values into lesser number of threads with more number
%of group by values. As clear from our model, this helps in reducing a large overhead of 900ms that is incurred on creating a new thread, resulting in 
%an improvment of 15-20\% in the response time over speculate.

%\noindent
%\textbf{Time for data retrievel vs post-processing}
%As depicted in Figure \ref{fig:optrealnviz} right, the SQL execution dominated the overall runtime with the post-processing time taking much less time(<500ms) 
%for all three queries. There are three reasons why taskprocessors take less time.First, computation time heavily depends on the number of cache line misses or memory access, however we found that since a large number of visualizations (10k visualizations of 10 groups each) can be cached in L caches (~8MB in size), performing even complicated operations over cached data takes less than 500ms (a minor fraction of the overall query execution times). Secondly, we have implemented functional primitives using array-based data structures, which are 50-60X faster than hash based implementations. Moreover, since arrays are stored sequentially in memory, it leads to comparatively lesser number of cache line misses. Finally, we make use of block based computions while applying functional primitives which minimize multiple memory access while iterating multiple times on the same set of data. 
%
%
%\noindent
%\textbf{Impact of number of visualizations}
%Figure \ref{fig:optsynviz} (left) shows the performance of no-opt,speculate and smartfuse algorithms on
%synthetic dataset as we increase the number of visualizations that a \zq query operates on.
%With the increase in visualizations, the overall response time increases for all optimization
%since the amount of processing per thread increases. smartfuse shows better performance than speculate upto
%10k visualizations due to reduction in thread overhead. However, at 10k visualization, we reach the threshold of 100k groups (since each visualization consists 
%10 X values) per thread at which point it is less optimal to merge thread, in that scenario smartfuse becomes similar to speculate. 
%



%\noindent
%\textbf{Impact of complexity of task-processors}
%Figure \ref{fig:optsynviz} (right) depicts that functional primitives such as T
%which iterate once over visualizations take maximum of 50ms even for large
%number of visualizations (25k). For task processors that need to iterate twice
%over the visualizations, such as once that need to find top k outlier or
%representative visualizations, we observed that there are not much difference
%between block based and without block based operations until 5k visualizations
%(all data in cache). After 5k visualizations, not all visualizations could be
%cached in L caches at a time, and thus the block based task processors depict
%an improvement of 30-50\% as the number of visualizations increased from 5k to
%25k, though still a minor improvement as compared to the overall query
%execution time.

%\begin{figure}[!h]
%\vspace{0pt}
%\begin{center}
%\includegraphics[width=0.48\columnwidth]{figs/optsynzqlvsqltwoloop.pdf}
%\end{center}
%\vspace{-10pt}
%\caption{Performance of zql vs sql for a query where we want to find top 10 similar products (using euclidean distance) for every product. We vary the number of products from 10 to 5000.}
%\vspace{-15pt}
%\label{fig:opt_syn_zqlvssql}
%\end{figure}


%\noindent
%\textbf{Impact of complexity of ZQL queries}
%For evaluating the impact of complexity of \zq queries on query optimizations, 
%we tried varying the number of sequential visual component nodes in a chain  from 1 to 10 (Figure \ref{fig:opt_syn_nodes} left)
%as well as the number of independent visual component nodes by varying the number of chains from 1 to 5 (Figure \ref{fig:opt_syn_nodes} right).
%In both cases, as the number of visual component nodes increases, the number of queries and thus the number of 
%threads and amount of processing per thread increases which leads to an increase in overall time. In the first case, no-opt and parallel show
%similar behaviour since the added nodes are dependent on the nodes earlier in the chain, while in the second case parallel optimization results 
%in simultaneous processing of multiple chains  resulting in a substantail improvement over the no-opt. Similarly,in both cases, speculate
%incurs an overhead of creating a thread for every new node while smartfuse avoids creating additional threads if they can be merged into the existing threads,
%and thus shows an improvement of about 20\% over speculate.

\begin{figure}[!h]
\vspace{-10pt}
\begin{center}
\includegraphics[width=0.48\columnwidth]{figs/optrealrowdataset.pdf}
\includegraphics[width=0.48\columnwidth]{figs/optrealcoldataset.pdf}
\end{center}
\vspace{-20pt}
\caption{\fuse  on PostgreSQL (left) and Vertica (right)}
\vspace{-15pt}
\label{fig:optrowcolumstores}
\end{figure}


%\noindent
%\textbf{Interactivity}
%Figure\ref{fig:optrowcolumstores}  depicts the time taken by three real world
%queries when applying swiftfuse optimization based query execution as compared
%to a single group by query on datasets of size 2M, 20M and 120M. As the size of
%dataset increases we observe that it is impossible to provide interative
%response time over disk-based relational databases since the time take to apply
%a single group by itself takes multiple seconds and a typical \zq involves
%multiple group by queries even after optimizations. For providing
%interactivity, existing visual analytics tools either cache all the data
%inmemory, or make use of large inmemory databases for avoiding expensive disk
%ios, which are orthogonal to the query optimization technique we propose in
%this paper. Even for \zv, we find (as depicted in
%Figure\ref{fig:optrowcolumstores}) that if we use vertica with large memory
%(7GB) to cache majority of the rows, there is an improvement upto 50X over
%postgresql. For 20M dataset (1.5GB in size and thus completely cached), the
%sub-second overall reponse times, and for 120M dataset (11 GB, about 70\% rows
%cached), we see a reduction in response times from multiple 100s of seconds to
%a few seconds. 
%   


==> docs copy/expressiveness.tex <==
%!TEX root=zenvisageql.tex

\later{
\section{Expressiveness}
\label{subsec:expressivenesss}

So far, we have described, via a collection of examples,
the various types of queries that can be posted using \zq.
A natural question now arises: {\em how can we characterize
the space of queries expressible via \zq?}
In this section, we provide both intuition for the space
of queries expressible via \zq, as well as more formal arguments.
Note, however, that \zq provides considerable flexibility to the user,
specifically via the Process and the Viz column;
as a result, there may be uses of \zq we still haven't foreseen,
and thus, our arguments will be necessarily incomplete.

\subsection{Formalized Capabilities}

We now discuss
the capabilities of \zq more formally.
For the rest of our discussion, 
we will assume that the Viz column 
uses
a simple aggregate, 
as opposed to user-defined interpolation or summarization.
We will relax this restriction later on in the section.






\paragraph{Language Formalization.}
The \zq language is straightforward to describe 
at a high level.
A \zq query $Q$ is formally defined
to be a collection of expressions $E$,
where each 
expression\footnote{\scriptsize Note that while we enforced that every Process must be associated with a Visual Component in our tabular interface, it need not be so; this decision 
was made primarily for compactness and intuitiveness. Here,
we decouple the two.} 
$E$
can be either a Visual Component expression $V$,
or a Process expression $P$.
A Visual Component expression $V$
must contain a tuple of sub-expressions,
for each of $X, Y$ and optionally, $Z_1,$$ Z_2,$$ \ldots,$$ Constraints,$ $Viz$.
A Process expression $P$
consists of three parts: a ranking function expression $S$
describing how the visualizations must be ranked,
a functional expression $F$ describing the computation that determines the ranking, and $k$, describing how many outputs are desired from the ranking.
Thus, formally:

$Q:= \{R\}$ where $ R:= V | P$

$V:= (X, Y, Z_1, Z_2, \ldots, Z_q, Constraints)$

$P:= (S, F, k)$

\noindent We next describe how $V$ and $P$ are interpreted.

\paragraph{Visual Components and Unit Visualizations.}
To describe how $V$ is interpreted,
we begin with the notion
of a {\em unit visualization}.
A unit visualization corresponds to 
a table that is the result of
a query of the following type:
\begin{quote} \small
\begin{verbatim}
SELECT X, A(Y)
FROM R1, R2, ..., Rp
WHERE Conditions
GROUP BY X 
ORDER BY X
\end{verbatim}
\end{quote}
where {\tt X, Y, A, Conditions} can vary.
Thus, a unit visualization corresponds to
a two-attribute aggregated table.
Such two-attribute tables can be readily visualized.
It is easy to see that the following holds:
\vspace{-5pt}
\begin{lemma}
Every visual component generates one or more unit visualizations.
\end{lemma}
We define a {\em unit visualization cross-product}
to be all unit visualizations formed from:
 combining
any $X_i$ in a set of attributes \overl{$X$}, 
any $Y_j$ in a set of attributes \overl{$Y$},
such that attribute $Z_i$ is equated to any attribute value $v_i$ in a set \overl{$V_i$}.
These visualizations can be represented using the following query,
where $X_i, Y_j, v_1, ..., v_q$ can vary:
\begin{quote} \small
\begin{verbatim}
SELECT Xi, A(Yj) 
FROM R1, R2, ..., Rp
WHERE Z1 = v1 AND ... AND Zq = vq AND Conditions
GROUP BY Xi
ORDER BY Xi
\end{verbatim}
\end{quote}
We have the following:
\begin{lemma}
Any unit visualization cross-product can be represented using a visual component.
\end{lemma}
\vspace{-5pt}
Thus, unit visualizations have close ties
to the visual components:
essentially, the visual components enable us
to assemble a collection of unit visualizations
by retrieving data from the database.

\paragraph{Visual Component Processor.}
%\agp{correspondence to axis variables? to polaris table algebra?}
We now describe how a visual component expression $V$ 
is processed
within \zv. 
To do that, we need to formally define name and axis variables. 
Name variables are variables that contain an array of unit
visualizations.
(As a result, we can say that each name variable corresponds
to a sequence of visualizations.)
Axis variables, on the other hand are variables 
that contain an array of elements: this could be attribute values,
or names of attributes themselves. 


\begin{figure}[!h]
\vspace{-5pt}

\begin{center}
\includegraphics[width=0.9\columnwidth]{figs/types.pdf}
\includegraphics[width=0.9\columnwidth]{figs/process-types.pdf}

\end{center}
\vspace{-10pt}
\caption{Visual Component Processor Flow (above) Task Processor Flow (below)}
\label{fig:flow}
\vspace{-5pt}
\end{figure}

A visual component processor 
(depicted in Figure~\ref{fig:flow} (top)) 
accepts as input
a visual component expression $V$,
as well as values for unspecified 
input axis variables $u_1, ..., u_n$,
within the visual component expression.
The output is an instantiation of the 
name variable: that is, it is an array of 
unit visualizations.
Additional outputs may include 
instantiations of output axis variables.
(These are used to refer to 
specific aspects or metadata of the unit visualizations.)
For instance, one axis variable $v_i$ may hold
an array with the values taken on by attribute $Z_i$
for each unit visualization in the name variable array.

\begin{figure}
\begin{center}
\vspace{-10pt}
\includegraphics[width=\columnwidth]{figs/patterns.pdf}
\end{center}
\vspace{-10pt}
\caption{Patterns in Task Computation (left: star pattern,  middle: complete graph pattern, right: bipartite pattern)}
\label{fig:patterns}
\vspace{-15pt}
\end{figure}

\paragraph{Task Processor.}
A task processor takes as a process expression $P$, 
as well as values for the 
unspecified input axis variables $u_1, ..., u_n$,
and unspecified name variables 
(or arrays of unit visualizations) $f_1, ..., f_m$.
It then generates instantiations of output axis variables. 



Thus, the Task Processor accepts a 
sequence of unit visualizations as input via name variables,
and performs some sub-selection (filtration) and/or ordering on these visualizations.
The eventual result is some subset of the unit visualizations that
are provided as input, ordered in some way.
Note that instead of generating an instantiation of
a single name variable (like the Visual Component Processor), the task processor instantiates
multiple axis variables: this distinction is important, because
by instantiating multiple axis variables, 
these axis variables could be used to generate multiple sets
of output unit visualizations via Visual Components.
It is the role of the Visual Component Processor to
generate the unit visualizations.

\paragraph{Process Primitives.} For populating
the Process Expression, 
\zq provides a few default functional primitives, 
including $D, T, R$.
Since the process can be overloaded by users
to specify their own user defined functions, it is not clear a-priori 
what types of computation may be possible via the Process expression.

Notice however, that all three of $D, T, R$ are computing
distance of some sort:
$D$ is explicitly computing a distance between a pair of visualizations,
$T$ is checking the overall trend of a visualization 
so is computing a distance between a visualization and the
trend,
$R$ is identifying representatives, and implicitly needs
to compute distances between all pairs of visualizations
in the collection.

Using these three primitives, and how we've used them in queries,
we have identified three patterns of distance computation 
that are expressible
in tasks, and capture all the examples described in the paper.
These patterns are depicted in Figure~\ref{fig:patterns}.
Each node depicts a visualization, while each edge between two visualizations corresponds to a distance computation between them.
The pattern on the left is a {\em star} pattern,
which compares the distance between 
a collection of unit visualizations to
a reference. 
This pattern is used for queries in Table~\ref{tab:motiv-ex-2} and Table~\ref{tab:name-1}.
The pattern in the middle is a {\em complete graph} pattern,
where unit visualizations are all compared against each other.
This pattern is used for queries in Table~\ref{tab:process-2}, Table~\ref{tab:ex-1}, and Table~\ref{tab:ex-4}.
Lastly, the pattern on the right is a {\em bipartite graph} pattern,
where pairs of corresponding unit visualizations
are compared against each other.
This pattern is used for queries in Table~\ref{tab:vars-1} and Table~\ref{tab:vars-3}.


\paragraph{Overall Capabilities.}
Thus, at a high level, 
\zv is tailored towards first, enumerating an array of unit visualizations
using visual components, and second,
task-based computation involving one of the three patterns 
displayed in Figure~\ref{fig:patterns},
to identify unit visualizations within this array 
with desired properties,
followed by repetitions of these two above steps.


% Note that the task cannot be used to compare an arbitrary
% collection of unit visualizations with each other:
% specifically, the schema of these unit visualizations
% must be the same, even if XXX


% \zv provides a few functional primitives by default as discussed in sub-section~\ref{sec:process}, and users can add their own simple primitives, or build complex functions using the simple functions. $F$ takes as input one or more name variables $v*$ pointing to a set of visualizations, and axis variable $a*$ to iterate over the sets. In particular, for each input axis variable, a {\tt for} loop is created and nested. The input axis variables are then used to step through the arrays specified by the name variables $v*$, and F is called at each iteration. $F$ can step through a set of visualizations and give a score based on how closely the visualization meets the objective. $F$ can also iterate through multiple sets of visualizations and compare mutiple visualizations corresponding to the same axis variable value. The output of $F$ is a list of axis variable values, and their scores. A ranking (and filtering) function $R$ is then applied to sort and pick top $k$ axis variable values. The output of the P is an iterator to the top $k$ values returned by $R$ which can be used in $V$ of successive rows.

% \tar{add examples of specific applications that the language can support}

\paragraph{Viz Column.}
So far, we have assumed that the Viz column
uses a simple aggregate for $Y$:
in fact, the Viz column could
apply some restricted set of 
data transformations, binning in arbitrary ways, noise removal,
and mappings to different types of visualizations,
as described in Section~\ref{sec:viz}.
However, as described in that section, we are
directly leveraging the capabilities of the grammar
of graphics to support these operations. 

% Through the Viz column, the language supports data transformations, data summarization, and mapping to different types of visualizations as discussed in sub-section~\ref{sec:viz}: If the summarization is specified in the Viz column, additional clauses and keywords such as {\tt GROUP BY}s and aggregations may be added. Additionally, result visualizer can map the fetched data into the visualization type specified under the Viz column. 

}

\section{Discussion of the Space of Use Cases}

As described above, \zq is targeted at 
generating simple unit visualizations 
via visual components, and then filtrating 
and ordering them via tasks,
which can be fed as input to 
other visual components or output to the user.

The visual components generate unit visualizations: 
the unit visualizations \zq is capable of 
handling correspond to a single 
SELECT-FROM-WH\-ERE-GROUPBY-ORDER; 
complicated nested queries are not the target
of \zv, since they are not usually the target 
of visual data exploration.
The tasks computation is limited to selecting 
visualizations with specific properties
from a set: even this encompasses a large collection of use-cases,
ranging from similarity and 
dissimilarity search, or to check if a visualization
has a specific property, to outlier detection and 
identification of representatives, to finding differences between 
corresponding visualizations, as we saw in the previous sections.

This implies that there is a large swath of data mining 
tasks that are 
not captured by \zq: this includes prediction of any sort, classification,
regression, dimensionality reduction, 
or frequent pattern mining. 
There are other data processing tasks that are not captured
by \zq, including data cleaning or pre-processing, data integration,
or expressing complex queries or computation that don't correspond to the unit visualization template described above.

\later{
\begin{figure}[!htb]
\begin{center}
\includegraphics[width=0.8\columnwidth]{figs/steps.pdf}
\end{center}
\vspace{-20pt}
\caption{The three stages of data analytics currently: the shaded box
is our focus}
\label{fig:steps}
\vspace{-10pt}
\end{figure}
}

Indeed, \zq is not meant to be a one-stop-shop for all of the computation on data:
it is meant to be the next logical step for current data visualization tools,
that severely lack the functionality of helping users find desired patterns
in visualizations
or compare visualizations.
This means that the data is already cleaned before it is
visualized: this is assumed in all data visualization tools. 
This also means that complex analytics, including prediction or mining,
and are not the focus of simple visualization, are better suited for 
subsequent tools.

%In Figure~\ref{fig:steps}, we depict our conceptualization of the three stages of data analytics;
%our target is not the first or the third stages, 
%which are better handled by other tools.
%Instead, our focus is on the middle, second stage,
%which is also the focus of current visual analytics tools.








% \newpage
% \tar{I have merged expressiveness and naive translation into one as they are related, next section could directly be on Query Optimisation.}
% A \zq query $Q$ can be broken up into two parts: the visual components $V$ and the
% the Process column $P$. In the \zq compiler, $V$
% determines the set of data \zv needs to retrieve from the database,and $P$ translates into the post-processing computation to be done on
% the returned data. Formally,

% $Q:$  $R+$  

% $R:$  $V[P]$

% \textbf{[Lemma 1] Since $V$ is translated into one or more relational algebra queries, \zq queries can be executed on relational data, and are limited to the expressive power of relational queries for retrieving data:}
% For each row, the \zq compiler loops over all combinations of values \tar{we can say we use Polaris Table Algebra to determine the combination} for each of the $n$ axis variables in $V$ and for each combination, issues a \sql query, the results of which are stored in the corresponding location in an $n$ dimensional array denoted as $N$. In other words, for each row, at a high level, the \zq compiler issues a \sql query corresponding to each visualization. Each generated \sql query has the form:
% \begin{quote} \small
% \begin{verbatim}
% SELECT X, Y 
% WHERE Z=v and (CONSTRAINTS) 
% ORDER BY X
% \end{verbatim}
% \end{quote}
% \textbf{[Lemma 2] Through the Viz column, the language supports data transformations, data summarization, and mapping to different types of visualizations as discussed in sub-section}~\ref{sec:viz}: If the summarization is specified in the Viz column, additional clauses and keywords such as {\tt GROUP BY}s and aggregations may be added. Additionally, result visualizer can map the fetched data into the visualization type specified under the Viz column. 

% Once the name variable array $N$ has been filled in with results from the \sql queries, the \zq compiler can directly visualize it or pass it as an input to to the Process column $P$. 

% \textbf{[Lemma 3] Process column P supports two kinds of explorations: a) single visualization exploration: how close a visualization matches a specific visual property, and/or b) comparative exploration: compare multiple visualizations and measure how similar they are:} $P$ consists of a functional primitive $F$ and a ranking function $R$.  $F$ are considered black boxes to the \zq compiler and are unaltered. \zv provides a few funtional primitives by default as discussed in sub-section~\ref{sec:process}, and users can add their own simple primitives, or build complex functions using the simple functions. $F$ takes as input one or more name variables $v*$ pointing to a set of visualizations, and axis variable $a*$ to iterate over the sets. In particular, for each input axis variable, a {\tt for} loop is created and nested. The input axis variables are then used to step through the arrays specified by the name variables $v*$, and F is called at each iteration. $F$ can step through a set of visualizations and give a score based on how closely the visualization meets the objective. $F$ can also iterate through multiple sets of visualizations and compare mutliple visualizations corresponding to the same axis variable value. The output of $F$ is a list of axis variable values, and their scores. A ranking (and filtering) function $R$ is then applied to sort and pick top $k$ axis variable values. Formally,

% $P:$  $R(F(v*,a*),k)$

% The output of the P is an iterator to the top $k$ values returned by $R$ which can be used in $V$ of successive rows.
 
% \textbf{Applications}: Using single and comparative visualization exploration based functional primitives, \zv can filter 2D visualizations based on a visual property, can find similar or dissimilar visualizations, can find outliers, can find k nearest- neighbour visualizations, can cluster and pick trends representing each cluster or combinations of these across any of the X, Y or Z dimensions. Other similar data mining tasks can integrated by introducing a functional primitive.

% \textbf{Limitations}: \zq is currently limited to exploration of visualization with only two dimensions. Given that \zq supports only single and comparative visaualization explorations, predictive explorations such as classification, or frequent pattern mining tasks are beyond the scope of the language. Moreover, since V is translated to relational queries, \zq cannot be used where fetching data needed for visualizations depends on recursion, and other query patterns that cannot be expressed using relational algebra \tar{the last point can be more clear}. 



==> docs copy/formal-expressiveness.tex <==
%!TEX root=zenvisageql.tex
\section{Expressiveness}
\label{sec:formal-expr}

In this section, we formally quantify the expressive power of \zq. To this end,
we formulate an algebra, called the \emph{\vzalg}.
Like relational algebra, \vzalg contains a basic
set of operators that we believe all \vzlans should be able to
express.
At a high level, the operators of
our \vzalg operate on sets of visualizations and are not
mired by the data representations of those visualizations, nor the details of how
the visualizations are rendered. Instead, the \vzalg is primarily
concerned with the different ways in which visualizations can be selected,
refined, and compared with each other.

Given a function $T$ that operates on a visualization at a time, 
and a function $D$ that operates on a pair of visualizations at a time, 
both returning real-valued numbers,
a \vzlan $L$ is defined to be
\emph{\vzcmp} $VEC_{T,D}(L)$ with respect to $T$ and $D$ if it supports
all the operators of the \vzalg.
These functions $T$ and $D$ (also defined previously) 
are ``functional primitives'' without which the resulting
algebra would have been unable to manipulate visualizations in the way
we need for data exploration. 
Unlike relational algebra, which does not have any ``black-box''
functions, \vzalg requires these functions for operating on visualizations
effectively. 
That said, these two functions are flexible and configurable and up to the user
to define (or left as system defaults).
Next, we formally define the \vzalg operators and prove
that \zq is  \vzcmp. 

\input{ordered-bag-algebra}

\subsection{Basic Notation}
Assume we are given a $k$-ary relation $\calR$ with attributes
$(A_1,A_2,\dots,A_k)$.
Let $\calX$ be the unary relation with attribute X whose values are the
names of the attributes in $\calR$ that can appear on the x-axis. If the
x-axis attributes are not specified by the user for relation $\calR$, the
default behavior is to include all attributes in $\calR$: $\{A_1,\dots,A_k\}$. Let
$\calY$ be defined similarly with Y for attributes that can appear on the y-axis.
Given $\calR$, $\calX$, and $\calY$, we define $\calV$, the \emph{\vzuni},
as follows: $
  \calV = \nu(\calR) = \calX \times \calY \times
  \left(
    \mathlarger{\mathlarger{\times}}_{i=1}^k \pi_{A_i}(\calR) \cup \{*\}
  \right)$
where $\pi$ is the projection operator from relational algebra and \wild
is a special wildcard symbol, used to denote all values of an attribute.
Table~\ref{tab:setup} shows an example of what a sample $\calR$ and
corresponding $\calX$, $\calY$, and $\calV$ would look like.
\techreport{
    At a high level, the visual universe specifies all subsets of data that may
    be of interest, along with the intended attributes to be visualized. Unlike
    relational algebra, \vzalg mixes schema and data elements, but in a special
    way in order to operate on a collection of visualizations.
}


% \scalebox{0.71}{
%    \begin{tabular}{|c|c|c|c|c|c|}
%       \hline
%       year & month & product & location & sales & profit \\ \hline
%       2016 & 4 & chair & US & 623,000 & 314,000 \\ \hline
%       2016 & 3 & chair & US & 789,000 & 410,000 \\ \hline
%       2016 & 4 & table & US & 258,000 & 169,000 \\ \hline
%       2016 & 4 & chair & UK & 130,000 & 63,000 \\
%       \multicolumn{6}{|c|}{\vdots} \\
%     \end{tabular}
% }
% \quad
% \scalebox{0.71}{
%     \begin{tabular}{|c|}
%       \hline
%       X \\ \hline
%       year \\ \hline
%       month \\ \hline
%     \end{tabular}
% }
% \quad
% \scalebox{0.71}{
%      \begin{tabular}{|c|}
%       \hline
%       Y \\ \hline
%       sales \\ \hline
%       profit \\ \hline
%   \end{tabular}
% }

% \scalebox{0.71}{
% \begin{tabular}{|c|c|c|c|c|c|c|c|}
%       \hline
%       X & Y & year & month & product & location & sales & profit \\ \hline
%       year & sales & \wild & \wild & \wild & \wild & \wild & \wild \\ \hline
%       year & profit & \wild & \wild & \wild & \wild & \wild & \wild \\ \hline
%       year & sales & \wild & \wild & chair & \wild & \wild & \wild \\ \hline
%       year & sales & \wild & \wild & chair & US & \wild & \wild \\
%       \multicolumn{8}{|c|}{\vdots} \\
%     \end{tabular}
% }


\begin{table*}[!t]
  \vspace{10pt}
  \begin{subtable}{0.4\linewidth}
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|}
      \hline
      year & month & product & location & sales & profit \\ \hline
      2016 & 4 & chair & US & 623,000 & 314,000 \\ \hline
      2016 & 3 & chair & US & 789,000 & 410,000 \\ \hline
      2016 & 4 & table & US & 258,000 & 169,000 \\ \hline
      2016 & 4 & chair & UK & 130,000 & 63,000 \\
      \multicolumn{6}{|c|}{{\bf \vdots}} \\
    \end{tabular}
    \caption{Example $\calR$}
    \label{subtab:ex-R}
     \end{subtable}
       \hspace{-10pt}
  \begin{subtable}{.1\linewidth}
    \scriptsize
    \begin{tabular}{|c|}
      \hline
      X \\ \hline
      year \\ \hline
      month \\ \hline
    \end{tabular}
    \caption{$\calX$\hphantom{ for $\calR$}}
    \label{subtab:ex-X}
  \end{subtable}
  \hspace{-10pt}
  \begin{subtable}{.1\linewidth}
        \scriptsize
    \begin{tabular}{|c|}
      \hline
      Y \\ \hline
      sales \\ \hline
      profit \\ \hline
    \end{tabular}
    \caption{$\calY$\hphantom{  for $\calR$}}
    \label{subtab:ex-Y}
  \end{subtable}
  \hspace{-10pt}
  \begin{subtable}{0.3\linewidth}
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
      \hline
      X & Y & year & month & product & location & sales & profit \\ \hline
      year & sales & \wild & \wild & \wild & \wild & \wild & \wild \\ \hline
      year & profit & \wild & \wild & \wild & \wild & \wild & \wild \\ \hline
      year & sales & \wild & \wild & chair & \wild & \wild & \wild \\ \hline
      year & sales & \wild & \wild & chair & US & \wild & \wild \\
      \multicolumn{8}{|c|}{{\bf \vdots}} \\
    \end{tabular}
    \caption{$\calV$ for $\calR$}
    \label{subtab:ex-V}
  \end{subtable}
  \vspace{-5pt}
\caption{An example relation $\calR$ and its resultant $\calX$, $\calY$,
  and $\calV$.}
  \label{tab:setup}
  \vspace{-15pt}
\end{table*}


Any subset relation $V \subseteq \calV$ is called a \emph{\vzgrp}, and any
$k+2$-tuple from $\calV$ is called a \emph{\vzchn}.
The last $k$ portions (or attributes) of a tuple from $\calV$
comprise the {\em data source} of the \vzchn.
Overall, a \vzchn
represents a visualization that can be rendered from a selected data source, and a
set of \vzchns is a \vzgrp. The X
and Y attributes of the \vzchn determine the x- and y- axes, and the
selection on the data source is determined by attributes $A_1,\dots,A_k$. If
an attribute has the wildcard symbol \wild as its value, no subselection is
performed on that attribute for the data source.
For example, the third row of Table~\ref{subtab:ex-V} is a \vzchn that
represents the visualization with year as the x-axis and sales as the y-axis for
chair products. Since the value of location is \wild, all locations are
considered valid or pertinent for the data source.
In relational algebra, the data source
for the third row can be written 
as $\sigma_{\text{product=chair}}(\calR)$.
The
\wild symbol therefore attempts to emulate the lack of presence 
of a selection condition on that attribute in the $\sigma$
operator of the relational algebra. 
Readers familiar with OLAP will notice the similarity between the use of the
symbol \wild here 
and the GROUPING SETS functionality in SQL.

Note that infinitely many
visualizations can be produced from a single visual source, due to different
granularities of binning, aggregation functions, and types
of visualizations that can be constructed, 
since a visualization generation engine can use a
visualization rendering grammar like ggplot~\cite{ggplot} that provides that functionality.
Our focus in defining the \vzalg is to specify the inputs to a visualization
and attributes of interest as opposed to the aesthetic aspects and encodings.
Thus, for our discussion, we assume that each visual source maps 
to a singular visualization.
Even if the details of the encoding and aesthetics are not provided,
standard rules may be applied for this mapping as alluded
earlier~\cite{wongvoyager2015,DBLP:journals/cacm/StolteTH08} in
Section~\ref{subsec:formalization}.
Furthermore,
a \vzchn does not specify the data representation of the underlying data source;
therefore the expressive power of \vzalg is not tied to any specific backend data storage
model.
The astute reader will have noticed that the format for a \vzchn looks fairly
similar to a collections of visualizations in \zq; this is no accident. In fact, we
will use the visualization collections of \zq as a proxy to \vzchns when proving that
\zq is \vzcmp.

\subsection{Functional Primitives}

Earlier, we mentioned that a \vzalg is \vzexp complete 
with respect to two functional primitives: $T$ and $D$.
Here we define the formal types for these functional primitives with respect to
\vzalg.


The function $T: \calV \rightarrow \mathbb{R}$ returns a real number given
a \vzchn. This function can be used to assess whether a trend:
defined by the visualization corresponding to a specific \vzchn,
is ``increasing'', or ``decreasing'', or satisfies some other fixed property. Many such $T$ can be defined and used within the \vzalg.

The function $D: \calV \times \calV \rightarrow \mathbb{R}$ returns a real
number given a pair of \vzchns. This function can be used
to compare pairs of visualizations (corresponding to the \vzchns)
with respect to each other. The most natural way to define $D$ is
via some notion of distance, e.g., Earth Mover's or Euclidian distance, 
but once again, the definition can be provided by the user or assumed as a fixed black box.


\input{viz-exp-operators}
\input{viz-exp-proof}


==> docs copy/formal-process.tex <==
%!TEX root=zenvisageql.tex


\begin{table*}[!htbp]
  \centering\scriptsize
 \vspace{-10pt}
  {\tt
    %\resizebox{\linewidth}{!}{%
      \begin{tabular}{|r|l|l|l|l|} \hline
        \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Z} & \textbf{Process}
        \\ \hline
        f1 & `year' & `sales' & v1 \IN `product'.* & v2 \IN $R(10, v1, f1)$ \\
        f2 & `year' & `sales' & v2 & v3 \IN $argmax_{v1}[k=10] \; min_{v2}
        D(f1,f2)$ \\
        *f3 & `year' & `sales' & v3  & \\ \hline
      \end{tabular}
    %}
  }
  \vspace{-10pt}\caption{A \zq query which returns 10 sales over years visualizations for
  products which are outliers compared to the rest.}
  \label{tab:process-2}
\vspace{-10pt}\end{table*}


\subsubsection{Process Column}
\label{sec:process}
%\tar{Maybe we need to revise this section, and make it more consistent with expressiveness section}
Once the visual component for a row has been named, the user may use the
Process column to sort, filter, and compare the visual component with
previously defined
visual components to isolate the set of visualizations she is interested in.
While the user is free to define her own functions for the Process column,
we have come up with a core set of primitives based on our case
studies which we believe can handle the vast majority of the common operations.
Each non-empty Process column entry is defined to be a {\em task}. 
Implicitly, a task may be impacted by one or more rows of a \zq query\techreport{ (which would be input to the process optimization),}
and may also impact one or more rows\techreport{ (which will use the outputs of the process optimization)}, 
as we will see below.

\noindent {\bf Functional Primitives.}
First, we introduce three simple functions that can be applied to
visualizations: $T$, $D$, and $R$.
\zv will use default settings for each of these functions, but
the user is free to specify their own variants for each of these functions
that are more suited to their application.


\noindent $\bullet \  T(f)$ measures the overall trend of visualization $f$. 
It is positive
if the overall trend indicates ``growth'' and negative if the overall trend goes
``down''.
There are obviously many ways that such a function can be
implemented, but one example implementation might be to measure the slope of a
linear fit to the given input visualization $f$.

\noindent $\bullet \ D(f,f')$ measures the distance between the two visualizations $f$ and
$f'$. For example, this might mean calculating the Earth Mover's Distance or the 
Kullback-Leibler Divergence between the induced probability distributions. 

\noindent $\bullet \ R(k,v,f)$ computes the set of $k$-representative visualizations given an axis
variable, $v$, and an iterator over the set of visualizations, $f$. Different
users might have different notions of what representative means, but one
example would be to run $k$-means clustering on the given set of visualizations
and return the $k$ centroids. In addition to taking in a single
axis variable, $v$, $R$ may also take in a tuple of axis variables to iterate
over. The return value of $R$ is the set of axis variable values which produced
the representative visualizations.


\noindent {\bf Processing.}
Given these functional primitives, 
\zq also provides some default sorting and filtering mechanisms: 
$argmin$, $argmax$, and $argany$. Although $argmin$ and $argmax$ are usually
used to find the best value for which the objective function is optimized, \zq
typically returns the top-$k$ values, sorted in order. $argany$ is used to
return any $k$ values. In addition to the top-$k$, the user might also like to
specify that she wants every value for which a certain threshold is met, and
\zq is able to support this as well.
Specifically, the expression {\tt v2 \IN $argmax_{v1}[k=10] D(f1,f2)$} returns
the top 10 {\tt v1} values for which $D(f1,f2)$ are maximized, sorts those in
decreasing order of the distance, and declares the variable {\tt v2} to iterate
over that set. 
This could be useful, for instance, to find the 10 visualizations with
the most variation on some attributes.
 The expression {\tt v2 \IN $argmin_{v1}[t<0] D(f1,f2)$} returns
the {\tt v1} values for which the objective function $D(f1,f2)$ is below the
threshold 0, sorts the values in increasing order of the objective function,
and declares {\tt v2} to iterate over that set. If a filtering option ($k$,$t$)
is not specified, the mechanism simply sorts the values, so {\tt v2} \IN
$argmin_{v1} T(f1)$ would bind {\tt v2} to iterate over the values of {\tt v1}
sorted in increasing order of $T(f1)$. {\tt v2 \IN $argany_{v1}[t>0] T(f1)$}
would set {\tt v2} to iterate over the values of {\tt v1} for which the $T(f1)$
is greater than 0. 
\later{Note that when using the $k$ filtering option for $argany$,
no objective function is required: {\tt v2 \IN $argany_{v1}[k=10]$}.}

Note that the mechanisms may also take in multiple axis variables, as we saw
from Table~\ref{tab:vars-3}.  The mechanism iterates over the Cartesian
product of its input variables. If a mechanism is given $k$ axis variables to
iterate over, the resulting set of values must also be bound to $k$ declared
variables. In the case of Table~\ref{tab:vars-3}, since there were two
variables to iterate over, {\tt x1} and {\tt y1}, there are two output
variables, {\tt x2} and {\tt y2}. The order of the variables is important as
the values of the $i$th input variable are set to the $i$th output variable.

\noindent 
{\bf User Exploration Tasks.}
By building on these mechanisms, the user can perform most
common tasks.
This includes the {\em similarity/dissimilarity search} 
performed in Table~\ref{tab:vars-1},
to find products that are dissimilar;
the {\em comparative search} performed in Table~\ref{tab:vars-3},
to identify attributes on which
two slices of data are dissimilar, or even the {\em outlier search}
query shown in Table~\ref{tab:process-2}, to identify the products
that are outliers on the sales over year visualizations. 
%\alkim{Verify that the outlier case is
%correct and similar to what Tarique's implementation of outliers.} 
Note that in
Table~\ref{tab:process-2}, we use two levels of iteration. 
%\agp{we should explain what these tasks mean}
\later{Other mathematical
operations such as $\sum$ and $\prod$ are also available to the user. However,
other mathematical operations such as $max$ and $min$ retain their original
meaning.}



==> docs copy/formal-viz.tex <==
%!TEX root=zenvisageql.tex


\begin{table*}[!htbp]
  \centering\scriptsize
  {\tt
    %\resizebox{\linewidth}{!}{%
      \begin{tabular}{|r|l|l|l|} \hline
        \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Viz} \\ \hline
        *f1 & `weight' & `sales' & bar.(x=bin(20), y=agg(`sum')) \\ \hline
      \end{tabular}
    %}
  }
  \vspace{-10pt}\caption{A \zq query which returns the bar chart of overall sales for
  different weight classes.}
  \label{tab:viz-1}
\vspace{-10pt}\end{table*}

\subsubsection{Viz Column}
\label{sec:viz}
Given the data from the X, Y, Z, and Constraints columns, the Viz column 
determines how the data is shaped 
before returning it as a visualization. 
There are two aspects to the Viz column:
first, the visualization type 
(e.g., bar chart, scatter plot),
and the summarization type
(e.g., binning or grouping, aggregating in some way).
These two aspects are akin to the
geometric and statistical transformation layers
from the Grammar of Graphics, a visualization specification language, and the inspiration behind
\ggplot~\cite{ggplot}.


In \zq, the Viz column specifies the visualization type
and the summarization using a period delimiter.
Functions are used to represent both
the visualization type and the summarization.
Consider the query in Table~\ref{tab:viz-1}. 
Here, the user specifies that she wants a bar chart,
with {\tt bar}, and 
specifies the type of summarization in the accompanying tuple:
{\tt x=bin(20)} denotes that x-axis should be binned into bins
of size 20, and {\tt y=agg(`sum')} runs the {\tt SUM} aggregation on the
y-values when grouped by both the bins of the x-axis and the values in the z-axis,
(if any are specified). 

%Although we can explicitly specify the Viz column,
Often we can leave the Viz column blank.
In such cases, we would apply well-known rules of thumb for what types of
visualization and summarization would be appropriate given specific X and Y axes.
Work on recommending appropriate visualization types
dates back to the 80s~\cite{Mackinlay:1986:ADG:22949.22950},
that both Polaris/Tableau~\cite{DBLP:journals/cacm/StolteTH08}, and recent work builds on~\cite{wongvoyager2015,DBLP:conf/avi/KandelPPHH12}, determining
the best visualization type by examining the schema and statistical properties.
\techreport{In many of our examples of \zq queries, we omit the Viz column for this reason.}



==> docs copy/inter-proc-opt.tex <==
%!TEX root=zenvisageql.tex




\paragraph{Inter-Task Optimization.}
%Our final optimization is less straightforward than the previous methods.
It is not generally not possible
to batch \sql queries across tasks, since
subsequent tasks may depend on the outputs of previous tasks.
However, for more sophisticated \zq queries, it may be possible 
to identify batching opportunities across tasks.
For instance, a visual component defined after a task may be
independent of the task. 
Formally, if visual component $V$ is defined in a
row later than the row task $T$ is defined in, 
and no column of $V$ depends on the
output of $T$, then $V$ is independent of $T$. The advantage of 
independence is that now we can batch $V$ into an earlier request because we do
not need to wait for the results of $T$.
Thus, in Table~\ref{tab:exec-1}, we can batch the \sql queries for the first and second
rows into a single request since the visual component in the second row is independent of
the task in the first row.


% \papertext{Since the visualizations from subsequent rows may depend on
% the output values of previous tasks, so it is not possible to batch
% queries across tasks}
% \techreport{As mentioned previously, it is generally not possible to batch \sql queries
% across tasks}.
% However, sometimes a visual component defined after a task may be
% independent of the task. 
% \papertext{Nothing prevents the user from combining 
% many non-related visual queries into a single \zq query with many output rows.
% Particularly for the case of exploratory visual analysis, the user may want to submit
% one \zq query which contains many different tasks to explore interesting trends,
% representative sets, and outliers in an unknown dataset.}

% \techreport{More formally, if visual component $V$ is defined in a
% row later than the row task $T$ is defined in, and no column of $V$ depends on the
% output of $T$, then $V$ is independent of $T$. The advantage of 
% independence is that now we can batch $V$ into an earlier request because we do
% not need to wait for the results of $T$.} 
% More concretely, in Table~\ref{tab:exec-1}, we can batch the \sql queries for the first and second
% rows into a single request since the visual component in the second row is independent of
% the task in the first row.

To determine all cases for which this independence can be taken advantage of,
the \zq compiler builds a query tree for the \zq queries it
parses. All axis variables, name variables, and tasks of a \zq query are 
nodes in its query tree. Name variables become the parents of the axis variables
in its visual component. Tasks become the parents of the visualizations it
operates over. Axis variables become the parents over the nodes which are used
in its declaration, which may be either tasks nodes or other axis variable
nodes.
The query tree for Table~\ref{tab:exec-1} is given in
Figure~\ref{fig:query-tree}. Here, the children point to their parents, and the
tasks in rows 1 and 2 are labeled {\tt t1} and {\tt t2} respectively. As
we can clearly see from the tree, the visual component for {\tt f2}
is independent of {\tt t1}.

\begin{figure}[!]
  \centering
  \vspace{-10pt}
  \includegraphics[scale=0.3]{figs/querytree1.pdf}
    \vspace{-10pt}
  \caption{The query tree for the \zq query in Table~\ref{tab:exec-1}.}
  \vspace{-15pt}
  \label{fig:query-tree}
\end{figure}

The \zv execution engine uses the query tree to determine which \sql queries to
batch in which step. At a high level, all \sql queries for name variable nodes
whose children have all been satisfied or completed can be batched into a single request.
More
specifically, the execution engine starts out by coloring all leaf nodes in the
query tree. Then, the engine repeats the following until the entire
query tree has been colored:
\begin{inparaenum}[i)]
  \item Batch the \sql queries for name variable nodes, who have all their
    children colored, into a single request and submit to the database.
  \item Once a response is received for the request, color all name variables
    nodes whose \sql queries were just submitted.
  \item Until no longer possible, color all axis variable and task nodes whose
    children are all colored. If a task is about to be colored, run the task
    first.
\end{inparaenum}
This execution plan ensures the maximal amount of batching is done while still
respecting dependencies. Parts of the execution plan may also be parallelized
(such as simultaneously running two independent, computation-expensive tasks
like representative sets), to improve overall throughput.



\techreport{While this optimization may seem like overkill for the short \zq examples
presented in this paper, nothing prevents the user from combining many non-related visual
queries into a single \zq query with many output rows. Particularly for the
case of exploratory visual analysis, the user may want to submit
one \zq query which contains many different tasks to explore interesting trends,
representative sets, and outliers in an unknown dataset.
}


==> docs copy/intra-proc-opt.tex <==
%!TEX root=zenvisageql.tex

\paragraph{Intra-Task Optimization.}
\papertext{In addition to combining \sql queries within a row, the second level 
of optimization batches \sql across all rows that are input to the same task.
In Table~\ref{tab:exec-2}, this optimization would batch
rows 1 and 2 together and rows 3 and 4 together.
}
\techreport{In addition to combining \sql queries within a row, \sql queries may also
be batched across \zq rows. However, in general, it may not be possible to
compose queries across rows into a single \sql query,
since different rows may access completely
different attributes. Instead, our optimization is to batch multiple \sql
queries from different rows into a single \emph{request} to the database,
effectively pipelining the data retrieval.
However, tasks in \zq frequently filter and limit the space of visualizations
being looked at. Moreover, visualizations from subsequent rows may depend on
the output values of previous tasks, so it is not possible to batch
queries across tasks. Therefore, we batch into a single request all \sql queries for task-less rows leading up to
a row with a task. In Table~\ref{tab:exec-2}, this optimization would batch
rows 1 and 2 together and rows 3 and 4 together.
}


==> docs copy/introduction.tex <==
%!TEX root=zenvisageql.tex

\section{Introduction}
\label{sec:intro}
Interactive visualization tools, such as Tableau~\cite{tableau}
and Spotfire~\cite{spotfire}, have paved the way for the 
democratization of data exploration and data science. 
These tools have witnessed an ever-expanding user base---as a concrete example, 
Tableau's revenues last year were in the hundreds of millions of US Dollars and is 
expected to reach tens of billions soon~\cite{tableau-increases}.
Using such tools, or even tools like Microsoft Excel, the standard 
data analysis recipe is as follows:
the data scientists load a dataset into the tool,  
select visualizations to examine, 
study the results, and then repeat the process
until they find ones that match
their desired pattern or need. 
Thus, using this repeated process of manual examination, or {\em trial-and-error},
data scientists are able to formulate and test hypothesis, 
and derive insights. 
The key premise of this work is that 
 to find
desired patterns in datasets, 
{\bf \em manual examination of each visualization in a collection  is 
simply unsustainable}, especially
on large, complex datasets.
Even on moderately sized datasets, a data scientist may need to examine as many as 
tens of thousands of visualizations, all to test a single hypothesis, 
a severe impediment to data exploration.

To illustrate, we describe the challenges of 
several collaborator groups who have been hobbled by the ineffectiveness of current 
data exploration tools: 


\paraem{Case Study 1: Engineering Data Analysis.}
Battery scientists at Carnegie Mellon University
perform visual exploration of datasets of solvent
properties to design better batteries.
A specific task may involve finding solvents
with desired behavior: e.g.,
those whose 
solvation energy
of Li$^+$ vs.~the boiling point is a 
{\em roughly increasing trend}. 
To do this using current tools, 
these scientists manually examine
the plot of Li$^+$ solvation energy vs.~boiling point for each of the thousands of solvents, to find those that match 
the desired pattern of a roughly increasing trend.



\paraem{Case Study 2: Advertising Data Analysis.}
Advertisers at ad analytics
firm Turn, Inc., 
often examine their portfolio of advertisements to see
if their campaigns are performing as expected.
For instance, an advertiser may be interested in seeing if there are any keywords
that are {\em behaving unusually} with respect to other keywords in Asia---for example,
maybe most keywords have a specific trend for 
click-through rates (CTR) over time, 
while a small number of them
have a different trend.
To do this using the current tools available at Turn, 
the advertiser needs to manually examine the plots of 
CTR over time for each 
keyword (thousands of such plots),
and remember what are the typical trends. 

\paraem{Case Study 3: Genomic Data Analysis.}
Clinical researchers at the NIH-funded genomics center
at UIUC and Mayo Clinic 
are interested in studying 
data from clinical trials.
One such task involves finding pairs of genes
that {\em visually explain the differences} 
in clinical trial outcomes (positive vs.~negative)---visualized 
via a scatterplot with the x- and y- axes each referring
to a gene, and each outcome depicted as a point 
in the scatterplot---with the positive outcomes
depicted in one color, and the negative ones as another.
Current tools require the researchers to
generate and manually evaluate tens of thousands of scatter plots of pairs of
genes to determine whether
the outcomes can be clearly
distinguished in the scatter plot. 




\techreport{
\paraem{Case Study 4: Environmental Data Analysis.}
Climate scientists at the National Center for
Supercomputing Applications at Illinois are interested
in studying the nutrient and water property readings on sensors within buoys
at various locations in the Great Lakes. 
Often, they find that a sensor is displaying unusual behavior
for a specific property, and want
to figure out {\em what is different} about this sensor relative to others,
and if other properties for this sensor are {\em showing similar behavior}.
In either case, the scientists would need to separately examine each
property for each sensor (in total 100s of thousands of visualizations)
to identify explanations or similarities.

\paraem{Case Study 5: Server Monitoring Analysis.}
 The server monitoring team at Facebook has noticed a spike in the
per-query response time for Image Search in Russia on August 15, after which the response time flattened out.
The team would like to identify if there are {\em other attributes 
that have a similar behavior} with
per-query response time, which may indicate the reason for the spike and subsequent flattening.
To do this, the server monitoring team generates visualizations for
different metrics as a function of the date, and assess if any of them has similar behavior
to the response time for Image Search. Given that the number of metrics is likely 
in the thousands, this takes a very long time.

\paraem{Case Study 6: Mobile App Analysis.} 
The complaints section of the Google mobile platform team 
have noticed that a certain mobile app has 
received many complaints.
They would like to figure out {\em what is different} about this app relative to others.
To do this, they need to plot various metrics for this app to figure out 
why it is behaving anomalously. 
For instance, they may look at network traffic generated by this app over time,
or at the distribution of energy consumption across different users.
In all of these cases, the team would need to generate several visualizations manually 
and browse through all of them in the hope of finding what could be the issues with the app.
}

\vspace{2pt}
\noindent 
Thus, in these examples, the recurring theme is 
the manual examination of a large number of generated visualizations for a specific visual pattern.
Indeed, we have found that in these scenarios\papertext{, as well as others that we have encountered 
via other collaborators---in {\em climate science, server monitoring, and mobile app analysis}}---data exploration 
can be a tedious and time-consuming process with current
visualization tools.

\paragraph{Key Insight.} The goal of this paper is to develop \zv, a visual analytics
system that can {\bf \em automate the search for desired
visual patterns}.
Our key insight in developing \zv is that the data exploration 
needs in all of these scenarios 
can be captured within a common set of operations
on collections of visualizations.
These operations include:
{\em composing}  
collections of visualizations,
{\em filtering} visualizations
based on some conditions,
{\em comparing} visualizations,
and {\em sorting} them based on some condition.
The conditions include 
similarity or dissimilarity to a specific pattern, 
``typical'' or anomalous behavior,
or the ability to provide 
explanatory or discriminatory power.
These operations and conditions form the kernel of a 
new data exploration language, \zq ("zee-quel"), that forms
the foundation upon which  \zv is built.

\paragraph{Key Challenges.} 
We encountered many challenges in building the \zv visual analytics platform, 
a substantial advancement over manually-intensive visualization
tools like Tableau and Spotfire; these tools
enable the examination of {\em one visualization at a time},
without the ability to automatically identify
relevant visualizations from a collection of visualizations.

First, there were many challenges in developing \zq,
the underlying query language for \zv.
Unlike relational query languages that operate
directly on data, \zq operates on collections of visualizations,
which are themselves aggregate queries on data. 
\techreport{Thus, in a sense \zq is a query language that operates
on other queries as a first class citizen.}
This leads to a number of challenges that are not addressed
in a relational query language context. For example,
we had to develop a natural way to users to specify
a collection of visualizations to operate on, without
having to explicitly list them;
even though the criteria on which the visualizations
were compared varied widely, we had to develop a 
small number of general mechanisms that capture all of these
criteria.
Often, the visualizations that we operated on had
to be modified in various ways---e.g., we
might be interested in visualizing the sales of
a product whose profits have been dropping---composing
these visualizations from existing ones is not straightforward.
Lastly, drilling down into specific visualizations
from a collection also required special care.
Our \zq language is a synthesis of desiderata
after discussions with data scientists
from a variety of domains, and has been under
development for the past two years. 
To further show that \zq is {\em complete} under
a new \vzalg that we develop involved additional challenges.

Second, in terms of front-end development, 
\zv, as an interactive analytics tool,
needs to support the ability for users to 
interactively specify \zq queries---specifically, 
interactive short-cuts for commonly used \zq queries, 
as well as the ability to pose extended \zq queries
for more complex needs.
Identifying common interaction ``idioms'' for these
needs took many months. 

Third,  
an important challenge in building \zv is
the back-end that supports the execution of \zq.
A single \zq query can lead to the generation of 10,000s of 
visualizations---executing each one 
independently as an aggregate query,
would take several hours, rendering the 
tool somewhat useless.
\techreport{(As it turns out, this time would be what an analyst aiming
to discover the same pattern would have to spend
with present visualization tools,
so the naive automation may still help reducing the amount of
manual effort.) }%
\zv's query optimizer 
operates as a wrapper
over any traditional relational database system. 
This query optimizer compiles \zq queries
down to a directed acyclic graph of 
operations on collections of visualizations,
followed with the optimizer
using 
a combination of intelligent speculation and combination, 
to issue queries to the underlying database. 
We also demonstrate that the underlying problem
is {\sc NP-Hard}.
Our query optimizer leads
to substantial improvements over the naive
schemes adopted within relational 
database systems for multi-query optimization.


\techreport{
\paragraph{Related Work.}
There are a number of
tools one could use for interactive analysis;
here, we briefly describe why those tools are inadequate 
for the important need of 
automating the search
for desired visual insights.
We describe related work in detail in Section~\ref{sec:related}.
To start, visualization tools like
Tableau and Spotfire only generate and provide one visualization
at a time, 
while \zv analyzes collections of visualizations at a time,
and identifies relevant ones from that collection---making it
substantially more powerful.
While we do use relational database systems
as a computation layer,
it is 
cumbersome to near-impossible to express
these user needs in \sql. 
As an example, finding visualizations of 
solvents for whom a given property
follows a roughly increasing trend is impossible to write
within native SQL, and would require custom UDFs---these UDFs 
would need to be hand-written for every \zq query.
\techreport{Similarly, finding visualizations of 
keywords where CTR over time in Asia is behaving
unusually with respect to other keywords 
is challenging to write within SQL. }%
For the small space of queries 
where it is possible to write
the queries within \sql 
these queries require non-standard constructs,
and are both complex and cumbersome to write,
even for expert \sql users, 
and are optimized very poorly
(see Section~\ref{sec:related}).
\techreport{It is also much more natural 
for end-users to operate directly on visualizations
than on data. 
Indeed, users who have never programmed or written
SQL before find it easy to understand and write 
a subset of \zq queries, as we
will show subsequently.} 
Statistical, 
data mining, and machine learning
 certainly provide functionality beyond \zv
in supporting prediction
and statistics; 
these functionalities are exposed as ``one-click'' algorithms
that can be applied on data.
However, no functionality is provided for searching for desired
patterns; no querying functionality beyond the one-click algorithms,
and no optimization. To use such tools for \zq, many
lines of code and hand-optimization is needed.
\techreport{As such, these tools are beyond the reach of
novice data scientists who simply want to explore 
and visualize their datasets.}
}%metatechreport

\paragraph{Outline.}
We first describe our
query language for \zv, \zq (Section~\ref{sec:querylanguage})%
\techreport{, and formalize the notion of a {\em \vzalg}, an analog of relational
algebra, describing a core set of capabilities for any 
language that supports visual data exploration and
demonstrate that \zq is {\em complete} in that
it subsumes these capabilities (Section~\ref{sec:formal-expr})}.
We then describe the graph-based query translator and optimizer for \zq
(Section~\ref{subsec:query_execution}).
Next, our initial prototype of \zv is presented (Section~\ref{sec:architecture}).
We also describe our performance experiments
(Section~\ref{sec:experiments}), and
present a user survey and study focused on evaluating the 
effectiveness and usability of \zv (Section~\ref{sec:userstudy}).
\techreport{In the appendix, we present additional details of 
our query language,
along with complete examples, 
and additional details on user study.}%
\papertext{%
Lastly, we describe how \zv differs from related work (Section~\ref{sec:related}).

In our extended technical report~\cite{techreport}, we provide
additional details that we weren't able to fit into the paper.
In particular, we formalize
the notion of a {\em \vzalg}, an analog of relational
algebra, describing a core set of capabilities for any language that supports visual
 data exploration, and demonstrate that \zq is {\em complete} in that
it subsumes these capabilities.
 We also provide additional details of our query language.}
% In the appendix, we present additional details of our query language,
% with complete examples (Appendix~\ref{subsec:examples}) and describe the capabilities of our language in some detail (Appendix~\ref{subsec:expressivenesss}).





==> docs copy/new-qexec.tex <==
%!TEX root=zenvisageql.tex

\vspace{-4pt}
\section{Query Execution}
\label{subsec:query_execution}
\vspace{-2pt}

In \zv, \zq queries are automatically parsed and executed by the back-end.
The \zq compiler translates \zq queries into a combination of \sql
queries to fetch the visualization collections and processing tasks to
operate on them.
We present a basic graph-based translation for \zq
 and then provide 
several optimizations to the graph which reduce the
overall runtime considerably.
%
%retrieve data and a series of processing tasks which performs
%that are issued to a relational database and performs
%the processing computation on the results to arrive at the final results.
%By translating to \sql, we do not tie ourselves down to any specific
%  relational database and can seamlessly leverage benefits from improvements to
%databases.
\vspace{4pt}
\subsection{Basic Translation}
% \alkim{If a specification is invalid, skip}
% \alkim{We translate into each \zq query into a graph-based query plan}
Every valid \zq query can be transformed into a query plan 
in the form of a directed
acyclic graph (DAG). 
The DAG contains \cnode[s] (or \emph{collection nodes})
to represent the collections of visualizations in the \zq query and \pnode[s]
(or \emph{process nodes}) to represent the optimizations (or
\emph{processes}) in the \zqproc column. 
Directed edges are drawn between nodes
that have a dependency relationship. 
Using this query plan,
the \zq engine can determine at each step which visualization collection to
fetch from the database or which process to execute.
The full steps to build a query plan for any \zq query is as follows: 
\begin{inparaenum}[(i)]
\item
  Create a \cnode[] or \emph{collection node} for every collection of
  visualizations (including singleton collections).
\item
  Create a \pnode[] or \emph{processor node} for every optimization (or
  \emph{process}) in the \zqproc column.
\item
  For each \cnode[], if any of its \axvar[s] are derived as a result of a
  process, connect a directed edge from the corresponding \pnode[].
\item
  For each \pnode[], connect a directed edge from the \cnode[] of each
  collection which appears in the process.
\end{inparaenum}
\later{
\begingroup
\plitemsep=.2em
\pltopsep=.2em
\begin{compactenum}
\item
  Create a \cnode[] or \emph{collection node} for every collection of
  visualizations (including singleton collections).
\item
  Create a \pnode[] or \emph{processor node} for every optimization (or
  \emph{process}) in the \zqproc column.
\item
  For each \cnode[], if any of its \axvar[s] are derived as a result of a
  process, connect a directed edge from the corresponding \pnode[].
\item
  For each \pnode[], connect a directed edge from the \cnode[] of each
  collection which appears in the process.
\end{compactenum}
\endgroup
}
%These steps split a \zq query into its collection components (\cnode[s]) and
%its process components (\pnode[s]), and the directed edges between the nodes
%represent the dependencies between these components.
%
Following these steps, we can translate our realistic query example in
Table~\ref{tab:real2} to its query plan presented in
Figure~\ref{fig:real2-plan}. The \cnode[s] are annotated with {\tt f\#},
and the \pnode[s] are annotated with {\tt p\#} (the $i$th \pnode[] refers to the
process in the $i$th row of the table). Here, {\tt f1} is a root node
with no dependencies since it does not depend on any process, whereas {\tt f5}
depends on the results of both {\tt p3} and {\tt p4} and have edges coming from
both of them.
\begin{figure}
\vspace{-5pt}
  \centering
  \includegraphics[width=.6\linewidth]{figs/real2-plan}
  \caption{The query plan for the query presented in Table~\ref{tab:real2}.}
  \label{fig:real2-plan}
  \vspace{-15pt}
\end{figure}
Once the query plan has been constructed, 
the \zq engine can execute it using the simple algorithm presented in
in Algorithm~\ref{simplealg:basic}.

  \vspace{-0.75em}
\begin{framed}
  \vspace{-1.5em}
\begin{simplealg}
\small
  %\begin{simplealg}
%\begingroup
%\plitemsep=.2em
%\pltopsep=.2em
Algorithm to execute \zq query plan:
\begin{compactenum}
\item
  Search for a node with either no parents or one whose parents have all been
  marked as done.
\item 
  Run the corresponding task for that node and mark the node as done.
\item
  Repeat steps 1 and 2 until all nodes have been marked as done.
\end{compactenum}
%\endgroup
%\caption{Basic algorithm to execute a \zq query based on its query plan.}
%\end{simplealg}
\label{simplealg:basic}
\end{simplealg}
  \vspace{-1.5em}
\end{framed}
  \vspace{-1em}
For \cnode[s], the corresponding task is to retrieve the data for visualization
collection, while for \pnode[s], the corresponding task is to execute the
process.

\paragraph{\cnode[] translation:}
At a high level, for \cnode[s], the appropriate \sql group-by queries
are issued to the database to compose the data for multiple visualizations
at once. 
Specifically,
for the simplest setting where there are no collections specified
for X or Y, a \sql query in the form of:
\begin{quoting}\small
\begin{verbatim}
      SELECT X, A(Y), Z, Z2, ...  WHERE C(X, Y, Z, Z2, ...)
        GROUP BY X, Z, Z2, ...  ORDER BY X, Z, Z2, ...
\end{verbatim}
\end{quoting}
is issued to the database, where {\tt X} is the X column attribute, {\tt Y} is
the Y column attribute, {\tt A(Y)} is the aggregation function on Y (specified
in the Viz column), {\tt Z, Z2, ...} are the attributes/dimensions we are
iterating over in the Z columns, 
while {\tt C(X, Y, Z, Z2, ...)} refers to any additional constraints
specified in the {\tt Z} columns. The {\tt ORDER BY} is inserted to ensure
that all rows corresponding to a visualization are grouped together, in order. 
As an example, the \sql
query for the \cnode[] for {\tt f1} in Table~\ref{tab:outlier} would have the form:
\begin{quoting}\small
\begin{verbatim}
      SELECT year, SUM(sales), product
        GROUP BY year, product  ORDER BY year, product
\end{verbatim}
\end{quoting}
If a collection is specified for the y-axis, each attribute in the collection
is appended to the {\tt SELECT} clause. If a collection is specified for the
x-axis, a separate query must be issued for every X attribute in the collection.
The results of the \sql query are then packed into a $m$-dimensional array
(each dimension in the array corresponding to a dimension in the collection)
and labeled with its {\tt f\#} tag. 
%\alkim{Do I need to explain the process of
%going from the resultset to the $m$-dimensional array more?}

\paragraph{\pnode[] translation:} 
At a high level, for \pnode[s], depending on the structure
of the expression within the process, 
the appropriate pseudocode is generated
to operate on the visualizations.
To illustrate, say our process is trying to find the
top-10 values for which a trend is maximized/minimized 
with respect to various
dimensions (using $T$), and the process has the form:
\vspace{-5pt}
\begin{equation}
  \langle argopt \rangle_{v0}[k=k']
  \; \bigg[ \langle op_1 \rangle_{v1}
    \bigg[
      \langle op_2 \rangle_{v2}
      \cdots
      \bigg[
        \langle op_m \rangle_{vm}
        T(f1)
      \bigg]
    \bigg]
  \bigg]
  \label{eq:trend}
  \vspace{-5pt}
\end{equation}
where $\langle argopt \rangle$ is one of {\tt argmax} or {\tt argmin}, and
$\langle op \rangle$ refers to one of 
$(\max|\min|\sum|\prod)$. 
Given this, the pseudocode which optimizes this
process can automatically be generated based on the actual values of $\langle
argopt \rangle$, $\langle op \rangle$, and the number of operations. 
In short, for each $\langle op \rangle$ or
dimension traversed over, the \zq engine generates a new nested for loop.
Within each for loop, we iterate over all values of that dimension,
evaluate the inner expression, and then eventually apply the overall 
operation (e.g., max, $\sum$). 
\iftechreportcode
\vspace{10pt}
For Equation~\ref{eq:trend}, 
the generated pseudocode would look like the one given by
Listing~\ref{lst:pseudocode}. Here, {\tt f} refers to the visualization
collection being operated on by the \pnode[], which the parent \cnode[] should
have already retrieved.  
% At the outermost level, instead of returning raw values,
% the generated code returns the top-$k$ dimensional values which most optimize
% the overall expression.

\vspace{-5pt}
\begin{lstlisting}[columns=fullflexible,basicstyle=\ttfamily\scriptsize,
    caption={Pseudocode for a process in the form of
  Equation~\ref{eq:trend}.}, label={lst:pseudocode}, captionpos=b]
  f = make_ndarray(SQL(...))
  tmp0 = make_array(size=len(v0))
  for i0 in [1 .. len(v0)]:
    tmp1 = make_array(size=len(v1))
    for i1 in [1 .. len(v1)]:
      tmp2 = make_array(size=len(v2))
      for i2 in [1 .. len(v2)]:
        ...
          tmpm = make_array(size=len(vn))
          for im in [1 .. len(vn)]:
            tmpm[im] = T(f[0, i1, i2, ..., im])
          tmpm-1[im-1] = opm(tmpm)
        ...
      tmp1[i1] = op1(tmp2)
    tmp0[i0] = op0(tmp1)
  return argopt(tmp0)[:k']
\end{lstlisting}
\vspace{-5pt}

\fi

%\begin{quoting}
%\begin{verbatim}
%f = make_ndarray(SQL(...))
%results = make_array(size=k')
%\end{verbatim}
%\end{quoting}

\techreport{Although this is the translation for one specific type of process, it is easy
to see how the code generation would generalize to other patterns.}

\vspace{-3pt}
\subsection{Optimizations}
We now present several optimizations to the previously introduced basic
translator. 
In preliminary experiments, we found that the \sql queries for the \cnode[s] 
took the majority of the runtime for \zq queries, 
so we concentrate our efforts on
reducing the cost of computing \cnode[s]. 
However, we do present one \pnode[]-based
optimization for process-intensive \zq queries.
We start with the simplest optimization schemes, and add more sophisticated
variations later.
%\alkim{Do we want to use the word I/O-bound?}

\vspace{-4pt}
\subsubsection{Parallelization}\label{sec:para}
\vspace{-3pt}
One natural way to optimize the graph-based query plan is to take advantage of
the multi-query optimization (MQO)~\cite{DBLP:journals/tods/Sellis88} present
in databases and issue in parallel the \sql queries for independent \cnode[s]---the \cnode[s]
for which there is no dependency between them.
With MQO, the database can receive multiple \sql queries at the same time and
share the scans for those queries, thereby reducing the number of
times the data needs to be read from disk.
% Note, however, that naively applying this 
% can lead to performance penalties, as we will discuss
% later on.

To integrate this optimization, we make two simple
modifications to Algorithm~\ref{simplealg:basic}. 
In the first step, instead of searching for a
single node whose parents have all been marked done, search for \emph{all}
nodes whose parents have been marked as done. Then in step 2, issue the
\sql queries for all \cnode[s] which were found in step 1 in parallel at the
same time. For example, the \sql queries for {\tt f1} and {\tt f2}
could be issued at the same time in Figure~\ref{fig:real2-plan}, and once {\tt
p1} and {\tt p2} are executed, \sql queries for {\tt f3} and {\tt f4} can
be issued in parallel.

\vspace{-6pt}
\subsubsection{Speculation}\label{sec:spec}
\vspace{-3pt}

While parallelization gives the \zq engine a substantial increase in
performance, we found that many realistic \zq queries intrinsically 
have a high level
of interdependence between the nodes in their query plans. 
% As a result, the \sql query runtimes
% still dominated the overall runtimes for \zq queries.
To further optimize the performance, we use \emph{speculation}:
the \zq engine pre-emptively issues \sql
queries to retrieve the superset of visualizations for each \cnode[],
considering all possible outcomes for the \axvar[s]. 
Specifically, by tracing the provenance of each \axvar[] 
back to the root, we can determine the superset of all values for each \axvar[];
then, by considering the Cartesian products of these sets, 
we can determine a superset of the relevant visualization collection for a \cnode[].
After the \sql queries have returned, the \zq
engine proceeds through the graph as before, and
once all parent \pnode[s] for a \cnode[] have been
evaluated, the \zq engine isolates the correct subset of data for that
\cnode[] from the pre-fetched data.

% Specifically,
% when composing a visualization collection,
% some columns are fixed by the user, while others
% are the results of processes by way of \axvar[s].
% It is because we do not know the results of these processes that we must wait
% until the corresponding \pnode[s] have been executed.
% However, as mentioned before, 
% a strict rule
% for processes is that the resulting collection of values must be a subset of
% the input collection of values.
% \alkim{Make sure to mention this in limitations.}
% Furthermore, the input collection of values must be either defined directly in
% a visualization collection or be the resulting values of a previous process.
% Therefore, by tracing the provenance of the unresolved \axvar[s] back to the
% root, we can determine the set of all possible values contained by an \axvar[].
% The \zq engine can take the Cartesian product of these sets to determine
% the superset of visualizations for a \cnode[].
For example, in the query in Table~\ref{tab:real2}, {\tt f3} depends on
the results of {\tt p1} and {\tt p2} since it has constraints based on {\tt v2}
and {\tt v4}; specifically {\tt v2} and {\tt v4} should be locations and
categories for which {\tt f1} and {\tt f2} have a negative trend. However, we
note that {\tt v2} and {\tt v4} are derived as a result of {\tt v1} and {\tt
v3}, specified to take on all locations and categories in rows 1 and
2. So, a
superset of {\tt f3}, the set of profit over year
visualizations for various products for all locations and categories 
(as opposed to just those that satisfy {\tt p1} and {\tt p2}), could be
retrieved pre-emptively.
Later, when the \zq engine executes {\tt p1} and {\tt p2}, this superset
can be filtered down correctly.

% \alkim{Note that this requires a change in the \sql code as well, as we have to
%   group the data for the {\tt f3} node by `origin' and `dest' as well, so they
% can be correctly filtered later. (should we add this line?)}
% In practice, this optimization allows the \zq engine to first concurrently
% issue the \sql queries for all \cnode[s] in the query plan, and after executing
% the \pnode[s], correctly filter down the supersets into their corresponding
% collections. 
One downside of speculation is that a lot more data must be
retrieved from the database, but we found that blocking on the retrieval of
data was more expensive in runtime than retrieving extra data. Thus,
speculation ends up being a powerful optimization which compounds the positive
effects of parallelization.
\vspace{-6pt}
\subsubsection{Query Combination}\label{sec:comb}
\vspace{-3pt}
From extensive modeling of relational databases,
we found that the overall runtime of concurrently 
running issuing \sql queries 
is heavily dependent on the number of queries being run in parallel.
Each additional query constituted a $T_q$ increase in
the overall runtime (e.g., for our settings of PostgreSQL, we found $T_q$ =
\texttildelow900ms). 
To reduce the total number of running queries, we use \emph{query combination}; that is,
given two \sql queries $Q_1$ and $Q_2$, we
combine these two queries into a new $Q_3$ 
which returns the data for both
$Q_1$ and $Q_2$. 
In general, if we have $Q_1$ (and $Q_2$) in the form of:
\begin{quoting}\small
\begin{verbatim}
SELECT X1, A(Y1), Z1    WHERE C1(X1, Y1, Z1)
       GROUP BY X, Z1    ORDER BY X, Z1
\end{verbatim}
\end{quoting}
we can produce a combined $Q_3$ which has the
form:
\begin{quoting}\small
\begin{verbatim}
SELECT X1, A(Y1), Z1, C1, X2, A(Y2), Z2, C2
    WHERE C1 or C2
    GROUP BY X1, Z1, C1, X2, Z2, C2
    ORDER BY X1, Z1, C1, X2, Z2, C2
\end{verbatim}
\end{quoting}
where {\tt C1 = C1(X1, Y1, Z1)} and {\tt C2} is defined similarly.
From the combined query $Q_3$, it is possible to regenerate the data which would
have been retrieved using queries $Q_1$ and $Q_2$ by aggregating over the
non-related groups for each query. For $Q_1$, we would select the data for which
{\tt C1} holds, and for each {\tt (X1, Z1)} pair, we would aggregate over the
{\tt X2}, {\tt Z2}, and {\tt C2} groups.
% \alkim{Btw, if we want to do AVG, we also need to return COUNTs, but this is a
% super minor detail. Probably can omit?}

While query combining is an effective optimization, there are limitations. We found
that the overall runtime also depends on the number of unique group-by values
per query, and the number of unique group-by values for a combined query is the
product of the number of unique group-by values of the constituent queries.
Thus, the number of average group-by values per query grows super-linearly with
respect to the number of combinations. However, we found that as long as the
combined query had less than $M_G$ unique group-by values, it was more
advantageous to combine than not (e.g., for our settings of PostgreSQL, we
found $M_G$ = 100k).

\paragraph{Formulation.} Given the above findings, we can now formulate the problem of deciding which
queries to combine as an optimization problem:
{\em Find the best combination of \sql queries that 
minimizes: $\alpha \times$(total number
of combined queries) + $\sum_i$ (number of unique group-by values in combined query $i$),
such that no single combination has more than $M_G$ unique group-by
values.} 

\papertext{
As we show in the technical report~\cite{techreport}, this optimization
problem is {\sc NP-Hard} via a reduction from the {\sc Partition Problem}.
}
%An interesting detail is that the choice of the queries to be combined is
%significant. Since the overall runtime depends on the average number of unique
%group-by values across the queries, it
%is more advantageous to combine queries with smaller numbers of unique group-by
%values.
\input{nphardnessproof}


\paragraph{Wrinkle and Solution.} However, a wrinkle to the above formulation is that it assumes no two \sql
queries share a group-by attribute.
If two queries have a shared group-by attribute, it may be
more beneficial to combine those two, since the number of group-by values does
not increase upon combining them. 
Overall, we developed the metric $EFGV$
or the effective increase in the number of group-by values to determine the
utility of combining query $Q'$ to query $Q$:
$EFGV_{Q}(Q') = \prod_{g \in G(Q')} \#(g)^{[[g \notin G(Q)]]}$
where $G(Q)$ is the set of group-by values in $Q$, $\#(g)$ calculates the
number of unique group-by values in $g$,  and $[[g \notin G(Q)]]$
returns 1 if $g \notin G(Q)$ and 0 otherwise. In other words, this calculates
the product of group-by values of the attributes which are in $Q'$ but not in $Q$.
Using the $EFGV$ metric, we then apply a variant of agglomerative
clustering~\cite{anderberg2014cluster} to decide the best choice of
queries to combine. 
As we show in the experiments section, this technique 
leads to very good performance. 

% \alkim{Do we want to say the full algorithm is omitted due to lack of space but
% present in the tech report here?}

\vspace{-4pt}
\subsubsection{Cache-Aware Execution}\label{sec:cache}
\vspace{-2pt}
Although the previous optimizations were all I/O-based optimizations for \zq,
there are cases in which optimizing the execution of \pnode[s] is important as
well. In particular, when a process has multiple nested for loops, the cost of
the \pnode[] may start to dominate the overall runtime. To address this
problem, we adapt techniques developed in high-performance computing---specifically,
cache-based optimizations similar to those used in matrix
multiplication~\cite{goto2008anatomy}. With cache-aware execution, the \zq
engine partitions the iterated values in the for loops into blocks of data
which fit into the L3 cache. Then, the \zq engine reorders the order of
iteration in the for loops to maximize the time that each block of data remains
in the L3 cache. This allows the system to reduce the amount of data transfer between
the cache and main memory, minimizing the time taken by the
\pnode[s].
%This allows the system to minimize the amount of data the cache needs to eject and thus the amount of data that needs to be copied
% from main memory to the cache, minimizing the time taken by the \pnode[s].
% This is also akin to the techniques for speeding up the nested-loops join algorithm.

%\alkim{Do we like ``{Block-Based Iteartion}'' better for the title?}


==> docs copy/new-qlang.tex <==
%!TEX root=zenvisageql.tex
\vspace{-6pt}
\section{Query Language}
\label{sec:querylanguage}
\vspace{-2pt}
\zv's query language, \zq, provides users with a powerful mechanism to operate 
on collections of visualizations. 
In fact, \zq treats visualizations as a {\em first-class citizen}, 
enabling users to operate at a high level on collections of visualizations
much like one would operate on relational data with \sql.
For example, a user may want to filter out all visualizations 
where the visualization shows a roughly decreasing trend from a collection,
or 
a user may want to create a collection of visualizations which are most
similar to a visualization of interest. 
Regardless of the query, \zq
provides an intuitive, yet flexible specification mechanism for
users to express the desired patterns of interest (in other words, their {\em exploration needs})
using a small number
of \zq lines. 
Overall, \zq provides users the ability to compose collections of visualizations,
filter them, and sort and compare them in various ways. 

\zq draws heavy inspiration from the
Query by Example (QBE) language~\cite{qbe} and uses a similar table-based
specification interface. 
Although \zq components are not fundamentally
tied to the tabular interface, we found that our end-users felt
more at home with it; many of them are
non-programmers who are used to spreadsheet tools like Microsoft
Excel.
Users may either directly write \zq, or they may use the \zv front-end, which
supports interactions that are transformed internally into \zq.



We now provide a formal introduction to \zq in the rest of this section. We introduce
many sample queries to make it easy to follow along, and we use a relatable
fictitious product sales-based dataset throughout this paper in our
query examples---we will reveal attributes of
this dataset as we go along.


\vspace{-4pt}
\subsection{Formalization}
\label{subsec:formalization}
\vspace{-3pt}
For describing \zq, we assume that we are operating on a single relation
or a star schema where the attributes are unique
(barring key-foreign key joins), allowing \zq to seamlessly support
  natural joins.
In general, \zq could be applied to arbitrary collections
of relations by letting the user precede an attribute $A$
with the relation name $R$, e.g., $R.A$.
For ease of exposition, we focus on the single relation case.

\vspace{-2pt}
\subsubsection{Overview}
\vspace{-3pt}
\begin{figure}
\vspace{-10pt}
  \centering
  \begin{tikzpicture}[scale=0.6]
    \begin{axis}[
        %cycle list name = color list,
        %axis lines=left,
       % xlabel=Year,
        ylabel=Sales (million \$),
        ylabel near ticks,
        yscale=0.3,
        ybar,
        /pgf/number format/1000 sep={},
        xtick pos =left,
        ytick pos=left
      ]
      \addplot
        coordinates {
          (2012, 50)
          (2013, 33)
          (2014, 40)
          (2015, 50)
          (2016, 70)
        };
    \end{axis}
  \end{tikzpicture}
  \vspace{-12pt}
  \caption{Sales over year visualization for the product chair.}
  \vspace{-18pt}
  \label{fig:sample-viz}
\end{figure}

\paragraph{The concept of visualizations.} We start by defining the notion of a visualization.
We use a sample visualization in Figure~\ref{fig:sample-viz} to guide our discussion.
Of course, different visual
analysis tasks may require different types of visualizations (instead of bar charts, 
we may want scatter plots or trend lines), but across all types,
a visualization is defined by the following five main components:
\begin{inparaenum}[(i)]
\item the x-axis attribute,
\item the y-axis attribute,
\item the subset of data used,
\item the type of visualization (e.g., bar chart, scatter plot), and
\item the binning and aggregation functions for the x- and y- axes.
\end{inparaenum}


\begin{table}[!]
\vspace{-6pt}
  \centering\scriptsize
  {\tt
    \begin{tabular}{|r|l|l|l|l|}
      \hline
      \zqname & X & Y & Z & Viz \\ \hline
      *f1 & `year' & `sales' & `product'.`chair' & bar.(y=agg(`sum')) \\ \hline
    \end{tabular}
  }
  \vspace{-7pt}
  \caption{Query for the bar chart of sales over year for the
    product chair.}
  \label{tab:overview-ex}
  \vspace{-5pt}
\end{table}

\begin{table}[!]
\vspace{-6pt}
  \centering\scriptsize
  {\tt
    \begin{tabular}{|r|l|l|l|l|}
      \hline
      \zqname & X & Y & Z & Viz \\ \hline
      *f1 & `year' & `sales' & `product'.* & bar.(y=agg(`sum')) \\ \hline
    \end{tabular}
  }
  \vspace{-6pt}
  \caption{Query for the bar chart of sales over year for
  each product.}
  \label{tab:overview-ex2}
  \vspace{-18pt}
\end{table}

\paragraph{Visualization collections in \zq:} \zq has four columns to support the specification of
visualizations that the five aforementioned components map into:
\begin{inparaenum}[(i)]
\item {\em \textbf{X}},
\item {\em \textbf{Y}},
\item {\em \textbf{Z}}, and
\item {\em \textbf{Viz}}.
\end{inparaenum}


Table~\ref{tab:overview-ex} gives an example of a valid \zq query that uses
these columns to specify a bar chart visualization of overall sales
over the years for the product chair 
(i.e., the visualization in
Figure~\ref{fig:sample-viz})---ignore the Name column for now. 
The details for each of these columns 
are presented subsequently.
In short, the x-axis (\texttt{X}) is the attribute \texttt{year},
the y-axis (\texttt{Y}) is the attribute \texttt{sales},
and the subset of data (\texttt{Z}) is the product chair,
while the type of visualization is a bar chart (\texttt{bar}),
and the binning and aggregation functions indicate that the y axis is an aggregate (\texttt{agg}) --- the sum of sales.  


In addition to specifying a single visualization, users may often want to
retrieve multiple visualizations. \zq supports this in two ways. Users
may use multiple rows, and specify one visualization per row. The user may also
specify a \emph{collection} of visualizations in a single row by iterating over
a collection of values for one of the X, Y, Z, and Viz columns.
Table~\ref{tab:overview-ex2} gives an example of how one may iterate over all products
(using the notation * to indicate that the attribute product can take
on all possible values),
returning a separate sales bar chart for each product.


\paragraph{High-level structure of \zq.} Starting from these two examples, we can now move onto
the general structure of \zq queries.
Overall, each \zq query consists of multiple rows, where each row operates on collections of visualizations.
Each row contains three sets of columns, as depicted in Table~\ref{tab:zq-breakdown}:
(i) the first column corresponds to an identifier for the visualization collection,
(ii) the second set of columns defines the visualization collection,
while (iii) the last column corresponds to some operation on 
the visualization collection.
All columns can be left empty if needed
(in such cases, to save space, for convenience, we do not display these columns in our paper). 
For example, the last column may be empty if no operation is to be 
performed, like it was in Table~\ref{tab:overview-ex} and~\ref{tab:overview-ex2}.
We have already discussed (ii); now we will briefly discuss (i) and (iii), corresponding
to {\em \textbf{\zqname}} and {\em \textbf{\zqproc}} respectively.

\paragraph{Identifiers and operations in \zq.} 
The {\em \textbf{\zqproc}} column allows the user to operate on the defined collections of
visualizations, applying high-level filtering, sorting, and comparison. 
The {\em \textbf{\zqname}} column provides a way to label and combine
specified
collections of
visualizations, so users may refer to them in the
\zqproc column. 
Thus, by repeatedly using the X, Y, Z,
and Viz columns to compose visualizations and the \zqproc column to process
those visualizations, the user is able derive the exact set of visualizations
she is looking for.
Note that the result of a \zq query is the \emph{data} used to
generate visualizations. The \zv front-end then uses this data to render the
visualizations for the user to peruse.
\vspace{-2pt}
\begin{table}
\vspace{-15pt}
  \centering\scriptsize
  {\tt
    \begin{tabular}{|r|l|l|l|l|r|}
      \hline
      \zqname & X & Y & Z & Viz & \zqproc \\ \hline
      \vspace{10pt}
      $\overbrace{\textrm{Identifier}}$ & \multicolumn{4}{l|}{$\overbrace{\textrm{Visualization Collection}}$} & $\overbrace{\textrm{Operation}}$ \\
    \end{tabular}
  }
  \vspace{-15pt}
  \caption{\zq query structure.}
  \label{tab:zq-breakdown}
  \vspace{-15pt}
\end{table}

\vspace{-5pt}
\subsubsection{X, Y, and Z}
The X and Y columns specify the attributes used for the x- and y- axes. 
For example, Table~\ref{tab:overview-ex} dictates that the returned
visualization should
have `year' for its x-axis and `sales' for its y-axis.
As mentioned, the user
may also specify a collection of values for the X and Y columns if they wish to
refer to a collection of visualizations in one \zq row. Table~\ref{tab:xy-coll}
refers the collection of both sales-over-years and profit-over-years bar
charts for the chair---the missing values in this query (``...'') are the same as 
Table~\ref{tab:overview-ex}.
As we can see, a collection is constructed using \{\}. If the user wishes to denote
all possible values, the shorthand * symbol may be used, as is shown by
Table~\ref{tab:overview-ex2}. In the case that multiple columns contain
collections, a Cartesian product is performed, and visualizations for every
combination of values is returned. For example, Table~\ref{tab:xy-coll2} would
return the collection of visualizations with specifications:
{\tt \{\mbox{(X: `year', Y: `sales')}, (X: `year', Y: `profit'), (X: `month', Y:
`sales'), (X: `month', Y: `profit')\}}. \techreport{Additionally, \zq allows composing 
multiple attributes in the X and Y columns by supporting Polaris table 
algebra [4] over the operators: +, x, / (Appendix
\ref{querylang-appendix}).} 


\begin{table}[!t]
  \vspace{-8pt}
  \centering\scriptsize
  \begin{adjustbox}{center}
    {\tt
      \begin{tabular}{|r|l|l|l|l|}
        \hline
        \zqname & X & Y & Z & Viz \\ \hline
        ... & ... & \{`sales', `profit'\} & ... & ... \\ \hline
      \end{tabular}
    }
  \end{adjustbox}
  \vspace{-8pt}
  \caption{Query for the sales and profit bar charts
  for the product chair (missing values are the same as that in Table~\ref{tab:overview-ex})}
  \label{tab:xy-coll}
\end{table}

\begin{table}[!t]
\vspace{-6pt}
  \centering\scriptsize
  \begin{adjustbox}{center}
    {\tt
      \begin{tabular}{|r|l|l|l|l|}
        \hline
        \zqname & X & Y & Z & Viz \\ \hline
        ... & \{`year', `month'\} & \{`sales', `profit'\} & ... & ... \\ \hline
      \end{tabular}
    }
  \end{adjustbox}
  \vspace{-8pt}
  \caption{Query for the sales and profit bar charts
    over years and months for chairs (missing values are the same as in Table~\ref{tab:overview-ex}).}
  \label{tab:xy-coll2}
  \vspace{-7pt}
\end{table}

\begin{table}[!t]
  \centering\scriptsize
  \begin{adjustbox}{center}
    {\tt
      \begin{tabular}{|r|l|l|l|l|l|}
        \hline
        \zqname & X & Y & Z & Z2 & Viz \\ \hline
        ... & ... & ... & ... & `location'.`US' & ... \\ \hline
      \end{tabular}
    }
  \end{adjustbox}
  \vspace{-8pt}
  \caption{Query which returns the overall sales bar chart
  for the chairs in US (all missing values are the same as that in Table~\ref{tab:overview-ex}).}
  \label{tab:z-mul-col}
  \vspace{-14pt}
  \end{table}



With the Z column, the user can select which subset of the data they wish to
construct their visualizations from.
\zq uses the
\mbox{\emph{$\langle$attribute$\rangle$.$\langle$attribute-value$\rangle$}}
notation
to denote
the selection of data.
Consequently,
the query in Table~\ref{tab:overview-ex}
declares that
the user wishes to retrieve the sales bar chart only for the
chair product.
\techreport{Note that unlike the X and Y columns, both the attribute and the
attribute value must be specified for the Z column; otherwise, a proper subset
of the data would not be identified.}%
Collections are allowed for both the attribute and the attribute value in the Z
column. Table~\ref{tab:overview-ex2} shows an example of using the * shorthand
to specify a collection of bar charts, one for each product.
A Z column which has a collection over attributes might look like:
\mbox{\tt \{`location', `product'\}.*}
(i.e., a visualization for every product and a visualization for every
location).
In addition, the Z column allows users to specify predicate constraints
using syntax like \mbox{\tt `weight'.[? < 10]}; this
specifies all items whose weight is less than 10 lbs. To evaluate, the ? is
replaced with the attribute and the resulting expression is passed to \sql's
{\tt WHERE} clause.
\techreport{The predicate constraint syntax has an analogous predicate collection syntax,
which creates a collection of the values which satisfy the condition.
\mbox{\tt `weight'.[? < 10]} specifies that the resulting visualizations must
only contains items with less than 10 lbs,  \mbox{\tt `weight'.\{? < 10\}}
creates a collection of values, one for each item which is less than 10 lbs. }%

\zq supports multiple constraints on different attributes through the use of multiple Z
columns. In addition to the basic Z column, the user may choose to add Z2,
Z3, ... columns depending on how many constraints she requires.
Table~\ref{tab:z-mul-col} gives an example of a query which looks at sales
plots for chairs only in the US. Note that Z columns are combined using
conjunctive semantics.
\vspace{-4pt}
\subsubsection{Viz}
  \vspace{-2pt}
The Viz column decides the visualization type, binning, and aggregation
functions for the row.
Elements in this column have the format:
\mbox{\emph{$\langle$type$\rangle$.$\langle$bin+aggr$\rangle$}}. 
All examples so far have been bar charts with no binning and {\tt SUM}
aggregation for the y-axis, but other variants
are supported.
The visualization types are derived from the Grammar of
Graphics~\cite{grammar-of-graphics}
specification language, so all plots from the geometric transformation layer of
\ggplot~\cite{ggplot} (the tool that implements Grammar of Graphics) are supported.
For instance, scatter plots are
requested with {\tt point} and heat maps with {\tt bin2d}.
As for binning, binning based on bin width ({\tt bin}) and number of bins
({\tt nbin}) are supported for numerical attributes---we may want to use 
binning, for example, when we are plotting the total number of products whose
prices lie within 0-10, 10-20, and so on. 

Finally, \zq supports all
the basic \sql aggregation functions such as {\tt AVG}, {\tt COUNT}, and {\tt
MAX}. Table~\ref{tab:viz} is an example of a query which uses a different
visualization type, heat map, and creates 20 bins for both x- and y- axes.

\begin{table}[!t]
  \centering\scriptsize
  \begin{adjustbox}{center}
    {\tt
      \begin{tabular}{|r|l|l|l|}
        \hline
        \zqname & X & Y & Viz \\ \hline
        *f1 & `weight' & `sales' & bin2d.(x=nbin(20), y=nbin(20)) \\ \hline
      \end{tabular}
    }
  \end{adjustbox}
  \vspace{-8pt}
  \caption{Query which returns the heat map of sales vs.~weights across all transactions.}
  \label{tab:viz}
    \vspace{-10pt}
\end{table}

\begin{table}[!t]
  \centering\scriptsize
  \begin{adjustbox}{center}
    {\tt
      \begin{tabular}{|r|l|l|l|}
        \hline
        \zqname & X & Y & Z \\ \hline
        f1 & `year' & `sales' & `product'.`chair' \\ \hline
        f2 & `year' & `profit' & `location'.`US' \\ \hline
        *f3 \IN f1 + f2 & & & `weight'.[? < 10] \\ \hline
      \end{tabular}
    }
  \end{adjustbox}
  \vspace{-8pt}
  \caption{Query which returns the sales for chairs or profits for US
    visualizations for all items less than 10 lbs.}
  \label{tab:name-plus}
      \vspace{-15pt}
\end{table}


\techreport{Like the earlier columns, the Viz column also allows collections of
values. Similar to the Z column, collections may be specified
for both the visualization type or the binning and aggregation. If the user wants to
view the same data binned at different granularities, she might specify a bar
chart with several different bin widths: \mbox{\tt bar.(x=\{bin(1), bin(5),
bin(10)\}, y=agg(`sum'))}. On the other hand, if the user wishes to view the
same data in different visualizations, she might write:
\mbox{\tt \{bar.(y=agg(`sum')), point.()\}}.}


The Viz column allows users powerful control over the structure of
the rendered visualization. However, there has been work from the visualization community
which automatically tries to determine the most appropriate visualization type,
binning, and aggregation for a
dataset based on the x- and y- axis
attributes~\cite{wongvoyager2015,Mackinlay:1986:ADG:22949.22950}. 
Thus, we can frequently leave the Viz
column blank and \zv will use these rules of thumb to automatically decide the appropriate setting for us. With this in
mind, we omit the Viz column from the remaining examples with the assumption
that \zv will determine the ``{best}'' visualization structure for us.

\vspace{-5pt}
\subsubsection{\zqname}
\vspace{-2pt}
Together, the values in the X, Y, Z, and Viz columns of each row specify a
collection of visualizations.  The \zqname column allows us to label these
collections so that they can be referred to be in the \zqproc column. For
example, {\tt f1} is the label or identifier given to the collection of sales bar charts in
Table~\ref{tab:overview-ex2}. The * in front of {\tt f1} signifies that 
the collection is an output collection; that is, \zq should return this
collection of visualizations to the user. 


However, not all rows need to have a * associated with their \zqname identifier.
A user may define intermediate
collections of visualizations if she wishes to further process them in the \zqproc
column before returning the final results. 
In the case of Table~\ref{tab:name-plus},
{\tt f1} and {\tt f2} are examples of intermediate collections. 

Also in Table~\ref{tab:name-plus}, we have an example of how
the \zqname column allows us to perform high-level set-like operations
to combine visualization collections directly.
For example, {\tt f3 \IN f1 + f2} assigns {\tt f3} to the
collection which includes all visualizations in {\tt f1} and {\tt f2} (similar
to set union). 
This can be useful if the user wishes to combine
variations of values without considering the full Cartesian product.
In our example in Table~\ref{tab:name-plus}, the user is able to combine the sales for chairs plots
with the profits for the US plots without also having to consider the sales for the
US plots or the profits for chairs plots; she would have to do so if she had used
the specification: {\tt \mbox{(Y: \{`sales', `profit'\}}, \mbox{Z: \{`product'.`chair',
`location'.`US'\}})}. 

An interesting aspect of Table~\ref{tab:name-plus}
is that the X and Y columns of the third row are devoid of values, and the Z
column refer to the seemingly unrelated weight attribute. The values in
the X, Y, Z, and Viz columns all help to specify a particular collection of
visualizations from a larger collection. 
When this collection is defined via the \zqname column, 
we no longer need to fill in the values for X, Y, Z, or Viz, except to select from
the collection---here, \zq only selects the items which satisfy the
constraint, {\tt weight < 10}.  

\techreport{Other set-like operators include
{\tt f1 - f2} for set minus and {\tt f1 \^{} f2} for intersection.}
 


\begin{table*}[t]
\vspace{-1pt}
  \centering\scriptsize
  \begin{adjustbox}{center}
    {\tt
      \begin{tabular}{|r|l|l|l|l|}
        \hline
        \zqname & X & Y & Z & \zqproc \\ \hline
        f1 & `year' & `profit' & v1 \IN `product'.* & \\ \hline
        %f2 & `year' & y1 \IN \{`sales', `sold'\} & v1 & v2 \IN argmax$_{v1}[k=10] \sum_{y1} D(f1,f2)$ \\ \hline
        f2 & `year' & `sales' & v1 & v2 \IN argmax$_{v1}[k=10] D(f1,f2)$ \\ \hline
        *f3  & `year' & `profit' & v2 & \\ \hline
      \end{tabular}
    }
   \end{adjustbox}
  \vspace{-10pt}  
  \caption{Query which returns the top 10 profit visualizations for products
    which are most different from their sales visualizations.}
  \label{tab:proc1}
\vspace{-5pt}
\end{table*}

\subsubsection{\zqproc}
%\alkim{
%  \begin{itemize}
%    \item
%      Defined iterators on variables, and how labels from Name column iterates
%      through
%    \item
%      The real power of \zq comes not from its ability to specify collections,
%      but to operate on them.
%    \item
%      Allows things like trend-based filtering, similarity search,
%      representative search, outlier search
%    \item
%      To operate on these levels, naturally we need a way to iterate over the
%      collections in some way: in \zq, we use \axvar[cs] and \nmvar[s] for this.
%    \item
%      There's many different ways to iterate over things based on what we want
%      to do exactly, but we opted for dimension-based iteration because we
%      found that's what served our needs for the majority of the cases.
%    \item
%      We also need to specify a way to iterate over collections because there
%      might be multiple dimensions along which they have multiple values.
%    \item
%      Here is how we assign \axvar[Cs] \axvar[] \axvar[c], \axvar[s]
%    \item
%      Now that we have a way to iterate, we define our process primitives (T,D)
%      and our iterators
%    \item
%      Basic ways to check for identity or one-pair, etc
%    \item
%      We found all the tasks by our visual analysts could be summarized as an
%      optimization function
%    \item
%      Give examples of sim, trend, etc.
%    \item
%      We also allow black-box which is how we implement k-mediodes.
%  \end{itemize}
%}
%
The real power of \zq as a query language comes not from its ability to
effortlessly specify collections of visualizations, but rather from its ability
to operate on these collections somewhat declaratively. 
With \zq's processing
capabilities, users can filter visualizations based on trend, search for 
similar-looking visualizations, identify representative visualizations, and
determine outlier visualizations. 
Naturally, to operate on collections, \zq
must have a way to iterate over them; however, 
since different visual analysis tasks
might require different forms of traversals over the collections, 
we expose the iteration
interface to the user.

\paragraph{Iterations over collections.}
Since collections may be composed of varying values from multiple columns,
iterating over the collections is not straight-forward.
Consider
Table~\ref{tab:proc1}---the goal is to return profit
by year visualizations for the top-10 products whose profit by year visualizations 
look the most different
from the sales by year visualizations.
\techreport{This may indicate a product that deserves special attention. }%
While we will describe this query in 
detail below, at a high level the first row assembles
the visualizations for profit over year for all products ({\tt f1}),
the second row assembles the visualizations for sales over year for all products ({\tt f2}), 
followed by operating (via the \zqproc column) on these two collections 
by finding the top-10 products who
sales over year is most different from profit over year,
while the third row displays the profit over year for those top-10 products.
A array-based representation of the visualization collections {\tt f1} and {\tt f2},
would look like the following:
\vspace{-5pt}
\begin{align*}
\scriptsize
  {\tt f1} = 
  \begin{Bmatrix}
    \texttt{X: `year', Y: `profit'} \\
    \begin{array}{l}
      \hline
      \texttt{Z: `product.chair'} \\
      \texttt{Z: `product.table'} \\
      \texttt{Z: `product.stapler'}
    \end{array} \\
    \vdots
  \end{Bmatrix}
  {\tt f2} = 
  \begin{Bmatrix}
    \texttt{X: `year', Y: `sales'}  \\
    \begin{array}{l}
      \hline
      \texttt{Z: `product.chair'} \\
      \texttt{Z: `product.table'} \\
      \texttt{Z: `product.stapler'}
    \end{array} \\
    \vdots 
  \end{Bmatrix}
\end{align*}
We would like to iterate over the products, the Z dimension values, of both {\tt f1}
and {\tt f2} to make our comparisons. Furthermore, we must
iterate over the products in the \emph{same order} for both {\tt f1} and {\tt
f2} to ensure that a product's profit visualization correctly matches with its
sales visualization. 
Using a single index for this would be
complicated and need to take into account the sizes of each of the columns.
\techreport{While there may be other ways to architect this iteration for
a single attribute, it is virtually impossible to do when there are multiple
attributes that are varying. }%
Instead, \zq opts for a more powerful \emph{dimension-based} iteration, which
assigns each column (or dimension) a separate iterator called an
\emph{\axvar[]}.
This dimension-based iteration is a powerful idea that extends to any number of dimensions. 
%In this example, we would like for each product in {\tt f1} to match their respective
%visualizations in {\tt f2}. So, for each value in the Z (product) dimension,
%we would like to
%iterate over the Y dimension in {\tt f2} to compare
%the profit visualization with the sales and sold visualizations.
%With a single
%index, this iteration would be complicated and need to take
%into account the sizes of each of the dimensions. However, this
%dimension-based iteration is a powerful idea which extends to any number of
%dimensions and is formalized in the algebra in Section~\ref{sec:formal-expr}.
%
%Now that we have established the need for dimension-based iteration, we
%introduce the mechanism to label the dimensions: \axvar[s].
%\alkim{Note that only columns which have collections of
%values are counted as dimensions in this scheme.}
%All dimension labels or \emph{\axvar[s]} use the syntax:
As shown in Table~\ref{tab:proc1}, \axvar[s] are defined and assigned
using the syntax:
\mbox{$\langle variable \rangle $\IN$ \langle collection \rangle$};
\axvar[] {\tt v1} is assigned to
the Z dimension of {\tt f1} and iterates over all product values. 
For cases in which multiple collections must traverse
over a dimension in the same order, an \axvar[] must be shared across those
collections for that
dimension;
%
%\axvar[cs] may be shared across collections if we want
%the \zqproc column to iterate over the collections in a consistent manner with
%respect to a dimension;
in Table~\ref{tab:proc1}, {\tt f1} and {\tt f2}
share {\tt v1} for their Z dimension, since we want
to iterate over the products in lockstep.

\paragraph{Operations on collections.}
With the \axvar[s] defined, the user can then formulate the high-level
operations on collections of visualizations as an optimization function which
maximizes/minimizes for their desired pattern. Given that {\tt
argmax$_{x}[k=10] \; g(x)$} returns the top-10 {\tt x} values which maximizes the
function $g(x)$, and $D(x,y)$ returns the ``{distance}'' between {\tt x} and
{\tt y}, now consider the expression in the \zqproc
column for Table~\ref{tab:proc1}.
Colloquially, the expression says to
find the top-10 {\tt v1} values whose $D(f1,f2)$ values are the
largest.
The $f1$ and $f2$ in $D(f1,f2)$ refer to the collections of
visualizations in the first and second row and are bound to the current value
of the iteration for {\tt v1}. In other words, for each product
{\tt v1'} in {\tt v1}, retrieve the
visualizations {\tt f1[z: v1']} from collection {\tt f1} and {\tt f2[z: v1']} 
from collection {\tt f2} and calculate the
``{distance}'' between these visualizations; then, retrieve the 10 {\tt
v1'} values for which this distance is the largest---these are the products, and assign {\tt v2} to this
collection. 
Subsequently, we can access this set of products, as we do in the Z column of 
the third line of Table~\ref{tab:proc1}.

\begin{table*}[t]
\vspace{0pt}
  \centering\scriptsize
  \begin{adjustbox}{center}
    {\tt
      \begin{tabular}{|r|l|l|l|l|}
        \hline
        \zqname & X & Y & Z & \zqproc \\ \hline
        f1 & `year' & `sales' & v1 \IN `product'.* & v2 \IN argmax$_{v1}[t<0]
        T(f1)$ \\ \hline
        *f2 & `year' & `sales' & v2 &  \\ \hline
      \end{tabular}
    }
  \end{adjustbox}
  \vspace{-8pt}
  \caption{Query which returns the sales visualizations for all products which
  have a negative trend.}
  \label{tab:trend}
\vspace{-15pt}
\end{table*}

\begin{table*}[t]
  \centering\scriptsize
  \begin{adjustbox}{center}
    {\tt
      \begin{tabular}{|r|l|l|l|l|}
        \hline
        \zqname & X & Y & Z & \zqproc \\ \hline
        f1 & `year' & `sales' & `product'.`chair' & \\ \hline
        f2 & `year' & `sales' & v1 \IN `product'.(* -  `chair') &
        v2 \IN argmin$_{v1}[k=10] D(f1,f2)$\\ \hline
        *f3 & `year' & `sales' & v2 & \\ \hline
      \end{tabular}
    }
  \end{adjustbox}
  \vspace{-10pt}
  \caption{Query which returns the sales visualizations for the 10 products
    whose sales visualizations are the most similar to the sales visualization
  for the chair.}
  \label{tab:similarity}
\vspace{-10pt}
\end{table*}

\begin{table*}[t]
  \centering\scriptsize
  \begin{adjustbox}{center}
    {\tt
      \begin{tabular}{|r|l|l|l|l|}
        \hline
        \zqname & X & Y & Z & \zqproc \\ \hline
        f1 & `year' & `sales' & v1 \IN `product'.* & \\ \hline
        f2 & `year' & `sales' & v2 \IN `product'.* & v3 \IN argmax$_{v1}[k=10]
        \sum_{v2} D(f1, f2)$ \\ \hline
        *f3 & `year' & `sales' & v3 & \\ \hline
      \end{tabular}
    }
  \end{adjustbox}
  \vspace{-10pt}
  \caption{Query which returns the sales visualizations for the 10 products
  whose sales visualizations are the most different from the others.}
  \label{tab:outlier}
  \vspace{-8pt}
\end{table*}

\paragraph{Formal structure.}
More generally, the basic structure of the \zqproc column is:
{\small
\vspace{-5pt}
\[
  \langle argopt \rangle_{\langle \axvar[a] \rangle}[\langle limiter \rangle] \langle expr \rangle \textrm{ \ \ \  where}
\]
\vspace{-2em}
\begin{align*}
  \langle expr \rangle \; & \rightarrow \; \left(\max | \min | \sum | \prod \right)_{\langle
  \axvar[a] \rangle} \langle expr \rangle \\
  & \rightarrow \; \langle expr \rangle \; (+|-|\times|\div) \; \langle expr \rangle \\
  & \rightarrow \; T(\langle \nmvar[a] \rangle) \\
  & \rightarrow \; D(\langle \nmvar[a] \rangle, \langle \nmvar[a] \rangle) \\
  \langle argopt \rangle \; & \rightarrow \; \left( \text{argmax} | \text{argmin} |
\text{argany} \right) \\
\langle limiter \rangle \; & \rightarrow  \; \left(k=\mathbb{N} \; | \; t>\mathbb{R}
\; | \; p=\mathbb{R} \right)
\end{align*}
}
%
\noindent where $\langle \axvar[a] \rangle$ refers to the \axvar[s], and $\langle \nmvar[a]
\rangle$ refers to collections of visualizations. $\langle argopt \rangle$ may
be one of argmax, argmin, or argany, which returns the values which have the largest, smallest, and
any expressions respectively. The $\langle limiter \rangle$ limits the number of results: 
$k = \mathbb{N}$ returns only the top-$k$ values;
$t>\mathbb{R}$ returns only values who are larger than a threshold value $t$
(may also be smaller, greater than equal, etc.); $p=\mathbb{R}$ returns
the top $p$-percentile values.
$T$ and $D$ are
two simple \emph{functional primitives} supported by \zq that can be applied to
visualizations to find desired patterns:
\begin{denselist}
    \item \ [$T(f) \rightarrow \mathbb{R}$]: $T$ is a function which takes a
    visualization $f$ and returns a real number measuring some visual property of the trend of
    $f$. One such property is ``growth'', which returns a positive number if the overall trend is
    ``{upwards}'' and a negative number otherwise; an
    example implementation might be to measure the slope of a linear fit to the
    given input visualization $f$.
    Other properties may measure the skewness, or the number of peaks, or noisiness
    of a visualization. 
  \item \ [$D(f, f') \rightarrow \mathbb{R}$]: $D$ is a function which takes two
    visualizations $f$ and $f'$ and measures the distance (or dissimilarity)
    between these visualizations. Examples of distance functions may include
    a pointwise distance function like 
    Euclidean distance, Earth Mover's Distance, or the Kullback-Leibler Divergence. 
    The distance $D$ could also be measured using 
    the difference in the number of peaks, or slopes, or some
    other property. 
\end{denselist}
\zq supports many different implementations for these two functional
primitives, and the user is free to choose any one. If
the user does not select one, \zv will
automatically detect the ``{best}'' primitive based on the data
characteristics. Furthermore, if \zq does not have an implementation of the
$T$ or $D$ function that the user is looking for, the user may write and use their own
function.

\paragraph{Concrete examples.}
With just dimension-based iteration, the optimization structure of the \zqproc
column, and the functional primitives $T$ and $D$, we found that we were able
to support the majority of the visual analysis tasks required by our users.
Common patterns include filtering based on overall trend
(Table~\ref{tab:trend}), searching for the most similar visualization
(Table~\ref{tab:similarity}), and determining outlier visualizations
(Table~\ref{tab:outlier}).
\techreport{
Table~\ref{tab:trend} describes a query where in the first row, the variable {\tt v2}
selects all products whose trend is decreasing, and the second row visualizes
these product's sales over year.
Table~\ref{tab:similarity} starts with the visualization 
sales over year for chair in the first row, then in the second row
computes the visualizations of sales over year for all products, and in the process
column computes the similarity with chair, assigning the top 10 to {\tt v2},
and the third row visualizes the sales over year for these products.
Table~\ref{tab:outlier} starts with the visualization collection of sales over year
for all products in the first row, followed by another collection of the same
in the second row, and in the process column computes the sum of pairwise distances,
assigning the 10 products whose visualizations are most distant to others to {\tt v3}, 
after which they are visualized.
}%
Table~\ref{tab:real2} features a realistic query inspired by one of our case
studies. The overall goal of the query is to find the
products which have positive sales and profits trends in locations and
categories which have overall negative trends; the user may want to look at
this set of products to see what makes them so special.
Rows 1 and 2 specify the sales and profit visualizations for all locations and
categories respectively, and the processes for these rows filter down to the
locations and categories which have negative trends. Then rows 3 and 4 specify
the sales and profit visualizations for products in these locations and
categories, and the processes filter the visualizations down to the ones that
have positive trends. Finally, row 5 takes the list of output products from the
processes in rows 3 and 4 and takes the intersection of the two returning the
sales and profits visualizations for these products.




\paragraph{Pluggable functions.}
While the general structure of the \zqproc column does cover the majority of
the use cases requested by our users, users may want to write their own
functions to run in a \zq query. To support this, \zq exposes a {\tt Java}-based API
for users to write their own functions. In fact, we use this interface to
implement the $k$-means algorithm for
\zq.
While the pluggable functions do allow virtually any capabilities to be
implemented, it is preferred that users write their queries using the syntax of
the \zqproc column; pluggable functions are considered black-boxes
and cannot be automatically optimized by the \zq compiler.

% \subsection{Realistic Examples}

% \alkim{
%   Now that we have looked at basic examples, to show the true power and
%   flexibility of \zq, we now show some real-world example queries. These are
%   all queries that visual analysts had to do by hand before.
% }

%\input{real-examples}

\begin{table*}
  \centering\scriptsize
  \begin{adjustbox}{center}
    {\tt
      \begin{tabular}{|r|l|l|l|l|l|l|}
        \hline
        \zqname & X & Y & Z & Z2 & Z3 & \zqproc \\ \hline
        f1 & `year' & `sales' & v1 \IN `location'.* & & & v2 \IN
        argany$_{v1}[t<0] T(f1)$\\ \hline
        f2 & `year' & `profit' & v3 \IN `category'.* & & & v4 \IN
        argany$_{v3}[t<0] T(f2)$\\ \hline
        f3 & `year' & `profit' & v5 \IN `product'.* & `location'.[? IN v2] &
        `category'.[? IN v4] & v6 \IN argany$_{v5}[t>0] T(f3)$ \\ \hline
        f4 & `year' & `sales' & v5 & `location'.[? IN v2] &
        `category'.[? IN v4] & v7 \IN argany$_{v5}[t>0] T(f4)$ \\ \hline
        *f5 & `year' & \{`profit', `sales'\} & v6 \^{} v7 & & & \\ \hline
      \end{tabular}
    }
  \end{adjustbox}
  \vspace{-10pt}
  \caption{Query which returns the profit and sales visualizations for products
    which have positive trends in profit and sales in locations and categories
  which have overall negative trends.}
  \label{tab:real2}
  \vspace{-15pt}
\end{table*}

 \vspace{-2pt}
\subsection{Discussion of Capabilities and Limitations}\label{subsec:cap-lim}
Although \zq can capture 
a wide range of visual exploration queries, it is not
limitless. Here, we give a brief description of what \zq can do.
A more formal quantification can be found in
\papertext{\cite{techreport}}\techreport{Section~\ref{sec:formal-expr}}.

\zq's primary goal is to support queries over visualizations---which are themselves
aggregate group-by queries on data. 
Using these queries, \zq can compose a collection of visualizations, 
filter them in various ways, compare them against benchmarks or against
each other, and sort the results. 
The functions $T$ and $D$, while intuitive, support the ability
to perform a range of computations on visualization collections---for example, 
any filter predicate on a single visualization, checking for a specific
visual property, can be captured under $T$.
\techreport{With the pluggable functions, the ability to perform sophisticated computation
on visualization collections is enhanced even further. }%
Then, via the dimension-based iterators, \zq supports the ability to chain
these queries with each other and compose new visualization collections.
These simple set of operations offer unprecedented power in being able to
sift through visualizations to identify desired trends.

Since \zq already operates one layer above the data---on the visualizations---it does
not support the {\em creation of new derived data}:
that is, \zq does not support the generation of derived attributes or values 
not already present in the data. 
The new data that is generated via \zq is limited to those from binning 
and aggregating via the Viz column.
This limits \zq's ability to perform prediction---since feature engineering is
an essential part of prediction; it also limits \zq's ability to 
compose visualizations on combinations of attributes at a time,
e.g., $\frac{A1}{A2}$ on the X axis. 
Among other drawbacks of \zq: \zq does not support 
\begin{inparaenum}[(i)] 
\item recursion; 
\item any data modification; 
\item non-foreign-key joins nor arbitrary nesting; 
\item dimensionality reduction or other changes to the attributes; 
\item other forms of processing visualization collections not expressible via $T$, $D$ or the
black box;
\techreport{\item multiple-dimensional visualizations;}
\techreport{\item intermediate variable definitions;}
\item merging of visualizations (e.g., by aggregating two visualizations);
and 
\item 
statistical tests.
\end{inparaenum}


==> docs copy/nphardnessproof.tex <==
%!TEX root=zenvisageql.tex
\techreport{
The cost of adding a thread, $\alpha$, is generally more than $M_G$---for instance, in PostgreSQL we found $\alpha$ > 100k ($M_G$) for different experimental settings. By further 
assuming that the cost of processing all group by values < $M_G$ is same, we can simplify the problem to finding the minimum number of combined queries such that the maximum number of group by values per 
combined query is less than $M_G$. We prove that the solution to this problem is {\sc NP-Hard} by reduction from the {\sc Partition Problem}. 
\begin{proof} 
Let $g_1,g_2,...g_n$ be the group by values for the queries $Q_1,Q_2,...,Q_n$ we want to combine.
We want to find minimum number $m$ of combined queries, such that each combined query $G_i$ 
has at most $M_G$ maximum group by values. 
Recall that in the Partition problem, we are given an instance of n numbers $a_1,a_2,...,a_n$, and we are asked to decide if
there is a set $S$ such that $\sum_{a_i \subset S}a_i=\sum_{a_i \not \subset S}a_i$. 
Let $A=\sum a_i$ and consider an instance of Query Combination problem with $g_i=M_G^{\frac{2\times a_i}{A}}$. 
With this setting, it is easy to see that the answer to the Partition instance is YES 
if and only if the minimum number of combined queries is 2.
\end{proof} 
}


==> docs copy/ordered-bag-algebra.tex <==
%!TEX root=zenvisageql.tex

\subsection{Ordered Bag Semantics}
\label{subsec:ordered-bag}
In \vzalg, relations have bag semantics. However, since users want to
see the most relevant visualizations first, ordering is critical. So, we
adapt the operators from relational algebra to preserve ordering
information.


Thus, we operate on {\em ordered bags} (i.e., a bag that has an inherent
order). 
We describe the details of how to operate on ordered bags below.
We use the variables $R,S$ to denote ordered bags. 
We also use the notation $R = [t_1, \ldots, t_n]$ to refer to an ordered bag,
where $t_i$ are the tuples. 

The first operator that we define is an indexing operator, much like
indexing in arrays.
The notation $R[i]$ refers to the $i$th tuple within $R$, and $R[i:j]$ refers
to the ordered bag corresponding to the list of tuples from the $i$th
to the $j$th tuple, both inclusive. In the notation $[i:j]$ if either one of
$i$ or $j$ is omitted, then it is assumed to be $1$ for $i$, and $n$ for $j$,
where $n$ is the total number of tuples.

Next, we define a union operator $\cup$: $R \cup S$ refers to the concatenation
of the two ordered bags $R$ and $S$.  
If one of $R$ or $S$ is empty, then the result of the union is simply the other
relation. We define the union operation first 
because it will come in handy for subsequent operations.
 
We define the $\sigma$ operator like in relational algebra, via a recursive definition:
$$\sigma_\theta (R) = \sigma_\theta ([R[1]]) \cup \sigma_\theta (R[2:])$$
where $\sigma_\theta$ when applied to an ordered bag with a single tuple ([t])
behaves exactly like in the relational algebra case, returning the same
ordered bag ([t]) if the condition is satisfied, and the empty ordered bag
([]) if the condition is not satisfied.
The $\pi$ operator for projection is defined similarly to $\sigma$ in the equation above,
with the $\pi$ operator on an ordered bag with a 
single tuple simply removing the irrelevant attributes from that tuple,
like in relational algebra. 

Then, we define the $\setminus$ operator, for ordered bag difference. 
Here, the set difference operator operates on every tuple in the first ordered
bag and removes it if it finds it in the second ordered bag.
Thus:
$$R \setminus S = ([R[1]] \setminus S) \cup (R[2:] \setminus S)$$
where $[t] \setminus S$ is defined like in relational algebra, 
returning $[t]$ if $[t]$ is not in $S$, and $[]$ otherwise. The intersection
operator $\cap$ is defined similarly to $\cup$ and $\setminus$.

Now, we can define the duplicate elimination operator as follows:
$$\delta(R) = [R[1]] \cup (R[2:] \setminus [R[1]])$$
Thus, the duplication elimination operator preserves ordering, while maintaining the first
copy of each tuple at the first position that it was found in the ordered bag.

Lastly, we have the cross product operator, as follows:
$$R \times S = ([R[1]] \times S) \cup (R[2:] \times S)$$
where further we have
$$[t] \times S = ([t] \times [S[1]]) \cup ([t] \times S[2:])$$
where $[t] \times [u]$ creates an ordered bag with the result of the cross product 
as defined in relational algebra.

Given these semantics for ordered bags, we can develop the visual exploration algebra.


% \begin{description}
%   \item[$\sigma(R) = S$:] 
%     $\forall t,t' \in S \times S \quad
%     i_t(S) < i_{t'}(S) \implies i_t(R) < i_{t'}(R)$
%   \item[$\pi(R) = S$:]
%     %$t' \subseteq t \implies i_{t'}(S) \le i_{t}(R) \quad \forall t,t' \in R
%     %\times S$
%     $\forall t,u \in S \times S, \exists t' \in R, \forall u' \in R \quad
%     i_{t}(S) < i_{u}(S)
%     \land (t \subseteq t') \land (u \subseteq u')
%     \implies
%     i_{t'}(R) < i_{u'}(R)
%     $
%   \item[$R \times S = T$:]
%     $\forall t,t' \in R \times S \quad
%     i_{t+t'}(T) = i_t(R) |S| + i_{t'}(S)$
%   \item[$R \cup S = T$:]
%     $\forall t, t' \in T \times T \quad
%     i_t(T) < i_{t'}(T) \implies \min(i_t(R), |R|+i_t(S)) < \min(i_{t'}(R),
%     |R|+i_{t'}(S))$
%   \item[$R \setminus S = T$:]
%     $\forall t,t' \in T \times T \quad
%     i_t(T) < i_{t'}(T) \implies i_t(R) < i_{t'}(R)$
% \end{description}

%\alkim{Someone needs to double check whether the properties above properly
%  constrain what I want, which is basically that later duplicates should all be
%erased in favor of the first appearance, in addition to their natural
%definitions.}



==> docs copy/queryexecution.tex <==
%!TEX root=zenvisageql.tex

\begin{table*}[!htbp]
%\vspace{-5pt}
  \centering\scriptsize
 {\tt
  %\resizebox{\linewidth}{!}{%
    \begin{tabular}{|r|l|l|l|l|l|l|} \hline
      \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Z} &
      \textbf{Constraints}
      & \textbf{Viz} & \textbf{Process} \\ \hline
      f1 & `year' & `sales' & v1 \IN P & location=`US' & bar.(y=agg('sum')) &
      v2 \IN
      $argany_{v1}[t>0] T(f1)$ \\
      f2 & `year' & `sales' & v1 & location=`UK' & bar.(y=agg('sum')) & v3 \IN $argany_{v1}[t<0] T(f2)$ \\
      *f3 & `year' & `profit' & v4 \IN (v2.range | v3.range) &
      & bar.(y=agg('sum')) & \\ \hline
    \end{tabular}
  %}
  %\end{alltt}
  }
    \vspace{-10pt}
  \caption{
    A \zq query which returns the profit over time visualizations for products
    in user-specified set {\tt P}
    that have positive sales over time trends for the US but have negative sales
    over time trends for the UK.
  }
  \label{tab:exec-1}
  {\tt
  %\resizebox{\linewidth}{!}{%
    \begin{tabular}{|r|l|l|l|l|l|l|} \hline
      \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Z} &
      \textbf{Constraints} & Viz
      & \textbf{Process} \\ \hline
      f1 & `location' & `sales' & v1 \IN P & year=`2010' & bar.(y=agg('sum')) & \\
      f2 & `location' & `sales' & v1 & year=`2015' & bar.(y=agg('sum')) & v2 \IN $argmax_{v1}[k=10] D(f1,f2)$ \\
      *f3 & `location' & `profit' & v2 & year=`2010' & bar.(y=agg('sum')) & \\
      *f4 & `location' & `profit' & v2 & year=`2015' & bar.(y=agg('sum')) & \\ \hline
	  	
    \end{tabular}
  %}
  %\end{alltt}
  }
  \vspace{-10pt}
  \caption{
    A \zq query which returns the profit over location visualizations for
    products in user-specified set {\tt P}
    that have the most different sales over location trends between 2010 and 2015.
  }
  \label{tab:exec-2}
    \vspace{-10pt}
\end{table*}

\section{Query Execution}
\label{subsec:query_execution}
In \zv, \zq queries are automatically parsed and executed by the backend.
The \zq compiler translates \zq queries into a collection of \sql queries
that are issued to a relational database and performs
post-processing computation on the results
of the \sql queries. 
By translating to \sql, we do not tie ourselves down to any specific
  relational database and can seamlessly leverage benefits from improvements to
databases.
%\new{By operating outside standard relational databases, we can seamlessly
%leverage benefits from improvements to the database; further, we can replace
%one relational database for another. 
%That said, we may be able to leverage benefits from moving computation
%``closer to'' the data; we plan to explore this in future work.}

\subsection{Translation to Database Queries}
Each row of a \zq query can be broken up into two parts: the visual component and the
the Process column. The visual components 
determine the set of data \zv needs to retrieve from the database, and the
Process column translates into the post-processing computation to be done on
the returned data. \techreport {\zv's naive \zq compiler performs the following operations for each row of a 
\zq query.}
For each row, the \zq compiler issues a \sql query 
corresponding to each visualization in the set specified in the visual component.
\techreport{Notice that this approach is akin to what a visual analyst manually
generating each visualization of interest and perusing it would do;
here, we are ignoring the human perception cost.}
More formally, for each row (i.e., each name variable),
the \zq compiler loops over all combinations of values
for each of the $n$ axis variables in the visual component corresponding
to that row, and for each combination, 
issues a \sql query,
the results of which are stored in the corresponding
location in an $n$ dimensional array.
\techreport{(Essentially, this corresponds to a nested for loop $n$ levels
deep.)}
Each
generated \sql query has the form:
{\tt \small SELECT X, Y FROM R WHERE Z=V AND (CONSTRAINTS) ORDER BY X}.
% \vspace{-5pt}
% \begin{quote} \small
% \begin{verbatim}
% SELECT X, Y 
% WHERE Z=V and (CONSTRAINTS) 
% ORDER BY X
% \end{verbatim}
% \end{quote}
% \vspace{-5pt}
If the summarization is specified, additional clauses
such as {\tt GRO\-UP BY}s and aggregations may be added. 
The results of each visualization are stored 
in an $n$-dimensional array
at the current
index. If $n$ is 0, the name variable points directly to the data.
\techreport{Going forward, we will omit the \texttt{FROM} clause: this is implied
and always fixed.}



Once the name variable array has been filled in with results
from the \sql queries,  
the \zq compiler generates the
post-processing code from the task in the Process
column. 
At a high level, \zq loops through all the visualizations, and applies
the objective function on each one. 
In particular, for each input axis variable in the mechanism, a 
{\tt for} loop is created and nested. The input axis variables are then used to
step through the arrays specified by the name variable, and the objective
function is called at each iteration. Instances of name variables are
updated with the correct index based on the axis variables it depends on. The
functions themselves are considered black boxes to the \zq compiler and are unaltered.
% \agp{This may be precise from a procedural standpoint but this is rather
% opaque. Can we talk about what you're trying to do? seems like all you're doing is to
% pass along each generated visualization to the objective function which has access
% to all the characteristics/attributes/properties of that visualization}
\papertext{We provide the psuedocode of the compiled version of the
query in~\cite{techreport}.}
\techreport{We provide the psuedocode of the compiled version of the
query expressed in Table~\ref{tab:exec-1} in Listing~\ref{lst:exec-1} in
the appendix.}


\subsection{External Optimizations}
Processing each visualization as an independent \sql query can be 
both wasteful and lead to unacceptable latencies.
We now describe how to rewrite and batch the \sql queries
via three levels of optimizations to reduce latency.
These optimizations are reminiscent of multi-query optimization
(MQO)~\cite{DBLP:journals/tods/Sellis88}; however, MQO techniques require
significant changes to the underlying database
engine~\cite{giannikis2013workload,psaroudakis2013sharing,DBLP:journals/pvldb/KementsietsidisNCV08,giannikis2014shared},
whereas our
syntactic rewriting techniques operate completely outside the database and are
tailored to the \zq setting.
\papertext{We omit many details that can be found in~\cite{techreport}.}
%The first two are straightforward and are 
%are reminiscent of multi-query optimization (MQO)~\cite{DBLP:journals/tods/Sellis88}---\new{however,
%MQO requires significant changes to the underlying
%engine, as opposed to our syntactic rewriting techniques
%that operate outside the database.}
%We focus on the third level, tailored to \zq.


% \techreport{While the translation process of the naive \zq compiler is simple and easy to
% follow, there is plenty of room for optimization. In particular, we look at
% three levels of optimization which focus on \emph{batching} \sql queries. 
% We found that the time it took to submit and wait for \sql queries was a
% bottleneck, and reducing the overall number of \sql queries can reduce performance 
% significantly.
% While none of these optimizations may seem particularly surprising,
% it required a substantial amount of effort to identify how these optimizations
% may be applied automatically to any \zq query. 
% \new{Our proposed optimizations are
% reminiscent of multi-query optimization techniques~\cite{DBLP:journals/tods/Sellis88}, but are tailored
% to \zq queries.}
% }

\paragraph{Intra-Line Optimization.}
\papertext{The first optimization level batches the \sql queries from a \zq row into one
query. For example, we can retrieve the data for all products in the first row
Table~\ref{tab:exec-1} in one \sql query. Similarly, if
the axis variable is in either the X or Y columns, we retrieve the data for
the entire set of attributes the axis variable iterates over. 
To ensure that the overhead of computation outside of the database
is minimal, we add appropriate {\tt ORDER BY} clauses to ensure
that additional sorting is not needed.
}
\iftechreportcode
The first level of optimization batches the \sql queries for a row into one
query. For example, we see that for the first row in Table~\ref{tab:exec-1}, that
a separate query is being made for every product in Listing~\ref{lst:exec-1}
in the appendix.
Instead, we can retrieve the data for all products in one \sql query:
\vspace{-5pt}
\begin{quote}\small
\begin{verbatim}
SELECT year, SUM(sales), product
  WHERE product IN P and location=`US'
  GROUP BY product, year
  ORDER BY product, year
\end{verbatim}
\end{quote}
\vspace{-5pt}
If the axis variable is in either the X or Y columns, we retrieve the data for
the entire set of attributes the axis variable iterates over. More concretely,
if we have axis variable {\tt y1 \IN \{`sales', `profit'\}}, our \sql
query would look like:
\vspace{-5pt}
\begin{quote}\small
\begin{verbatim}
SELECT year, SUM(sales), SUM(profit), product
  WHERE product IN P and location=`US'
  GROUP BY product, year
  ORDER BY product, year
\end{verbatim}
\end{quote}
\vspace{-5pt}
This optimization cuts down the number of queries by the sizes of sets the axis
variables range over, and therefore will lead to substantial performance benefits,
as we will see in the experiments.
Note that a side effect of batching queries is that the compiled code must now have an
extra phase to extract the data for different visualizations from the combined
results. However, since the \zq compiler includes an {\tt ORDER BY} clause, the
overhead of this phase is minimal.
\fi



\input{intra-proc-opt}
\input{inter-proc-opt}


==> docs copy/querylanguage.tex <==
%!TEX root=zenvisageql.tex





%\begin{table*}[h]
%  \centering
%  \begin{alltt}
%  %\resizebox{\linewidth}{!}{%
%    \begin{tabular}{|r|l|l|l|l|l|l|} \hline
%      \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Z} & \textbf{Constraints}
%      & \textbf{Viz} & \textbf{Process} \\ \hline
%      f1 & `time' & `profit' & v1 IN `product'.* & location=`US' & & \\
%      f2 & `time' & `profit' & v1 & location=`UK' & & v2
%      IN $argmax_{v1}[k=10] D(f1, f2)$ \\
%      *f3 & `time' & `sales' & v2 & & & \\ \hline
%    \end{tabular}
%  %}
%  \end{alltt}
%  \vspace{-10pt}\caption{An example \zq query.}
%  \label{tab:overview-ex}
%\vspace{-10pt}\end{table*}
%
%\begin{table*}[h]
%  \centering
%  \resizebox{\linewidth}{!}{%
%    \begin{tabular}{|r|l|l|l|l|l|l|} \hline
%      \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Z}
%      & \textbf{Process} \\ \hline
%      f1 & x1 IN \{* - Y - `product'\} & y1 in (Y = \{`profit', `sales', `revenue'\}) &
%      `product'.`desk' & \\
%      f2 & x1 & y1 & `product'.`chair' &x2, y2 IN $argmax_{x1, y2} D(f1,f2)$ \\
%      *f3 & x2 & y2 & v1 IN `product'.\{`desk', `chair'\} & \\ \hline
%    \end{tabular}
%  }
%  \vspace{-10pt}\caption{A SeeDB-style query written in \zq.}
%  \label{tab:seedb}
%\vspace{-10pt}\end{table*}

%\alkim{Go back through these examples and see which ones need
%aggregating/binning}

We now formally describe the \zq syntax.
We assume that we are operating on a single relation
or a star schema where the attributes are unique
(barring key-foreign key joins).
In general, \zq could be applied to arbitrary collections
of relations by letting the user precede an attribute $A$
with the relation name $R$, e.g., $R.A$.
For ease of exposition, we focus on the single relation case.

\subsubsection{Overview}
As described earlier, a \zq query is composed using a table,
much like a QBE query.
Unlike QBE, the columns of a \zq query do not refer to attributes
of the table being operated on; instead, they are predefined, and have
fixed semantic meanings.
In particular, at a high level, the columns are:
\begin{inparaenum}[(i)]
\item {\em Name:} providing an identifier for a set or collection of visualizations,
and allowing us to indicate if a specific set of visualizations
are to be output
\item {\em X, Y:} specifying the X and Y axes of the collections of visualizations,
restricted to sets of attributes
\item {\em Z (optional):} specifying the ``slice'' (or subset) of data that we're varying
restricted to sets of attributes along with values for those attributes;
\item {\em Constraints (optional):} specifying optional constraints applied to
the data prior to any visualizations or collections of visualizations being generated
\item {\em Viz (optional):} specifying the mechanism of visualization,
e.g., a bar chart, scatterplot, as well as the associated
transformation, or aggregation, e.g., the X axis is binned in groups of 20,
while the Y axis attribute is aggregated using SUM.
If this is not specified, standard rules of thumb are used
to determine the appropriate visualization~\cite{wongvoyager2015,Mackinlay:1986:ADG:22949.22950}.
\item {\em Process (optional):} specifying the ``optimization'' operation performed
on a collection of visualizations, typically intended towards identifying
desired visualizations. 
\end{inparaenum}

A \zq query may have any number of rows, and conceptually each row represents a
set of visualizations of interest. 
The user can then process and
filtrate these rows until she is left 
with only the output visualizations she is
interested in.
The result of a \zq query is the \emph{data} used to generate visualizations.
The \zv front-end then generates the visualizations for the user to peruse.

\paragraph{The Merits of a Tabular Interface.} 
The reader may wonder why we chose a table as an interface
for entering \zq queries. 
Our choice is due to our end-users: primarily non-programmers
who are used to drop-down menus and spreadsheet tools like Microsoft
Excel, and feel more at home with a tabular interface.
Specifically, the tabular skeleton ensures that users would not 
``miss out'' on key columns, and can view the query on the web-client front-end 
as a collection
of correct steps, each of which corresponds to a row.
Indeed, our user study validates this point; even users
with minimal programming experience can still use \zq proficiently after a
short tutorial.
Additionally, this interface is much more suited for embedding into an
interactive web-client.
That said, a user with more experience in programming
may find the interface restrictive, and may prefer
issuing the query as a function call within a programming language.
Nothing in our underlying \zq backend is tied to the tabular interface:
specifically, we already support the issuing of \zq queries within our 
Java client library: users can easily embed \zq queries into other computation. 
\techreport{In the future, we plan to write wrappers for other libraries
so that users can embed \zq into computation in other settings.
We are exploring the use of Thrift~\cite{slee2007thrift} for this purpose.}
% An astute reader may wonder why we chose table as an interface for entering a \zq query. Our thinking is that the formulation of a complex query as a table captures the user\textquotesingle s thought process - the user first breaks a complex query into multiple subqueries, and represents each sub-query as a row. Unlike in a programming language or a text based language where the user needs to remember the phrase structure of the language, table provides an easy to understand skeleton for users to write a syntactically admissible query. That said, a user with more experience in programming can directly write the query using our java client library (currently used by the front-end). In future, we plan to write libraries in other languages atop which users can build their own graphical interface, or can use them directly to make a query to the \zv backend.
%Table~\ref{tab:overview-ex} gives an example of what a fully-fledged \zq query
%would look like. At a high level, this example returns the general sales over
%time visualizations for the top 10 products whose profit over time
%visualizations for the US and the UK have the greatest discrepancy.
%%In the rest of this section, we define how to declare and use variables in the
%%context of \zq and discuss the characteristics of each column in a
%%\zq query.
%Table~\ref{tab:seedb} gives an example of a SeeDB-style query using \zq where
%we try to find the most distinguishing x- and y- axes for the desk and chair.
%Note that in Table~\ref{tab:seedb}, we have chosen to omit the Constraints and
%Viz columns to reduce space. The reader may assume that for this and future
%examples, any omitted column has blanks for every table cell in that column.
%In the rest of this section, we delve more deeply into what each of the columns
%in a \zq query semantically refers to and what values the columns can take on.

\subsubsection{X and Y Columns}
As mentioned, each row can be thought of as a set of visualizations, and the X
and Y columns represent the x- and y- axes for those visualizations. In
Table~\ref{tab:motiv-ex-1}, the first row's visualizations will have `year'
as their x-axis and `profit' as their y-axis. 

The only permissible entries for the X or Y column are either
a single attribute from the table, or 
a {\em set} of attributes, with a variable to iterate over them.
\techreport{The exact semantics of variables and sets are discussed later in
Section~\ref{sec:variables}, 
but essentially, a column is allowed to take on any
attribute from the set.}
For example, in Table~\ref{tab:y-set}, the y-axis is allowed to take on either
`profit' or `sales' as its attribute. 
Because the y-axis value can be
taken from a set of attributes, the resulting output of this query is actually
the \emph{set} of visualizations whose x-axis is the `time' and the y-axis is
one of `profit' and `sales' for the `stapler'. 
This becomes a powerful
notion later in the Process column where we try to iterate over a set of
visualizations and identify desired ones to return to the user
or select for down-stream processing.
\begin{table}[H]
\vspace{-10pt}
 \centering\scriptsize
  {\tt    
  \begin{tabular}{|r|l|l|l|} \hline
      \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Constraints} \\ \hline
      *f1 & `year' & y1 \IN \{`profit', `sales'\} & product=`stapler' \\ \hline
    \end{tabular}
  }
  \vspace{-10pt}\caption{A query for a set of visualizations, one of which plots profit
  over year and one of which plots sales over time for the stapler.}
  \label{tab:y-set}
\vspace{-10pt}
\end{table}

%y-axis is allowed to for the first row can take on
%any one of `profit', `sales', and `revenue', and the x-axis can take
%on any attribute that is not `profit', `sales', `revenue', and
%`product'. Note that, however, 
%The second row takes on the same sets as the first
%row for its X and Y columns, and the third row takes on the sets of X and Y
%values output by the process column of the second row.
%values output by the process column of the second row. The full semantics of As a side note, with
%Table~\ref{tab:seedb} and other examples queries presented
%; the process column is
%discussed further in Section~\ref{sec:process}.


\subsubsection{Z Column}
The Z column is used to either focus our attention on a specific slice 
(or subset) of the dataset or
iterate over a set of slices for one or more attributes. 
To specify a set of slices,
the Z column must specify (a) one or more attributes,
just like the X and Y column, and
(b) one or more attribute values for each of those attributes --- which 
allows us to slice the data in some way.
For both (a) and (b) the Z column could specify a single 
entry, or a variable associated with a set of entries.
Table~\ref{tab:z-1} gives an example of using the Z column to visualize the
sales over time data specifically with regards to the `chair' and `desk'
products, one per line. 
Note that the attribute name and the attribute value are separated
using a period.


Table~\ref{tab:z-2} depicts an example where we iterate over
a set of slices (attribute values)
for a given attribute. 
This query returns the set of sales over time
visualizations for each product. Here, {\tt v1} binds to
the values of the `product' category. Since \zq internally associates
attribute values with their respective attributes, there is no need to
specify the attribute explicitly
for {\tt v1}. 
\techreport{Another way to think about this is to think of v1 \IN `product'.* as
syntactic sugar for `product'.v1 \IN `product'.*. The * symbol denotes all
possible values; in this case, all possible values of the `product'
attribute.}

\begin{table}[H]
\vspace{-10pt}
  \centering\scriptsize
  {\tt  
    \begin{tabular}{|r|l|l|l|} \hline
      \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Z} \\ \hline
      *f1 & `year' & `sales' & `product'.`chair' \\
      *f2 & `year' & `sales' & `product'.`desk' \\ \hline
    \end{tabular}
  }
  \vspace{-10pt}\caption{A \zq query that returns the sales over year visualization for
  chairs and the sales over time visualization for desks.}
  \label{tab:z-1}
\vspace{-10pt}\end{table}

\begin{table}[H]
\vspace{-10pt}
  \centering\scriptsize
  {\tt  
    \begin{tabular}{|r|l|l|l|} \hline
      \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Z} \\ \hline
      *f1 & `year' & `sales' & v1 \IN `product'.* \\ \hline
    \end{tabular}
  }
  \vspace{-10pt}\caption{A \zq query that returns the set of sales over year visualizations
  for each product.}
  \label{tab:z-2}
\vspace{-10pt}\end{table}

\techreport{Furthermore, the Z column can be left blank if the user does not wish to slice the data in any way.}


\subsubsection{Constraints Column}
\label{sec:constraints}
The Constraints column is used to specify further constraints on the set of
data used to generate the set of visualizations. 
Conceptually, we can view the Constraints column as being applied
to the dataset first, following which a collection of visualizations
are generated on the constrained dataset.
While the Constraints column may appear to overlap in functionality with 
the Z column, the Constraints column does not admit iteration via
variables in the way the Z, X or Y column, admits.
It is instead intended to apply a fixed boolean predicate to each tuple of 
the dataset prior to visualization in much the same way the \texttt{WHERE} clause
is applied in \sql. 
\techreport{(We discuss this issue further in Section~\ref{sec:variables}.)}
A blank Constraints column means no constraints are applied\techreport{ to the
data prior to visualization}.


% This may appear to overlap in
% functionality with the Z columns, but there are a few key differences which
% distinguish the two columns. First, variables can be declared and
% used generally in the Z columns but not in the Constraints column. Only a
% single exception exists for when the user can use a variable in the
% Constraints column, and this exception is covered in Section~\ref{sec:variables}.
% However, any other use of variables and declarations of variables are
% prohibited in the Constraints column. This rule essentially precludes the
% Constraints column from taking on a set of values as a variable must always be
% associated with a set of values in \zq, for reasons we discuss in
% Section~\ref{sec:variables}.




\input{formal-viz}

\subsubsection{Name Column}
For any row of a \zq query, 
the combination of X, Y, Z, Constraints, and Viz
columns together represent the \emph{visual component} of that row. 
A visual component formally represents a set of visualizations. 
The Name column allows us to provide a name to this visual component 
by binding a variable to it.
These variables can be used in the Process column
to subselect the desired visualizations from the set of visualizations,
as we will see subsequently.

\begin{table*}[!htbp]
  \centering\scriptsize
  {\tt
    \begin{tabular}{|r|l|l|l|l|} \hline
      \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Z} & \textbf{Process} \\ \hline
      *f1 & `year' & `sales' & `product'.`stapler' & \\
      f2 & `year' & `sales' & v1 \IN `product'.(* - `stapler') & v2 \IN
      $argmin_{v1}[k=10] D(f1,f2)$ \\
      *f3 & `year' & `sales' & v2 & \\ \hline
    \end{tabular}
  }
  \vspace{-10pt}\caption{A \zq query retrieving the sales over year visualization for the top
    10 products whose sales over year visualization looks the most similar to that
  of the stapler.}
  \label{tab:name-1}
\techreport{
\centering\scriptsize
  {\tt
    \begin{tabular}{|r|l|l|l|l|} \hline
      \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Z} & \textbf{Process} \\ \hline
      -f1 & & & & \\
      f2 & x1 \IN \{`time', `location'\} & y1 \IN \{`sales', `profit'\} &
      `product'.`stapler' & x2, y2 \IN $argmin_{x1,y1}[k=10] D(f1,f2)$ \\
      *f3 & x2 & y2 & `product'.`stapler' & \\ \hline
    \end{tabular}
  }
  \vspace{-10pt}\caption{A \zq query retrieving two different visualisations (among different combinations of x and y) of stapler which are most similar to each other}
  \label{tab:name-2}}
\vspace{-10pt}\end{table*}


\papertext{
In Table~\ref{tab:name-1}, {\tt f1} is bound to the single visualization in
the first row, while {\tt f2} is bound to the variable which iterates over the
set of visualizations in the second row. Any rows prefaced with a * symbol are
output rows; visualizations corresponding to these rows are processed and
displayed by the \zv frontend.
}
\techreport{
In the \zq query given by Table~\ref{tab:name-1}, 
we see that the names for the visual components of
the rows are named {\tt f1}, {\tt f2}, and {\tt f3} in order of the rows. 
For the first row, the
visual component is a single visualization, since there are no sets, and {\tt f1}
binds to the single visualization. 
For the second row, we see that the visual
component is over the set of visualizations with varying Z column values, and
{\tt f2} binds to the variable which iterates over this set. 
Note that {\tt f1} and {\tt f3} in Table~\ref{tab:name-1} are prefaced
by a * symbol.
This symbol indicates that the visual component of the row
is designated to be part of the output.
As can be seen in the example, multiple rows can be part of the output,
and in fact, a row could correspond to multiple visualizations.
Visualizations corresponding to all the rows marked with * are 
processed and displayed by the \zv frontend.
}


%Table~\ref{tab:name-2} depicts another example.
%We see that f1 of Table~\ref{tab:name-2} is prefaced with a - and has no other
%column set except for the Name column. This is an example of a user input row.
%f1 refers to a visualization that the user has input either via by drawing it
%directly using the \zv front-end, providing a set of data values, or specifying
%a list of constraints of what the visualization could be. The variable
%associated with the user input visualization can then be treated like any other
%singular visualization for the rest of the \zq query.
%This could be useful, for instance, if the user intends to find visualizations
%similar to the one that she drew, for example, a scatterplot with a correlation
%along the x=y line, or a line chart with two peaks.



\later{If multiple columns'
values are sets, the visual component becomes the set of visualizations that
would span over the Cartesian product of these column sets.
Table~\ref{tab:name-2} provides an example of this in the second row.
}


\later{Name cells may be blank, but then there would be no way to refer to the
visual component of that row, obviating the need for the row in the first place. If not blank,
Name cells may only have variable names possibly prefaced with either * or - as
it only possible values.}


\input{sets-and-vars}
\input{formal-process}

\later{
\subsubsection{Limitations}
\alkim{We probably want to move this section to another place}
\begin{itemize}
  \item \zq fundamentally assumes a 2-D visualization
\end{itemize}
}


==> docs copy/real-examples.tex <==
\begin{table*}
  \centering\scriptsize
  \begin{adjustbox}{center}
    {\tt
      \begin{tabular}{|r|l|l|l|l|l|l|}
        \hline
        \zqname & X & Y & Z & Z2 & Z3 & \zqproc \\ \hline
        f1 & `year' & `depdelay' & v1 \IN `origin'.* & & & v2 \IN
        argany$_{v1}[t<0] T(f1)$\\ \hline
        f2 & `year' & `arrdelay' & v3 \IN `dest'.* & & & v4 \IN
        argany$_{v3}[t<0] T(f2)$\\ \hline
        f3 & `year' & `arrdelay' & v5 \IN `carrier'.* & `origin'.[? IN v2] &
        `dest'.[? IN v4] & v6 \IN argany$_{v5}[t>0] T(f3)$ \\ \hline
        f4 & `year' & `depdelay' & v5 & `origin'.[? IN v2] &
        `dest'.[? IN v4] & v7 \IN argany$_{v5}[t>0] T(f4)$ \\ \hline
        *f5 & `year' & \{`arrdelay', `depdelay'\} & v6 \^{} v7 & & & \\ \hline
      \end{tabular}
    }
  \end{adjustbox}
  \caption{Query which returns the sales visualizations for the 10 products
  whose sales visualizations are the most different from the others.}
  \label{tab:real2}
\end{table*}


==> docs copy/related.tex <==
%!TEX root=zenvisageql.tex
\vspace{-5pt}
\section{Related Work}
\label{sec:related}
\vspace{-2pt}


We now discuss related prior work in a number of areas.
We begin with analytics tools --- visualization tools,
statistical packages and programming libraries, and relational databases.
Then, we talk about other tools that overlap somewhat with  \zv.
% To aid our discussion, in Figure \ref{fig:steps}, 
% we depict our abstract conceptualization of the three stages of data analytics;
% our specific target, with \zv, is not on the first or third stages, which 
% are better handled by other tools,
% but instead on the middle stage, 
% which is also the focus of current visual analytics tools. 
% Many of these tools target both programmers
% and non-programmers (like we do).
% \begin{figure}[!htb]
% \begin{center}
% \vspace{-5pt}
% \includegraphics[width=0.65\columnwidth]{figs/steps.pdf}
% \end{center}
% \vspace{-20pt}
% \caption{The stages of data analytics: the shaded box
% is our focus}
% \label{fig:steps}
% \vspace{-10pt}
% \end{figure}



\paragraph{Visual Analytics Tools.} 
Visualization tools, such as ShowMe, Spotfire, 
and Tableau~\cite{DBLP:journals/cacm/StolteTH08, DBLP:journals/tvcg/MackinlayHS07,Ahlberg:1996:SIE:245882.245893},
along with similar tools from the 
database community~\cite{DBLP:conf/sigmod/GonzalezHJLMSSG10,DBLP:conf/sigmod/KeyHPA12,DBLP:conf/sigmod/LivnyRBCDLMW97,DBLP:conf/avi/KandelPPHH12}
have recently gained in popularity, catering to 
data scientists who lack programming skills.
Using these tools, these scientists can 
select and view one visualization at a time.
However, these tools do not operate on 
collections of visualizations at a time---and thus
they are much less powerful and the 
optimization challenges are minimal.
\zv, on the other hand, supports queries over collections
of visualizations, returning results not much slower than the
time to execute a single query (See Section~\ref{sec:experiments}). 
Since these systems operate one visualization at a time, users are 
also not able to directly identify desired patterns or needs. 

\begin{table}[t]
\scriptsize
\begin{verbatim}
with ranking    as (
with distances as (
with distance_ product_year  as (
with aggregate_ product_year as (
   select   product, year, avg(profit) as avg_profit 
   from   table group by  product, year) )
   select  s. product as source, d. product as destination, s.year, 
           power(s.avg_profit - d.avg_profit,2) as distance_year 
   from   aggregate_ product_year s, aggregate_ product_year d 
   where  s. product!=d. product and s.year=d.year )
   select  source, destination, sum(distance_year) as distance 
   from   distance_ product_year   groupby  source, destination )
   select  source, destination, distance, 
           rank() over (partition by source order by distance asc) 
           rank from distances )
   select  source, destination, distance 
   from   ranking   where  rank < 10;
\end{verbatim}
\vspace{-15pt}
\caption{Verbose \sql query}\label{tab:verbose}
\vspace{-20pt}
\end{table}

\paragraph{Statistical Packages and Programming Libraries:}
Statistical tools (e.g., KNIME, RapidMiner, SAS, SPSS)
support the easy application of 
data mining and statistical primitives---including
prediction algorithms and statistical tests. 
While these tools support the selection of a prediction
algorithm (e.g., decision trees) 
to apply, and the appropriate parameters,
they offer no querying capabilities, 
and as a result do not need
extensive optimization.
As a result, these tools cannot support user needs like 
those describe in the examples in the introduction. 
Similarly, programming libraries such as 
Weka~\cite{holmes1994weka}
and Scikit-learn~\cite{pedregosa2011scikit} embed machine learning
 within programs.
However, manually translating the user desired patterns
into code that uses these libraries
will require substantial user effort and hand-optimization.
In addition, writing new code and hand-optimization will need
to be performed every time the exploration needs change.
Additionally, for both statistical tools and programming libraries, 
there is a need for programming ability and understanding
of machine learning and statistics to be useful---something 
we cannot expect all data scientists to possess.


\paragraph{Relational Databases.}
Relational databases can certainly support interactive analytics
via \sql. \zv uses relational databases as a backend computational
component, augmented with an engine that uses \fuse to optimize
accesses to the database, along with efficient processing code.
% an in-memory processing component and a sophisticated optimization layer
% that optimizes across this in-memory component and the databases backend.
Thus, one can certainly express some \zq queries 
by writing multiple \sql queries (via procedural \sql), 
using complex constructs only found in some databases, 
such as common table expressions (CTE) 
and window functions.
As we saw in Section~\ref{sec:userstudy}, these \sql queries are too cumbersome to write, and 
are not known to most users of databases---during our user study, we found that
all participants who had experience with \sql were not aware of these constructs; in fact,
they responded that they did not know of any way of issuing \zq queries in \sql, preferring
instead to express these needs in Python.
In Table~\ref{tab:verbose}, we list the verbose \sql query that
computes the following: for each product,
find 10 other products that have most similar profit over year trends. 
The equivalent 
\zq query takes two lines.
Further, we were able to write the \sql query only because the 
function $D$ is Euclidean distance: for other functions, we are unable
to come up with appropriate \sql rewritings.
On the other hand, for \zq, it is effortless to change the function by selecting it from a drop-down menu.
% \begin{wrapfigure}{l}{0.5\columnwidth}
% \vspace{-10pt}
%   \begin{center}
%     \includegraphics[width=0.48\columnwidth]{figs/optsynzqlvsqltwoloop.pdf}
%   \end{center}
% \vspace{-10pt}
% \caption{Performance of \zq vs \sql where we want to find top 10 similar products for every product. 
% We vary the number of products from 10 to 5000.}
% \vspace{-15pt}
% \label{fig:opt_syn_zqlvssql}
% \end{wrapfigure}
Beyond being cumbersome to write, the constructs required 
lead to severe performance penalties on most databases---for instance,
PostgreSQL materializes intermediate results when executing queries with CTEs.
To illustrate, we took the \sql query in Table~\ref{tab:verbose}, 
and compared its execution with the execution of the equivalent \zq. 
As depicted in Figure \ref{fig:opt_syn_zqlvssql}, 
the time taken by PostgreSQL increases sharply as 
the number of visualizations increases, taking up to 
10$\times$ more time as compared to \zq query executor.
This indicates that \zv is still important even for the restricted
cases where we are able to correctly write the queries in \sql.


\begin{figure}[!h]
\vspace{-10pt}
\begin{center}
\includegraphics[width=0.48\columnwidth]{figs/optsynzqlvsqltwoloop.pdf}
\end{center}
\vspace{-15pt}
\caption{\zq vs \sql: we want to find top 10 similar products for every product
on varying the number of products from 10---5000.}
\vspace{-13pt}
\label{fig:opt_syn_zqlvssql}
\end{figure}


% Lastly, these queries are extremely verbose and complex, and are error-prone to write,
% compared to a few lines of \zq.


\paragraph{OLAP Browsing.} There has been some work on 
interactive browsing of data cubes~\cite{DBLP:conf/vldb/Sarawagi99,DBLP:conf/vldb/SatheS01}.
%While we may be able to reuse some of the metrics from that line of work,
The work focuses on suggestions for raw aggregates to examine
that are informative given past browsing, or those that show a generalization 
or explanation of a specific cell---an easier problem meriting simpler techniques---not
addressing the full exploration capabilities provided by \zq.

\paragraph{Data Mining Languages:} 
There has been some limited work in data mining query languages, all from the early 90s, 
on association rule mining (DMQL~\cite{han1996dmql}, MSQL~\cite{imielinski2000query}),
or on storing and retrieving models on data
(OLE DB~\cite{netz2001integrating}),
as opposed to a general-purpose visual data exploration language
aimed at identifying visual trends. 

\paragraph{Visualization Suggestion Tools:}
There has been some recent work on building systems that 
suggest visualizations.
Voyager~\cite{wongvoyager2015} recommends
visualizations based on aesthetic properties of the
visualizations, as opposed to queries.
SeeDB~\cite{Vartak:2015:SED:2831360.2831371} 
recommends visualizations that best display the 
difference between two sets of data. 
SeeDB and Voyager can be seen to be special cases of \zv.
The optimization techniques outlined are a substantial generalization
of the techniques described in SeeDB; 
while the techniques in SeeDB are special-cased to one setting 
(a simple comparison),
here, our goal is to support and optimize all \zq queries.






% but require extensive knowledge of the underlying 
% algorithms and para\-metrization, limiting their use to experts,
% e.g., a user can select to use decision trees, with a certain depth
% and splitting criteria
% on their dataset using any of these tools. 
% Programming libraries such as Weka~\cite{holmes1994weka}
% and Scikit-learn~\cite{pedregosa2011scikit} support embedding machine
% learning and data mining within programs. 
% The statistical analysis and programming libraries falls under
% the third box of Figure~\ref{fig:steps}, representing the
% third stage of data analytics, following data exploration.
% Indeed, complex statistical tasks\techreport{ such as classification,
% regression, and dimensionality reduction}
% are hugely important, but 
% require programming ability or an understanding of machine learning
% and statistics to be useful.
% \zv is instead intended to be a substantial generalization over existing
% data exploration tools (second box in Figure~\ref{fig:steps}),
% aimed at identifying the patterns and trends that hold in the data,
% by non-programmers,
% which can be then used to train a machine learning algorithm later on.



% \tar{One can express a portion of ZQL queries by writing multiple SQL queries (procedural SQL) with complex constructs such as common table expressions (CTE), nested queries, and window (analytic) functions. However:
% --Only a handful of databases support these options. Still, most of the databases don't optimize these constructs, and so execution of these tend to take a lot of time. For instance, postgres materializes intermediate results while executing CTEs.
% --Hacky and cumbersome to write. Only users who are extremely proficient in SQL can write these. Will take many more lines than equivalent ZQL queries. During our user-study, almost all participants who had experience with SQL weren't aware of these options - all clearly said SQL can't express ZQL type of queries. Participants were more comfortable using python than SQL.
% }




% A number of interactive data analytics tools have been developed, such as ShowMe, Spotfire, and Tableau~\cite{DBLP:journals/cacm/StolteTH08, polaris,DBLP:journals/tvcg/MackinlayHS07,Ahlberg:1996:SIE:245882.245893}. While these tools are effective in retrieval, and automatic visualization mapping and encoding of the data the user specifies in a query, these tools do not let the users specify the kind of patterns or insights that they are looking for, and thus the onus is on the users to manually search for interesting visualizations among all possible output visualizations.

%\paragraph{OLAP:} \tar{got rid of the first line}
% Visual specification tools have also been introduced by the database community\cite{DBLP:conf/sigmod/GonzalezHJLMSSG10,DBLP:conf/sigmod/KeyHPA12,DBLP:conf/sigmod/LivnyRBCDLMW97,DBLP:conf/avi/KandelPPHH12}.
% %, including Fusion Tables~\cite{DBLP:conf/sigmod/GonzalezHJLMSSG10},
% VizDeck~\cite{DBLP:conf/sigmod/KeyHPA12}, 
% and Devise~\cite{DBLP:conf/sigmod/LivnyRBCDLMW97}.
% Profiler~\cite{DBLP:conf/avi/KandelPPHH12} and Potter's Wheel~\cite{DBLP:conf/vldb/RamanH01}
% identifies mistakes in datasets. 







% although support a number of complex data mining tasks,
% require extensive knowledge of the algorithms and their parameterizations making them limited only to expert users. Moreover, these tools are loosely coupled with databases, 
% providing limited opportunities for query optimizations, and do not scale well as size of 
% the data increases. \zv, unlike these tools, is not meant for complex data analytics tasks such
% as classification, prediction, regression, or dimensionality reduction, but 
% augments the functionalities of existing visual data exploration tools such as Tableau and ggplot by 
% automatically identifying interesting visualizations that match user specified insights.

% \paragraph{Programming libraries:} Several programming and workflow languages support machine
% learning (e.g, WEKA) and visualization libraries using which users can write imperative code to retreive data, and search for visualizations
% with specific insights. However, most of the users, especially  with less programming experience, only know the insights that they are interested in
% instead of the actual procedure to find them. \zv is more accessible to such users as it exposes a more general purpose declarative interface for describing
% their insights. Moreover, as the path of data exploration is mostly unpredictable and iterative, zenvisage leads to a faster data exploration
% since the users can rapidly modify their queries as their desired insights change.



\techreport{
\paragraph{Multi-Query Optimization:} 
There has been a lot of work on Multi-Query Optimization (MQO), both classic, 
e.g.,~\cite{DBLP:journals/tods/Sellis88,shim1994improvements,roy2000efficient}, and
recent work, e.g.,~\cite{giannikis2013workload,psaroudakis2013sharing,DBLP:journals/pvldb/KementsietsidisNCV08,giannikis2014shared}.
Overall, the approach adopted is to batch queries, decompose into operators,
and build ``meta''-query plans that process multiple queries at once,
with sharing at the level of scans, or at the level of higher level operators
(either via simultaneous pipelining or a true global query plan~\cite{psaroudakis2013sharing}).
Unlike these techniques which require significant modifications
to the underlying database engine---indeed, some of these systems do not even provide
full cost-based optimization and only support hand-tuned plans~\cite{giannikis2013workload}, 
in this paper, we adopted two 
syntactic rewriting techniques that operate outside of any relational database as a backend
without 
requiring any modification, and can thus seamlessly leverage improvements
to the database. 
Our third optimization is tailored to the \zq setting and does not apply more broadly.
}



% \papertext{
% \smallskip
% \noindent In our technical report, we describe other areas of related work,
% including multi-query optimization, anomaly discovery, and time-series similarity indexing~\cite{techreport}.
% }


\techreport{
\paragraph{Anomaly Discovery:}
Anomaly detection is a well-studied topic~\cite{Chandola:2009:ADS:1541880.1541882,Agyemang:2006:CSN:1609942.1609946,Patcha:2007:OAD:1269989.1270131}. Our goal in that
\zv is expected to be interactive, especially on large datasets; most work in anomaly detection focuses on accuracy at the cost of latency and is typically a batch operation. In our case, since interactiveness is of 
the essence, and requests can come at any time, the emphasis is on scalable on-the-fly data processing aspects.
}

\techreport{
\paragraph{Time Series Similarity and Indexing:}
There has been some work on indexing of
of time series data, e.g., \cite{timeseries1,timeseries2,timeseries3,timeseries4,timeseries5,
timeseries6,timeseries7};
for the attributes that are queried frequently, 
we plan to reuse these techniques for similarity search.
For other attributes, indexing and maintaining all trends
is impossible, since the number of trends grows exponentially with the
number of indexed attributes.
}


\later{
\tar{Previous text}
Our work is related to prior work in a number of areas.
\paragraph{Visual Analytics Tools:} A number of 
interactive data analytics tools have been developed, such as ShowMe, Polaris, Spotfire, and
Tableau~\cite{DBLP:journals/cacm/StolteTH08, DBLP:journals/tvcg/MackinlayHS07,Ahlberg:1996:SIE:245882.245893}.
Here, the onus is on the user to specify the visualization to be generated,
and then repeat until the desired visualization is identified. 
Similar specification tools have also been introduced
by the database community\cite{DBLP:conf/sigmod/GonzalezHJLMSSG10,DBLP:conf/sigmod/KeyHPA12,DBLP:conf/sigmod/LivnyRBCDLMW97,DBLP:conf/avi/KandelPPHH12}.
%%, including Fusion Tables~\cite{DBLP:conf/sigmod/GonzalezHJLMSSG10},
%VizDeck~\cite{DBLP:conf/sigmod/KeyHPA12}, 
%and Devise~\cite{DBLP:conf/sigmod/LivnyRBCDLMW97}.
%Profiler~\cite{DBLP:conf/avi/KandelPPHH12} and Potter's Wheel~\cite{DBLP:conf/vldb/RamanH01}
%identifies mistakes in datasets. 
\zv is related to work on browsing data cubes---finding explanations, getting suggestions for cubes to visit,
or identifying generalizations from a single cube, 
e.g., \cite{DBLP:conf/vldb/Sarawagi99, 
DBLP:conf/vldb/SatheS01}. 
While we may be able to reuse the metrics from that line of work,
the same techniques will not directly apply to the identification of
trends, patterns, and anomalies for interactive visualizations.  
Specifically, no OLAP techniques capture the interestingness of slices
of the data cube that can be visualized via two (or more) dimensional
visualizations: instead, the focus is more on 
raw aggregate data, on interestingness of cells of the cube, 
displayed within multidimensional tables.  
Thus, the emphases are different. 
Indeed, we believe that, given the popularity of tools like Tableau,
users prefer to browse and explore data visually rather than in tables.
% \new{Moreover, while the OLAP applications try to model relational data as multidimensional cubes for analysis, our system searches for insights among multiple two-dimensional visualizations that are created from one or more attributes of a relational data.}
There has been some work sketch-based interfaces for visualization~\cite{visual1, visual2,visual3, visual4}: however, none of this work addresses
the deep scalability issues at play if these techniques are to be applied on large
datasets.
There is limited work on visual query interfaces~\cite{gesturedb, dbtouch, qbe, dataplay}, but the goal there is to make it easier to pose SQL queries.

% Furthermore, unlike traditional anomaly detection, our anomaly identification goals are query-driven,
% and not one-shot
% scientists can explore the same dataset or multiple datasets in many different
% ways, and we need to be able to surface interesting insights or anomalies
% in real-time whenever a query is issued.
\paragraph{Time Series Similarity and Indexing:}
There has been some work on indexing of
of time series data, e.g., \cite{timeseries1,timeseries2,timeseries3,timeseries4,timeseries5,
timeseries6,timeseries7};
for the attributes that are queried frequently, 
we plan to reuse these techniques for similarity search.
For other attributes, indexing and maintaining all trends
is impossible, since the number of trends grows exponentially with the
number of indexed attributes.
\paragraph{Visualization Recommendation Tools:}
There has been some recent work on building systems that 
recommend visualizations
to analysts.
Voyager~\cite{wongvoyager2015} recommends
visualizations based on aesthetic properties of the
visualizations, as opposed to user queries.
SeeDB~\cite{tr} 
recommends visualizations that best display the 
difference between two sets of data. 
Both SeeDB and Voyager can be seen to be special cases of \zv,
since \zv can be viewed to be a user-driven visualization
recommendation engine as well.
The optimization techniques outlined are a generalization
of the techniques described in SeeDB; 
while the techniques in SeeDB are special-cased to the 
query considered (a simple comparative query),
here, our goal is to support and optimize all \zq queries.
\paragraph{Data Mining Query Languages:}
There has been some limited work in the space of data mining query languages, all from the early 90s, 
focusing
either on
association rule mining (languages such as DMQL~\cite{han1996dmql} and MSQL~\cite{imielinski2000query}),
or on storing and retrieving models on data
(languages such as OLE DB~\cite{netz2001integrating}),
as opposed to a visual exploration language like \zq.
\paragraph{Multi-Query Optimization:} 
Our proposed primitive query optimization techniques are currently 
tailored to the \zv setting, specifically trying to identify 
opportunities for batching of 
individual visualization generation \sql queries 
so as to ``combine work''
as much as possible, even before they are issued to the database. 
These optimization techniques are external to the database system,
are completely interpreted based on the rows of \zq, and do not 
require any modifications to the underlying database.
Indeed, there are very powerful multi-query optimization techniques
in related work, e.g.,~\cite{DBLP:journals/tods/Sellis88,shim1994improvements,dalvi2003pipelining,roy2000efficient,DBLP:journals/pvldb/KementsietsidisNCV08},
that we plan to leverage as future work to further improve the performance
of \zv, when we attempt to holistically
process \zq queries by making modifications to the underlying database
query processor, rather than simply operating as a ``wrapper'' on top
of a database.
}%techreport

% \new {Our proposed query optimization technqiues fall into the cateogory of Multi-Query Optimization techniques ~\cite{DBLP:journals/tods/Sellis88} with a similar goal of batching multiple SQL queries to reduce the overall number of queries that the system needs to execute. However, our query optimization technqiues are specific to the semantics of \zq query model, and analyze visualisation and process column attributes for optimization opportunities rather than the SQL constructs.}




==> docs copy/sets-and-vars.tex <==
%!TEX root=zenvisageql.tex


\begin{table*}[!htbp]
  \centering\scriptsize
  {\tt
    %\resizebox{\linewidth}{!}{%
      \begin{tabular}{|r|l|l|l|l|} \hline
        \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Z} & \textbf{Process}
        \\ \hline
        f1 & `year' & `sales' & v1 \IN `product'.* & \\
        f2 & `year' & `profit' & v1 & v2 \IN $argmax_{v1}[k=10]
        D(f1, f2)$ \\
        *f3 & `year' & `sales' & v2  & \\
        *f4 & `year' & `profit' & v2  & \\ \hline
      \end{tabular}
    %}
  }
  \vspace{-10pt}\caption{A \zq query which returns the set sales over years and the profit
    over years visualizations for the top 10 products for which these two
  visualizations are the most dissimilar.}
  \label{tab:vars-1}

  \centering\scriptsize
  {\tt
    %\resizebox{\linewidth}{!}{%
      \begin{tabular}{|r|l|l|l|l|l|} \hline
        \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Z} &
        \textbf{Constraints} & \textbf{Process}
        \\ \hline
        f1 & `year' & `sales' & v1 \IN `product'.* & & v2 \IN $argmax_{v1}[k=10]
        T(f1)$ \\
        *f2 & `year' & `profit' & & product IN (v2.range) & \\ \hline
      \end{tabular}
    %}
  }
  \vspace{-10pt}\caption{A \zq query which plots the profit over years for the top 10
  products with the highest sloping trend lines for sales over the years.}
  \label{tab:vars-2}

  \centering\scriptsize
  {\tt
    %\resizebox{\linewidth}{!}{%
      \begin{tabular}{|r|l|l|l|l|} \hline
        \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Z} &
        \textbf{Process}
        \\ \hline
        f1 & x1 \IN C & y1 \IN  M & `product'.`chair' & \\
        f2 & x1 & y1 & `product'.`desk' & x2,y2 \IN $argmax_{x1,y1}[k=10] D(f1,f2)$ \\
        *f3 & x2 & y2 & `product'.`chair' & \\
        *f4 & x2 & y2 & `product'.`desk' & \\ \hline
      \end{tabular}
    %}
  }
  \vspace{-10pt}\caption{A \zq query which finds the x- and y- axes which
  differentiate the chair and the desk most.}
  \label{tab:vars-3}
\vspace{-10pt}\end{table*}

\subsubsection{Sets and Variables}
\label{sec:variables}
As we described previously, sets in \zq must
always be accompanied by a variable which iterates over that set, to 
ensure that \zq traverses over sets of visualizations
in a consistent order when making comparisons. 
Consider Table~\ref{tab:vars-1}, which shows
a query that iterates over
the set of products, and for each, compares the sales over
years with the profits over years. Without a
variable enforcing a consistent iteration order over the set of products,
it is possible that the set of visualizations could be
traversed in unintended ways. For example, the sales vs.~year plot for chairs
from the first set could be compared with the profit vs.~year plot for desks in
the second set. By reusing {\tt
v1} in both the first and second rows, the user can force the \zv back-end to
step through the sets in sync.

\noindent {\bf Operations on Sets.} 
Constant sets in \zq must use \{\} to denote that the enclosed elements are
part of a set. As a special case, the user may also use * to represent the set of
all possible values. The union of
sets can be taken using the  sign {\tt |}, set difference can be taken using the
{\tt $\setminus$}
sign, and the intersection can be taken with {\tt \&}. 
\later{Users must take the
explicit difference between * and a set to get the complement.
Set operators have lower precedence than most other operators, so the use of
parentheses is encouraged:
{\tt `product'.(* $\setminus$ \{`stapler'\})}.
As a matter of convenience, all operands of a set operation
which are not sets are automatically converted into singleton sets which
contain that operand. This allows us to simplify the previous expression a
little
further to {\tt `product'.(* $\setminus$ `stapler')}.
The valid elements of sets are literals, the set expansion of variables ({\tt
.range}), and other valid sets. Variables in their raw form cannot be elements
in a set. The \zq, the only a Cartesian products of sets can be specified is
when a period is used (e.g., {\tt \{`product', 'color'\}.*}).}

\later{Labels for sets maybe used with the {\tt @} notation so that the user does not
need to specify the same set over and over again. For example, if the user has
decided that the measure attributes she is interested in are {\tt \{`profit',
`sales', 'revenue'\}}, she could use {\tt M @ \{`profit', `sales', `revenue'\}}
the first time when she defines the set, and {\tt M} every time afterwards.
Once a label has been set, it cannot be redefined.}

\noindent {\bf Ordering.} 
All sets in \zv are ordered, but when defined using the \{\}, the ordering is
defined arbitrarily. Only after a set has passed through a Process
column's ordering mechanism can the user depend on the ordering of the set.
Ordering mechanisms are discussed further in Section~\ref{sec:process}.
However, even for arbitrarily ordered sets, if a variable iterator is defined
for that set and reused, \zq guarantees at least a \emph{consistent} ordering
of traversal, allowing the sets in
Table~\ref{tab:vars-1} to be traversed in the intended order.
\later{
\alkim{
Variable names must start with a letter and can only contain letters, numbers,
and the underscore for the remaining characters. 
To be used, variables must either be defined in the current or a previous row.
}
}

\noindent {\bf Axis Variables.} 
In \zq, there are two types of variables: \emph{axis variables} and \emph{name
variables}.
Axis variables are the common variables used in any of the columns except the
Name column.  The declaration has the form:
\emph{$\langle$variable~name$\rangle$} \IN \emph{$\langle$set$\rangle$}.
The variable then can be used as an iterator in the Process column or reused in
a different table cell to denote that the set be traversed in the same way for
that cell. It is possible to declare multiple axis variables at once,
as we have seen from the Z and Process columns: (e.g., {\tt z.v \IN *.*}).

Sometimes, it is necessary to retrieve the set that an axis variable iterates
over. The {\tt .range} notation allows the user to expand variables to
their corresponding sets and apply arbitrary \zv set
operations on them. For example, {\tt v4 \IN (v2.range |
v3.range)} binds v4 to the union of the sets iterated by {\tt v2}
and {\tt v3}. 
\later{However, the expanded set for a variable may not be the final
value for any table cell in \zq; it must always be either a literal or a
raw variable.}

Axis
variables can be used freely in any column except the Constraints column. In
the Constraints column, only the expanded set form of a variable may be used.
Table~\ref{tab:vars-2} demonstrates how to use an axis variable in the
Constraints column. In this example, the user is trying to plot the overall
profits over years for the top 10 products which have had the most growth in
sales over the years. The user finds these top 10 products in the first row
and declares the variable {\tt v2} to iterate over that set. Afterwards, she
uses the constraint {\tt product \IN (v2.range)} to get the overall profits
across all 10 of these products in the second row.

\noindent {\bf Name Variables.}
Name variables (e.g., \texttt{f1, f2}) are declared only in the Name column and used only in the
Process column.  
Named variables are iterators
over the set of visualizations represented by the visual component. If the
visual component represents only a single visualization, the name variable is
set to that specific visualization. Name variables are \emph{bound} to the axis
variables present in their row. In Table~\ref{tab:vars-2}, {\tt f1} is bound
{\tt v1}, so if {\tt v1} progresses to the next product in the set {\tt f1}
also progresses to the next visualization in the set. This is what allows the
Process column to iterate over the axis variable ({\tt v1}), and still compare
using the name variable ({\tt f1}).
If multiple axis variables are present in the visual component, the name
variable iterates over set of visualizations produced by the Cartesian product
of the axis variables. 
\techreport{If the axis variables have been declared independently
of each other in the visual component, the ordering of the Cartesian product
  follows the ordered bag semantics described in
  Section~\ref{subsec:ordered-bag} in order of the columns laid out in \zq.
  However, the user may also superscript variables to control the order in
  which Cartesian product is done as well.
  However, if the variables were declared together in the Process 
column as is the case
with {\tt x2} and {\tt
y2} in Table~\ref{tab:vars-3}, the ordering is the same as the set in the
declaration.}


==> docs copy/userstudy-cuts.tex <==
%!TEX root=zenvisageql.tex

\section{User Study}
\label{subsec:userstudy}
We conducted a mixed methods study~\cite{creswell2007designing} 
in order to assess the efficacy of \zv. 
We wanted to: 
a) examine and compare the usability of the drag and drop 
interface and the custom query builder interface of \zv; 
b) compare the performance and usefulness of \zv 
with existing tools;
c) identify if, when, and how people would use \zv in their workflow;
and d) receive general feedback for future improvements.

\subsection{User Study Methodology}
\paragraph{Participants.} We recruited 12 graduate students 
as participants with varying degrees of expertise in data analytics. 
Table \ref{tab:toolsrep} depicts the participants' experience of participants in different tool categories of tools.
\begin{table}[H]
\vspace{-10pt}
 \centering\scriptsize
  {\tt    
  \begin{tabular}{|l|l|} \hline
      \textbf{Tools} & \textbf{Count} \\ \hline
      Excel, Google spreadsheet, Google Charts  & 8 \\ \hline
      Tableau & 4 \\ \hline
      SQL, Databases & 6 \\ \hline
      Matlab,R,Python,Java & 8 \\ \hline
      Data mining tools such as weka, JNP & 2 \\ \hline
      Other tools like D3 & 2 \\ \hline
     \end{tabular}
  }
  \vspace{-10pt}\caption{Participants' prior experience with data analytic tools}
  \label{tab:toolsrep}
\vspace{-10pt}\end{table}

\paragraph{Dataset.} 
To conduct the study, we used a housing dataset from Zillow.com~\cite{housing_data} consisting of housing sales data for different cities, counties, and states from 2004--15, with over 245K rows, and 15 attributes. We selected this dataset for two reasons:
First, housing data is often explored by data analysts using existing \john{visualization tools} \cite{elmqvist2008datameadow}. Second, looking for housing is commonplace for graduate students while in school and upon graduation; the participants could relate to the dataset and understand the usefulness of the tasks in the real world.
  
\paragraph{Comparison Points.} 
There are no tools that offer the same functionalities as
\zv: visual analytics tools do not offer the ability
to search for specific patterns, or issue complex data exploration queries; 
data mining toolkits do not offer the ability to generate visualizations, 
search for visual patterns and are instead tailored for general machine learning and prediction.
Since visual analytics tools are closer in spirit and functionality 
to \zv, we decided to implement a visual analytics tool as our baseline.
Thus, our baseline tool replicated the basic query specification and output visualization
capabilities of existing tools such as Tableau \john{(see Figure \ref{fig:baseline})}.  
We augmented the baseline tool with the ability to specify an arbitrary number of filters, allowing
users to use filters to drill-down on specific visualizations.
This baseline visualization tool was implemented with a styling scheme similar to \zv to control for external factors. 
%As depicted in Figure \ref{fig:baseline}, the baseline allowed users to visualize data by allowing them to specify the x-axis, y-axis, category, and filters. The baseline tool would populate all the visualizations, which fit the user specifications, using an alpha-numeric sort order.
In addition to task-based comparisons with this baseline, we
also explicitly asked participants to compare \zv with existing data mining and visual analytics 
tools that they use in their workflow.
 
\paragraph{Study Protocol.} The user study was 
conducted using a within-subject study design~\cite{bordens2002research}. 
The study consisted of three parts. 
In the first part, participants described 
their previous experience with data analytics and visualization tools. 
In the second part, participants performed visual analytics 
tasks using one tool at a time. 
\techreport{\zv was introduced as Tool A and the baseline tool was introduced as Tool B.}
Before starting the tasks on each of the tools, 
participants completed a 15-minute tutorial 
which included an overview of the interface and two practice questions 
to get a general understanding of the tool. 
The order of the tools was randomized to reduce the order effects. 
In order to compare the effectiveness of the drag and drop interface 
and the custom query builder interface of \zv, 
participants performed two separate sets of tasks on \zv, one for each component. Finally, in the third part, participants completed a survey that measured 
their satisfaction levels and preferences, followed by open-ended questions on the strengths and weaknesses 
of the tools, and whether they would use the two tools in their workflow. 
\techreport{
The study lasted for 1 hour and 15 minutes on average. 
Participants were paid 10 dollars per hour for their participation.}

\paragraph{Tasks.}
We prepared three sets of different tasks for the three interfaces (baseline, drag and drop, and custom query builder interfaces). The tasks differed only in the selection attributes so that the performance of the interfaces could be measured objectively (Section~\ref{sec:frontend} lists a few example queries that were used in the study). We carefully selected tasks which can surface during a search for a house. To demonstrate the efficacy of \zv, the tasks were focused on identifying similar trends or anomalies in housing data, which are non-trivial tasks to complete with a large dataset with existing tools. Specifically, the tasks were targeted to test the core features of \zv and solicit responses from participants on how it can complement existing data analytics workflows.

%The tasks that the participants performed on the two tools were designed to be similar in nature (differing only in selection attributes) so that we could compare the performance more objectively. The tasks focused on identifying visualizations with specific insights. Section~\ref{sec:frontend} lists a few example queries that were used in the study. 

\paragraph{Metrics.} 
We manually recorded how participants used the tool, their answers for each task, tracked their browser activity using a screen capture software, collected system interaction logs, recorded audio, and asked the participants to fill in a survey form. Using this data, we collected the following metrics: task completion time, task accuracy, the number of visualizations browsed for each task, the number of edits made on the drawing panel and the query table, survey results, and the answers to open-ended questions.

\paragraph{Ground Truth.} 
We took help of two expert data analysts to prepare the ground truth consisting of ranked answers for each of the tasks. Their inter-rater agreement, measured using Kendall\textquotesingle s Tau rank correlation coefficient, was 0.854. 
% The experts further discussed and resolved the conflicting answers to produce a final single ranked list of answers for each task. 
Then, each expert independently rated the answers on their ranked list on a 0 to 5 scale, with a score of 5 for the highest ranked answer and a score of 0 for the lowest ranked answer. We took the average of the two scores to rate the participants\textquotesingle~answers.


\begin{figure}
\vspace{-10pt}
\begin{center}
\fbox{\includegraphics[width=0.6\columnwidth]{figs/baseline.png}}
\end{center}
\vspace{-20pt}
\caption{The baseline interface implemented for the user study.}
\label{fig:baseline}
\vspace{-15pt}
\end{figure}


\subsection{Key Findings}
Now, we describe the key findings that we discovered through our analysis on the metrics collected during the study. We use $\mu$, $\sigma$, $\chi^2$ to denote average, standard deviation, and Chi-square test scores respectively.

\begin{table}[H]
\vspace{-10pt}
 \centering\scriptsize
  {\tt    
  \begin{tabular}{ | l | l | l  | } \hline
      \textbf{Tool} & \textbf{Time} (\textbf{sd}) & \textbf{Accuracy} (\textbf{sd}) \\ \hline
      Baseline & 172.5s (50.5) & 69.9\% (13.3) \\ \hline
      Drag and drop & 74s (15.1) & 85.3\% (7.61) \\ \hline
      Custom query builder & 115s (51.6) & 96.3\% (5.82) \\ \hline
     \end{tabular}
  }
  \vspace{-10pt}\caption{Average task completion time and average accuracy of the three interfaces.}
  \label{tab:taskresults}
\vspace{-10pt}\end{table}

\paraem{Finding 1: \zv enables over 50\% and 100\% faster task completion time than the baseline for custom query builder and drag and drop interface respectively.} We timed the task completion time for all participants,
and we found that the drag and drop interface has the smallest, and most predictable completion time (Table \ref{tab:taskresults}). The custom query builder has a higher completion time, but also with higher variance, while the baseline had a significantly higher completion time, more than twice the completion time of the drag and drop interface, and almost 50\% more than the custom query builder (Table \ref{tab:taskresults}).
This is not surprising, given that the baseline tool requires more manual exploration of the results, as opposed to either of the other two interfaces. We tested for statistical significance on the difference between the three interfaces using 
one-way between-subject ANOVA, followed by a post-hoc Tukey's test~\cite{tukey1949comparing}.
We found that the drag and drop interface and the custom query builder interface had statistically significantly 
faster task completion times compared to the baseline interface, with $p$ values of 0.0010 and 0.0069 respectively, both $<0.01$, while the difference between drag and drop and custom query builder was not statistically significant,
with a $p$ value of $0.06$. \papertext{Detailed statistics can be found in the technical report~\cite{techreport}.}

% One-way between subject ANOVA~\cite{tukey1949comparing} on the completion time of the tasks revealed that the differences between the three interfaces were significant F(2, 33) = 16.02, p < 0.001. On further applying the post hoc Tukey's test\cite{tukey1949comparing} for comparing the pairwise task completion times among the three interfaces (Table \ref{tab:turkeytest}), we found that both the drag and drop interface and the custom query builder had significantly faster task completion times compared to the baseline tool (p < 0.01), whereas the difference between the drag and drop interface, and the custom query builder was not significantly different.  
\techreport{
\begin{table}[H]
 \centering \scriptsize
  {\tt    
  \scalebox{0.75}{
  \begin{tabular}{|l|l|l|l|} \hline
      \textbf{Treatments} & \textbf{Q statistic} & \textbf{p-value} & \textbf{inference} \\ \hline
	Drag and drop interface vs. Custom query builder & 3.3463 & 0.0605331 & insignificant \\ \hline
	Drag and drop interface vs. Baseline tool & 7.9701 & 0.0010053 & significant (p<0.01) \\ \hline
	Custom query builder vs. Baseline tool & 4.6238 & 0.0069276 & significant (p<0.01) \\ \hline    
     \end{tabular}
  }
  }
\vspace{-10pt}
\caption{Tukey's test on task completion time}
\label{tab:turkeytest}
\vspace{-10pt}
\end{table}
}

\begin{figure}
\begin{center}
\includegraphics[width=0.6\columnwidth]{figs/accuracyvstime.pdf}
\end{center}
\vspace{-25pt}
\caption{Accuracy over time results for zenvisage and baseline}
\label{fig:accuracyvstime}
\vspace{-20pt}
\end{figure}

\paraem{Finding 2: \zv helps retrieve 20\% and 35\% more accurate results than the baseline for drag and drop and custom query builder interface respectively.} 
We rated the participant's answers based on the ground truth answers. 
The ratings revealed that participants performed poorly on the baseline tool (Table \ref{tab:taskresults})
\techreport{Further, any tasks that required comparing multiple
pairs of visualizations or trends ended up having lower accuracy than those that looked
for a pattern, such as a peak or an increasing trend, in a single visualization.}
Overall the low accuracy can be attributed to the
fact that the participants got tired of browsing through
large collections of visualizations and return the first result 
that approximately matches the conditions. 
On the other hand, since \zv is able to
accept more fine-grained user input, and
rank output visualizations, 
assisting participants in retrieving accurate answers
with less effort.
Among the two interfaces in \zv,
while the drag and drop interface had a faster task completion time, it was less accurate. The custom query builder had the highest accuracy (Table \ref{tab:taskresults}).
Thus accuracy is greater than the baseline by over 20\% (for the drag and drop interface)
or over 35\% (for the custom builder interface).
Finally, looking at both accuracy and task completion times together in Figure~\ref{fig:accuracyvstime}, we can conclude that \zv \emph{helps in ``fast-forwarding to desired visualizations'' with high accuracy.}

% In the baseline, comparing multiple pairs of visualizations or trends revealed to be more difficult than looking for a visual property, such as a peak, or an increasing pattern, in a single visualization. on the other hand, since \zv returns a ranked list of filtered answers based on the user specification, which allowed the participants to browse through a smaller number of visualizations compared to the baseline tool. Among the two interfaces in \zv, participants completed the tasks faster ($\mu=74s$, $\sigma=15.1$) on the drag and drop interface, but at the price of accuracy ($\mu=85.3\%$, $\sigma=7.61$). Participants using the custom query builder had the highest accuracy ($\mu=96.3\%$, $\sigma=5.82$) while maintaining comparable speeds to the drag and drop interface ($\mu=115s$, $\sigma=51.6$). Finally, looking at both accuracy and task completion times together (as depicted in Figure~\ref{fig:accuracyvstime}), we can conclude that \zv \textbf{helps in fast-forwarding to desired visualizations with a high accuracy.}

% Figure \ref{fig:accuracyvstime} depicts the average accuracy over time results of each of the participants on each of the interfaces. \agp{move this later.} 



%\textbf{\zv helps retrieve accurate results}: We rated the participant's answers based on the expert's gold set answers. The ratings revealed that participants performed poorly with the baseline, with the lowest accuracy ($\mu=69.9\%$, $\sigma=13.3$) and longest task completion time. In the baseline, comparing multiple pairs of trends or graphs revealed to be more difficult than looking for a single trend such as a peak, or an increasing pattern. \zv, on other hand, returns a ranked list of results based on the user specification, which allowed the participants to browse through a smaller number of visualizations compared to the baseline tool. Among the two interfaces in \zv, participants completed the tasks fastest ($\mu=74s$, $\sigma=15.1$) on the drag and drop interface, but at the price of accuracy ($\mu=85.3\%$, $\sigma=7.61$). Participants using the custom query builder had the highest accuracy ($\mu=96.3\%$, $\sigma=5.82$) while maintaining comparable speeds to the drag and drop interface ($\mu=115s$, $\sigma=51.6$). \textbf{\zv, thus, helps in fast-forwarding to desired visualizations with a high accuracy}.


\paraem{Finding 3: The drag and drop interface, and the custom query builder complement each other.} 
The large majority of participants (8/12) 
mentioned that the drag and drop interface, 
and the custom query builder complement each other in 
making \zv powerful in searching for specific insights. 
About 25 percent (3/12) of the participants 
(all with backgrounds in machine learning and data mining) 
preferred using only the custom query builder while 
just one participant 
(with no prior experience with query languages or programming languages) 
found only the drag and drop interface as useful. 
Participants stated that they would use the drag and drop interface for exploration and simple pattern search, and the custom query builder for specific and complex queries. One participant stated: \textit{``When I know what I am looking for is something exact, I want to use the query table. The other one [drag and drop interface] is for exploration when you are not so sure.''} 
\techreport{We next discuss the participants\textquotesingle responses to the individual components of \zv.}

\paraem{Finding 4: The drag and drop interface is intuitive.} 
Participants liked the simplicity and intuitiveness of the drag and drop interface. 
One stated: \textit{``[The drawing feature] is very easy and intuitive, I can draw the trend and automatically get the results.''} 
The participants rated the usability of this feature on 
a 5-point Likert scale ranging from strongly disagree 
(1) to strongly agree (5), and 
found the drawing feature easy to use, with $\mu=4.45$, $\sigma=0.674$. 
Despite the positive feedback, participants did identify limitations,
specifically that the functionality is restricted to identifying trends
similar to a single hand-drawn trend.

\paraem{Finding 5: The custom query builder is useful for complex queries.}
The majority of the participants (11/12) 
said that the custom query builder 
allowed them to search for complex insights which might be 
difficult to answer in the drag and drop interface. 
When asked if the custom query builder is comparatively difficult
to the drag-and-drop interface, participants tended to agree,
with $\mu=3.73$, $\sigma=0.866$ on a 5-point scale (5 is strongly agree).
At the same time, participants acknowledged 
the flexibility and the efficacy supported by the custom query builder. 
One participant explicitly stated that they 
preferred the custom query builder over the drag and drop interface 
for this reason: 
\textit{``When the query is very complicated, [the drag and drop interface] has its limitations, so I think I will use the query table most of the times unless I want to get a brief impression.''} 
Another participant stated that the custom query builder \textit{``has more functionality and it lets me express what I want to do clearly more than the sketch''}. This is consistent with other responses. 
Participants with a background in machine learning, 
data mining, and statistics (3/12) preferred always 
using the custom query builder over the drag and drop interface.

\paraem{Finding 6: \zv is much more effective (4.27 vs. 2.67 on a 5 point scale)
than the baseline tool at visual data exploration}
 In response to survey question \emph{``I found the tool to be effective in visualizing the data I want to see''}, the participants rated \zv (drag and drop interface + custom query builder) much higher ($\mu=4.27$, $\sigma=0.452$) than the baseline tool ($\mu=2.67$, $\sigma=0.890$) on a 5 point Likert scale.
 A participant experienced in Tableau commented:\textit{``In Tableau, there is no pattern searching. For example, if I see some pattern in Tableau, such as a decreasing pattern, and I want to see if any other variable is decreasing in that month, I have to go one by one to find this trend. But here I can find this through the query table.''}.  

\tar{Point 7 was earlier part of point 6, made it a separate point for emphasis}
\paraem{Finding 7: \zv would be a valuable addition to the participants' analytics workflow, can lead to a quicker initial data exploration before performing complex anaysis using machine learning and imperative programing languages:}
When asked about using the two tools in their current workflow, 9/12 participants stated that they would use \zv in their workflow, whereas only 2/12 participants stated that they would use our baseline tool ($\chi^2=8.22$, p<0.01). When the participants were asked how they would use \zv in their workflow, most of the them mentioned that they would use this tool for tasks such as finding common patterns, gaining an initial understanding of data distribution before running a machine learning task and finding outliers during data cleaning. One participant provided a specific scenario: \textit{``If I am doing my social science study and I want to see some specific behavior among users, then I can use tool A [\zv] since I can find the trend I am looking for and easily see what users fit into the pattern.''}. \nnew{While the pariticpants who had no programming experience considered the insight specification functionality of \zv as something very useful as they had to do it manually before, those with experince in programming languages such as python and MATLAB said \zv would take less time and fewer number of lines of code to do basic data exploration tasks. On asking participants (2/12) who had considerable experince with machine learning and data-mining libraries to write code for a task similar to the one in Table 11 in their favorite language, it took them several minutes and many more operations as compared to a few lines of \zq. \papertext{Example code can be found in our
technical report~\cite{techreport}}}. 

\techreport{
\begin{verbatim}[language=MATLAB]
% x1 = year, x2 = quarter, x3 = month, 
% y1 = sold price, y2 = listing price,
% y3 = turnover ratio
% X = [x1 x2 x3]
% Y_CA = [x1_y1_CA x1_y2_CA ... x3_y3_CA];
% Y_NY = [x1_y1_NY x1_y2_NY ... x3_y3_NY];

% similarity matrix (nX by nY matrix)
% nX = # of x (in this case, 3), 
% nY = # of y (in this case, 3)
sim = zeros(nX,nY);
for i = 1 : nX
    for j = 1 : nY
        val_CA = Y_CA(nX*(i-1)+j);
	val_NY = Y_NY(nX*(i-1)+j);
	sim(nX,nY) = pdist([val_CA,val_NY],'euclidean');
    end
end

% Find max entry M and its index 
% I in the sim matrix
[M,I] = max(sim);   

% Plot line chart (I_x and I_y 
% are the indices from the previous step)
plot(X(I_x), Y_CA(I_y), X(I_x), Y_NY(I_y));
\end{verbatim}
}

% \textbf{\zv is novel with real world applications}: All the participants described \zv as a novel tool and mentioned that they have not seen the declarative pattern searching functionality in any other tool.

\paraem{Finding 8: \zv can be improved.} While the participants looked forward to using the custom query builder in their own workflow, a few of them were interested in directly exposing the commonly-used trends/patterns such as outliers, through the drag and drop interface. Some of them were interested in knowing how they could integrate custom functional primitives (we could not cover it in the tutorial due to time constraints). In order to improve the user experience, participants suggested adding instructions and guidance for new users as part of the interface. Participants also commented on the unrefined look and feel of the tool, as well as the lack of the diverse set of usability related features, such as bookmarking and search history, that are offered in existing systems.






==> docs copy/userstudy-revised.tex <==
%!TEX root=zenvisageql.tex

\vspace{-5pt}
\section{User Study}
\label{sec:userstudy}
\vspace{-3pt}

We conducted a user study to evaluate the utility of \zv for data exploration versus two types of systems---first, visualization tools, similar to Tableau, and second, general database and data mining tools, which also support interactive analytics to a certain extent.
%In order to set up the 
In preparation for the user study, we conducted interviews with data analysts to identify the typical exploration tasks and tools used in their present workflow. Using these interviews, we identified a set of tasks to be used in the user study for \zv. We describe these interviews first, followed by the user study details.

% We conducted a mixed methods study~\cite{creswell2007designing} 
% to compare \zv with a custom-made baseline visual analytics tool to assess how \zv can aid in visualizing interesting patterns, trends, or insights from large datasets. Additional interviews with data analysts were conducted to identify the low level tasks and tools used in their typical workflow, and explore how \zv can help with their everyday activities.

\vspace{-5pt}
\subsection{Analyst Interviews and Task Selection}
\label{sec:interviews}
\vspace{-2pt}

We hired seven data analysts via Upwork~\cite{upwork},
a freelancing plat\-form---we 
found these analysts by searching for freelancers
who had the keywords \texttt{analyst} or \texttt{tableau}
in their profile. 
We conducted one hour interviews with them
to understand how they perform data exploration tasks.
The interviewees had 3---10 years of prior experience
and explained every step of their workflow;
from receiving the dataset to presenting the
analysis to clients.
The rough workflow of all interviewees identified 
was the following: first, data cleaning is performed;
%if the data is not already presented in structured form;
subsequently, the analysts perform data exploration;
then, the analysts develop presentations using their findings.
We then drilled down onto the data exploration step.

We first asked the analysts what types of tools 
they use for data exploration.
Analysts reported nine different tools---the most popular ones 
included Excel (5), Tableau (3), and SPSS (2). 
The rest of the tools were reported by just one analyst:
Python, SQL, Alteryx, Microsoft Visio, Microsoft BI, SAS. 
Perhaps not surprisingly, analysts use both visualization
tools (Tableau, Excel, BI), programming languages (Python),
statistical tools (SAS, SPSS), and relational databases (SQL)
for data exploration.

Then, to identify the common tasks used in data exploration, 
%while not being biased by \zv's targeted use-cases, 
we used a taxonomy of
abstract exploration tasks proposed by Amar et al.~\cite{amar2005low}.
Amar et al. developed their taxonomy through summarizing
the analytical questions that arose
during the analysis of five different datasets, 
independent of the capabilities of existing tools or interfaces.
The exploration tasks in Amar et al.~include:
filtering ({\sf f}), sorting ({\sf s}), determining range ({\sf r}), 
characterizing distribution ({\sf d}),
finding anomalies ({\sf a}), clustering ({\sf c}), 
correlating attributes ({\sf co}), retrieving value ({\sf v}),  
computing derived value ({\sf dv}), and finding extrema ({\sf e}).
When we asked the data analysts which tasks they use in their workflow, 
the responses were consistent in that all of them use all of these
tasks, except for three exceptions---{\textsf c}, reported by four participants,
and {\sf e, d}, reported by six participants. 

%We hired seven data analysts on Upwork \cite{upwork}, an online freelancing platform, and conducted one hour interviews to probe how analysts explore data to find meaningful trends and patterns from large datasets. The interviewees had 3 to 10 years of prior experience as data analysts, and were asked to walk through each step of their workflow; from receiving the dataset to presenting the analysis to clients. \john{To identify the common analytical tasks utilized by analysts, we referenced the taxonomy of low level analytical tasks proposed by Amar et al. \cite{amar2005low}. Amar et al. developed the taxonomy through summarization of the analytical questions that arose during analysis of five different datasets, and generated a comprehensive list of tasks that are not limited by the expressive capability of specific tools or interfaces. Considering that analysts use a wide variety of tools for analysis, the taxonomy provides a fair baseline for comparing the type of tasks analysts work on, rather than focusing on the tools used during their workflow (we identified nine different tools used by the seven data analysts). When we asked the data analysts which low level analytical tasks they used during their workflow, and how they approached these tasks, responses were consistent among the analysts with the exception of clustering; only four analysts reported to use clustering, while at least six analysts utilized the other remaining tasks.}

Given these insights, we selected a small number of appropriate tasks for our user study
encompassing eight of the ten exploration tasks described above:
{\sf f}, {\sf s}, {\sf r}, {\sf d}, {\sf a}, {\sf c}, {\sf co}, {\sf v}.
The other two---{\sf dv} and {\sf e}---finding derived values
and computing extrema, are important tasks in data analysis,
but existing tools (e.g., Excel) already provide adequate
capabilities for these tasks, and we did not expect \zv to 
provide additional benefits. 


\vspace{-3pt}
\subsection{User Study Methodology}
\vspace{-2pt}

The goal of our user study was to evaluate \zv with other tools,
on its ability to effectively support data exploration.

\paragraph{Participants.} 
We recruited 12 graduate students as participants with 
varying degrees of expertise in data analytics.
\papertext{In short, half of them used databases; eight of them 
used Matlab, R, Python or Java; eight of them used
spreadsheet software; and four of them used Tableau.
Data for other not as popular tools are not reported. 
}
\techreport{Table \ref{tab:toolsrep} depicts the participants' experience with different categories of tools.
\begin{table}[H]
\vspace{-10pt}
 \centering\scriptsize
  {\tt    
  \begin{tabular}{|l|l|} \hline
      \textbf{Tools} & \textbf{Count} \\ \hline
      Excel, Google spreadsheet, Google Charts  & 8 \\ \hline
      Tableau & 4 \\ \hline
      SQL, Databases & 6 \\ \hline
      Matlab,R,Python,Java & 8 \\ \hline
      Data mining tools such as weka, JNP & 2 \\ \hline
      Other tools like D3 & 2 \\ \hline
     \end{tabular}
  }
  \vspace{-10pt}\caption{Participants' prior experience with data analytic tools}
  \label{tab:toolsrep}
\vspace{-10pt}\end{table}
}

\paragraph{Baselines.}
For the purposes of our study, we explicitly wanted to
do a head-to-head qualitative and quantitative comparison with visual analytics tools,
and thus we developed a baseline tool to compare \zv against directly.
Further, via qualitative interviews, we compared \zv versus
against other types of tools, such as databases, data mining, and programming tools.
Our baseline tool was developed by replicating the visualization 
selection capabilities of visual analytics tools with a styling scheme identical to \zv to control for external factors.
The tool allowed users to specify the x-axis, y-axis, dimensions, and filters.
The tool would then populate all visualizations meeting the specifications.

\techreport{
\paragraph{Comparison Points.} 
There are no tools that offer the same functionalities as
\zv. Visual analytics tools do not offer the ability
to search for specific patterns, or issue complex visual exploration queries; 
data mining toolkits do not offer the ability to search for visual patterns 
and are instead tailored for general machine learning and prediction. 
\papertext{We decided to implement our baseline tool by replicating
the basic visualization specification capabilities of tools like Tableau,
augmented with additional filtering capabilities. 
The styling scheme was similar to \zv to control for external factors;
details can be found in \cite{techreport}.}\techreport{Since visual analytics tools are closer in spirit and functionality 
to \zv, we decided to implement a visual analytics tool as our baseline.
Thus, our baseline tool replicated the basic query specification and output visualization
capabilities of existing tools such as Tableau.  
We augmented the baseline tool with the ability to specify an arbitrary number of filters, allowing
users to use filters to drill-down on specific visualizations.
This baseline visualization tool was implemented with a styling scheme similar to \zv to control for external factors. 
As depicted in Figure \ref{fig:baseline}, the baseline allowed users to visualize data by allowing them to specify the x-axis, y-axis, category, and filters. The baseline tool would populate all the visualizations, which fit the user specifications, using an alpha-numeric sort order.} In addition to task-based comparisons with this baseline, we
also explicitly asked participants to compare \zv with existing data mining and visual analytics 
tools that they use in their workflow.
}

\paragraph{Dataset.}
We used a housing dataset from Zillow.com \cite{housing_data}, 
consisting of housing sales data for different cities, counties, and states from 2004-15, 
with over 245K rows, and 15 attributes. We selected this dataset since participants could relate to the dataset and understand the usefulness of the tasks.

% We designed the user study tasks with the case studies in Section~\ref{sec:intro} in mind, and we translated the case study tasks into tasks applicable to the real estate dataset. We prepared two sets of tasks for the baseline tool and \zv. The tasks differed only in the selection attributes so that the performance of the interfaces could be measured objectively. Section~\ref{sec:frontend} lists a few example queries that were used in the study.

\paragraph{Tasks.}
We designed the user study tasks with the case studies 
from Section~\ref{sec:intro} in mind,
and translated them into the housing dataset. 
Further, we ensured that these tasks together evaluate 
eight of the exploration tasks described above---{\sf f}, {\sf s}, {\sf r}, {\sf d}, {\sf a}, {\sf c}, {\sf co}, 
and {\sf v}.
One task used in the user study is as follows: ``Find three cities in the state
of NY where the sold price vs year trend is very different from the
state\textquotesingle s overall trend.'' This query required the participants to
first retrieve the trend of NY ({\sf v}) and characterize its distribution ({\sf
d}), then separately filter to retrieve the cities of NY ({\sf f}), compare the
values to find a negative correlation ({\sf co}), sort the results ({\sf s}),
and report the top three cities on the list.

\paragraph{Study Protocol.} 
The user study was conducted using a within-subjects study design~\cite{bordens2002research},
forming three phases.
First, participants described their previous experience with data 
analytics tools. 
Next, participants performed exploration tasks using 
\zv (Tool A) and the baseline tool (Tool B), with the orders 
randomized to reduce order effects.
Participants were provided a 15-minute tutorial-cum-practice session
per tool to get familiarized before performing the tasks.
Finally, participants completed a survey
that both measured their satisfaction levels and preferences,
along with open-ended questions on the strengths
and weaknesses of \zv and the baseline, when compared to 
other analytics tools they may have used.\techreport{ The average study session lasted for 75 minutes on average. 
Participants were paid ten dollars per hour for their participation.}
After the study, we reached out to participants with backgrounds
in data mining and programming, and asked if they could complete
a follow-up interview where they use their favorite analytics tool for performing
one of the tasks. 

\paragraph{Metrics.} 
% We recorded how the participants used the tool, their answers for each task, the audio of discussions, and 
% the responses to the survey. 
Using data that we recorded, we collected the following metrics: 
completion time, accuracy, and the usability ratings 
and satisfaction level from the survey results. 
In addition, we also explicitly 
asked participants to compare \zv with tools that they use in their workflow.
For comparisons between \zv and general database and data mining tools
via follow-up interviews, 
we used the number of lines of code to evaluate the differences. 

\paragraph{Ground Truth.} 
Two expert data analysts prepared the ground truth 
for each the tasks in the form of ranked answers,
along with score cut-offs on a 0 to 5 scale (5 highest). 
Their inter-rater agreement, measured using Kendall's Tau coefficient, 
was 0.854. 
% Then, each expert independently rated the answers on their 
% ranked list on a 0 to 5 scale (5 highest). 
We took the average of the two scores to rate the participants' answers.

\techreport{
\begin{figure}
\vspace{-5pt}
\begin{center}
\fbox{\includegraphics[width=0.6\columnwidth]{figs/baseline.png}}
\end{center}
\vspace{-20pt}
\caption{The baseline interface implemented for the user study.}
\label{fig:baseline}
\vspace{-10pt}
\end{figure}
}

\vspace{-8pt}
\subsection{Key Findings}
\vspace{-2pt}

Three key findings emerged from the study and are described below.
We use $\mu$, $\sigma$, $\chi^2$ to denote average, standard deviation, 
and Chi-square test scores, respectively.

\paraem{Finding 1: \zv enables faster and more accurate exploration than existing visualization tools.}
Since all of our tasks involved generating multiple visualizations
and comparing them to find desired ones, participants were not only able to complete the tasks
 {\em faster}---$\mu$=115s, $\sigma$=51.6 for 
\zv vs.~$\mu$=172.5s, $\sigma$=50.5 for the baseline---but also more 
{\em accurately}---$\mu$=96.3\%, $\sigma$=5.82 for \zv vs.~$\mu$=69.9\%, $\sigma$=13.3 for the baseline.
\techreport{A one-way between-subjects ANOVA,
followed by a post-hoc Tukey's test~\cite{tukey1949comparing},
we found that \zv
had statistically significant
faster task completion times compared to the baseline interface,
with $p$ value of 0.0069.}
The baseline required considerable manual exploration to complete
the same task, explaining the high task completion times. In addition, participants frequently compromised
by selecting suboptimal answers before browsing
the entire list of results for better ones, explaining the 
low accuracy.
On the other hand, \zv was able to 
automate the task of finding desired visualizations, considerably reducing manual
effort.
Also of note is the fact that the accuracy with \zv was close to 100\%---indicating
that a short 15 minute tutorial on \zq was enough to equip users with the knowledge they
needed to address the tasks---and that too, within 2 minutes (on average). 

When asked about using \zv vs.~the baseline in their current workflow, 
9 of the 12 participants stated that they would use \zv in their workflow, 
whereas only two participants stated that they would use our baseline tool ($\chi^2=8.22$, p<0.01). 
When the participants were asked how, 
one participant provided a specific scenario: \textit{``If I am doing my social science study, 
and I want to see some specific behavior among users, then I can use tool A [\zv] 
since I can find the trend I am looking for and easily see what users fit into the pattern.''} (P7). 
In response to the survey question \emph{``I found the tool to be effective in visualizing the data I want to see''}, 
the participants rated \zv higher ($\mu$=4.27, $\sigma$=0.452) than the baseline ($\mu$=2.67, $\sigma$=0.890) 
on a five-point Likert scale. A participant experienced in Tableau 
commented: \textit{``In Tableau, there is no pattern searching. If I see some pattern in Tableau, 
such as a decreasing pattern, and I want to see if any other variable is decreasing in that month, 
I have to go one by one to find this trend. But here I can find this through the query table.''} (P10). 

%we just need to say that all participants were able to successfully use a 15 min tutorial to write zql queries and receive accurate answers

\paraem{Finding 2: \zv complements existing database and data mining systems, and programming languages.}
When explicitly asked about comparing \zv with the
tools they use on a regular basis for data analysis, 
all participants acknowledged that \zv adds %\zq and \zv adds 
value in data exploration not encompassed by their tools. 
\zq augmented with inputs from the sketching canvas proved to be extremely effective.
For example P8 stated: \emph{``you can just [edit] and draw to find out similar patterns. You\textquotesingle ll 
need to do a lot more through Matlab to do the same thing.''}
Another experienced participant mentioned the benefits of not needing to know much programming to accomplish certain tasks: \emph{``The obvious good thing is that you can do complicated queries, and you don\textquotesingle t have to write SQL queries... I can imagine a non-cs student [doing] this.''} (P9).
When asked about the specific tools they would use to solve the user study tasks,
all participants reported a programming language like Matlab or Python. 
This is despite half of the participants reporting using a relational database regularly,
and a smaller number of participants (2) reporting using a data mining tool regularly.
Additionally, multiple participants, even those with extensive programming experience,
reported that \zv would take less time and fewer lines of code for certain data exploration tasks.
(Indeed, we found that all participants were able to complete the user study tasks in under 2 minutes.)
In follow-up email interviews, we asked a few participants to respond with code from their
favorite data analytics tool for the user study tasks.
Two participants responded --- one with Matlab code, one with Python code.
Both these code snippets were much longer than \zq:
as a concrete example, the participant accomplished the same task with 
38 lines of Python code compared to 4 lines of \zq.
While comparing code may not be fair, the roughly order of magnitude
difference demonstrates the power of \zv over existing systems.
% While simply considering the number of lines of code 
% may not be a truly fair comparison, we argue that ZQL requiring 
% roughly only one tenth of the python code demonstrates the value of \zv, 
% and how it can complement existing database and data mining systems.

 % \john{Even those with considerable experience with programming languages such as Python and Matlab argued that \zv would take less time and fewer lines of code for certain data exploration tasks. Considering that all participants were able to complete the provided tasks under 2 minuets (as described in Finding 1) after a brief 15 minute tutorial, it reflects on the learnability of ZQL. Relatively simple queries in \zv can be difficult to reproduce in other languages. If a user wishes to identify trends which are similar to a specific graph, or locate trends which have been consistently decreasing, it would require the users substantial effort to accomplish such tasks. When we asked about the benefits of \zv over existing systems, P8 stated: \emph{``you can just [edit] and draw to find out similar patterns. You\textquotesingle ll need to do a lot more through Matlab to do the same thing.''} Another experienced participant mentioned the benefits of not needing to know programming languages to accomplish these tasks: \emph{``The obvious good thing is that you can do complicated queries, and you don\textquotesingle t have to write SQL queries... I can imagine a non-cs student [doing] this.''} (P9). We include a sample code written by a participant in their favorite language; the participants accomplished the same task with 38 lines of python code compared to 4 lines of instructions in \zv. While simply considering the number of lines of code may not be a truly fair comparison, we argue that ZQL requiring roughly only one tenth of the python code demonstrates the value of \zv, and how it can complement existing database and data mining systems. \papertext{Example code can be found in~\cite{techreport}.} \techreport{Example code can be found in the appendix \ref{sec:userstudy-appendix}.}}

\paraem{Finding 3: \zv can be improved.}  
\papertext{Participants outlined some areas for improvement: some requested drag-and-drop interactions 
to support additional operations, such as outlier finding; others wanted a more polished interface;
and some desired bookmarking and search history capabilities.}
%Others commented on how the interface could be more polished, and suggested that we add bookmarking and search history capabilities.}
\techreport{
 While the participants looked forward to using custom query builder in their own workflow, a few of them were interested in directly exposing the commonly-used trends/patterns such as outliers, through the drag and drop interface. Some were interested in knowing how they could integrate custom functional primitives (we could not cover it in the tutorial due to time constraints). In order to improve the user experience, participants suggested adding instructions and guidance for new users as part of the interface. Participants also commented on the unrefined look and feel of the tool, as well as the lack of a diverse set of usability related features, such as bookmarking and search history, that are offered in existing systems.
}


\later{
\paraem{Finding 1: \zv enabled over 50\% and 100\% faster task completion times than the baseline for the custom query builder and drag and drop interfaces, respectively.} 
%We timed the task completion time for all participants,
%and 
We found that the drag and drop interface
had the smallest, and most predictable completion time ($\mu=74s$, $\sigma=15.1$),
the custom query builder had a higher completion time and a higher variance ($\mu=115s$, $\sigma=51.6$),
while the baseline had a significantly higher completion time ($\mu=172.5s$, $\sigma=50.5$), more than twice the completion time of the drag and drop interface,
and almost 50\% higher than the custom query builder interface.
This is not surprising, given that the baseline tool requires more
manual exploration compared to the other two interfaces.
%We tested for statistical significance on the difference between the three interfaces 
Using 
a one-way between-subjects ANOVA,
followed by a post-hoc Tukey's test~\cite{tukey1949comparing},
we found that the
drag and drop interface and the custom query builder interface
had statistically significant
faster task completion times compared to the baseline interface,
with $p$ values of 0.0010 and 0.0069, respectively.
The difference between the drag and drop interface
and the custom query builder interface was not statistically significant,
with a $p$ value of $0.06$. Detailed statistics can be found in Table\ref{tab:turkeytest}.


% One-way between subject ANOVA~\cite{tukey1949comparing} on the completion time of the tasks revealed that the differences between the three interfaces were significant F(2, 33) = 16.02, p < 0.001. On further applying the post hoc Tukey's test\cite{tukey1949comparing} for comparing the pairwise task completion times among the three interfaces (Table \ref{tab:turkeytest}), we found that both the drag and drop interface and the custom query builder had significantly faster task completion times compared to the baseline tool (p < 0.01), whereas the difference between the drag and drop interface, and the custom query builder was not significantly different.  
\techreport{
\begin{table}[H]
 \centering \scriptsize
  {\tt    
  \scalebox{0.75}{
  \begin{tabular}{|l|l|l|l|} \hline
      \textbf{Treatments} & \textbf{Q statistic} & \textbf{p-value} & \textbf{inference} \\ \hline
	Drag and drop interface vs. Custom query builder & 3.3463 & 0.0605331 & insignificant \\ \hline
	Drag and drop interface vs. Baseline tool & 7.9701 & 0.0010053 & significant (p<0.01) \\ \hline
	Custom query builder vs. Baseline tool & 4.6238 & 0.0069276 & significant (p<0.01) \\ \hline    
     \end{tabular}
  }
  }
\vspace{-10pt}
\caption{Tukey's test on task completion time}
\label{tab:turkeytest}
\vspace{-10pt}
\end{table}
}

\begin{figure}
\begin{center}
\includegraphics[width=0.6\columnwidth]{figs/accuracyvstime.pdf}
\end{center}
\vspace{-25pt}
\caption{Accuracy over time results for zenvisage and baseline}
\label{fig:accuracyvstime}
\vspace{-20pt}
\end{figure}


\paraem{Finding 2: \zv helped retrieve 20\% and 35\% more accurate results than the baseline for drag and drop and custom query builder interfaces, respectively.} 
Comparing the participants' responses against the ground truth responses, 
we found that participants achieved the lowest accuracy with the baseline tool ($\mu=69.9\%$, $\sigma=13.3$). 
\techreport{Further, any tasks that required comparing multiple
pairs of visualizations or trends ended up having lower accuracy than those that looked
for a pattern, such as a peak or an increasing trend, in a single visualization.}
The low accuracy could be attributed to the fact that the participants selected suboptimal answers before browsing through the entire list of results for better answers. Conversely, \zv is able to
accept more fine-grained user input, and
rank output visualizations. With \zv,
participants were able to retrieve accurate answers
with less effort.
Between the two interfaces in \zv,
while the drag and drop interface had a faster task completion time,
it also had a lower accuracy ($\mu=85.3\%$, $\sigma=7.61$).
The custom query builder interface had the
highest accuracy ($\mu=96.3\%$, $\sigma=5.82$).
The accuracy was greater than the baseline by over 20\% (for drag and drop)
and over 35\% (for custom builder).
Finally, looking at both accuracy and task completion times together in Figure~\ref{fig:accuracyvstime}, we see that \zv \emph{helps in ``fast-forwarding to desired visualizations'' with high accuracy.} 


\paraem{Finding 3: The drag and drop interface and the custom query builder complemented each other.
The drag and drop interface was intuitive, while the custom builder was useful for complex queries.} 
The majority of participants (8/12) 
mentioned that the drag and drop 
and custom query builder interfaces complemented each other \techreport{in making \zv powerful}
when searching for specific insights.\techreport{ 25 percent (3/12) of the participants (all with backgrounds in machine learning and data mining) 
preferred using only the custom query builder interface, while just one participant (with no prior experience with query languages or programming languages) found only the drag and drop interface as useful.}
Participants stated that they would use drag and drop for exploration and simple pattern search and custom query builder for specific / complex queries. One stated: \textit{``When I know what I am looking for is exact, I want to use the query table. The other one [drag and drop] is for exploration when you are not so sure.'' (P9).} 
Participants liked the simplicity and intuitiveness of the drag and drop interface. 
One stated: \textit{``[The drawing feature] is very easy and intuitive, I can draw... and automatically get the results.''} (P2).
On a five-point Likert (5 is strongly agree), participants
found the drawing feature easy to use ($\mu=4.45$, $\sigma=0.674$). 
Despite the positive feedback, participants did identify limitations,
specifically, that the functionality was restricted to identifying trends
similar to a single hand-drawn trend.

The majority of the participants (11/12) 
stated that the custom query builder 
allowed them to search for complex insights that might be 
difficult to answer via drag and drop. 
When asked if the custom query builder was difficult to use compared to
the drag-and-drop interface, participants tended to agree ($\mu=3.73$, $\sigma=0.866$ on a five-point Likert scale where five is strongly agree).
At the same time, participants acknowledged 
the flexibility and the efficacy supported by the custom query builder interface. 
One participant explicitly stated why they 
preferred the custom query builder over the drag and drop interface: 
\textit{``When the query is very complicated, [the drag and drop] has its limitations, 
so I think I will use the query table most of the times unless I want to get a brief impression.''} (P6).
Another participant stated that the custom query builder interface \textit{``has more functionality and it lets me express what I want to do clearly more than the sketch''} (P4). This was consistent with other responses. 
Participants with a background in machine learning, 
data mining, and statistics (3/12) preferred
using the custom query builder over the drag and drop interface.

\paraem{Finding 4: \zv was more effective (4.27 vs. 2.67 on a five-point Likert scale)
than the baseline tool at visual data exploration, and would be
a valuable addition to the participants' analytics workflow.} 
In response to the survey question \emph{``I found the tool to be effective in visualizing the data I want to see''}, the participants rated \zv (the drag and drop interface and the custom query builder interface) higher ($\mu=4.27$, $\sigma=0.452$) than the baseline tool ($\mu=2.67$, $\sigma=0.890$) on a five-point Likert scale.
A participant experienced in Tableau commented: \textit{``In Tableau, there is no pattern searching. If I 
see some pattern in Tableau, such as a decreasing pattern, and I want to see if any other variable is 
decreasing in that month, I have to go one by one to find this trend. But here I can find this through the query table.''} (P10).

\paraem{Finding 5: \zv complements existing database and data mining systems, and programming languages.}
When explicitly asking participants about comparing \zv with the
tools they use on a regular basis for data analysis, 
all participants acknowledged that \zv adds %\zq and \zv adds 
value in data exploration not encompassed by their tools. 
\zq augmented with inputs from the sketching canvas proved to be extremely effective.
For example P8 stated: \emph{``you can just [edit] and draw to find out similar patterns. You\textquotesingle ll 
need to do a lot more through Matlab to do the same thing.''}
Another experienced participant mentioned the benefits of not needing to know much programming to accomplish certain tasks: \emph{``The obvious good thing is that you can do complicated queries, and you don\textquotesingle t have to write SQL queries... I can imagine a non-cs student [doing] this.''} (P9).
When asked about the specific tools they would use to solve the user study tasks,
all participants reported a programming language like Matlab or Python. 
This is despite half of the participants reporting using a relational database regularly,
and a smaller number of participants (2) reporting using a data mining tool regularly.
Additionally, multiple participants even with extensive programming experience
reported that \zv would take less time and fewer lines of code for certain data exploration tasks.
(Indeed, we found that all participants were able to complete the user study tasks in under 2 minutes.)
In follow-up email interviews, we asked a few participants to respond with code from their
favorite data analytics tool for the user study tasks.
Two participants responded --- one with Matlab code, one with Python code.
Both these code snippets were much longer than \zq:
as a concrete example, the participant accomplished the same task with 
38 lines of Python code compared to 4 lines of \zq.
While comparing code may not be fair, the roughly order of magnitude
difference demonstrates the power of \zv over existing systems.


\paraem{Finding 6: \zv can be improved.} While the participants looked forward to using custom query builder in their own workflow, a few of them were interested in directly exposing the commonly-used trends/patterns such as outliers, through the drag and drop interface. Some were interested in knowing how they could integrate custom functional primitives (we could not cover it in the tutorial due to time constraints). In order to improve the user experience, participants suggested adding instructions and guidance for new users as part of the interface. Participants also commented on the unrefined look and feel of the tool, as well as the lack of a diverse set of usability related features, such as bookmarking and search history, that are offered in existing systems.
}

%\papertext{Participants also outlined some areas for improvement; details can be found in~\cite{techreport}.
%In brief, the participants requested drag-and-drop interactions to support additional operations, such as outlier finding. Others commented on how the interface could be more polished, and suggested that we add bookmarking and search history capabilities.}
%\john{\techreport{
%While the participants looked forward to using \zv in their own workflow, \zv is not without limitations. The algorithm for finding similar trends and patterns is abstracted to the backend, and participants wanted to learn about the algorithm behind the blackbox. ``I don\textquotesingle t know how the function is working behind the process... Knowing how this works is important'' (P1). They further wished to program their own similarity metrics for their datasets. It is unlikely that a single similarity metric will fit all users needs, and users asked for customizable similarity metrics. Another limitation of \zv is the lack of general features as a visual analytics tool. Existing tools such as Excel or Tableau allows users to directly edit data and generate resulting visualizations or apply statistical methods onto the results. These features are not offered with \zv. In order to improve the user experience, participants also suggested adding instructions and guidance for new users as part of the interface. Participants also commented on the unrefined look and feel of the tool, as well as the lack of a diverse set of usability related features, such as bookmarking and search history, that are offered in existing systems.
%}}


%In order to assess how \zv can aid data analysts in their workflow, we first identified the various analytical tasks commonly performed by data analysts, then designed a user study focused on visual data exploration tasks and how \zv compares to existing tools in this domain. 

%\john{There are no tools that offer the same functionalities as \zv. Existing visual analytics tools do not offer the ability to directly search for specific patterns, or issue complex visual exploration queries. Conversely, the current implementation of \zv is not capable of performing all tasks necessary for data analysts.} to evaluate how \zv can improve the current workflow of data analysts in searching for visual trends and patterns.}

% Following the taxonomy of low level analytical tasks by Amar et al. [cite], we identified four types of visual data exploration tasks that can be streamlined by the features offered by \zv. The four type of tasks are - characterizing distribution, finding anomalies, clustering, and correlating attributes. 
% In order to evaluate how the features of \zv can aid data analyst in these four types of tasks, we conducted a mixed methods study comparing \zv with a baseline tool. In addition, through the user study, we anticipated to a) examine and compare the usability of the drag and drop interface and the custom query builder interface of \zv; b) identify if, when, and how people would use \zv in their workflow; and c) receive general feedback for future improvements.

%can help in visualizing interesting patterns, trends, or insights from large datasets.
%focus on how it helps visual data exploration, make clear of limitations

%\john{We focused our user study tasks on three of the ten low level analytical tasks (finding anomalies, clustering, and correlating attributes) which have no straightforward solutions \cite{lee2006task}. In addition, existing tools already provide well defined functions for the other seven tasks (retrieving value, filtering, computing derived value, finding extremum, sorting, determining range, characterizing distribution). All seven analysts answered that they actively looked for correlation and anomalies in their datasets, and four analysts answered that they cluster data during their exploration stage. Six analysts used visualizations for these three tasks, with the exception of one analyst who used python libraries and customized code for his analysis. These three low level analytical tasks were most relevant to the potential improvements \zv offered to data analysts over existing tools, and we did not expect the features of \zv to offer significant improvements for the remaining seven tasks. With this in mind, we brainstormed realistic tasks using examples from the case studies in Section~\ref{sec:intro} as reference and translated the case study tasks into tasks applicable to the real estate dataset. We prepared three sets of tasks for the three interfaces (baseline, drag and drop, and custom query builder interfaces). The tasks differed only in the selection attributes so that the performance of the interfaces could be measured objectively. Section ~\ref{sec:frontend} lists a few example queries that were used in the study.}

%\papertext{The detailed responses can be found in our technical report~\cite{techreport}.} 
%\techreport{
%Table \ref{tab:tasks} shows the response for commonly used low level analytical tasks.}
%\techreport{
%\begin{table}[H]
%\vspace{-10pt}
 %\centering\scriptsize
 % {\tt    
  %\begin{tabular}{|l|l|} \hline
    %  \textbf{Tasks} & \textbf{Count} \\ \hline
      %Retrieve value & 7  \\ \hline
      %Filter & 7 \\ \hline
      %Compute derived value & 7 \\ \hline
      %Find extreme & 6 \\ \hline
      %Determine range & 7 \\ \hline
      %Characterize distribution & 6 \\ \hline
      %Find anomalies & 7 \\ \hline
      %Cluster & 4 \\ \hline
      %Correlate & 7 \\ \hline
     %\end{tabular}
  %}
  %\vspace{-10pt}\caption{Commonly used low level analytical tasks}
  %\label{tab:tasks}
%\vspace{-10pt}\end{table}
%}





==> docs copy/userstudy-tr-revised.tex <==
%!TEX root=zenvisageql.tex

\vspace{-2pt}
\section{User Study}
\label{sec:userstudy}
\vspace{-2pt}

We conducted a user study to evaluate the utility of \zv for data exploration versus two types of systems---first, visualization tools, similar to Tableau, and second, general database and data mining tools, which also support interactive analytics to a certain extent.
%In order to set up the 
In preparation for the user study, we conducted interviews with data analysts to identify the typical exploration tasks and tools used in their present workflow. Using these interviews, we identified a set of tasks to be used in the user study for \zv. We describe these interviews first, followed by the user study details.

% We conducted a mixed methods study~\cite{creswell2007designing} 
% to compare \zv with a custom-made baseline visual analytics tool to assess how \zv can aid in visualizing interesting patterns, trends, or insights from large datasets. Additional interviews with data analysts were conducted to identify the low level tasks and tools used in their typical workflow, and explore how \zv can help with their everyday activities.

\vspace{-2pt}
\subsection{Analyst Interviews and Task Selection}
\label{sec:interviews}
\vspace{-2pt}

We hired seven data analysts via Upwork~\cite{upwork},
a freelancing plat\-form---we 
found these analysts by searching for freelancers
who had the keywords \texttt{analyst} or \texttt{tableau}
in their profile. 
We conducted one hour interviews with them
to understand how they perform data exploration tasks.
The interviewees had 3---10 years of prior experience,
and told about every step of their workflow;
from receiving the dataset to presenting the
analysis to clients.
The rough workflow of all interviewees identified 
was the following: first, data cleaning is performed;
%if the data is not already presented in structured form;
subsequently, the analysts perform data exploration;
then, the analysts develop presentations using their findings.
We then drilled down onto the data exploration step.

We first asked the analysts what types of tools 
they use for data exploration.
Analysts reported nine different tools---the most popular ones 
included Excel (5), Tableau (3), and SPSS (2). 
The rest of the tools were reported by just one analyst:
Python, SQL, Alteryx, Microsoft Visio, Microsoft BI, SAS. 
Perhaps not surprisingly, analysts use both visualization
tools (Tableau, Excel, BI), programming languages (Python),
statistical tools (SAS, SPSS), and relational databases (SQL)
for data exploration.

Then, to identify the common tasks used in data exploration, 
%while not being biased by \zv's targeted use-cases, 
we used a taxonomy of
abstract exploration tasks proposed by Amar et al.~\cite{amar2005low}.
Amar et al. developed their taxonomy through summarizing
the analytical questions that arose
during the analysis of five different datasets, 
independent of the capabilities of existing tools or interfaces.
The exploration tasks in Amar et al.~include:
filtering ({\sf f}), sorting ({\sf s}), determining range ({\sf r}), 
characterizing distribution ({\sf d}),
finding anomalies ({\sf a}), clustering ({\sf c}), 
correlating attributes ({\sf co}), retrieving value ({\sf v}),  
computing derived value ({\sf dv}), and finding extrema ({\sf e}).
When we asked the data analysts which tasks they use in their workflow, 
the responses were consistent in that all of them use all of these
tasks, except for three exceptions---{\textsf c}, reported by four participants,
and {\sf e, d}, reported by six participants. 

%We hired seven data analysts on Upwork \cite{upwork}, an online freelancing platform, and conducted one hour interviews to probe how analysts explore data to find meaningful trends and patterns from large datasets. The interviewees had 3 to 10 years of prior experience as data analysts, and were asked to walk through each step of their workflow; from receiving the dataset to presenting the analysis to clients. \john{To identify the common analytical tasks utilized by analysts, we referenced the taxonomy of low level analytical tasks proposed by Amar et al. \cite{amar2005low}. Amar et al. developed the taxonomy through summarization of the analytical questions that arose during analysis of five different datasets, and generated a comprehensive list of tasks that are not limited by the expressive capability of specific tools or interfaces. Considering that analysts use a wide variety of tools for analysis, the taxonomy provides a fair baseline for comparing the type of tasks analysts work on, rather than focusing on the tools used during their workflow (we identified nine different tools used by the seven data analysts). When we asked the data analysts which low level analytical tasks they used during their workflow, and how they approached these tasks, responses were consistent among the analysts with the exception of clustering; only four analysts reported to use clustering, while at least six analysts utilized the other remaining tasks.}

Given these insights, we selected a small number of appropriate tasks for our user study
encompassing eight of the ten exploration tasks described above:
{\sf f}, {\sf s}, {\sf r}, {\sf d}, {\sf a}, {\sf c}, {\sf co}, {\sf v}.
The other two---{\sf dv} and {\sf e}---finding derived values
and computing extrema, are important tasks in data analysis,
but existing tools (e.g., Excel) already provide adequate
capabilities for these tasks, and we did not expect \zv to 
provide additional benefits. 


\vspace{-2pt}
\subsection{User Study Methodology}
\vspace{-2pt}

The goal of our user study was to evaluate \zv with other tools,
on its ability to effectively support data exploration.

\paragraph{Participants.} 
We recruited 12 graduate students as participants with 
varying degrees of expertise in data analytics.
\papertext{In short, half of them used databases; eight of them 
used Matlab, R, Python or Java; eight of them used
spreadsheet software; and four of them used Tableau.
Data for other not as popular tools are not reported. 
}
\techreport{Table \ref{tab:toolsrep} depicts the participants' experience with different categories of tools.
\begin{table}[H]
\vspace{-10pt}
 \centering\scriptsize
  {\tt    
  \begin{tabular}{|l|l|} \hline
      \textbf{Tools} & \textbf{Count} \\ \hline
      Excel, Google spreadsheet, Google Charts  & 8 \\ \hline
      Tableau & 4 \\ \hline
      SQL, Databases & 6 \\ \hline
      Matlab,R,Python,Java & 8 \\ \hline
      Data mining tools such as weka, JNP & 2 \\ \hline
      Other tools like D3 & 2 \\ \hline
     \end{tabular}
  }
  \vspace{-10pt}\caption{Participants' prior experience with data analytic tools}
  \label{tab:toolsrep}
\vspace{-10pt}\end{table}
}

\paragraph{Baselines.}
For the purposes of our study, we explicitly wanted to
do a head-to-head qualitative and quantitative comparison with visual analytics tools,
and thus we developed a baseline tool to compare \zv against directly.
Further, via qualitative interviews, we compared \zv versus
against other types of tools, such as databases, data mining, and programming tools.
Our baseline tool was developed by replicating the visualization 
selection capabilities of visual analytics tools with a styling scheme identical to \zv to control for external factors.
The tool allowed users to specify the X-axis, Y-axis, dimensions, and filters.
The tool would then populate all visualizations meeting the specifications.


\paragraph{Dataset.}
We used a housing dataset from Zillow.com \cite{housing_data}, 
consisting of housing sales data for different cities, counties, and states from 2004-15, 
with over 245K rows, and 15 attributes. We selected this dataset since participants could relate to the dataset and understand the usefulness of the tasks.

% We designed the user study tasks with the case studies in Section~\ref{sec:intro} in mind, and we translated the case study tasks into tasks applicable to the real estate dataset. We prepared two sets of tasks for the baseline tool and \zv. The tasks differed only in the selection attributes so that the performance of the interfaces could be measured objectively. Section~\ref{sec:frontend} lists a few example queries that were used in the study.
\paragraph{Comparison Points.} 
There are no tools that offer the same functionalities as
\zv. Visual analytics tools do not offer the ability
to search for specific patterns, or issue complex visual exploration queries; 
data mining toolkits do not offer the ability to search for visual patterns 
and are instead tailored for general machine learning and prediction. 
\papertext{We decided to implement our baseline tool by replicating
the basic visualization specification capabilities of tools like Tableau,
augmented with additional filtering capabilities. 
The styling scheme was similar to \zv to control for external factors;
details can be found in \cite{techreport}.}\techreport{Since visual analytics tools are closer in spirit and functionality 
to \zv, we decided to implement a visual analytics tool as our baseline.
Thus, our baseline tool replicated the basic query specification and output visualization
capabilities of existing tools such as Tableau.  
We augmented the baseline tool with the ability to specify an arbitrary number of filters, allowing
users to use filters to drill-down on specific visualizations.
This baseline visualization tool was implemented with a styling scheme similar to \zv to control for external factors. 
As depicted in Figure \ref{fig:baseline}, the baseline allowed users to visualize data by allowing them to specify the x-axis, y-axis, category, and filters. The baseline tool would populate all the visualizations, which fit the user specifications, using an alpha-numeric sort order.} In addition to task-based comparisons with this baseline, we
also explicitly asked participants to compare \zv with existing data mining and visual analytics 
tools that they use in their workflow.

\paragraph{Tasks.}
We designed the user study tasks with the case studies 
from Section~\ref{sec:intro} in mind,
and translated them into the housing dataset. 
Further, we ensured that these tasks together evaluate 
eight of the exploration tasks described above---{\sf f}, {\sf s}, {\sf r}, {\sf d}, {\sf a}, {\sf c}, {\sf co}, 
and {\sf v}.
One task used in the user study is as follows: ``Find three cities in the state of NY where the Sold Price vs Year trend is very different from the state\textquotesingle s overall trend.'' This query required the participants to first retrieve the trend of NY ({\sf v}) and characterize its distribution ({\sf d}), then separately filter to retrieve the cities of NY ({\sf f}), compare the values to find a negative correlation ({\sf co}), sort the results ({\sf s}), and report the top three cities on the list.

\paragraph{Study Protocol.} 
The user study was conducted using a within-subjects study design~\cite{bordens2002research},
forming three phases.
First, participants described their previous experience with data 
analytics tools. 
Next, participants performed exploration tasks using 
\zv (Tool A) and the baseline tool (Tool B), with the orders 
randomized to reduce order effects.
Participants were provided a 15-minute tutorial-cum-practice session
per tool to get familiarized before performing the tasks.
Finally, participants completed a survey
that both measured their satisfaction levels and preferences,
along with open-ended questions on the strengths
and weaknesses of \zv and the baseline, when compared to 
other analytics tools they may have used.\techreport{ The average study session lasted for 75 minutes on average. 
Participants were paid ten dollars per hour for their participation.}
After the study, we reached out to participants with backgrounds
in data mining and programming, and asked if they could complete
a follow-up interview where they use their favorite analytics tool for performing
one of the tasks, via email. 

\paragraph{Metrics.} 
% We recorded how the participants used the tool, their answers for each task, the audio of discussions, and 
% the responses to the survey. 
Using data that we recorded, we collected the following metrics: 
completion time, accuracy, and the usability ratings 
and satisfaction level from the survey results. 
In addition, we also explicitly 
asked participants to compare \zv with tools that they use in their workflow.
For comparisons between \zv and general database and data mining tools
via follow-up interviews, 
we used the number of lines of code to evaluate the differences. 

\paragraph{Ground Truth.} 
Two expert data analysts prepared the ground truth 
for each the tasks in the form of ranked answers,
along with score cut-offs on a 0 to 5 scale (5 highest). 
Their inter-rater agreement, measured using Kendall's Tau coefficient, 
was 0.854. 
% Then, each expert independently rated the answers on their 
% ranked list on a 0 to 5 scale (5 highest). 
We took the average of the two scores to rate the participants' answers.

\techreport{
\begin{figure}
\vspace{-5pt}
\begin{center}
\fbox{\includegraphics[width=0.6\columnwidth]{figs/baseline.png}}
\end{center}
\vspace{-20pt}
\caption{The baseline interface implemented for the user study.}
\label{fig:baseline}
\vspace{-10pt}
\end{figure}
}

\vspace{-2pt}
\subsection{Key Findings}
\vspace{-2pt}

Three key findings emerged from the study and are described below.
We use $\mu$, $\sigma$, $\chi^2$ to denote average, standard deviation, 
and Chi-square test scores, respectively.

\paraem{Finding 1: \zv enabled over 50\% and 100\% faster task completion times than the baseline for the custom query builder and drag and drop interfaces, respectively.} 
%We timed the task completion time for all participants,
%and 
We found that the drag and drop interface
had the smallest, and most predictable completion time ($\mu=74s$, $\sigma=15.1$),
the custom query builder had a higher completion time and a higher variance ($\mu=115s$, $\sigma=51.6$),
while the baseline had a significantly higher completion time ($\mu=172.5s$, $\sigma=50.5$), more than twice the completion time of the drag and drop interface,
and almost 50\% higher than the custom query builder interface.
This is not surprising, given that the baseline tool requires more
manual exploration compared to the other two interfaces.
%We tested for statistical significance on the difference between the three interfaces 
Using 
a one-way between-subjects ANOVA,
followed by a post-hoc Tukey's test~\cite{tukey1949comparing},
we found that the
drag and drop interface and the custom query builder interface
had statistically significant
faster task completion times compared to the baseline interface,
with $p$ values of 0.0010 and 0.0069, respectively.
The difference between the drag and drop interface
and the custom query builder interface was not statistically significant,
with a $p$ value of $0.06$. Detailed statistics can be found in Table\ref{tab:turkeytest}.


% One-way between subject ANOVA~\cite{tukey1949comparing} on the completion time of the tasks revealed that the differences between the three interfaces were significant F(2, 33) = 16.02, p < 0.001. On further applying the post hoc Tukey's test\cite{tukey1949comparing} for comparing the pairwise task completion times among the three interfaces (Table \ref{tab:turkeytest}), we found that both the drag and drop interface and the custom query builder had significantly faster task completion times compared to the baseline tool (p < 0.01), whereas the difference between the drag and drop interface, and the custom query builder was not significantly different.  
\techreport{
\begin{table}[H]
 \centering \scriptsize
  {\tt    
  \scalebox{0.75}{
  \begin{tabular}{|l|l|l|l|} \hline
      \textbf{Treatments} & \textbf{Q statistic} & \textbf{p-value} & \textbf{inference} \\ \hline
	Drag and drop interface vs. Custom query builder & 3.3463 & 0.0605331 & insignificant \\ \hline
	Drag and drop interface vs. Baseline tool & 7.9701 & 0.0010053 & significant (p<0.01) \\ \hline
	Custom query builder vs. Baseline tool & 4.6238 & 0.0069276 & significant (p<0.01) \\ \hline    
     \end{tabular}
  }
  }
\vspace{-10pt}
\caption{Tukey's test on task completion time}
\label{tab:turkeytest}
\vspace{-10pt}
\end{table}
}

\begin{figure}
\begin{center}
\includegraphics[width=0.6\columnwidth]{figs/accuracyvstime.pdf}
\end{center}
\vspace{-25pt}
\caption{Accuracy over time results for zenvisage and baseline}
\label{fig:accuracyvstime}
\vspace{-20pt}
\end{figure}


\paraem{Finding 2: \zv helped retrieve 20\% and 35\% more accurate results than the baseline for drag and drop and custom query builder interfaces, respectively.} 
Comparing the participants' responses against the ground truth responses, 
we found that participants achieved the lowest accuracy with the baseline tool ($\mu=69.9\%$, $\sigma=13.3$). 
\techreport{Further, any tasks that required comparing multiple
pairs of visualizations or trends ended up having lower accuracy than those that looked
for a pattern, such as a peak or an increasing trend, in a single visualization.}
The low accuracy could be attributed to the fact that the participants selected suboptimal answers before browsing through the entire list of results for better answers. Conversely, \zv is able to
accept more fine-grained user input, and
rank output visualizations. With \zv,
participants were able to retrieve accurate answers
with less effort.
Between the two interfaces in \zv,
while the drag and drop interface had a faster task completion time,
it also had a lower accuracy ($\mu=85.3\%$, $\sigma=7.61$).
The custom query builder interface had the
highest accuracy ($\mu=96.3\%$, $\sigma=5.82$).
The accuracy was greater than the baseline by over 20\% (for drag and drop)
and over 35\% (for custom builder).
Finally, looking at both accuracy and task completion times together in Figure~\ref{fig:accuracyvstime}, we see that \zv \emph{helps in ``fast-forwarding to desired visualizations'' with high accuracy.} 


\paraem{Finding 3: The drag and drop interface and the custom query builder complemented each other.
The drag and drop interface was intuitive, while the custom builder was useful for complex queries.} 
The majority of participants (8/12) 
mentioned that the drag and drop 
and custom query builder interfaces complemented each other \techreport{in making \zv powerful}
when searching for specific insights.\techreport{ 25 percent (3/12) of the participants (all with backgrounds in machine learning and data mining) 
preferred using only the custom query builder interface, while just one participant (with no prior experience with query languages or programming languages) found only the drag and drop interface as useful.}
Participants stated that they would use drag and drop for exploration and simple pattern search and custom query builder for specific / complex queries. One stated: \textit{``When I know what I am looking for is exact, I want to use the query table. The other one [drag and drop] is for exploration when you are not so sure.'' (P9).} 
Participants liked the simplicity and intuitiveness of the drag and drop interface. 
One stated: \textit{``[The drawing feature] is very easy and intuitive, I can draw... and automatically get the results.''} (P2).
On a five-point Likert (5 is strongly agree), participants
found the drawing feature easy to use ($\mu=4.45$, $\sigma=0.674$). 
Despite the positive feedback, participants did identify limitations,
specifically, that the functionality was restricted to identifying trends
similar to a single hand-drawn trend.

The majority of the participants (11/12) 
stated that the custom query builder 
allowed them to search for complex insights that might be 
difficult to answer via drag and drop. 
When asked if the custom query builder was difficult to use compared to
the drag-and-drop interface, participants tended to agree ($\mu=3.73$, $\sigma=0.866$ on a five-point Likert scale where five is strongly agree).
At the same time, participants acknowledged 
the flexibility and the efficacy supported by the custom query builder interface. 
One participant explicitly stated why they 
preferred the custom query builder over the drag and drop interface: 
\textit{``When the query is very complicated, [the drag and drop] has its limitations, 
so I think I will use the query table most of the times unless I want to get a brief impression.''} (P6).
Another participant stated that the custom query builder interface \textit{``has more functionality and it lets me express what I want to do clearly more than the sketch''} (P4). This was consistent with other responses. 
Participants with a background in machine learning, 
data mining, and statistics (3/12) preferred
using the custom query builder over the drag and drop interface.

\paraem{Finding 4: \zv was more effective (4.27 vs. 2.67 on a five-point Likert scale)
than the baseline tool at visual data exploration, and would be
a valuable addition to the participants' analytics workflow.} 
In response to the survey question \emph{``I found the tool to be effective in visualizing the data I want to see''}, the participants rated \zv (the drag and drop interface and the custom query builder interface) higher ($\mu=4.27$, $\sigma=0.452$) than the baseline tool ($\mu=2.67$, $\sigma=0.890$) on a five-point Likert scale.
A participant experienced in Tableau commented: \textit{``In Tableau, there is no pattern searching. If I 
see some pattern in Tableau, such as a decreasing pattern, and I want to see if any other variable is 
decreasing in that month, I have to go one by one to find this trend. But here I can find this through the query table.''} (P10).

\paraem{Finding 5: \zv complements existing database and data mining systems, and programming languages.}
When explicitly asking participants about comparing \zv with the
tools they use on a regular basis for data analysis, 
all participants acknowledged that \zv adds %\zq and \zv adds 
value in data exploration not encompassed by their tools. 
\zq augmented with inputs from the sketching canvas proved to be extremely effective.
For example P8 stated: \emph{``you can just [edit] and draw to find out similar patterns. You\textquotesingle ll 
need to do a lot more through Matlab to do the same thing.''}
Another experienced participant mentioned the benefits of not needing to know much programming to accomplish certain tasks: \emph{``The obvious good thing is that you can do complicated queries, and you don\textquotesingle t have to write SQL queries... I can imagine a non-cs student [doing] this.''} (P9).
When asked about the specific tools they would use to solve the user study tasks,
all participants reported a programming language like Matlab or Python. 
This is despite half of the participants reporting using a relational database regularly,
and a smaller number of participants (2) reporting using a data mining tool regularly.
Additionally, multiple participants even with extensive programming experience
reported that \zv would take less time and fewer lines of code for certain data exploration tasks.
(Indeed, we found that all participants were able to complete the user study tasks in under 2 minutes.)
In follow-up email interviews, we asked a few participants to respond with code from their
favorite data analytics tool for the user study tasks.
Two participants responded --- one with Matlab code, one with Python code.
Both these code snippets were much longer than \zq:
as a concrete example, the participant accomplished the same task with 
38 lines of Python code compared to 4 lines of \zq.
While comparing code may not be fair, the roughly order of magnitude
difference demonstrates the power of \zv over existing systems.


\paraem{Finding 6: \zv can be improved.} While the participants looked forward to using custom query builder in their own workflow, a few of them were interested in directly exposing the commonly-used trends/patterns such as outliers, through the drag and drop interface. Some were interested in knowing how they could integrate custom functional primitives (we could not cover it in the tutorial due to time constraints). In order to improve the user experience, participants suggested adding instructions and guidance for new users as part of the interface. Participants also commented on the unrefined look and feel of the tool, as well as the lack of a diverse set of usability related features, such as bookmarking and search history, that are offered in existing systems.



\later{
\paraem{Finding 1: \zv enables faster and more accurate exploration than existing visualization tools.}
Since all of our tasks involved generating multiple visualizations
and comparing them to find desired ones, participants were not only able to complete the tasks
 {\em faster}---$\mu$=115s, $\sigma$=51.6 for 
\zv vs.~$\mu$=172.5s, $\sigma$=50.5 for the baseline---but also more 
{\em accurately}---$\mu$=96.3\%, $\sigma$=5.82 for \zv vs.~$\mu$=69.9\%, $\sigma$=13.3 for the baseline.
The baseline requires considerable manual exploration to complete
the same task, explaining the high task completion times; in addition, participants frequently compromised
by selecting suboptimal answers before browsing
the entire list of results for better ones, explaining the 
low accuracy.
On the other hand, \zv is able to 
automate the task of finding desired visualizations, considerably reducing manual
effort.
Also of note is the fact that the accuracy with \zv is close to 100\%---indicating
that a short 15 minute tutorial on \zq was enough to equip users with the knowledge they
needed to address the tasks---and that too, within 2 minutes (on average). 

When asked about using \zv vs.~the baseline in their current workflow, 
9 of the 12 participants stated that they would use \zv in their workflow, 
whereas only two participants stated that they would use our baseline tool ($\chi^2=8.22$, p<0.01). 
When the participants were asked how, 
one participant provided a specific scenario: \textit{``If I am doing my social science study, 
and I want to see some specific behavior among users, then I can use tool A [\zv] 
since I can find the trend I am looking for and easily see what users fit into the pattern.''} (P7). 
In response to the survey question \emph{``I found the tool to be effective in visualizing the data I want to see''}, 
the participants rated \zv higher ($\mu$=4.27, $\sigma$=0.452) than the baseline ($\mu$=2.67, $\sigma$=0.890) 
on a five-point Likert scale. A participant experienced in Tableau 
commented: \textit{``In Tableau, there is no pattern searching. If I see some pattern in Tableau, 
such as a decreasing pattern, and I want to see if any other variable is decreasing in that month, 
I have to go one by one to find this trend. But here I can find this through the query table.''} (P10). 

%we just need to say that all participants were able to successfully use a 15 min tutorial to write zql queries and receive accurate answers

\paraem{Finding 2: \zv complements existing database and data mining systems, and programming languages.}
When explicitly asking participants about comparing \zv with the
tools they use on a regular basis for data analysis, 
all participants acknowledged that \zv adds %\zq and \zv adds 
value in data exploration not encompassed by their tools. 
\zq augmented with inputs from the sketching canvas proved to be extremely effective.
For example P8 stated: \emph{``you can just [edit] and draw to find out similar patterns. You\textquotesingle ll 
need to do a lot more through Matlab to do the same thing.''}
Another experienced participant mentioned the benefits of not needing to know much programming to accomplish certain tasks: \emph{``The obvious good thing is that you can do complicated queries, and you don\textquotesingle t have to write SQL queries... I can imagine a non-cs student [doing] this.''} (P9).
When asked about the specific tools they would use to solve the user study tasks,
all participants reported a programming language like Matlab or Python. 
This is despite half of the participants reporting using a relational database regularly,
and a smaller number of participants (2) reporting using a data mining tool regularly.
Additionally, multiple participants even with extensive programming experience
reported that \zv would take less time and fewer lines of code for certain data exploration tasks.
(Indeed, we found that all participants were able to complete the user study tasks in under 2 minutes.)
In follow-up email interviews, we asked a few participants to respond with code from their
favorite data analytics tool for the user study tasks.
Two participants responded --- one with Matlab code, one with Python code.
Both these code snippets were much longer than \zq:
as a concrete example, the participant accomplished the same task with 
38 lines of Python code compared to 4 lines of \zq.
While comparing code may not be fair, the roughly order of magnitude
difference demonstrates the power of \zv over existing systems.
% While simply considering the number of lines of code 
% may not be a truly fair comparison, we argue that ZQL requiring 
% roughly only one tenth of the python code demonstrates the value of \zv, 
% and how it can complement existing database and data mining systems.

 % \john{Even those with considerable experience with programming languages such as Python and Matlab argued that \zv would take less time and fewer lines of code for certain data exploration tasks. Considering that all participants were able to complete the provided tasks under 2 minuets (as described in Finding 1) after a brief 15 minute tutorial, it reflects on the learnability of ZQL. Relatively simple queries in \zv can be difficult to reproduce in other languages. If a user wishes to identify trends which are similar to a specific graph, or locate trends which have been consistently decreasing, it would require the users substantial effort to accomplish such tasks. When we asked about the benefits of \zv over existing systems, P8 stated: \emph{``you can just [edit] and draw to find out similar patterns. You\textquotesingle ll need to do a lot more through Matlab to do the same thing.''} Another experienced participant mentioned the benefits of not needing to know programming languages to accomplish these tasks: \emph{``The obvious good thing is that you can do complicated queries, and you don\textquotesingle t have to write SQL queries... I can imagine a non-cs student [doing] this.''} (P9). We include a sample code written by a participant in their favorite language; the participants accomplished the same task with 38 lines of python code compared to 4 lines of instructions in \zv. While simply considering the number of lines of code may not be a truly fair comparison, we argue that ZQL requiring roughly only one tenth of the python code demonstrates the value of \zv, and how it can complement existing database and data mining systems. \papertext{Example code can be found in~\cite{techreport}.} \techreport{Example code can be found in the appendix \ref{sec:userstudy-appendix}.}}

\paraem{Finding 3: \zv can be improved.}  
\papertext{Participants outlined some areas for improvement: some requested drag-and-drop interactions 
to support additional operations, such as outlier finding; others wanted a more polished interface;
and some desired bookmarking and search history capabilities.}
%Others commented on how the interface could be more polished, and suggested that we add bookmarking and search history capabilities.}
\techreport{
 While the participants looked forward to using custom query builder in their own workflow, a few of them were interested in directly exposing the commonly-used trends/patterns such as outliers, through the drag and drop interface. Some were interested in knowing how they could integrate custom functional primitives (we could not cover it in the tutorial due to time constraints). In order to improve the user experience, participants suggested adding instructions and guidance for new users as part of the interface. Participants also commented on the unrefined look and feel of the tool, as well as the lack of a diverse set of usability related features, such as bookmarking and search history, that are offered in existing systems.
}
}

%\papertext{Participants also outlined some areas for improvement; details can be found in~\cite{techreport}.
%In brief, the participants requested drag-and-drop interactions to support additional operations, such as outlier finding. Others commented on how the interface could be more polished, and suggested that we add bookmarking and search history capabilities.}
%\john{\techreport{
%While the participants looked forward to using \zv in their own workflow, \zv is not without limitations. The algorithm for finding similar trends and patterns is abstracted to the backend, and participants wanted to learn about the algorithm behind the blackbox. ``I don\textquotesingle t know how the function is working behind the process... Knowing how this works is important'' (P1). They further wished to program their own similarity metrics for their datasets. It is unlikely that a single similarity metric will fit all users needs, and users asked for customizable similarity metrics. Another limitation of \zv is the lack of general features as a visual analytics tool. Existing tools such as Excel or Tableau allows users to directly edit data and generate resulting visualizations or apply statistical methods onto the results. These features are not offered with \zv. In order to improve the user experience, participants also suggested adding instructions and guidance for new users as part of the interface. Participants also commented on the unrefined look and feel of the tool, as well as the lack of a diverse set of usability related features, such as bookmarking and search history, that are offered in existing systems.
%}}


%In order to assess how \zv can aid data analysts in their workflow, we first identified the various analytical tasks commonly performed by data analysts, then designed a user study focused on visual data exploration tasks and how \zv compares to existing tools in this domain. 

%\john{There are no tools that offer the same functionalities as \zv. Existing visual analytics tools do not offer the ability to directly search for specific patterns, or issue complex visual exploration queries. Conversely, the current implementation of \zv is not capable of performing all tasks necessary for data analysts.} to evaluate how \zv can improve the current workflow of data analysts in searching for visual trends and patterns.}

% Following the taxonomy of low level analytical tasks by Amar et al. [cite], we identified four types of visual data exploration tasks that can be streamlined by the features offered by \zv. The four type of tasks are - characterizing distribution, finding anomalies, clustering, and correlating attributes. 
% In order to evaluate how the features of \zv can aid data analyst in these four types of tasks, we conducted a mixed methods study comparing \zv with a baseline tool. In addition, through the user study, we anticipated to a) examine and compare the usability of the drag and drop interface and the custom query builder interface of \zv; b) identify if, when, and how people would use \zv in their workflow; and c) receive general feedback for future improvements.

%can help in visualizing interesting patterns, trends, or insights from large datasets.
%focus on how it helps visual data exploration, make clear of limitations

%\john{We focused our user study tasks on three of the ten low level analytical tasks (finding anomalies, clustering, and correlating attributes) which have no straightforward solutions \cite{lee2006task}. In addition, existing tools already provide well defined functions for the other seven tasks (retrieving value, filtering, computing derived value, finding extremum, sorting, determining range, characterizing distribution). All seven analysts answered that they actively looked for correlation and anomalies in their datasets, and four analysts answered that they cluster data during their exploration stage. Six analysts used visualizations for these three tasks, with the exception of one analyst who used python libraries and customized code for his analysis. These three low level analytical tasks were most relevant to the potential improvements \zv offered to data analysts over existing tools, and we did not expect the features of \zv to offer significant improvements for the remaining seven tasks. With this in mind, we brainstormed realistic tasks using examples from the case studies in Section~\ref{sec:intro} as reference and translated the case study tasks into tasks applicable to the real estate dataset. We prepared three sets of tasks for the three interfaces (baseline, drag and drop, and custom query builder interfaces). The tasks differed only in the selection attributes so that the performance of the interfaces could be measured objectively. Section ~\ref{sec:frontend} lists a few example queries that were used in the study.}

%\papertext{The detailed responses can be found in our technical report~\cite{techreport}.} 
%\techreport{
%Table \ref{tab:tasks} shows the response for commonly used low level analytical tasks.}
%\techreport{
%\begin{table}[H]
%\vspace{-10pt}
 %\centering\scriptsize
 % {\tt    
  %\begin{tabular}{|l|l|} \hline
    %  \textbf{Tasks} & \textbf{Count} \\ \hline
      %Retrieve value & 7  \\ \hline
      %Filter & 7 \\ \hline
      %Compute derived value & 7 \\ \hline
      %Find extreme & 6 \\ \hline
      %Determine range & 7 \\ \hline
      %Characterize distribution & 6 \\ \hline
      %Find anomalies & 7 \\ \hline
      %Cluster & 4 \\ \hline
      %Correlate & 7 \\ \hline
     %\end{tabular}
  %}
  %\vspace{-10pt}\caption{Commonly used low level analytical tasks}
  %\label{tab:tasks}
%\vspace{-10pt}\end{table}
%}





==> docs copy/userstudy.tex <==
%!TEX root=zenvisageql.tex

\section{User Study}
\label{sec:userstudy}
We conducted a mixed methods study~\cite{creswell2007designing} 
in order to assess the efficacy of \zv. 
We wanted to: 
a) examine and compare the usability of the drag and drop 
interface and the custom query builder interface of \zv; 
b) compare the performance and usefulness of \zv 
with existing tools;
\papertext{and}
c) identify if, when, and how people would use \zv in their workflow\techreport{;
and d) receive general feedback for future improvements}.

\subsection{User Study Methodology}
\paragraph{Participants.} We recruited 12 graduate students 
as participants with varying degrees of expertise in data analytics. 
\papertext{Details of their prior experience can be found in our 
technical report~\cite{techreport}.}
\techreport{Table \ref{tab:toolsrep} depicts the participants' experience with different categories of tools.
\begin{table}[H]
\vspace{-10pt}
 \centering\scriptsize
  {\tt    
  \begin{tabular}{|l|l|} \hline
      \textbf{Tools} & \textbf{Count} \\ \hline
      Excel, Google spreadsheet, Google Charts  & 8 \\ \hline
      Tableau & 4 \\ \hline
      SQL, Databases & 6 \\ \hline
      Matlab,R,Python,Java & 8 \\ \hline
      Data mining tools such as weka, JNP & 2 \\ \hline
      Other tools like D3 & 2 \\ \hline
     \end{tabular}
  }
  \vspace{-10pt}\caption{Participants' prior experience with data analytic tools}
  \label{tab:toolsrep}
\vspace{-10pt}\end{table}
}

\paragraph{Dataset.} 
We used a housing dataset from Zillow.com~\cite{housing_data} consisting of
housing sales data for different cities, counties, and states from 2004--15,
with over 245K rows, and 15 attributes.
\papertext{Since looking for housing is commonplace, the participants could relate to the dataset and understand the
usefulness of the tasks.}
\techreport{
We selected this dataset for two
reasons: 
First, housing data is often explored by data analysts using existing
visualization tools~\cite{elmqvist2008datameadow}. Second, looking for housing
is commonplace for graduate students while in school and upon
graduation; the participants could relate to the dataset and understand the
usefulness of the tasks.
}
  
\paragraph{Comparison Points.} 
There are no tools that offer the same functionalities as
\zv. Visual analytics tools do not offer the ability
to search for specific patterns, or issue complex visual exploration queries; 
data mining toolkits do not offer the ability to search for visual patterns 
and are instead tailored for general machine learning and prediction. 
\papertext{We decided to implement our baseline tool by replicating
the basic visualization specification capabilities of tools like Tableau,
augmented with additional filtering capabilities. 
The styling scheme was similar to \zv to control for external factors;
details can be found in \cite{techreport}.}\techreport{Since visual analytics tools are closer in spirit and functionality 
to \zv, we decided to implement a visual analytics tool as our baseline.
Thus, our baseline tool replicated the basic query specification and output visualization
capabilities of existing tools such as Tableau.  
We augmented the baseline tool with the ability to specify an arbitrary number of filters, allowing
users to use filters to drill-down on specific visualizations.
This baseline visualization tool was implemented with a styling scheme similar to \zv to control for external factors. 
As depicted in Figure \ref{fig:baseline}, the baseline allowed users to visualize data by allowing them to specify the x-axis, y-axis, category, and filters. The baseline tool would populate all the visualizations, which fit the user specifications, using an alpha-numeric sort order.} In addition to task-based comparisons with this baseline, we
also explicitly asked participants to compare \zv with existing data mining and visual analytics 
tools that they use in their workflow.
 
\paragraph{Study Protocol.} The user study was 
conducted using a within-subjects study design~\cite{bordens2002research}. 
The study consisted of three phases. 
In the first phase, participants described 
their previous experience with data analytics and visualization tools. 
In the second phase, participants performed visual analytics 
tasks using each of the tools. 
\techreport{\zv was introduced as Tool A and the baseline tool was introduced as Tool B.}
This phase began with a 15-minute tutorial that included an overview of the interface and two practice questions. 
The order of the baseline tool and the \zv interface was randomized to reduce order effects.
To compare the effectiveness of the drag and drop interface 
and the custom query builder interface of \zv, 
participants performed two separate sets of tasks on \zv, one for each component. Finally, in the third phase, participants completed a survey that measured 
their satisfaction levels and preferences, followed by open-ended interview questions\techreport{ assessing the strengths and weaknesses 
of the tools, and whether they would use the two tools in their workflow}. 
\techreport{
The average study session lasted for 75 minutes on average. 
Participants were paid ten dollars per hour for their participation.}

\paragraph{Tasks.}
We prepared three sets of tasks for the three interfaces (baseline, drag and
drop, and custom query builder interfaces). The tasks differed only in the
selection attributes so that the performance of the interfaces could be
measured objectively (Section~\ref{sec:frontend} lists a few example queries
that were used in the study \papertext{; others can be found
in the techreport~\cite{techreport}}).
\techreport{We carefully selected tasks which can surface during a
search for a house.
}
To demonstrate the efficacy of \zv, the tasks focused on
identifying patterns, trends or anomalies in housing data; these are
non-trivial tasks to complete with a large dataset with existing tools. 
\techreport{The tasks were targeted to test the core features of \zv and solicit responses from participants on how \zv could complement existing data analytics workflows.}

%The tasks that the participants performed on the two tools were designed to be similar in nature (differing only in selection attributes) so that we could compare the performance more objectively. The tasks focused on identifying visualizations with specific insights. Section~\ref{sec:frontend} lists a few example queries that were used in the study. 

\paragraph{Metrics.} 
We manually recorded how participants used the tool and their answers for each task. We further collected browser activity using screen capture software, system interaction logs, audio of discussions, and asked the participants to complete a survey. 
\techreport{Using this data, we collected the following metrics: task completion time, task accuracy, the number of visualizations browsed for each task, the number of edits made on the drawing panel and the query table, and the usability ratings and satisfaction level from the survey results.}

\paragraph{Ground Truth.} 
Two expert data analysts prepared the ground truth for each the tasks in the form of ranked answers. Their inter-rater agreement, measured using Kendall\textquotesingle s Tau rank correlation coefficient, was 0.854. 
% The experts further discussed and resolved the conflicting answers to produce a final single ranked list of answers for each task. 
Then, each expert independently rated the answers on their ranked list on a 0 to 5 scale (5 highest). We took the average of the two scores to rate the participants\textquotesingle~answers.

\techreport{
\begin{figure}
\vspace{-5pt}
\begin{center}
\fbox{\includegraphics[width=0.6\columnwidth]{figs/baseline.png}}
\end{center}
\vspace{-20pt}
\caption{The baseline interface implemented for the user study.}
\label{fig:baseline}
\vspace{-10pt}
\end{figure}
}


\subsection{Key Findings}
Six key findings emerged from the study.  We describe them below.
We use $\mu$, $\sigma$, $\chi^2$ to denote average, standard deviation, and Chi-square test scores, respectively.

\paraem{Finding 1: \zv enabled over 50\% and 100\% faster task completion times than the baseline for the custom query builder and drag and drop interfaces, respectively.} 
%We timed the task completion time for all participants,
%and 
We found that the drag and drop interface
had the smallest, and most predictable completion time ($\mu=74s$, $\sigma=15.1$),
the custom query builder had a higher completion time and a higher variance ($\mu=115s$, $\sigma=51.6$),
while the baseline had a significantly higher completion time ($\mu=172.5s$, $\sigma=50.5$), more than twice the completion time of the drag and drop interface,
and almost 50\% higher than the custom query builder interface.
This is not surprising, given that the baseline tool requires more
manual exploration compared to the other two interfaces.
%We tested for statistical significance on the difference between the three interfaces 
Using 
a one-way between-subjects ANOVA,
followed by a post-hoc Tukey's test~\cite{tukey1949comparing},
we found that the
drag and drop interface and the custom query builder interface
had statistically significant
faster task completion times compared to the baseline interface,
with $p$ values of 0.0010 and 0.0069, respectively.
The difference between the drag and drop interface
and the custom query builder interface was not statistically significant,
with a $p$ value of $0.06$.
\papertext{Detailed statistics can be found in ~\cite{techreport}.}


% One-way between subject ANOVA~\cite{tukey1949comparing} on the completion time of the tasks revealed that the differences between the three interfaces were significant F(2, 33) = 16.02, p < 0.001. On further applying the post hoc Tukey's test\cite{tukey1949comparing} for comparing the pairwise task completion times among the three interfaces (Table \ref{tab:turkeytest}), we found that both the drag and drop interface and the custom query builder had significantly faster task completion times compared to the baseline tool (p < 0.01), whereas the difference between the drag and drop interface, and the custom query builder was not significantly different.  
\techreport{
\begin{table}[H]
 \centering \scriptsize
  {\tt    
  \scalebox{0.75}{
  \begin{tabular}{|l|l|l|l|} \hline
      \textbf{Treatments} & \textbf{Q statistic} & \textbf{p-value} & \textbf{inference} \\ \hline
	Drag and drop interface vs. Custom query builder & 3.3463 & 0.0605331 & insignificant \\ \hline
	Drag and drop interface vs. Baseline tool & 7.9701 & 0.0010053 & significant (p<0.01) \\ \hline
	Custom query builder vs. Baseline tool & 4.6238 & 0.0069276 & significant (p<0.01) \\ \hline    
     \end{tabular}
  }
  }
\vspace{-10pt}
\caption{Tukey's test on task completion time}
\label{tab:turkeytest}
\vspace{-10pt}
\end{table}
}

\begin{figure}
\begin{center}
\includegraphics[width=0.6\columnwidth]{figs/accuracyvstime.pdf}
\end{center}
\vspace{-25pt}
\caption{Accuracy over time results for zenvisage and baseline}
\label{fig:accuracyvstime}
\vspace{-20pt}
\end{figure}


\paraem{Finding 2: \zv helped retrieve 20\% and 35\% more accurate results than the baseline for drag and drop and custom query builder interfaces, respectively.} 
Comparing the participants' responses against the ground truth responses, 
we found that participants achieved the lowest accuracy with the baseline tool ($\mu=69.9\%$, $\sigma=13.3$). 
\techreport{Further, any tasks that required comparing multiple
pairs of visualizations or trends ended up having lower accuracy than those that looked
for a pattern, such as a peak or an increasing trend, in a single visualization.}
The low accuracy could be attributed to the fact that the participants selected suboptimal answers before browsing through the entire list of results for better answers. Conversely, \zv is able to
accept more fine-grained user input, and
rank output visualizations. With \zv,
participants were able to retrieve accurate answers
with less effort.
Between the two interfaces in \zv,
while the drag and drop interface had a faster task completion time,
it also had a lower accuracy ($\mu=85.3\%$, $\sigma=7.61$).
The custom query builder interface had the
highest accuracy ($\mu=96.3\%$, $\sigma=5.82$).
The accuracy was greater than the baseline by over 20\% (for drag and drop)
and over 35\% (for custom builder).
Finally, looking at both accuracy and task completion times together in Figure~\ref{fig:accuracyvstime}, we see that \zv \emph{helps in ``fast-forwarding to desired visualizations'' with high accuracy.} 

% In the baseline, comparing multiple pairs of visualizations or trends revealed to be more difficult than looking for a visual property, such as a peak, or an increasing pattern, in a single visualization. on the other hand, since \zv returns a ranked list of filtered answers based on the user specification, which allowed the participants to browse through a smaller number of visualizations compared to the baseline tool. Among the two interfaces in \zv, participants completed the tasks faster ($\mu=74s$, $\sigma=15.1$) on the drag and drop interface, but at the price of accuracy ($\mu=85.3\%$, $\sigma=7.61$). Participants using the custom query builder had the highest accuracy ($\mu=96.3\%$, $\sigma=5.82$) while maintaining comparable speeds to the drag and drop interface ($\mu=115s$, $\sigma=51.6$). Finally, looking at both accuracy and task completion times together (as depicted in Figure~\ref{fig:accuracyvstime}), we can conclude that \zv \textbf{helps in fast-forwarding to desired visualizations with a high accuracy.}

% Figure \ref{fig:accuracyvstime} depicts the average accuracy over time results of each of the participants on each of the interfaces. \agp{move this later.} 

%\textbf{\zv helps retrieve accurate results}: We rated the participant's answers based on the expert's gold set answers. The ratings revealed that participants performed poorly with the baseline, with the lowest accuracy ($\mu=69.9\%$, $\sigma=13.3$) and longest task completion time. In the baseline, comparing multiple pairs of trends or graphs revealed to be more difficult than looking for a single trend such as a peak, or an increasing pattern. \zv, on other hand, returns a ranked list of results based on the user specification, which allowed the participants to browse through a smaller number of visualizations compared to the baseline tool. Among the two interfaces in \zv, participants completed the tasks fastest ($\mu=74s$, $\sigma=15.1$) on the drag and drop interface, but at the price of accuracy ($\mu=85.3\%$, $\sigma=7.61$). Participants using the custom query builder had the highest accuracy ($\mu=96.3\%$, $\sigma=5.82$) while maintaining comparable speeds to the drag and drop interface ($\mu=115s$, $\sigma=51.6$). \textbf{\zv, thus, helps in fast-forwarding to desired visualizations with a high accuracy}.


\paraem{Finding 3: The drag and drop interface and the custom query builder complemented each other.
The drag and drop interface was intuitive, while the custom builder was useful for complex queries.} 
The majority of participants (8/12) 
mentioned that the drag and drop 
and custom query builder interfaces complemented each other \techreport{in making \zv powerful}
when searching for specific insights.\techreport{ 25 percent (3/12) of the participants (all with backgrounds in machine learning and data mining) 
preferred using only the custom query builder interface, while just one participant (with no prior experience with query languages or programming languages) found only the drag and drop interface as useful.}
Participants stated that they would use drag and drop for exploration and simple pattern search and custom query builder for specific / complex queries. One stated: \textit{``When I know what I am looking for is exact, I want to use the query table. The other one [drag and drop] is for exploration when you are not so sure.'' (P9).} 
Participants liked the simplicity and intuitiveness of the drag and drop interface. 
One stated: \textit{``[The drawing feature] is very easy and intuitive, I can draw... and automatically get the results.''} (P2).
On a five-point Likert (5 is strongly agree), participants
found the drawing feature easy to use ($\mu=4.45$, $\sigma=0.674$). 
Despite the positive feedback, participants did identify limitations,
specifically, that the functionality was restricted to identifying trends
similar to a single hand-drawn trend.

The majority of the participants (11/12) 
stated that the custom query builder 
allowed them to search for complex insights that might be 
difficult to answer via drag and drop. 
When asked if the custom query builder was difficult to use compared to
the drag-and-drop interface, participants tended to agree ($\mu=3.73$, $\sigma=0.866$ on a five-point Likert scale where five is strongly agree).
At the same time, participants acknowledged 
the flexibility and the efficacy supported by the custom query builder interface. 
One participant explicitly stated why they 
preferred the custom query builder over the drag and drop interface: 
\textit{``When the query is very complicated, [the drag and drop] has its limitations, 
so I think I will use the query table most of the times unless I want to get a brief impression.''} (P6).
Another participant stated that the custom query builder interface \textit{``has more functionality and it lets me express what I want to do clearly more than the sketch''} (P4). This was consistent with other responses. 
Participants with a background in machine learning, 
data mining, and statistics (3/12) preferred
using the custom query builder over the drag and drop interface.

\paraem{Finding 4: \zv was more effective (4.27 vs. 2.67 on a five-point Likert scale)
than the baseline tool at visual data exploration, and would be
a valuable addition to the participants' analytics workflow.} 
In response to the survey question \emph{``I found the tool to be effective in visualizing the data I want to see''}, the participants rated \zv (the drag and drop interface and the custom query builder interface) higher ($\mu=4.27$, $\sigma=0.452$) than the baseline tool ($\mu=2.67$, $\sigma=0.890$) on a five-point Likert scale.
A participant experienced in Tableau commented: \textit{``In Tableau, there is no pattern searching. If I 
see some pattern in Tableau, such as a decreasing pattern, and I want to see if any other variable is 
decreasing in that month, I have to go one by one to find this trend. But here I can find this through the query table.''} (P10).

\paraem{Finding 5: \zv is a valuable addition to the participants' analytics workflow, and allows a quicker initial data exploration before performing complex analysis:}
When asked about using the two tools in their current workflow, 9 of the 12 participants stated that they would use \zv in their workflow, whereas two participants stated that they would use our baseline tool ($\chi^2=8.22$, p<0.01). When the participants were asked how they would use \zv in their workflow, one participant provided a specific scenario: \textit{``If I am doing my social science study, and I want to see some specific behavior among users, then I can use tool A [\zv] since I can find the trend I am looking for and easily see what users fit into the pattern.''} (P7). Other participants mentioned that they would use this tool for finding outliers during data cleaning, common patterns search, and initial understanding of data distributions before running a machine learning task. 
Participants could not articulate specific reasons for using the baseline tool. As one participant put it, \textit{``the existing solutions can already do what tool B [the baseline interface] can do.''} (P10).
Even those with considerable experience with programming languages such as Python and Matlab 
argued that \zv would take less time and fewer lines of code for basic data exploration tasks. 
Participants (2/12) who had considerable experience with data mining libraries were asked a follow-up 
question to write code for a task similar to Table 11 in their favorite language;
this task took them multiple orders of magnitudes more time and lines of code compared to \zq. 
\papertext{Example code can be found in~\cite{techreport}.} \techreport{Example code can be found in the appendix \ref{sec:userstudy-appendix}.} 



% \textbf{\zv is novel with real world applications}: All the participants described \zv as a novel tool and mentioned that they have not seen the declarative pattern searching functionality in any other tool.

\paraem{Finding 6: \zv can be improved.}  
\papertext{Participants also outlined some areas for improvement; details can be found in~\cite{techreport}.
In brief, the participants requested drag-and-drop interactions to support additional operations, such as outlier finding.
Others commented on how the interface could be more polished, and suggested that we add bookmarking and search history capabilities.}
\techreport{
 While the participants looked forward to using custom query builder in their own workflow, a few of them were interested in directly exposing the commonly-used trends/patterns such as outliers, through the drag and drop interface. Some were interested in knowing how they could integrate custom functional primitives (we could not cover it in the tutorial due to time constraints). In order to improve the user experience, participants suggested adding instructions and guidance for new users as part of the interface. Participants also commented on the unrefined look and feel of the tool, as well as the lack of a diverse set of usability related features, such as bookmarking and search history, that are offered in existing systems.
}





==> docs copy/viz-exp-operators.tex <==
%!TEX root=zenvisageql.tex

\subsection{\VzAlg Operators}
\label{sec:viz-exp-oper}

Similar to how operators in
ordered bag algebra operate on and result in ordered bags, 
operators in \vzalg operate on and result in \vzgrps. 
Many of the symbols for operators in \vzalg are also derived from
relational algebra, with some differences. 
To differentiate, operators in \vzalg are superscripted
with a $v$ (e.g., $\vzsel$, $\vzsort$).
The unary operators for \vzalg include 
\begin{inparaenum}[\itshape (i)\upshape]
\item $\vzsel$ for selection, \item $\vzsort$ for
sorting a \vzgrp based on the trend-estimating function $T$, \item $\vzlimit$ for
limiting the number of \vzchns in a \vzgrp, and \item $\vzdedup$ for duplicate \vzchn removal.
\end{inparaenum}. 
The binary operators include 
\begin{inparaenum}[\itshape (i)\upshape]
\item  $\vzunion$ for union, \item $\vzdiff$ for
difference, \item $\vzswap$ for replacing the attribute values of the \vzchns in one \vzgrp's with
another's, \item $\vzdist$ to reorder the first \vzgrp based on the \vzchns'
distances to the \vzchns of another \vzgrp based on metric $D$, and \item $\vzfind$
to reorder the \vzchns in a \vzgrp based on their distance to a reference
\vzchn from a singleton \vzgrp based on $D$. 
\end{inparaenum}
These operators are described below, and listed
in Table~\ref{tab:vizalgebopt}.

\begin{table*}[!t]
  \vspace{0pt}
\scriptsize
    \centering
\begin{tabular}{|c|l|l|p{5cm}|l|}      \hline
       Operator & Name & Derived from Bag Algebra  & Meaning & Unary/Binary \\ \hline \hline
       $\vzsel$ & Selection & Yes  & Subselects \vzchns & Unary \\ \hline
       $\vzsort$ & Sort & No & Sorts \vzchns in increasing order & Unary \\ \hline
       $\vzlimit$ & Limit & Yes & Returns first k \vzchns & Unary \\ \hline 
       $\vzdedup$ & Dedup & Yes  & Removes duplicate \vzchns & Unary \\ \hline 
       $\vzunion/\vzdiff/\vzint$ & Union/Diff/Int & Yes & Returns the union
  of/differences between/intersection of two \vzgrps & Binary \\ \hline 
       $\vzswap$ & Swap & No & Returns a \vzgrp in which values of an attribute in  one \vzgrp is  replaced  with values of the same attribute in another \vzgrp & Binary \\ \hline 
       $\vzdist$ & Dist & No & Sorts a \vzgrp based on pairwise distance to another \vzgrp  & Binary \\ \hline 	
       $\vzfind$ & Find & No & Sorts a \vzgrp in increasing order based on their distances to a single reference \vzchn & Binary \\ \hline  
   \end{tabular}
   \caption{Visual Exploration Algebra Operators}
  \label{tab:vizalgebopt}
\end{table*}




\subsubsection{Unary Operators.}
\paragraph{$\vzsel_{\theta}(V)$:}
$\vzsel$ selects a \vzgrp from $V$ based on selection criteria
$\theta$, like ordered bag algebra. 
However, $\vzsel$ has a
more restricted $\theta$; while $\vee$ and $\wedge$ may still be used, 
only the binary comparison operators $=$ and
$\ne$ are allowed. 
As an example, \\
$\vzsel_\theta (\calV)$ where $\theta = ($X=`year' $\land$ Y=`sales' $\land$ year=\wild $\land$ month=\wild $\land$ product $\ne$ \wild $\land$ location=`US' $\land$ sales=\wild $\land$ profit=\wild$)$ from Table~\ref{subtab:vzsel} 
on $\calV$ from
Table~\ref{tab:setup} would result in the \vzgrp of time 
vs. sales visualizations for different products in the US.
% \alkim{The reason we have this restriction is because \zq does not support the
%   other comparisons. Also, we would have to redefine the comparison operators
%   to handle the semantics for what happens with \wild, which seemed annoying
% and long to do.}

In this example, note that the product is
specifically set to not equal \wild so that the resulting \vzgrp will include
all products.
On the other hand, the location is explicitly set to be equal to US. 
The other attributes, e.g., sales, profit, year, month are set to equal \wild: 
this implies that the visual groups are not employing any additional constraints
on those attributes. 
(This may be useful, for example when those attributes are not
relevant for the current visualization or set of visualizations.)
As mentioned before, \vzgrps have the semantics of ordered bags. Thus, $\vzsel$
operates on one tuple at a time in the order they appear in
$V$, and the result is in the same order the tuples are operated on. 

\paragraph{$\vzsort_{F(T)}(V)$:}
$\vzsort$ returns the \vzgrp sorted in an increasing order based on applying $F(T)$ on
each \vzchn in $V$, where $F(T)$ is a procedure that uses  
function $T$.  For example, $\vzsort_{-T}(V)$ might return the
visualizations in $V$ sorted in decreasing order of estimated slope.
This operator is not present in the ordered bag semantics,
but may be relevant when we want to reorder the ordered bag using a different criterion.
The function $F$ may be any higher-order function with no side effects. For a language to
\vzcmp, the language must be able to support any arbitrary $F$.

\paragraph{$\vzlimit_{k}(V)$:}
$\vzlimit$ returns the first $k$ \vzchns of $V$ ordered in the same way they
were in $V$. $\vzlimit$ is equivalent to the \texttt{LIMIT} statement in \sql.
$\vzlimit$ is often used in conjunction with $\vzsort$ to retrieve the top-$k$
visualizations with greatest increasing trends (e.g. $\vzlimit_{k}(\vzsort_{-T}(V))$).
When instead of a number $k$, the subscript to $\vzlimit$ is actually $[a: b]$, 
then the items of $V$ that are between
positions $a$ and $b$ in $V$ are returned.
Thus $\vzlimit$ offers identical functionality to the $[a:b]$ in ordered bag algebra,
with the convenient functionality of getting the top $k$ results by just having
one number as the subscript.
Instead of using $\vzlimit$, \vzalg also supports the use
of the syntax $V[i]$ to refer to the $i$th \vzchn in $V$, and 
$V[a:b]$ to refer to the ordered bag of \vzchns from positions $a$ to $b$.

\paragraph{$\vzdedup(V):$}
$\vzdedup$ returns the \vzchns in $V$ with the duplicates removed, in the order
of their first appearance.
Thus, $\vzdedup$ is defined identically to ordered bag algebra.

\subsubsection{Binary Operators.}
\paragraph{$V \vzunion U$ | $V \vzdiff U$ | $V \vzint U$:}
Returns the union / difference / intersection of $V$ and $U$.
These operations are just like the corresponding operations in
ordered bag algebra.


\paragraph{$\vzswap_{A}(V, U)$:}
$\vzswap$ returns a \vzgrp in which values of attribute
$A$ in $V$ are replaced with
the values of $A$ in $U$. 
Formally, assuming $A_i$ is the $i$th attribute of $V$
and $V$ has $n$ total attributes:
$\vzswap_{A_i}(V, U) = \pi_{A_1,\dots, A_{i-1}, A_{i+1}, \dots, A_{n}}(V) \times \pi_{A_i}(U)$. This can be useful for when the user would like to change
an axis: $\beta_{\text{X}}(V, \vzsel_{\text{X=year}}(\calV))$ will change the \vzchns in $V$
to have year as their x-axis. $\vzswap$ can also be used to combine multiple
dimensions as well. If we assume that $V$ has multiple Y values, we can do
$\vzswap_{\text{X}}(V, \vzsel_{\text{X}\ne*}(\calV))$ to have the \vzchns in
$V$ vary over both X and Y.
\techreport{This operator allows us to start with a set of visualizations and then ``pivot''
to focus on a different attribute, e.g., start with sales over time
visualizations and pivot to look at profit. 
Thus, the operator allows us to transform the space of \vzchns.}


\paragraph{$\vzdist_{F(D),A_1,...,A_j}(V, U)$:}
$\vzdist$ sorts the \vzchns in $V$ in increasing order based on their
distances to the corresponding \vzchns in $U$. More specifically, $\vzdist$
computes $F(D)(\vzsel_{A_1=a_1 \land ... \land A_j=a_j}(V),\\ \vzsel_{A_1=a_1
  \land ... \land A_j=a_j}(U)) \forall a_1,...,a_j \in
  \pi_{A_1,...,A_j}(V)$ and returns an increasingly sorted $V$ based on the
  results. If $\vzsel_{A_1=a_1 \land ... \land A_j=a_j}$ for either $V$ or $U$
  ever returns a non-singleton \vzgrp for any tuple
  $(a_1,...,a_j)$, the result of the operator is undefined.

\paragraph{$\vzfind_{F(D)}(V, U)$:}
$\vzfind$ sorts the \vzchns in $V$ in increasing order based on their distances
to a single reference \vzchn in singleton \vzgrp $U$. 
Thus, $U = [t]$.
$\vzfind$ computes $F(D)(V[i],
U[1]) \quad$ $\forall i \in \{1,\dots,|V|\}$, and returns a reordered $V$ based
on these values, where $F(D)$ is a procedure that uses $D$. 
If $U$ has
more than one \vzchn, the operation is undefined. 
$\vzfind$ is useful for
queries in which the user would like to find the top-$k$ most similar
visualizations to a reference: $\vzlimit_{k}(\vzfind_{D}(V,U))$,
where $V$ is the set of candidates and $U$ contains the reference.
Once again, this operator is similar to $\vzsort$, except that
it operates on the results of the comparison of individual \vzchns to a specific \vzchn.

\begin{table}[!]
  \scriptsize
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
      \hline
      X & Y & year & month & product & location & sales & profit \\ \hline
      year & sales & \wild & \wild & chair & US & \wild & \wild \\ \hline
      year & sales & \wild & \wild & table & US & \wild & \wild \\ \hline
      year & sales & \wild & \wild & stapler & US & \wild & \wild \\ \hline
      year & sales & \wild & \wild & printer & US & \wild & \wild \\
      \multicolumn{8}{|c|}{\vdots} \\
    \end{tabular}
  \caption{Results of performing unary operators on $\calV$ from Table~\ref{tab:setup}: $\vzsel_\theta (\calV)$ where $\theta = ($X=`year' $\land$ Y=`sales' $\land$ year=\wild $\land$ month=\wild $\land$ product $\ne$ \wild $\land$location=`US' $\land$ sales=\wild $\land$ profit=\wild$)$}.
  \label{tab:viz-un-opers}    \label{subtab:vzsel}
  \vspace{-10pt}
\end{table}



==> docs copy/viz-exp-proof.tex <==
%!TEX root=zenvisageql.tex

\subsection{Proof of \VzCmpness}
\label{subsec:viz-exp-proof}
We now attempt to quantify the expressiveness of \zq within the context of
\vzalg and the two functional primtives $T$ and $D$.
More
formally, we prove the following theorem:

\vspace{-7pt}
\begin{framed}
  \vspace{-12pt}
  \begin{theorem}
    Given well-defined functional primitives $T$ and $D$, \zq is \vzcmp
    with respect to $T$ and $D$: $VEC_{T,D}(\text{\zq})$ is true.
    \label{thm:main}
  \end{theorem}
  \vspace{-12pt}
\end{framed}
\vspace{-7pt}

% \papertext{
%   Although we omit the full proof here due to lack of space, the basic idea of
%   the proof is that the visualization collections in \zq are equivalent in expressive
%   power as \vzgrps in \vzalg and for each operator in \vzalg, there is a \zq
%   query that appropriately transforms the corresponding visualization collections.
%   For more details, see the extended technical report~\cite{techrepoort}.
% }


Our proof for this theorem involves two major steps:
\begin{description}
  \item[Step 1.] We show that a visualization collection in \zq has as much
    expressive power as a \vzgrp of \vzalg, and therefore a visualization
    collection in
    \zq serves as an appropriate proxy of a \vzgrp in \vzalg.
  \item[Step 2.] For each operator in \vzalg, we show that there exists a \zq
    query which takes in visualization collection semantically equivalent to the
    \vzgrp operands and produces visualization collection semantically equivalent to
    the resultant \vzgrp.
\end{description}

\begin{lemma}
  A visualization collection of \zq has at least as much expressive power as a
  \vzgrp in \vzalg.
  \label{lemma:1}
\end{lemma}
\begin{proof}
  A \vzgrp $V$, with $n$ \vzchns, is a relation with $k+2$ columns and $n$
  rows, where $k$ is the number of attributes in the original relation. We show
  that for any \vzgrp $V$, we can come up with a \zq query $q$ which can
  produce a visualization collection that represents the same set of visualizations as
  $V$.
  
  \begin{table}[H]
    \centering\scriptsize
    {\tt   
      \begin{tabular}{|r|l|l|l|l|l|} \hline
        \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Z1} & \textbf{...}
        & \textbf{Zk} \\ \hline
        f1 & $\pi_{\text{X}}(V[1])$ & $\pi_{\text{Y}}(V[1])$ & $E_{1,1}$ & ... &
        $E_{1,k}$ \\
        \vdots & \vdots & \vdots & \vdots & \vdots & \vdots \\
        fn & $\pi_{\text{X}}(V[n])$ & $\pi_{\text{Y}}(V[n])$ & $E_{n,1}$ & ... &
        $E_{n,k}$ \\
        *fn+1 \IN f1+...+fn & & & & & \\
        \hline
      \end{tabular}
    }
    \vspace{-10pt}\caption{\zq query $q$ which produces a visualization collection
    equal in expressiveness to \vzgrp $V$.}
    \label{tab:lemma-1}
  \vspace{-10pt}\end{table}

  Query $q$ has the format given by Table~\ref{tab:lemma-1}, where $V[i]$
  denotes the $i$th tuple of relation $V$ and:
  \[
    E_{i,j} = 
    \begin{cases}
      \text{`` ''} & \text{if } \pi_{A_j}(V[i]) = * \\
      A_j.\pi_{A_j}(V[i]) & \text{otherwise}
    \end{cases}
  \]
  Here, $A_j$ refers to the $j$th attribute of the original relation. The
  $i$th \vzchn of $V$ is represented with the {\tt fi} from $q$. The X and Y
  values come directly from the \vzchn using projection. For the {\tt Zj}
  column, if the $A_j$ attribute of \vzchn has any value than other
  than \wild, we must filter the data based on that value, so $E_{i,j} =
  A_j.\pi_{A_j}{V[i]}$. However, if the $A_j$ attribute is equal to
  \wild, then the corresponding element in {\tt fi} is left blank, signaling no
  filtering based on that attribute.

  After, we have defined a visualization collection {\tt fi} for each $i$th \vzchn in
  $V$, we take the sum (or concatenation) across all these visualization collections as
  defined in Appendix \ref{name-appex}, and the resulting
  {\tt fn+1} becomes equal to the \vzgrp $V$.
\end{proof}

\begin{lemma}
  $\vzsel_{\theta}(V)$ is expressible in \zq for all valid constraints $\theta$
  and \vzgrps $V$.
\end{lemma}
\begin{proof}
  We prove this by induction.
  
  The full context-free grammar (CFG) for $\theta$ in
  $\vzsel_{\theta}$ can be given by:
  \begin{flalign}
    \theta &\rightarrow E \;|\; E \land E \;|\; E \lor E \;|\; \epsilon &\\
    E &\rightarrow C \;|\; (E) \;|\; E \land C \;|\; E \lor C & \label{cfg:e}\\
    C &\rightarrow T_1 = B_1 \;|\; T_1 \ne B_1 \;|\; T_2 = B_2 \;|\; T_2 \ne
    B_2 &\\
    T_1 &\rightarrow X \;|\; Y &\\
    B_1 &\rightarrow A_1 \;|\; ... \;|\; A_k &\\
    T_2 &\rightarrow A_1 \;|\; ... \;|\; A_k &\\
    B_2 &\rightarrow \text{string} \;|\; \text{number} \;|\; *
  \end{flalign}
  where $\epsilon$ represents an empty string (no selection), and $X$, $Y$,
  and $A_1$, ..., $A_k$ refer to the attributes of $\calV$.

  To begin the proof by induction,
  we first show that \zq is capable of expressing the base expressions
  $\vzsel_{C}(V)$:
  $\vzsel_{T_1 = B_1}(V)$,
  $\vzsel_{T_1 \ne B_1}(V)$,
  $\vzsel_{T_2 = B_2}(V)$, and
  $\vzsel_{T_2 \ne B_2}(V)$.
  The high level idea for each of these proofs is to be come up with a
  \emph{filtering \vzgrp} $U$ which we take the intersection with to arrive at
  our desired result: $\exists U, \vzsel_{C}(V) = V \vzint U$.

  In the first two expressions, $T_1$ and $B_1$ refer to filters on the $X$ and
  $Y$ attributes of $V$; we
  have the option of either selecting a specific attribute ($T_1=B_1$) or
  excluding a specific attribute ($T_1 \ne B_1$). Tables \ref{tab:vzsel-c1} and
  \ref{tab:vzsel-c2} show \zq queries which express $\vzsel_{T_1=B_1}(V)$ for
  $T_1 \rightarrow X$ and $T_1 \rightarrow Y$ respectively. The \zq queries
  do the approximate equivalent of $\vzsel_{T_1=B_1}(V) = V \vzint
  \vzsel_{T_1=B_1}(\calV)$.

  \begin{table}[H]
    \centering\scriptsize
    {\tt   
      \begin{tabular}{|r|l|l|l|l|l|} \hline
        \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Z1} & \textbf{...}
        & \textbf{Zk} \\ \hline
        f1 & - & - & - & ... & - \\
        f2 \IN f1 & & y1 \IN \_ & v1 \IN $A_1$.\_ & ... & vk \IN $A_k$.\_ \\
        f3 & $B_1$ & y1 & v1 & ... & vk \\
        *f4 \IN f1\^{}f3 & & & & & \\
        \hline
      \end{tabular}
    }
    \vspace{-10pt}\caption{\zq query which expresses $\vzsel_{X=B_1}(V)$.}
    \label{tab:vzsel-c1}
  \vspace{-10pt}\end{table}

  \begin{table}[H]
    \centering\scriptsize
    {\tt   
      \begin{tabular}{|r|l|l|l|l|l|} \hline
        \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Z1} & \textbf{...}
        & \textbf{Zk} \\ \hline
        f1 & - & - & - & ... & - \\
        f2 \IN f1 & x1 \IN \_ & & v1 \IN $A_1$.\_ & ... & vk \IN $A_k$.\_ \\
        f3 & x1 & $B_1$ & v1 & ... & vk \\
        *f4 \IN f1\^{}f3 & & & & & \\
        \hline
      \end{tabular}
    }
    \vspace{-10pt}\caption{\zq query which expresses $\vzsel_{Y=B_1}(V)$.}
    \label{tab:vzsel-c2}
  \vspace{-10pt}\end{table}

  We have
  shown with Lemma~\ref{lemma:1} that a visualization collection is capable of
  expressing a \vzgrp, so we assume that {\tt f1}, the
  visualization collection which represents the operand $V$, is given to us for both of
  these tables. Since we
  do not know how {\tt f1} was derived, we use - for its axis variable columns.
  The second rows of these tables derive {\tt f2} from {\tt f1} and bind axis
  variables to the values of the non-filtered attributes. Here, although the
  set of visualizations present in {\tt f2} is exactly the same as {\tt f1},
  we now have a convenient way to iterate over the non-filtered attributes of
  {\tt f1} (for more information on derived visualization collections, please refer to
  Appendix~\ref{name-appex}).
  The third row
  combines the specified attribute $B_1$ with the non-filtered attributes of
  {\tt f2} to form the \emph{filtering visualization collection} {\tt f3}, which
  expresses the filtering \vzgrp $U$ from above. We then take the
  intersection between {\tt f1} and the filtering visualization collection {\tt f3} to
  arrive at our desired visualization collection {\tt f4}, which represents
  the resultant \vzgrp $\vzsel_{T_1=B_1}(V)$. Although, we earlier said that we
  would come up with {\tt f3} $=\vzsel_{T_1=B_1}(\calV)$, in truth, we come up
  with {\tt f3} $=B_1 \times \pi_{Y,A_1,...,A_k}(V)$ for $T_1 \rightarrow X$
  and {\tt f3} $=\pi_{X,A_1,...,A_k}(V) \times B_1$ for $T_1 \rightarrow Y$
  because they are easier to express in \zq; regardless we still end up with
  the correct resulting set of visualizations.

  Tables \ref{tab:vzsel-c3} and \ref{tab:vzsel-c4} show \zq queries which
  express $\vzsel_{T_1 \ne B_1}(V)$ for $T_1 \rightarrow X$ and $T_1
  \rightarrow Y$ respectively. Similar to the queries above, these queries
  perform the approximate
  equivalent of $\vzsel_{T_1 \ne B_1}(V) = V \vzint \vzsel_{T_1 \ne
  B_1}(\calV)$. We once again assume {\tt f1} is a given visualization collection which
  represents the operand $V$, and we come up with a filtering visualization collection
  {\tt f3} which mimics the effects of (though is not completely equivalent to) $\vzsel_{T_1
    \ne B_1}(\calV)$. We then take the intersection between {\tt f1} and {\tt
    f3} to arrive at {\tt f4} which represents the resulting $\vzsel_{T_1 \ne
    B_1}(V)$.

  \begin{table*}[!htbp]
    \centering\scriptsize
    {\tt   
      \begin{tabular}{|r|l|l|l|l|l|} \hline
        \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Z1} & \textbf{...}
        & \textbf{Zk} \\ \hline
        f1 & - & - & - & ... & - \\
        f2 \IN f1 & x1 \IN \_ & y1 \IN \_ & v1 \IN $A_1$.\_ & ... & vk \IN $A_k$.\_ \\
        f3 & x2 \IN x1 - \{$B_1$\} & y1 & v1 & ... & vk \\
        *f4 \IN f1\^{}f3 & & & & & \\
        \hline
      \end{tabular}
    }
    \vspace{-10pt}\caption{\zq query which expresses $\vzsel_{X \ne B_1}(V)$.}
    \label{tab:vzsel-c3}
  \vspace{-10pt}\end{table*}

  \begin{table*}[!htbp]
    \centering\scriptsize
    {\tt   
      \begin{tabular}{|r|l|l|l|l|l|} \hline
        \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Z1} & \textbf{...}
        & \textbf{Zk} \\ \hline
        f1 & - & - & - & ... & - \\
        f2 \IN f1 & x1 \IN \_ & y1 \IN \_ & v1 \IN $A_1$.\_ & ... & vk \IN $A_k$.\_ \\
        f3 & x1 & y2 \IN y1 - \{$B_1$\} & v1 & ... & vk \\
        *f4 \IN f1\^{}f3 & & & & & \\
        \hline
      \end{tabular}
    }
    \vspace{-10pt}\caption{\zq query which expresses $\vzsel_{Y \ne B_1}(V)$.}
    \label{tab:vzsel-c4}
  \vspace{-10pt}\end{table*}

  The expressions $\vzsel_{T_2=B_2}$ and $\vzsel_{T_2 \ne B_2}$ refer to filters on the
  $A_1,...,A_k$ attributes of $V$. Specifically, $T_2$ is some attribute $A_j
  \in \{A_1,...,A_k\}$ and $B_2$ is the attribute value which is selected or
  excluded.
  Here, we have an additional complication to the proof since any attribute
  $A_j$ can also filter for or exclude \wild. First, we
  show \zq is capable of expressing $\vzsel_{T_2 = B_2'}$ and $\vzsel_{T_2
  \ne B_2'}$ for which $B_2' \neq *$; that is $B_2'$ is any attribute
  value which is not \wild. Tables \ref{tab:vzsel-c5} and \ref{tab:vzsel-c6}
  show the \zq queries which express $\vzsel_{T_2 = B_2'}(V)$ and $\vzsel_{T_2
  \ne B_2'}(V)$ respectively. Note the similarity between these queries and the
  queries for $\vzsel_{T_1=B_1}(V)$ and $\vzsel_{T_1 \ne B_1}(V)$.

  \begin{table*}[!htbp]
    \centering\scriptsize
    {\tt   
      \begin{tabular}{|r|l|l|l|l|l|l|l|} \hline
        \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Z1} & \textbf{...} &
        \textbf{Zj} & \textbf{...} & \textbf{Zk} \\ \hline
        f1 & - & - & - & ... & - & ... & - \\
        f2 \IN f1 & x1 \IN \_ & y1 \IN \_ & v1 \IN $A_1$.\_ & ... & & ... & vk \IN $A_k$.\_ \\
        f3 & x1 & y1 & v1 & ... & $B_2'$ & ... & vk \\
        *f4 \IN f1\^{}f3 & & & & & & & \\
        \hline
      \end{tabular}
    }
    \vspace{-10pt}\caption{\zq query which expresses $\vzsel_{A_j =  B_2'}(V)$
    when $B_2' \ne *$.}
    \label{tab:vzsel-c5}
  \vspace{-10pt}\end{table*}

  \begin{table*}[!htbp]
    \centering\scriptsize
    {\tt   
      \begin{tabular}{|r|l|l|l|l|l|l|l|} \hline
        \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Z1} & \textbf{...} &
        \textbf{Zj} & \textbf{...} & \textbf{Zk} \\ \hline
        f1 & - & - & - & ... & - & ... & - \\
        f2 \IN f1 & x1 \IN \_ & y1 \IN \_ & v1 \IN $A_1$.\_ & ... & vj \IN $A_j$.\_ & ... & vk \IN $A_k$.\_ \\
        f3 & x1 & y1 & v1 & ... & uj \IN vj - \{$B_2'$\} & ... & vk \\
        *f4 \IN f1\^{}f3 & & & & & & & \\
        \hline
      \end{tabular}
    }
    \vspace{-10pt}\caption{\zq query which expresses $\vzsel_{A_j \ne
    B_2'}(V)$ when $B_2' \ne *$.}
    \label{tab:vzsel-c6}
  \vspace{-10pt}\end{table*}

  For $\vzsel_{T_2=*}(V)$ and $\vzsel_{T_2 \ne *}(V)$, Tables
  \ref{tab:vzsel-c7} and \ref{tab:vzsel-c8} show the corresponding queries. In
  Table~\ref{tab:vzsel-c7}, we explicitly avoid setting a value for {\tt Zj}
  for {\tt f3} to emulate $A_j=*$ for the filtering visualization collection. In
  Table~\ref{tab:vzsel-c8}, {\tt f3}'s {\tt Zj} takes on all possible values
  from $A_j${\tt.*}, but that means that a value is set for {\tt Zj} (i.e.,
  $T_2 \ne *$).

  \begin{table*}[!htbp]
    \centering\scriptsize
    {\tt   
      \begin{tabular}{|r|l|l|l|l|l|l|l|} \hline
        \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Z1} & \textbf{...} &
        \textbf{Zj} & \textbf{...} & \textbf{Zk} \\ \hline
        f1 & - & - & - & ... & - & ... & - \\
        f2 \IN f1 & x1 \IN \_ & y1 \IN \_ & v1 \IN $A_1$.\_ & ... & & ... & vk \IN $A_k$.\_ \\
        f3 & x1 & y1 & v1 & ... & & ... & vk \\
        *f4 \IN f1\^{}f3 & & & & & & & \\
        \hline
      \end{tabular}
    }
    \vspace{-10pt}\caption{\zq query which expresses $\vzsel_{A_j = *}(V)$.}
    \label{tab:vzsel-c7}
  \vspace{-10pt}\end{table*}

  \begin{table*}[!htbp]
    \centering\scriptsize
    {\tt   
      \begin{tabular}{|r|l|l|l|l|l|l|l|} \hline
        \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Z1} & \textbf{...} &
        \textbf{Zj} & \textbf{...} & \textbf{Zk} \\ \hline
        f1 & - & - & - & ... & - & ... & - \\
        f2 \IN f1 & x1 \IN \_ & y1 \IN \_ & v1 \IN $A_1$.\_ & ... & & ... & vk \IN $A_k$.\_ \\
        f3 & x1 & y1 & v1 & ... & vj \IN $A_j$.* & ... & vk \\
        *f4 \IN f1\^{}f3 & & & & & & & \\
        \hline
      \end{tabular}
    }
    \vspace{-10pt}\caption{\zq query which expresses $\vzsel_{A_j \ne *}(V)$.}
    \label{tab:vzsel-c8}
  \vspace{-10pt}\end{table*}

  Now that we have shown how to express the base operations, we next assume \zq
  is capable of expressing any arbitrary complex filtering operations
  $\vzsel_{E'}$ where $E'$ comes from Line~\ref{cfg:e} of the CFG.
  Specifically, we assume that given a visualization collection {\tt f1} which
  expresses $V$, there exists a filtering visualization collection {\tt f2} for which
  $\vzsel_{E'}(V)=$ {\tt f1\^{}f2}. Given this assumption, we now must take the
  inductive step, apply Line~\ref{cfg:e}, and prove that $\vzsel_{E \rightarrow (E')}(V)$,
  $\vzsel_{E \rightarrow E' \land C}(V)$, and $\vzsel_{E \rightarrow E' \lor
  C}(V)$ are all expressible in
  \zq for any base constraint $C$.

  %\begin{enumerate}
  %  \item
  %    $\vzsel_{E \rightarrow (E')}(V)$ is trivial. Given {\tt f1} which
  %    represents $V$ and {\tt f2} which is the filtering visualization collection for
  %    $E'$, we simply the intersect the two to get {\tt f4 \IN f1\^{}f2} which
  %    represents $\vzsel_{E \rightarrow (E')}$.
  %\end{enumerate}
  \paragraph{$\vzsel_{E \rightarrow (E')}(V)$:} This case is trivial. Given
  {\tt f1} which represents $V$ and {\tt f2} which is the filtering
  visualization
  collection for $E'$, we simply the intersect the two to get {\tt f3 \IN f1\^{}f2}
  which represents $\vzsel_{E \rightarrow (E')}$.

  \paragraph{$\vzsel_{E \rightarrow E' \land C}$:} Once again assume we are
  given {\tt f1} which represents $V$ and {\tt f2} which is the filtering
  visualization collection of $E'$. Based on the base expression proofs above, we know
  that given any base constraint $C$, we can find a filtering visualization collection
  for it; call this filtering visualization collection {\tt f3}. We can then see that
  {\tt f2\^{}f3} is the filtering visualization collection of $E \rightarrow E' \land C$, and {\tt
  f4 \IN f1\^{}(f2\^{}f3)} represents $\vzsel_{E \rightarrow E \land C}(V)$.

  \paragraph{$\vzsel_{E \rightarrow E' \lor C}$:} Once again assume we are
  given {\tt f1} which represents $V$, {\tt f2} which is the filtering
  visualization collection of $E'$, and we can find a filtering visualization collection {\tt
  f3} for $C$.  We can then see that {\tt f2+f3} is the filtering visualization
  collection of $E \rightarrow E' \lor C$, and {\tt f4 \IN f1\^{}(f2+f3)} represents $\vzsel_{E
  \rightarrow E \lor C}(V)$.

  With this inductive step, we have shown that for all complex constraints $E$
  of the form given by Line~\ref{cfg:e} of the CFG, we can find a \zq query
  which expresses $\vzsel_{E}(V)$. Given this, we can finally show that \zq is capable
  of expressing $\vzsel_{\theta}(V)$ for all $\theta$: $\vzsel_{\theta \rightarrow E}(V)$,
  $\vzsel_{\theta \rightarrow E \land E')}(V)$,
  $\vzsel_{\theta \rightarrow E \lor E'}(V)$, and
  $\vzsel_{\theta \rightarrow \epsilon}(V)$.

  \paragraph{$\vzsel_{\theta \rightarrow E}(V)$:} This case is once again
  trivial. Assume, we are given {\tt f1} which represents $V$, and {\tt f2},
  which is the filtering visualization collection of $E$, {\tt f3 \IN f1\^{}f2} represents
  $\vzsel_{\theta \rightarrow E}(V)$.

  \paragraph{$\vzsel_{\theta \rightarrow E \land E'}(V)$:} Assume, we are given
  {\tt f1} which represents $V$, {\tt f2}, which is the filtering visualization collection of
  $E$, and {\tt f3}, which is the filtering visualization collection of $E'$.
  {\tt f2\^{}f3} is the filtering visualization collection of $\theta \rightarrow E
  \land E'$, and {\tt f4 \IN f1\^{}(f2\^{}f3)} represents $\vzsel_{\theta
  \rightarrow E \land E'}(V)$.

  \paragraph{$\vzsel_{\theta \rightarrow E \lor E'}(V)$:} Assume, we are given
  {\tt f1} which represents $V$, {\tt f2} which is the filtering visualization collection of
  $E$, and {\tt f3} which is the filtering visualization collection of $E'$.
  {\tt f2+f3} is the filtering visualization collection of $\theta \rightarrow E
  \lor E'$, and {\tt f4 \IN f1\^{}(f2+f3)} represents $\vzsel_{\theta
  \rightarrow E \lor E'}(V)$.

  \paragraph{$\vzsel_{\theta \rightarrow \epsilon}(V)$:} This is the case in
  which no filtering is done. Therefore, given {\tt f1} which represents $V$,
  we can simply return {\tt f1}.
\end{proof}

\begin{lemma}
  $\vzsort_{F(T)}(V)$ is expressible in \zq for all valid
  functionals $F$ of $T$ and \vzgrps $V$.
\end{lemma}
\begin{proof}
  \begin{table*}[!htbp]
    \centering\scriptsize
    {\tt   
      \begin{tabular}{|r|l|l|l|l|l|l|} \hline
        \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Z1} & \textbf{...}
        & \textbf{Zk} & \textbf{Process} \\ \hline
        f1 & - & - & - & ... & - & \\
        f2 \IN f1 & x1 \IN \_ & y1 \IN \_ & v1 \IN $A_1$.\_ & .. & vk \IN $A_k$.\_
        &
        x2, y2, u1, ..., uk \IN $argmin_{x1,y1,v1,...,vk}[k=\infty] F(T)(f2)$ \\
        *f3 & x2 & y2 & u1 & ... & uk & \\
        \hline
      \end{tabular}
    }
    \vspace{-10pt}\caption{\zq query $q$ which expresses $\vzsort_{F(T)}(V)$.
    }
    \label{tab:proof-vzsort}
  \vspace{-10pt}\end{table*}

  Assume {\tt f1} is the visualization collection which represents $V$. Query $q$
  given by Table~\ref{tab:proof-vzsort} produces visualization collection {\tt f3}
  which expresses $\vzsort_{F(T)}(V)$.
\end{proof}

\begin{lemma}
  $\vzlimit_{[a:b]}(V)$ is expressible in \zq for all valid intervals $a:b$
  and \vzgrps $V$.
\end{lemma}
\begin{proof}
  \begin{table*}[!htbp]
    \centering\scriptsize
    {\tt   
      \begin{tabular}{|r|l|l|l|l|l|l|} \hline
        \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Z1} & \textbf{...}
        & \textbf{Zk} & \textbf{Process} \\ \hline
        f1 & - & - & - & ... & - & \\
        *f2 \IN f1[a:b] &  & & & & & \\
        \hline
      \end{tabular}
    }
    \vspace{-10pt}\caption{\zq query $q$ which expresses $\vzlimit_{[a:b]}(V)$.
    }
    \label{tab:proof-vzlimit}
  \vspace{-10pt}\end{table*}

  Assume {\tt f1} is the visualization collection which represents $V$. Query $q$
  given by Table~\ref{tab:proof-vzlimit} produces visualization collection {\tt f2}
  which expresses $\vzlimit_{[a:b]}(V)$.
\end{proof}

%\begin{lemma}
%  $\vzrep_{R,j}(V)$ is expressible in \zq for all valid numbers $j$
%  and \vzgrps $V$.
%\end{lemma}
%\begin{proof}
%  \begin{table*}[!htbp]
%    \centering\scriptsize
%    {\tt   
%      \begin{tabular}{|r|l|l|l|l|l|l|} \hline
%        \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Z1} & \textbf{...}
%        & \textbf{Zk} & \textbf{Process} \\ \hline
%        f1 & - & - & - & ... & - & \\
%        f2 \IN f1 & x1 \IN \_ & y1 \IN \_ & v1 \IN $A_1$.\_ & ... & vk \IN $A_k$.\_
%        & 
%        x2, y2, u1, ..., uk \IN $R(j,x1,y1,v1,...,vk,f2)$ \\
%        *f3 & x2 & y2 & u1 & ... & uk & \\
%        \hline
%      \end{tabular}
%    }
%    \vspace{-10pt}\caption{\zq query $q$ which expresses $\vzrep_{R,j}(V)$.
%    }
%    \label{tab:proof-vzrep}
%  \vspace{-10pt}\end{table*}
%
%  Assume {\tt f1} is the visualization collection which represents $V$ and $R'$ is the
%  corresponding representative-finding algorithm in \zq. Query $q$
%  given by Table~\ref{tab:proof-vzrep} produces visualization collection {\tt f3}
%  which expresses $\vzlimit_{[a:b]}(V)$.
%\end{proof}

\begin{lemma}
  $\vzdedup(V)$ is expressible in \zq for all valid \vzgrps $V$.
\end{lemma}
\begin{proof}
  \begin{table*}[!htbp]
    \centering\scriptsize
    {\tt   
      \begin{tabular}{|r|l|l|l|l|l|l|} \hline
        \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Z1} & \textbf{...}
        & \textbf{Zk} & \textbf{Process} \\ \hline
        f1 & - & - & - & ... & - & \\
        *f2 \IN f1 &  & & & & & \\
        \hline
      \end{tabular}
    }
    \vspace{-10pt}\caption{\zq query $q$ which expresses $\vzdedup(V)$.
    }
    \label{tab:proof-vzdedup}
  \vspace{-10pt}\end{table*}

  Assume {\tt f1} is the visualization collection which represents $V$. Query $q$
  given by Table~\ref{tab:proof-vzdedup} produces visualization collection {\tt f2}
  which expresses $\vzdedup(V)$.
\end{proof}

\begin{lemma}
  $V \vzunion U$ is expressible in \zq for all valid \vzgrps $V$ and $U$.
\end{lemma}
\begin{proof}
  \begin{table*}[!htbp]
    \centering\scriptsize
    {\tt   
      \begin{tabular}{|r|l|l|l|l|l|l|} \hline
        \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Z1} & \textbf{...}
        & \textbf{Zk} & \textbf{Process} \\ \hline
        f1 & - & - & - & ... & - & \\
        f2 & - & - & - & ... & - & \\
        *f3 \IN f1+f2 & & & & ... & & \\
        \hline
      \end{tabular}
    }
    \vspace{-10pt}\caption{\zq query $q$ which expresses $V \vzunion U$.
    }
    \label{tab:proof-vzunion}
  \vspace{-10pt}\end{table*}

  Assume {\tt f1} is the visualization collection which represents $V$ and {\tt f2}
  represents $U$.  Query $q$ given by Table~\ref{tab:proof-vzunion} produces
  visualization collection {\tt f3} which expresses $V \vzunion U$.
\end{proof}

\begin{lemma}
  $V \vzdiff U$ is expressible in \zq for all valid \vzgrps $V$ and $U$.
\end{lemma}
\begin{proof}
  \begin{table*}[!htbp]
    \centering\scriptsize
    {\tt   
      \begin{tabular}{|r|l|l|l|l|l|l|} \hline
        \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Z1} & \textbf{...}
        & \textbf{Zk} & \textbf{Process} \\ \hline
        f1 & - & - & - & ... & - & \\
        f2 & - & - & - & ... & - & \\
        *f3 \IN f1-f2 & & & & ... & & \\
        \hline
      \end{tabular}
    }
    \vspace{-10pt}\caption{\zq query $q$ which expresses $V \vzdiff U$.
    }
    \label{tab:proof-vzdiff}
  \vspace{-10pt}\end{table*}

  Assume {\tt f1} is the visualization collection which represents $V$ and {\tt f2}
  represents $U$.  Query $q$ given by Table~\ref{tab:proof-vzdiff} produces
  visualization collection {\tt f3} which expresses $V \vzdiff U$. The proof for
  $\vzint$ can be shown similarly.
\end{proof}

\begin{lemma}
  $\vzswap_{A}(V, U)$ is expressible in \zq for all valid attributes $A$ in
  $\calV$ and \vzgrps $V$ and $U$.
\end{lemma}
\begin{proof}

  \begin{table*}[!htbp]
    \centering\scriptsize
    {\tt   
      \begin{tabular}{|r|l|l|l|l|l|} \hline
        \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Z1} & \textbf{...}
        & \textbf{Zk} \\ \hline
        f1 & - & - & - & ... & - \\
        f2 & - & - & - & ... & - \\
        f3 \IN f1 & & y1 \IN \_ & v1 \IN $A_1$.\_ & ... & vk \IN $A_k$.\_ \\
        f4 \IN f2 & x1 \IN \_ & & & & \\
        *f5 & x1$^2$ & y1$^1$ & v1$^1$ & ... & vk$^1$ \\
        \hline
      \end{tabular}
    }
    \vspace{-10pt}\caption{\zq query $q$ which expresses $\vzswap_{A}(V, U)$
      where $A=X$.
    }
    \label{tab:proof-vzswap1}
  \vspace{-10pt}\end{table*}

  \begin{table*}[!htbp]
    \centering\scriptsize
    {\tt   
      \begin{tabular}{|r|l|l|l|l|l|} \hline
        \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Z1} & \textbf{...}
        & \textbf{Zk} \\ \hline
        f1 & - & - & - & ... & - \\
        f2 & - & - & - & ... & - \\
        f3 \IN f1 & x1 \IN \_ & & v1 \IN $A_1$.\_ & ... & vk \IN $A_k$.\_ \\
        f4 \IN f2 & & y1 \IN \_ & & & \\
        *f5 & x1$^1$ & y1$^2$ & v1$^1$ & ... & vk$^1$ \\
        \hline
      \end{tabular}
    }
    \vspace{-10pt}\caption{\zq query $q$ which expresses $\vzswap_{A}(V, U)$
      where $A=Y$.
    }
    \label{tab:proof-vzswap2}
  \vspace{-10pt}\end{table*}

  \begin{table*}[!htbp]
    \centering\scriptsize
    {\tt   
      \begin{tabular}{|r|l|l|l|l|l|l|l|l|l|} \hline
        \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Z1} & \textbf{...}
        & \textbf{Zj-1} & \textbf{Zj} & \textbf{Zj+1} & \textbf{...}
        & \textbf{Zk} \\ \hline
        f1 & - & - & - & ... & - & - & - &... & - \\
        f2 & - & - & - & ... & - & - & - &... & - \\
        f3 \IN f1 & x1 \IN \_ & y1 \IN \_ & v1 \IN $A_1$.\_ & ... & vj-1 \IN
        $A_{j-1}$.\_ & & vj+1 \IN $A_{j+1}$.\_ & ... & vk \IN $A_k$.\_ \\
        f4 \IN f2 & & & & & & uj \IN $A_{j}$.\_ & & & \\
        *f5 & x1$^1$ & y1$^1$ & v1$^1$ & ... & vj-1$^1$ & uj$^2$ & vj+1$^1$ & ... & vk$^1$ \\
        \hline
      \end{tabular}
    }
    \vspace{-10pt}\caption{\zq query $q$ which expresses $\vzswap_{A}(V, U)$
      where $A=A_j$ and $A_j$ is an attribute from $\calR$
    }
    \label{tab:proof-vzswap3}
  \vspace{-10pt}\end{table*}

  Assume {\tt f1} is the visualization collection which represents $V$ and {\tt f2}
  represents $U$. There are three cases we must handle depending on the value
  of $A$ due to the structure of columns in \zq: \begin{inparaenum}[\itshape
    (i)\upshape] \item $A=X$ \item $A=Y$ \item $A=A_j$ where $A_j$ is an
  attribute from the original relation $\calR$ \end{inparaenum}. For each
  of the three cases, we produce a separate query which expresses $\vzswap$.
  For $A=X$, the query given by Table~\ref{tab:proof-vzswap1} produces {\tt f5}
  which is equivalent to $\vzswap_{X}(V,U)$ We use the superscripts 
  in the last row so that cross product conforms to the ordering defined in
  Section~\ref{sec:viz-exp-oper}. For more information about the superscripts,
  please refer to Appendix~\ref{name-appex}. For $A=Y$, the query given by
  Table~\ref{tab:proof-vzswap2} produces {\tt f5} which is equivalent to
  $\vzswap_{Y}(V,U)$, and for $A=A_j$, the query given by
  Table~\ref{tab:proof-vzswap3} produces {\tt f5} which is equivalent to
  $\vzswap_{A_j}(V,U)$.
  %Query $q$ given by Table~\ref{tab:proof-vzswap} produces
  %visualization collection {\tt f5} which expresses $\vzswap_{A_j}(V,U)$.
\end{proof}

\begin{lemma}
  $\vzdist_{F(D),A_1,...,A_j}(V, U)$ is expressible in \zq for all valid
  attributes $A_1,...,A_j$ and \vzgrps $V$ and $U$.
\end{lemma}
\begin{proof}

  \begin{table*}[!htbp]
    \centering\scriptsize
    {\tt   
      \begin{tabular}{|r|l|l|l|l|l|l|} \hline
        \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Z1} & \textbf{...} &
        \textbf{Zj} &
        \textbf{Process} \\ \hline
        f1 & - & - & - & ... & - & \\
        f2 & - & - & - & ... & - & \\
        f3 \IN f1 & & & v1 \IN $A_1$.\_ & ...  & vj \IN
        $A_j$.\_ & \\
        f4 \IN f2.order & & & v1 \TO & ... & vj \TO & u1, ..., uj \IN
        $argmin_{v1,...,vj}[k=\infty] F(D)(f3,f4)$\\
        *f5 \IN f1.order & & & u1 \TO & ... & uj \TO & \\
        \hline
      \end{tabular}
    }
    \vspace{-10pt}\caption{\zq query $q$ which expresses
      $\vzdist_{F(D),A_1,...,A_j}(V, U)$.
    }
    \label{tab:proof-vzdist}
    \vspace{-10pt}\end{table*}

  Assume {\tt f1} is the visualization collection which represents $V$, and {\tt f2}
  represents $U$. Without loss of generality, assume the attributes we want to
  match on ($A_1,...,A_j$) are the first $j$ attributes of $\calR$.
  Query $q$ given by Table~\ref{tab:proof-vzdist} produces
  visualization collection {\tt f5} which expresses $\vzdist_{F(D),A_1,...,A_j}(V,U)$.
  In the table, we first retrieve the values for $(A_1,...,A_j)$ using {\tt f3} and reorder
  {\tt f2} based on these values to get {\tt f4}.
  %We are guaranteed by the
  %operator definition in Section~\ref{sec:viz-exp-oper} that there will be
  %exactly one visualization in both {\tt f1} and {\tt f2} $\forall a_1,...a_j
  %\in (A_1,...,A_j)$
  We then compare the visualizations in {\tt f3}
  and {\tt f4} with respect to $(A_1,...,A_j)$ using the distance function
  $F(D)$ and retrieve the increasingly sorted $(A_1,...,A_j)$ values from the
  $argmin$. We are guaranteed that visualizations in {\tt f3} and {\tt f4}
  match up perfectly with respect to $(A_1,...,A_j)$ since the definition in
  Section~\ref{sec:viz-exp-oper} allows exactly one \vzchn to result from any
  $\vzsel_{A_1=a_1 \land ... \land A_j=a_j}$. Finally, we
  reorder {\tt f1} according to these values to retrieve {\tt f5}.
  For more information on the {\tt .order} operation, please refer to
  Appendix~\ref{name-appex}.
  %Similar queries exist
  %We can imagine coming up with similar
  %Note that a
  %key assumption we make multiple times is that $\vzsel_{A_1,...,A_j}$ for 
\end{proof}

\begin{lemma}
  $\vzfind_{F(D)}(V, U)$ is expressible in \zq for all valid functionals $F$ of
  $D$ and \vzgrps $V$ and singleton \vzgrps $U$.
\end{lemma}
\begin{proof}
  \begin{table*}[!htbp]
    \centering\scriptsize
    {\tt   
      \begin{tabular}{|r|l|l|l|l|l|l|} \hline
        \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Z1} & \textbf{...}
        & \textbf{Zk} & \textbf{Process} \\ \hline
        f1 & - & - & - & ... & - & \\
        f2 & - & - & - & ... & - & \\
        f3 \IN f1 & x1 \IN \_ & y1 \IN \_ & v1 \IN $A_1$.\_ & ... & vk \IN $A_k$.\_
        &
        x2, y2, u1, ..., uk \IN $argmin_{x1,y1,v1,...,vk}[k=\infty] {F(D)}(f3,f2)$
        \\
        *f4 & x2 & y2 & u1 & ... & uk & \\
        \hline
      \end{tabular}
    }
    \vspace{-10pt}\caption{\zq query $q$ which expresses $\vzfind_{F(D)}(V, U)$.
    }
    \label{tab:proof-vzfind}
  \vspace{-10pt}\end{table*}

  Assume {\tt f1} is the visualization collection which represents $V$ and {\tt f2}
  represents $U$.  Query $q$ given by Table~\ref{tab:proof-vzfind} produces
  visualization collection {\tt f4} which expresses $\vzfind_{F(D)}(V, U)$.
\end{proof}

Although we have come up with a formalized algebra to measure the
expressiveness of \zq, \zq is actually more expressive than \vzalg. For
example, \zq allows the user to nest multiple levels of iteration in the
Process column as in Table~\ref{tab:outlier}.
Nevertheless,
\vzalg serves as a useful minimum metric for determining the expressiveness of
\vzlans.
Other visual analytics tools like Tableau are capable of expressing the
selection operator $\vzsel$ in \vzalg, but they are incapable of expressing
the other operators which compare and filter visualizations based on
functional primitives $T$ and $D$. 
General purpose programming
languages with analytics libraries such as Python and
Scikit-learn~\cite{pedregosa2011scikit} are \vzcmp since they are
Turing-complete, but \zq's declarative syntax strikes a novel balance between
simplicity and expressiveness which allows even non-programmers to become data
analysts as we see in Section~\ref{sec:userstudy}.


%\alkim{Should we mention much of \vzalg ggplot/tableau can express here or
%later in related work?} 
%\alkim{Do we need to talk about how the logic \vzalg is necessarily more complicated
%than relational algebra (mention Godel logic for min/max?}


==> expressiveness.tex <==
%!TEX root=zenvisageql.tex

\later{
\section{Expressiveness}
\label{subsec:expressivenesss}

So far, we have described, via a collection of examples,
the various types of queries that can be posted using \zq.
A natural question now arises: {\em how can we characterize
the space of queries expressible via \zq?}
In this section, we provide both intuition for the space
of queries expressible via \zq, as well as more formal arguments.
Note, however, that \zq provides considerable flexibility to the user,
specifically via the Process and the Viz column;
as a result, there may be uses of \zq we still haven't foreseen,
and thus, our arguments will be necessarily incomplete.

\subsection{Formalized Capabilities}

We now discuss
the capabilities of \zq more formally.
For the rest of our discussion, 
we will assume that the Viz column 
uses
a simple aggregate, 
as opposed to user-defined interpolation or summarization.
We will relax this restriction later on in the section.






\paragraph{Language Formalization.}
The \zq language is straightforward to describe 
at a high level.
A \zq query $Q$ is formally defined
to be a collection of expressions $E$,
where each 
expression\footnote{\scriptsize Note that while we enforced that every Process must be associated with a Visual Component in our tabular interface, it need not be so; this decision 
was made primarily for compactness and intuitiveness. Here,
we decouple the two.} 
$E$
can be either a Visual Component expression $V$,
or a Process expression $P$.
A Visual Component expression $V$
must contain a tuple of sub-expressions,
for each of $X, Y$ and optionally, $Z_1,$$ Z_2,$$ \ldots,$$ Constraints,$ $Viz$.
A Process expression $P$
consists of three parts: a ranking function expression $S$
describing how the visualizations must be ranked,
a functional expression $F$ describing the computation that determines the ranking, and $k$, describing how many outputs are desired from the ranking.
Thus, formally:

$Q:= \{R\}$ where $ R:= V | P$

$V:= (X, Y, Z_1, Z_2, \ldots, Z_q, Constraints)$

$P:= (S, F, k)$

\noindent We next describe how $V$ and $P$ are interpreted.

\paragraph{Visual Components and Unit Visualizations.}
To describe how $V$ is interpreted,
we begin with the notion
of a {\em unit visualization}.
A unit visualization corresponds to 
a table that is the result of
a query of the following type:
\begin{quote} \small
\begin{verbatim}
SELECT X, A(Y)
FROM R1, R2, ..., Rp
WHERE Conditions
GROUP BY X 
ORDER BY X
\end{verbatim}
\end{quote}
where {\tt X, Y, A, Conditions} can vary.
Thus, a unit visualization corresponds to
a two-attribute aggregated table.
Such two-attribute tables can be readily visualized.
It is easy to see that the following holds:
\vspace{-5pt}
\begin{lemma}
Every visual component generates one or more unit visualizations.
\end{lemma}
We define a {\em unit visualization cross-product}
to be all unit visualizations formed from:
 combining
any $X_i$ in a set of attributes \overl{$X$}, 
any $Y_j$ in a set of attributes \overl{$Y$},
such that attribute $Z_i$ is equated to any attribute value $v_i$ in a set \overl{$V_i$}.
These visualizations can be represented using the following query,
where $X_i, Y_j, v_1, ..., v_q$ can vary:
\begin{quote} \small
\begin{verbatim}
SELECT Xi, A(Yj) 
FROM R1, R2, ..., Rp
WHERE Z1 = v1 AND ... AND Zq = vq AND Conditions
GROUP BY Xi
ORDER BY Xi
\end{verbatim}
\end{quote}
We have the following:
\begin{lemma}
Any unit visualization cross-product can be represented using a visual component.
\end{lemma}
\vspace{-5pt}
Thus, unit visualizations have close ties
to the visual components:
essentially, the visual components enable us
to assemble a collection of unit visualizations
by retrieving data from the database.

\paragraph{Visual Component Processor.}
%\agp{correspondence to axis variables? to polaris table algebra?}
We now describe how a visual component expression $V$ 
is processed
within \zv. 
To do that, we need to formally define name and axis variables. 
Name variables are variables that contain an array of unit
visualizations.
(As a result, we can say that each name variable corresponds
to a sequence of visualizations.)
Axis variables, on the other hand are variables 
that contain an array of elements: this could be attribute values,
or names of attributes themselves. 


\begin{figure}[!h]
\vspace{-5pt}

\begin{center}
\includegraphics[width=0.9\columnwidth]{figs/types.pdf}
\includegraphics[width=0.9\columnwidth]{figs/process-types.pdf}

\end{center}
\vspace{-10pt}
\caption{Visual Component Processor Flow (above) Task Processor Flow (below)}
\label{fig:flow}
\vspace{-5pt}
\end{figure}

A visual component processor 
(depicted in Figure~\ref{fig:flow} (top)) 
accepts as input
a visual component expression $V$,
as well as values for unspecified 
input axis variables $u_1, ..., u_n$,
within the visual component expression.
The output is an instantiation of the 
name variable: that is, it is an array of 
unit visualizations.
Additional outputs may include 
instantiations of output axis variables.
(These are used to refer to 
specific aspects or metadata of the unit visualizations.)
For instance, one axis variable $v_i$ may hold
an array with the values taken on by attribute $Z_i$
for each unit visualization in the name variable array.

\begin{figure}
\begin{center}
\vspace{-10pt}
\includegraphics[width=\columnwidth]{figs/patterns.pdf}
\end{center}
\vspace{-10pt}
\caption{Patterns in Task Computation (left: star pattern,  middle: complete graph pattern, right: bipartite pattern)}
\label{fig:patterns}
\vspace{-15pt}
\end{figure}

\paragraph{Task Processor.}
A task processor takes as a process expression $P$, 
as well as values for the 
unspecified input axis variables $u_1, ..., u_n$,
and unspecified name variables 
(or arrays of unit visualizations) $f_1, ..., f_m$.
It then generates instantiations of output axis variables. 



Thus, the Task Processor accepts a 
sequence of unit visualizations as input via name variables,
and performs some sub-selection (filtration) and/or ordering on these visualizations.
The eventual result is some subset of the unit visualizations that
are provided as input, ordered in some way.
Note that instead of generating an instantiation of
a single name variable (like the Visual Component Processor), the task processor instantiates
multiple axis variables: this distinction is important, because
by instantiating multiple axis variables, 
these axis variables could be used to generate multiple sets
of output unit visualizations via Visual Components.
It is the role of the Visual Component Processor to
generate the unit visualizations.

\paragraph{Process Primitives.} For populating
the Process Expression, 
\zq provides a few default functional primitives, 
including $D, T, R$.
Since the process can be overloaded by users
to specify their own user defined functions, it is not clear a-priori 
what types of computation may be possible via the Process expression.

Notice however, that all three of $D, T, R$ are computing
distance of some sort:
$D$ is explicitly computing a distance between a pair of visualizations,
$T$ is checking the overall trend of a visualization 
so is computing a distance between a visualization and the
trend,
$R$ is identifying representatives, and implicitly needs
to compute distances between all pairs of visualizations
in the collection.

Using these three primitives, and how we've used them in queries,
we have identified three patterns of distance computation 
that are expressible
in tasks, and capture all the examples described in the paper.
These patterns are depicted in Figure~\ref{fig:patterns}.
Each node depicts a visualization, while each edge between two visualizations corresponds to a distance computation between them.
The pattern on the left is a {\em star} pattern,
which compares the distance between 
a collection of unit visualizations to
a reference. 
This pattern is used for queries in Table~\ref{tab:motiv-ex-2} and Table~\ref{tab:name-1}.
The pattern in the middle is a {\em complete graph} pattern,
where unit visualizations are all compared against each other.
This pattern is used for queries in Table~\ref{tab:process-2}, Table~\ref{tab:ex-1}, and Table~\ref{tab:ex-4}.
Lastly, the pattern on the right is a {\em bipartite graph} pattern,
where pairs of corresponding unit visualizations
are compared against each other.
This pattern is used for queries in Table~\ref{tab:vars-1} and Table~\ref{tab:vars-3}.


\paragraph{Overall Capabilities.}
Thus, at a high level, 
\zv is tailored towards first, enumerating an array of unit visualizations
using visual components, and second,
task-based computation involving one of the three patterns 
displayed in Figure~\ref{fig:patterns},
to identify unit visualizations within this array 
with desired properties,
followed by repetitions of these two above steps.


% Note that the task cannot be used to compare an arbitrary
% collection of unit visualizations with each other:
% specifically, the schema of these unit visualizations
% must be the same, even if XXX


% \zv provides a few functional primitives by default as discussed in sub-section~\ref{sec:process}, and users can add their own simple primitives, or build complex functions using the simple functions. $F$ takes as input one or more name variables $v*$ pointing to a set of visualizations, and axis variable $a*$ to iterate over the sets. In particular, for each input axis variable, a {\tt for} loop is created and nested. The input axis variables are then used to step through the arrays specified by the name variables $v*$, and F is called at each iteration. $F$ can step through a set of visualizations and give a score based on how closely the visualization meets the objective. $F$ can also iterate through multiple sets of visualizations and compare mutiple visualizations corresponding to the same axis variable value. The output of $F$ is a list of axis variable values, and their scores. A ranking (and filtering) function $R$ is then applied to sort and pick top $k$ axis variable values. The output of the P is an iterator to the top $k$ values returned by $R$ which can be used in $V$ of successive rows.

% \tar{add examples of specific applications that the language can support}

\paragraph{Viz Column.}
So far, we have assumed that the Viz column
uses a simple aggregate for $Y$:
in fact, the Viz column could
apply some restricted set of 
data transformations, binning in arbitrary ways, noise removal,
and mappings to different types of visualizations,
as described in Section~\ref{sec:viz}.
However, as described in that section, we are
directly leveraging the capabilities of the grammar
of graphics to support these operations. 

% Through the Viz column, the language supports data transformations, data summarization, and mapping to different types of visualizations as discussed in sub-section~\ref{sec:viz}: If the summarization is specified in the Viz column, additional clauses and keywords such as {\tt GROUP BY}s and aggregations may be added. Additionally, result visualizer can map the fetched data into the visualization type specified under the Viz column. 

}

\section{Discussion of the Space of Use Cases}

As described above, \zq is targeted at 
generating simple unit visualizations 
via visual components, and then filtrating 
and ordering them via tasks,
which can be fed as input to 
other visual components or output to the user.

The visual components generate unit visualizations: 
the unit visualizations \zq is capable of 
handling correspond to a single 
SELECT-FROM-WH\-ERE-GROUPBY-ORDER; 
complicated nested queries are not the target
of \zv, since they are not usually the target 
of visual data exploration.
The tasks computation is limited to selecting 
visualizations with specific properties
from a set: even this encompasses a large collection of use-cases,
ranging from similarity and 
dissimilarity search, or to check if a visualization
has a specific property, to outlier detection and 
identification of representatives, to finding differences between 
corresponding visualizations, as we saw in the previous sections.

This implies that there is a large swath of data mining 
tasks that are 
not captured by \zq: this includes prediction of any sort, classification,
regression, dimensionality reduction, 
or frequent pattern mining. 
There are other data processing tasks that are not captured
by \zq, including data cleaning or pre-processing, data integration,
or expressing complex queries or computation that don't correspond to the unit visualization template described above.

\later{
\begin{figure}[!htb]
\begin{center}
\includegraphics[width=0.8\columnwidth]{figs/steps.pdf}
\end{center}
\vspace{-20pt}
\caption{The three stages of data analytics currently: the shaded box
is our focus}
\label{fig:steps}
\vspace{-10pt}
\end{figure}
}

Indeed, \zq is not meant to be a one-stop-shop for all of the computation on data:
it is meant to be the next logical step for current data visualization tools,
that severely lack the functionality of helping users find desired patterns
in visualizations
or compare visualizations.
This means that the data is already cleaned before it is
visualized: this is assumed in all data visualization tools. 
This also means that complex analytics, including prediction or mining,
and are not the focus of simple visualization, are better suited for 
subsequent tools.

%In Figure~\ref{fig:steps}, we depict our conceptualization of the three stages of data analytics;
%our target is not the first or the third stages, 
%which are better handled by other tools.
%Instead, our focus is on the middle, second stage,
%which is also the focus of current visual analytics tools.








% \newpage
% \tar{I have merged expressiveness and naive translation into one as they are related, next section could directly be on Query Optimisation.}
% A \zq query $Q$ can be broken up into two parts: the visual components $V$ and the
% the Process column $P$. In the \zq compiler, $V$
% determines the set of data \zv needs to retrieve from the database,and $P$ translates into the post-processing computation to be done on
% the returned data. Formally,

% $Q:$  $R+$  

% $R:$  $V[P]$

% \textbf{[Lemma 1] Since $V$ is translated into one or more relational algebra queries, \zq queries can be executed on relational data, and are limited to the expressive power of relational queries for retrieving data:}
% For each row, the \zq compiler loops over all combinations of values \tar{we can say we use Polaris Table Algebra to determine the combination} for each of the $n$ axis variables in $V$ and for each combination, issues a \sql query, the results of which are stored in the corresponding location in an $n$ dimensional array denoted as $N$. In other words, for each row, at a high level, the \zq compiler issues a \sql query corresponding to each visualization. Each generated \sql query has the form:
% \begin{quote} \small
% \begin{verbatim}
% SELECT X, Y 
% WHERE Z=v and (CONSTRAINTS) 
% ORDER BY X
% \end{verbatim}
% \end{quote}
% \textbf{[Lemma 2] Through the Viz column, the language supports data transformations, data summarization, and mapping to different types of visualizations as discussed in sub-section}~\ref{sec:viz}: If the summarization is specified in the Viz column, additional clauses and keywords such as {\tt GROUP BY}s and aggregations may be added. Additionally, result visualizer can map the fetched data into the visualization type specified under the Viz column. 

% Once the name variable array $N$ has been filled in with results from the \sql queries, the \zq compiler can directly visualize it or pass it as an input to to the Process column $P$. 

% \textbf{[Lemma 3] Process column P supports two kinds of explorations: a) single visualization exploration: how close a visualization matches a specific visual property, and/or b) comparative exploration: compare multiple visualizations and measure how similar they are:} $P$ consists of a functional primitive $F$ and a ranking function $R$.  $F$ are considered black boxes to the \zq compiler and are unaltered. \zv provides a few funtional primitives by default as discussed in sub-section~\ref{sec:process}, and users can add their own simple primitives, or build complex functions using the simple functions. $F$ takes as input one or more name variables $v*$ pointing to a set of visualizations, and axis variable $a*$ to iterate over the sets. In particular, for each input axis variable, a {\tt for} loop is created and nested. The input axis variables are then used to step through the arrays specified by the name variables $v*$, and F is called at each iteration. $F$ can step through a set of visualizations and give a score based on how closely the visualization meets the objective. $F$ can also iterate through multiple sets of visualizations and compare mutliple visualizations corresponding to the same axis variable value. The output of $F$ is a list of axis variable values, and their scores. A ranking (and filtering) function $R$ is then applied to sort and pick top $k$ axis variable values. Formally,

% $P:$  $R(F(v*,a*),k)$

% The output of the P is an iterator to the top $k$ values returned by $R$ which can be used in $V$ of successive rows.
 
% \textbf{Applications}: Using single and comparative visualization exploration based functional primitives, \zv can filter 2D visualizations based on a visual property, can find similar or dissimilar visualizations, can find outliers, can find k nearest- neighbour visualizations, can cluster and pick trends representing each cluster or combinations of these across any of the X, Y or Z dimensions. Other similar data mining tasks can integrated by introducing a functional primitive.

% \textbf{Limitations}: \zq is currently limited to exploration of visualization with only two dimensions. Given that \zq supports only single and comparative visaualization explorations, predictive explorations such as classification, or frequent pattern mining tasks are beyond the scope of the language. Moreover, since V is translated to relational queries, \zq cannot be used where fetching data needed for visualizations depends on recursion, and other query patterns that cannot be expressed using relational algebra \tar{the last point can be more clear}. 



==> inter-proc-opt.tex <==
%!TEX root=zenvisageql.tex




\paragraph{Inter-Task Optimization.}
%Our final optimization is less straightforward than the previous methods.
It is not generally not possible
to batch \sql queries across tasks, since
subsequent tasks may depend on the outputs of previous tasks.
However, for more sophisticated \zq queries, it may be possible 
to identify batching opportunities across tasks.
For instance, a visual component defined after a task may be
independent of the task. 
Formally, if visual component $V$ is defined in a
row later than the row task $T$ is defined in, 
and no column of $V$ depends on the
output of $T$, then $V$ is independent of $T$. The advantage of 
independence is that now we can batch $V$ into an earlier request because we do
not need to wait for the results of $T$.
Thus, in Table~\ref{tab:exec-1}, we can batch the \sql queries for the first and second
rows into a single request since the visual component in the second row is independent of
the task in the first row.


% \papertext{Since the visualizations from subsequent rows may depend on
% the output values of previous tasks, so it is not possible to batch
% queries across tasks}
% \techreport{As mentioned previously, it is generally not possible to batch \sql queries
% across tasks}.
% However, sometimes a visual component defined after a task may be
% independent of the task. 
% \papertext{Nothing prevents the user from combining 
% many non-related visual queries into a single \zq query with many output rows.
% Particularly for the case of exploratory visual analysis, the user may want to submit
% one \zq query which contains many different tasks to explore interesting trends,
% representative sets, and outliers in an unknown dataset.}

% \techreport{More formally, if visual component $V$ is defined in a
% row later than the row task $T$ is defined in, and no column of $V$ depends on the
% output of $T$, then $V$ is independent of $T$. The advantage of 
% independence is that now we can batch $V$ into an earlier request because we do
% not need to wait for the results of $T$.} 
% More concretely, in Table~\ref{tab:exec-1}, we can batch the \sql queries for the first and second
% rows into a single request since the visual component in the second row is independent of
% the task in the first row.

To determine all cases for which this independence can be taken advantage of,
the \zq compiler builds a query tree for the \zq queries it
parses. All axis variables, name variables, and tasks of a \zq query are 
nodes in its query tree. Name variables become the parents of the axis variables
in its visual component. Tasks become the parents of the visualizations it
operates over. Axis variables become the parents over the nodes which are used
in its declaration, which may be either tasks nodes or other axis variable
nodes.
The query tree for Table~\ref{tab:exec-1} is given in
Figure~\ref{fig:query-tree}. Here, the children point to their parents, and the
tasks in rows 1 and 2 are labeled {\tt t1} and {\tt t2} respectively. As
we can clearly see from the tree, the visual component for {\tt f2}
is independent of {\tt t1}.

\begin{figure}[!]
  \centering
  \vspace{-10pt}
  \includegraphics[scale=0.3]{figs/querytree1.pdf}
    \vspace{-10pt}
  \caption{The query tree for the \zq query in Table~\ref{tab:exec-1}.}
  \vspace{-15pt}
  \label{fig:query-tree}
\end{figure}

The \zv execution engine uses the query tree to determine which \sql queries to
batch in which step. At a high level, all \sql queries for name variable nodes
whose children have all been satisfied or completed can be batched into a single request.
More
specifically, the execution engine starts out by coloring all leaf nodes in the
query tree. Then, the engine repeats the following until the entire
query tree has been colored:
\begin{inparaenum}[i)]
  \item Batch the \sql queries for name variable nodes, who have all their
    children colored, into a single request and submit to the database.
  \item Once a response is received for the request, color all name variables
    nodes whose \sql queries were just submitted.
  \item Until no longer possible, color all axis variable and task nodes whose
    children are all colored. If a task is about to be colored, run the task
    first.
\end{inparaenum}
This execution plan ensures the maximal amount of batching is done while still
respecting dependencies. Parts of the execution plan may also be parallelized
(such as simultaneously running two independent, computation-expensive tasks
like representative sets), to improve overall throughput.



\techreport{While this optimization may seem like overkill for the short \zq examples
presented in this paper, nothing prevents the user from combining many non-related visual
queries into a single \zq query with many output rows. Particularly for the
case of exploratory visual analysis, the user may want to submit
one \zq query which contains many different tasks to explore interesting trends,
representative sets, and outliers in an unknown dataset.
}


==> intra-proc-opt.tex <==
%!TEX root=zenvisageql.tex

\paragraph{Intra-Task Optimization.}
\papertext{In addition to combining \sql queries within a row, the second level 
of optimization batches \sql across all rows that are input to the same task.
In Table~\ref{tab:exec-2}, this optimization would batch
rows 1 and 2 together and rows 3 and 4 together.
}
\techreport{In addition to combining \sql queries within a row, \sql queries may also
be batched across \zq rows. However, in general, it may not be possible to
compose queries across rows into a single \sql query,
since different rows may access completely
different attributes. Instead, our optimization is to batch multiple \sql
queries from different rows into a single \emph{request} to the database,
effectively pipelining the data retrieval.
However, tasks in \zq frequently filter and limit the space of visualizations
being looked at. Moreover, visualizations from subsequent rows may depend on
the output values of previous tasks, so it is not possible to batch
queries across tasks. Therefore, we batch into a single request all \sql queries for task-less rows leading up to
a row with a task. In Table~\ref{tab:exec-2}, this optimization would batch
rows 1 and 2 together and rows 3 and 4 together.
}


==> queryexecution.tex <==
%!TEX root=zenvisageql.tex

\begin{table*}[!htbp]
%\vspace{-5pt}
  \centering\scriptsize
 {\tt
  %\resizebox{\linewidth}{!}{%
    \begin{tabular}{|r|l|l|l|l|l|l|} \hline
      \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Z} &
      \textbf{Constraints}
      & \textbf{Viz} & \textbf{Process} \\ \hline
      f1 & `year' & `sales' & v1 \IN P & location=`US' & bar.(y=agg('sum')) &
      v2 \IN
      $argany_{v1}[t>0] T(f1)$ \\
      f2 & `year' & `sales' & v1 & location=`UK' & bar.(y=agg('sum')) & v3 \IN $argany_{v1}[t<0] T(f2)$ \\
      *f3 & `year' & `profit' & v4 \IN (v2.range | v3.range) &
      & bar.(y=agg('sum')) & \\ \hline
    \end{tabular}
  %}
  %\end{alltt}
  }
    \vspace{-10pt}
  \caption{
    A \zq query which returns the profit over time visualizations for products
    in user-specified set {\tt P}
    that have positive sales over time trends for the US but have negative sales
    over time trends for the UK.
  }
  \label{tab:exec-1}
  {\tt
  %\resizebox{\linewidth}{!}{%
    \begin{tabular}{|r|l|l|l|l|l|l|} \hline
      \textbf{Name} & \textbf{X} & \textbf{Y} & \textbf{Z} &
      \textbf{Constraints} & Viz
      & \textbf{Process} \\ \hline
      f1 & `location' & `sales' & v1 \IN P & year=`2010' & bar.(y=agg('sum')) & \\
      f2 & `location' & `sales' & v1 & year=`2015' & bar.(y=agg('sum')) & v2 \IN $argmax_{v1}[k=10] D(f1,f2)$ \\
      *f3 & `location' & `profit' & v2 & year=`2010' & bar.(y=agg('sum')) & \\
      *f4 & `location' & `profit' & v2 & year=`2015' & bar.(y=agg('sum')) & \\ \hline
	  	
    \end{tabular}
  %}
  %\end{alltt}
  }
  \vspace{-10pt}
  \caption{
    A \zq query which returns the profit over location visualizations for
    products in user-specified set {\tt P}
    that have the most different sales over location trends between 2010 and 2015.
  }
  \label{tab:exec-2}
    \vspace{-10pt}
\end{table*}

\section{Query Execution}
\label{subsec:query_execution}
In \zv, \zq queries are automatically parsed and executed by the backend.
The \zq compiler translates \zq queries into a collection of \sql queries
that are issued to a relational database and performs
post-processing computation on the results
of the \sql queries. 
By translating to \sql, we do not tie ourselves down to any specific
  relational database and can seamlessly leverage benefits from improvements to
databases.
%\new{By operating outside standard relational databases, we can seamlessly
%leverage benefits from improvements to the database; further, we can replace
%one relational database for another. 
%That said, we may be able to leverage benefits from moving computation
%``closer to'' the data; we plan to explore this in future work.}

\subsection{Translation to Database Queries}
Each row of a \zq query can be broken up into two parts: the visual component and the
the Process column. The visual components 
determine the set of data \zv needs to retrieve from the database, and the
Process column translates into the post-processing computation to be done on
the returned data. \techreport {\zv's naive \zq compiler performs the following operations for each row of a 
\zq query.}
For each row, the \zq compiler issues a \sql query 
corresponding to each visualization in the set specified in the visual component.
\techreport{Notice that this approach is akin to what a visual analyst manually
generating each visualization of interest and perusing it would do;
here, we are ignoring the human perception cost.}
More formally, for each row (i.e., each name variable),
the \zq compiler loops over all combinations of values
for each of the $n$ axis variables in the visual component corresponding
to that row, and for each combination, 
issues a \sql query,
the results of which are stored in the corresponding
location in an $n$ dimensional array.
\techreport{(Essentially, this corresponds to a nested for loop $n$ levels
deep.)}
Each
generated \sql query has the form:
{\tt \small SELECT X, Y FROM R WHERE Z=V AND (CONSTRAINTS) ORDER BY X}.
% \vspace{-5pt}
% \begin{quote} \small
% \begin{verbatim}
% SELECT X, Y 
% WHERE Z=V and (CONSTRAINTS) 
% ORDER BY X
% \end{verbatim}
% \end{quote}
% \vspace{-5pt}
If the summarization is specified, additional clauses
such as {\tt GRO\-UP BY}s and aggregations may be added. 
The results of each visualization are stored 
in an $n$-dimensional array
at the current
index. If $n$ is 0, the name variable points directly to the data.
\techreport{Going forward, we will omit the \texttt{FROM} clause: this is implied
and always fixed.}



Once the name variable array has been filled in with results
from the \sql queries,  
the \zq compiler generates the
post-processing code from the task in the Process
column. 
At a high level, \zq loops through all the visualizations, and applies
the objective function on each one. 
In particular, for each input axis variable in the mechanism, a 
{\tt for} loop is created and nested. The input axis variables are then used to
step through the arrays specified by the name variable, and the objective
function is called at each iteration. Instances of name variables are
updated with the correct index based on the axis variables it depends on. The
functions themselves are considered black boxes to the \zq compiler and are unaltered.
% \agp{This may be precise from a procedural standpoint but this is rather
% opaque. Can we talk about what you're trying to do? seems like all you're doing is to
% pass along each generated visualization to the objective function which has access
% to all the characteristics/attributes/properties of that visualization}
\papertext{We provide the psuedocode of the compiled version of the
query in~\cite{techreport}.}
\techreport{We provide the psuedocode of the compiled version of the
query expressed in Table~\ref{tab:exec-1} in Listing~\ref{lst:exec-1} in
the appendix.}


\subsection{External Optimizations}
Processing each visualization as an independent \sql query can be 
both wasteful and lead to unacceptable latencies.
We now describe how to rewrite and batch the \sql queries
via three levels of optimizations to reduce latency.
These optimizations are reminiscent of multi-query optimization
(MQO)~\cite{DBLP:journals/tods/Sellis88}; however, MQO techniques require
significant changes to the underlying database
engine~\cite{giannikis2013workload,psaroudakis2013sharing,DBLP:journals/pvldb/KementsietsidisNCV08,giannikis2014shared},
whereas our
syntactic rewriting techniques operate completely outside the database and are
tailored to the \zq setting.
\papertext{We omit many details that can be found in~\cite{techreport}.}
%The first two are straightforward and are 
%are reminiscent of multi-query optimization (MQO)~\cite{DBLP:journals/tods/Sellis88}---\new{however,
%MQO requires significant changes to the underlying
%engine, as opposed to our syntactic rewriting techniques
%that operate outside the database.}
%We focus on the third level, tailored to \zq.


% \techreport{While the translation process of the naive \zq compiler is simple and easy to
% follow, there is plenty of room for optimization. In particular, we look at
% three levels of optimization which focus on \emph{batching} \sql queries. 
% We found that the time it took to submit and wait for \sql queries was a
% bottleneck, and reducing the overall number of \sql queries can reduce performance 
% significantly.
% While none of these optimizations may seem particularly surprising,
% it required a substantial amount of effort to identify how these optimizations
% may be applied automatically to any \zq query. 
% \new{Our proposed optimizations are
% reminiscent of multi-query optimization techniques~\cite{DBLP:journals/tods/Sellis88}, but are tailored
% to \zq queries.}
% }

\paragraph{Intra-Line Optimization.}
\papertext{The first optimization level batches the \sql queries from a \zq row into one
query. For example, we can retrieve the data for all products in the first row
Table~\ref{tab:exec-1} in one \sql query. Similarly, if
the axis variable is in either the X or Y columns, we retrieve the data for
the entire set of attributes the axis variable iterates over. 
To ensure that the overhead of computation outside of the database
is minimal, we add appropriate {\tt ORDER BY} clauses to ensure
that additional sorting is not needed.
}
\iftechreportcode
The first level of optimization batches the \sql queries for a row into one
query. For example, we see that for the first row in Table~\ref{tab:exec-1}, that
a separate query is being made for every product in Listing~\ref{lst:exec-1}
in the appendix.
Instead, we can retrieve the data for all products in one \sql query:
\vspace{-5pt}
\begin{quote}\small
\begin{verbatim}
SELECT year, SUM(sales), product
  WHERE product IN P and location=`US'
  GROUP BY product, year
  ORDER BY product, year
\end{verbatim}
\end{quote}
\vspace{-5pt}
If the axis variable is in either the X or Y columns, we retrieve the data for
the entire set of attributes the axis variable iterates over. More concretely,
if we have axis variable {\tt y1 \IN \{`sales', `profit'\}}, our \sql
query would look like:
\vspace{-5pt}
\begin{quote}\small
\begin{verbatim}
SELECT year, SUM(sales), SUM(profit), product
  WHERE product IN P and location=`US'
  GROUP BY product, year
  ORDER BY product, year
\end{verbatim}
\end{quote}
\vspace{-5pt}
This optimization cuts down the number of queries by the sizes of sets the axis
variables range over, and therefore will lead to substantial performance benefits,
as we will see in the experiments.
Note that a side effect of batching queries is that the compiled code must now have an
extra phase to extract the data for different visualizations from the combined
results. However, since the \zq compiler includes an {\tt ORDER BY} clause, the
overhead of this phase is minimal.
\fi



\input{intra-proc-opt}
\input{inter-proc-opt}


==> real-examples.tex <==
\begin{table*}
  \centering\scriptsize
  \begin{adjustbox}{center}
    {\tt
      \begin{tabular}{|r|l|l|l|l|l|l|}
        \hline
        \zqname & X & Y & Z & Z2 & Z3 & \zqproc \\ \hline
        f1 & `year' & `depdelay' & v1 \IN `origin'.* & & & v2 \IN
        argany$_{v1}[t<0] T(f1)$\\ \hline
        f2 & `year' & `arrdelay' & v3 \IN `dest'.* & & & v4 \IN
        argany$_{v3}[t<0] T(f2)$\\ \hline
        f3 & `year' & `arrdelay' & v5 \IN `carrier'.* & `origin'.[? IN v2] &
        `dest'.[? IN v4] & v6 \IN argany$_{v5}[t>0] T(f3)$ \\ \hline
        f4 & `year' & `depdelay' & v5 & `origin'.[? IN v2] &
        `dest'.[? IN v4] & v7 \IN argany$_{v5}[t>0] T(f4)$ \\ \hline
        *f5 & `year' & \{`arrdelay', `depdelay'\} & v6 \^{} v7 & & & \\ \hline
      \end{tabular}
    }
  \end{adjustbox}
  \caption{Query which returns the sales visualizations for the 10 products
  whose sales visualizations are the most different from the others.}
  \label{tab:real2}
\end{table*}


==> userstudy-cuts.tex <==
%!TEX root=zenvisageql.tex

\section{User Study}
\label{subsec:userstudy}
We conducted a mixed methods study~\cite{creswell2007designing} 
in order to assess the efficacy of \zv. 
We wanted to: 
a) examine and compare the usability of the drag and drop 
interface and the custom query builder interface of \zv; 
b) compare the performance and usefulness of \zv 
with existing tools;
c) identify if, when, and how people would use \zv in their workflow;
and d) receive general feedback for future improvements.

\subsection{User Study Methodology}
\paragraph{Participants.} We recruited 12 graduate students 
as participants with varying degrees of expertise in data analytics. 
Table \ref{tab:toolsrep} depicts the participants' experience of participants in different tool categories of tools.
\begin{table}[H]
\vspace{-10pt}
 \centering\scriptsize
  {\tt    
  \begin{tabular}{|l|l|} \hline
      \textbf{Tools} & \textbf{Count} \\ \hline
      Excel, Google spreadsheet, Google Charts  & 8 \\ \hline
      Tableau & 4 \\ \hline
      SQL, Databases & 6 \\ \hline
      Matlab,R,Python,Java & 8 \\ \hline
      Data mining tools such as weka, JNP & 2 \\ \hline
      Other tools like D3 & 2 \\ \hline
     \end{tabular}
  }
  \vspace{-10pt}\caption{Participants' prior experience with data analytic tools}
  \label{tab:toolsrep}
\vspace{-10pt}\end{table}

\paragraph{Dataset.} 
To conduct the study, we used a housing dataset from Zillow.com~\cite{housing_data} consisting of housing sales data for different cities, counties, and states from 2004--15, with over 245K rows, and 15 attributes. We selected this dataset for two reasons:
First, housing data is often explored by data analysts using existing \john{visualization tools} \cite{elmqvist2008datameadow}. Second, looking for housing is commonplace for graduate students while in school and upon graduation; the participants could relate to the dataset and understand the usefulness of the tasks in the real world.
  
\paragraph{Comparison Points.} 
There are no tools that offer the same functionalities as
\zv: visual analytics tools do not offer the ability
to search for specific patterns, or issue complex data exploration queries; 
data mining toolkits do not offer the ability to generate visualizations, 
search for visual patterns and are instead tailored for general machine learning and prediction.
Since visual analytics tools are closer in spirit and functionality 
to \zv, we decided to implement a visual analytics tool as our baseline.
Thus, our baseline tool replicated the basic query specification and output visualization
capabilities of existing tools such as Tableau \john{(see Figure \ref{fig:baseline})}.  
We augmented the baseline tool with the ability to specify an arbitrary number of filters, allowing
users to use filters to drill-down on specific visualizations.
This baseline visualization tool was implemented with a styling scheme similar to \zv to control for external factors. 
%As depicted in Figure \ref{fig:baseline}, the baseline allowed users to visualize data by allowing them to specify the x-axis, y-axis, category, and filters. The baseline tool would populate all the visualizations, which fit the user specifications, using an alpha-numeric sort order.
In addition to task-based comparisons with this baseline, we
also explicitly asked participants to compare \zv with existing data mining and visual analytics 
tools that they use in their workflow.
 
\paragraph{Study Protocol.} The user study was 
conducted using a within-subject study design~\cite{bordens2002research}. 
The study consisted of three parts. 
In the first part, participants described 
their previous experience with data analytics and visualization tools. 
In the second part, participants performed visual analytics 
tasks using one tool at a time. 
\techreport{\zv was introduced as Tool A and the baseline tool was introduced as Tool B.}
Before starting the tasks on each of the tools, 
participants completed a 15-minute tutorial 
which included an overview of the interface and two practice questions 
to get a general understanding of the tool. 
The order of the tools was randomized to reduce the order effects. 
In order to compare the effectiveness of the drag and drop interface 
and the custom query builder interface of \zv, 
participants performed two separate sets of tasks on \zv, one for each component. Finally, in the third part, participants completed a survey that measured 
their satisfaction levels and preferences, followed by open-ended questions on the strengths and weaknesses 
of the tools, and whether they would use the two tools in their workflow. 
\techreport{
The study lasted for 1 hour and 15 minutes on average. 
Participants were paid 10 dollars per hour for their participation.}

\paragraph{Tasks.}
We prepared three sets of different tasks for the three interfaces (baseline, drag and drop, and custom query builder interfaces). The tasks differed only in the selection attributes so that the performance of the interfaces could be measured objectively (Section~\ref{sec:frontend} lists a few example queries that were used in the study). We carefully selected tasks which can surface during a search for a house. To demonstrate the efficacy of \zv, the tasks were focused on identifying similar trends or anomalies in housing data, which are non-trivial tasks to complete with a large dataset with existing tools. Specifically, the tasks were targeted to test the core features of \zv and solicit responses from participants on how it can complement existing data analytics workflows.

%The tasks that the participants performed on the two tools were designed to be similar in nature (differing only in selection attributes) so that we could compare the performance more objectively. The tasks focused on identifying visualizations with specific insights. Section~\ref{sec:frontend} lists a few example queries that were used in the study. 

\paragraph{Metrics.} 
We manually recorded how participants used the tool, their answers for each task, tracked their browser activity using a screen capture software, collected system interaction logs, recorded audio, and asked the participants to fill in a survey form. Using this data, we collected the following metrics: task completion time, task accuracy, the number of visualizations browsed for each task, the number of edits made on the drawing panel and the query table, survey results, and the answers to open-ended questions.

\paragraph{Ground Truth.} 
We took help of two expert data analysts to prepare the ground truth consisting of ranked answers for each of the tasks. Their inter-rater agreement, measured using Kendall\textquotesingle s Tau rank correlation coefficient, was 0.854. 
% The experts further discussed and resolved the conflicting answers to produce a final single ranked list of answers for each task. 
Then, each expert independently rated the answers on their ranked list on a 0 to 5 scale, with a score of 5 for the highest ranked answer and a score of 0 for the lowest ranked answer. We took the average of the two scores to rate the participants\textquotesingle~answers.


\begin{figure}
\vspace{-10pt}
\begin{center}
\fbox{\includegraphics[width=0.6\columnwidth]{figs/baseline.png}}
\end{center}
\vspace{-20pt}
\caption{The baseline interface implemented for the user study.}
\label{fig:baseline}
\vspace{-15pt}
\end{figure}


\subsection{Key Findings}
Now, we describe the key findings that we discovered through our analysis on the metrics collected during the study. We use $\mu$, $\sigma$, $\chi^2$ to denote average, standard deviation, and Chi-square test scores respectively.

\begin{table}[H]
\vspace{-10pt}
 \centering\scriptsize
  {\tt    
  \begin{tabular}{ | l | l | l  | } \hline
      \textbf{Tool} & \textbf{Time} (\textbf{sd}) & \textbf{Accuracy} (\textbf{sd}) \\ \hline
      Baseline & 172.5s (50.5) & 69.9\% (13.3) \\ \hline
      Drag and drop & 74s (15.1) & 85.3\% (7.61) \\ \hline
      Custom query builder & 115s (51.6) & 96.3\% (5.82) \\ \hline
     \end{tabular}
  }
  \vspace{-10pt}\caption{Average task completion time and average accuracy of the three interfaces.}
  \label{tab:taskresults}
\vspace{-10pt}\end{table}

\paraem{Finding 1: \zv enables over 50\% and 100\% faster task completion time than the baseline for custom query builder and drag and drop interface respectively.} We timed the task completion time for all participants,
and we found that the drag and drop interface has the smallest, and most predictable completion time (Table \ref{tab:taskresults}). The custom query builder has a higher completion time, but also with higher variance, while the baseline had a significantly higher completion time, more than twice the completion time of the drag and drop interface, and almost 50\% more than the custom query builder (Table \ref{tab:taskresults}).
This is not surprising, given that the baseline tool requires more manual exploration of the results, as opposed to either of the other two interfaces. We tested for statistical significance on the difference between the three interfaces using 
one-way between-subject ANOVA, followed by a post-hoc Tukey's test~\cite{tukey1949comparing}.
We found that the drag and drop interface and the custom query builder interface had statistically significantly 
faster task completion times compared to the baseline interface, with $p$ values of 0.0010 and 0.0069 respectively, both $<0.01$, while the difference between drag and drop and custom query builder was not statistically significant,
with a $p$ value of $0.06$. \papertext{Detailed statistics can be found in the technical report~\cite{techreport}.}

% One-way between subject ANOVA~\cite{tukey1949comparing} on the completion time of the tasks revealed that the differences between the three interfaces were significant F(2, 33) = 16.02, p < 0.001. On further applying the post hoc Tukey's test\cite{tukey1949comparing} for comparing the pairwise task completion times among the three interfaces (Table \ref{tab:turkeytest}), we found that both the drag and drop interface and the custom query builder had significantly faster task completion times compared to the baseline tool (p < 0.01), whereas the difference between the drag and drop interface, and the custom query builder was not significantly different.  
\techreport{
\begin{table}[H]
 \centering \scriptsize
  {\tt    
  \scalebox{0.75}{
  \begin{tabular}{|l|l|l|l|} \hline
      \textbf{Treatments} & \textbf{Q statistic} & \textbf{p-value} & \textbf{inference} \\ \hline
	Drag and drop interface vs. Custom query builder & 3.3463 & 0.0605331 & insignificant \\ \hline
	Drag and drop interface vs. Baseline tool & 7.9701 & 0.0010053 & significant (p<0.01) \\ \hline
	Custom query builder vs. Baseline tool & 4.6238 & 0.0069276 & significant (p<0.01) \\ \hline    
     \end{tabular}
  }
  }
\vspace{-10pt}
\caption{Tukey's test on task completion time}
\label{tab:turkeytest}
\vspace{-10pt}
\end{table}
}

\begin{figure}
\begin{center}
\includegraphics[width=0.6\columnwidth]{figs/accuracyvstime.pdf}
\end{center}
\vspace{-25pt}
\caption{Accuracy over time results for zenvisage and baseline}
\label{fig:accuracyvstime}
\vspace{-20pt}
\end{figure}

\paraem{Finding 2: \zv helps retrieve 20\% and 35\% more accurate results than the baseline for drag and drop and custom query builder interface respectively.} 
We rated the participant's answers based on the ground truth answers. 
The ratings revealed that participants performed poorly on the baseline tool (Table \ref{tab:taskresults})
\techreport{Further, any tasks that required comparing multiple
pairs of visualizations or trends ended up having lower accuracy than those that looked
for a pattern, such as a peak or an increasing trend, in a single visualization.}
Overall the low accuracy can be attributed to the
fact that the participants got tired of browsing through
large collections of visualizations and return the first result 
that approximately matches the conditions. 
On the other hand, since \zv is able to
accept more fine-grained user input, and
rank output visualizations, 
assisting participants in retrieving accurate answers
with less effort.
Among the two interfaces in \zv,
while the drag and drop interface had a faster task completion time, it was less accurate. The custom query builder had the highest accuracy (Table \ref{tab:taskresults}).
Thus accuracy is greater than the baseline by over 20\% (for the drag and drop interface)
or over 35\% (for the custom builder interface).
Finally, looking at both accuracy and task completion times together in Figure~\ref{fig:accuracyvstime}, we can conclude that \zv \emph{helps in ``fast-forwarding to desired visualizations'' with high accuracy.}

% In the baseline, comparing multiple pairs of visualizations or trends revealed to be more difficult than looking for a visual property, such as a peak, or an increasing pattern, in a single visualization. on the other hand, since \zv returns a ranked list of filtered answers based on the user specification, which allowed the participants to browse through a smaller number of visualizations compared to the baseline tool. Among the two interfaces in \zv, participants completed the tasks faster ($\mu=74s$, $\sigma=15.1$) on the drag and drop interface, but at the price of accuracy ($\mu=85.3\%$, $\sigma=7.61$). Participants using the custom query builder had the highest accuracy ($\mu=96.3\%$, $\sigma=5.82$) while maintaining comparable speeds to the drag and drop interface ($\mu=115s$, $\sigma=51.6$). Finally, looking at both accuracy and task completion times together (as depicted in Figure~\ref{fig:accuracyvstime}), we can conclude that \zv \textbf{helps in fast-forwarding to desired visualizations with a high accuracy.}

% Figure \ref{fig:accuracyvstime} depicts the average accuracy over time results of each of the participants on each of the interfaces. \agp{move this later.} 



%\textbf{\zv helps retrieve accurate results}: We rated the participant's answers based on the expert's gold set answers. The ratings revealed that participants performed poorly with the baseline, with the lowest accuracy ($\mu=69.9\%$, $\sigma=13.3$) and longest task completion time. In the baseline, comparing multiple pairs of trends or graphs revealed to be more difficult than looking for a single trend such as a peak, or an increasing pattern. \zv, on other hand, returns a ranked list of results based on the user specification, which allowed the participants to browse through a smaller number of visualizations compared to the baseline tool. Among the two interfaces in \zv, participants completed the tasks fastest ($\mu=74s$, $\sigma=15.1$) on the drag and drop interface, but at the price of accuracy ($\mu=85.3\%$, $\sigma=7.61$). Participants using the custom query builder had the highest accuracy ($\mu=96.3\%$, $\sigma=5.82$) while maintaining comparable speeds to the drag and drop interface ($\mu=115s$, $\sigma=51.6$). \textbf{\zv, thus, helps in fast-forwarding to desired visualizations with a high accuracy}.


\paraem{Finding 3: The drag and drop interface, and the custom query builder complement each other.} 
The large majority of participants (8/12) 
mentioned that the drag and drop interface, 
and the custom query builder complement each other in 
making \zv powerful in searching for specific insights. 
About 25 percent (3/12) of the participants 
(all with backgrounds in machine learning and data mining) 
preferred using only the custom query builder while 
just one participant 
(with no prior experience with query languages or programming languages) 
found only the drag and drop interface as useful. 
Participants stated that they would use the drag and drop interface for exploration and simple pattern search, and the custom query builder for specific and complex queries. One participant stated: \textit{``When I know what I am looking for is something exact, I want to use the query table. The other one [drag and drop interface] is for exploration when you are not so sure.''} 
\techreport{We next discuss the participants\textquotesingle responses to the individual components of \zv.}

\paraem{Finding 4: The drag and drop interface is intuitive.} 
Participants liked the simplicity and intuitiveness of the drag and drop interface. 
One stated: \textit{``[The drawing feature] is very easy and intuitive, I can draw the trend and automatically get the results.''} 
The participants rated the usability of this feature on 
a 5-point Likert scale ranging from strongly disagree 
(1) to strongly agree (5), and 
found the drawing feature easy to use, with $\mu=4.45$, $\sigma=0.674$. 
Despite the positive feedback, participants did identify limitations,
specifically that the functionality is restricted to identifying trends
similar to a single hand-drawn trend.

\paraem{Finding 5: The custom query builder is useful for complex queries.}
The majority of the participants (11/12) 
said that the custom query builder 
allowed them to search for complex insights which might be 
difficult to answer in the drag and drop interface. 
When asked if the custom query builder is comparatively difficult
to the drag-and-drop interface, participants tended to agree,
with $\mu=3.73$, $\sigma=0.866$ on a 5-point scale (5 is strongly agree).
At the same time, participants acknowledged 
the flexibility and the efficacy supported by the custom query builder. 
One participant explicitly stated that they 
preferred the custom query builder over the drag and drop interface 
for this reason: 
\textit{``When the query is very complicated, [the drag and drop interface] has its limitations, so I think I will use the query table most of the times unless I want to get a brief impression.''} 
Another participant stated that the custom query builder \textit{``has more functionality and it lets me express what I want to do clearly more than the sketch''}. This is consistent with other responses. 
Participants with a background in machine learning, 
data mining, and statistics (3/12) preferred always 
using the custom query builder over the drag and drop interface.

\paraem{Finding 6: \zv is much more effective (4.27 vs. 2.67 on a 5 point scale)
than the baseline tool at visual data exploration}
 In response to survey question \emph{``I found the tool to be effective in visualizing the data I want to see''}, the participants rated \zv (drag and drop interface + custom query builder) much higher ($\mu=4.27$, $\sigma=0.452$) than the baseline tool ($\mu=2.67$, $\sigma=0.890$) on a 5 point Likert scale.
 A participant experienced in Tableau commented:\textit{``In Tableau, there is no pattern searching. For example, if I see some pattern in Tableau, such as a decreasing pattern, and I want to see if any other variable is decreasing in that month, I have to go one by one to find this trend. But here I can find this through the query table.''}.  

\tar{Point 7 was earlier part of point 6, made it a separate point for emphasis}
\paraem{Finding 7: \zv would be a valuable addition to the participants' analytics workflow, can lead to a quicker initial data exploration before performing complex anaysis using machine learning and imperative programing languages:}
When asked about using the two tools in their current workflow, 9/12 participants stated that they would use \zv in their workflow, whereas only 2/12 participants stated that they would use our baseline tool ($\chi^2=8.22$, p<0.01). When the participants were asked how they would use \zv in their workflow, most of the them mentioned that they would use this tool for tasks such as finding common patterns, gaining an initial understanding of data distribution before running a machine learning task and finding outliers during data cleaning. One participant provided a specific scenario: \textit{``If I am doing my social science study and I want to see some specific behavior among users, then I can use tool A [\zv] since I can find the trend I am looking for and easily see what users fit into the pattern.''}. \nnew{While the pariticpants who had no programming experience considered the insight specification functionality of \zv as something very useful as they had to do it manually before, those with experince in programming languages such as python and MATLAB said \zv would take less time and fewer number of lines of code to do basic data exploration tasks. On asking participants (2/12) who had considerable experince with machine learning and data-mining libraries to write code for a task similar to the one in Table 11 in their favorite language, it took them several minutes and many more operations as compared to a few lines of \zq. \papertext{Example code can be found in our
technical report~\cite{techreport}}}. 

\techreport{
\begin{verbatim}[language=MATLAB]
% x1 = year, x2 = quarter, x3 = month, 
% y1 = sold price, y2 = listing price,
% y3 = turnover ratio
% X = [x1 x2 x3]
% Y_CA = [x1_y1_CA x1_y2_CA ... x3_y3_CA];
% Y_NY = [x1_y1_NY x1_y2_NY ... x3_y3_NY];

% similarity matrix (nX by nY matrix)
% nX = # of x (in this case, 3), 
% nY = # of y (in this case, 3)
sim = zeros(nX,nY);
for i = 1 : nX
    for j = 1 : nY
        val_CA = Y_CA(nX*(i-1)+j);
	val_NY = Y_NY(nX*(i-1)+j);
	sim(nX,nY) = pdist([val_CA,val_NY],'euclidean');
    end
end

% Find max entry M and its index 
% I in the sim matrix
[M,I] = max(sim);   

% Plot line chart (I_x and I_y 
% are the indices from the previous step)
plot(X(I_x), Y_CA(I_y), X(I_x), Y_NY(I_y));
\end{verbatim}
}

% \textbf{\zv is novel with real world applications}: All the participants described \zv as a novel tool and mentioned that they have not seen the declarative pattern searching functionality in any other tool.

\paraem{Finding 8: \zv can be improved.} While the participants looked forward to using the custom query builder in their own workflow, a few of them were interested in directly exposing the commonly-used trends/patterns such as outliers, through the drag and drop interface. Some of them were interested in knowing how they could integrate custom functional primitives (we could not cover it in the tutorial due to time constraints). In order to improve the user experience, participants suggested adding instructions and guidance for new users as part of the interface. Participants also commented on the unrefined look and feel of the tool, as well as the lack of the diverse set of usability related features, such as bookmarking and search history, that are offered in existing systems.






==> userstudy-tr-revised.tex <==
%!TEX root=zenvisageql.tex

\vspace{-2pt}
\section{User Study}
\label{sec:userstudy}
\vspace{-2pt}

We conducted a user study to evaluate the utility of \zv for data exploration versus two types of systems---first, visualization tools, similar to Tableau, and second, general database and data mining tools, which also support interactive analytics to a certain extent.
%In order to set up the 
In preparation for the user study, we conducted interviews with data analysts to identify the typical exploration tasks and tools used in their present workflow. Using these interviews, we identified a set of tasks to be used in the user study for \zv. We describe these interviews first, followed by the user study details.

% We conducted a mixed methods study~\cite{creswell2007designing} 
% to compare \zv with a custom-made baseline visual analytics tool to assess how \zv can aid in visualizing interesting patterns, trends, or insights from large datasets. Additional interviews with data analysts were conducted to identify the low level tasks and tools used in their typical workflow, and explore how \zv can help with their everyday activities.

\vspace{-2pt}
\subsection{Analyst Interviews and Task Selection}
\label{sec:interviews}
\vspace{-2pt}

We hired seven data analysts via Upwork~\cite{upwork},
a freelancing plat\-form---we 
found these analysts by searching for freelancers
who had the keywords \texttt{analyst} or \texttt{tableau}
in their profile. 
We conducted one hour interviews with them
to understand how they perform data exploration tasks.
The interviewees had 3---10 years of prior experience,
and told about every step of their workflow;
from receiving the dataset to presenting the
analysis to clients.
The rough workflow of all interviewees identified 
was the following: first, data cleaning is performed;
%if the data is not already presented in structured form;
subsequently, the analysts perform data exploration;
then, the analysts develop presentations using their findings.
We then drilled down onto the data exploration step.

We first asked the analysts what types of tools 
they use for data exploration.
Analysts reported nine different tools---the most popular ones 
included Excel (5), Tableau (3), and SPSS (2). 
The rest of the tools were reported by just one analyst:
Python, SQL, Alteryx, Microsoft Visio, Microsoft BI, SAS. 
Perhaps not surprisingly, analysts use both visualization
tools (Tableau, Excel, BI), programming languages (Python),
statistical tools (SAS, SPSS), and relational databases (SQL)
for data exploration.

Then, to identify the common tasks used in data exploration, 
%while not being biased by \zv's targeted use-cases, 
we used a taxonomy of
abstract exploration tasks proposed by Amar et al.~\cite{amar2005low}.
Amar et al. developed their taxonomy through summarizing
the analytical questions that arose
during the analysis of five different datasets, 
independent of the capabilities of existing tools or interfaces.
The exploration tasks in Amar et al.~include:
filtering ({\sf f}), sorting ({\sf s}), determining range ({\sf r}), 
characterizing distribution ({\sf d}),
finding anomalies ({\sf a}), clustering ({\sf c}), 
correlating attributes ({\sf co}), retrieving value ({\sf v}),  
computing derived value ({\sf dv}), and finding extrema ({\sf e}).
When we asked the data analysts which tasks they use in their workflow, 
the responses were consistent in that all of them use all of these
tasks, except for three exceptions---{\textsf c}, reported by four participants,
and {\sf e, d}, reported by six participants. 

%We hired seven data analysts on Upwork \cite{upwork}, an online freelancing platform, and conducted one hour interviews to probe how analysts explore data to find meaningful trends and patterns from large datasets. The interviewees had 3 to 10 years of prior experience as data analysts, and were asked to walk through each step of their workflow; from receiving the dataset to presenting the analysis to clients. \john{To identify the common analytical tasks utilized by analysts, we referenced the taxonomy of low level analytical tasks proposed by Amar et al. \cite{amar2005low}. Amar et al. developed the taxonomy through summarization of the analytical questions that arose during analysis of five different datasets, and generated a comprehensive list of tasks that are not limited by the expressive capability of specific tools or interfaces. Considering that analysts use a wide variety of tools for analysis, the taxonomy provides a fair baseline for comparing the type of tasks analysts work on, rather than focusing on the tools used during their workflow (we identified nine different tools used by the seven data analysts). When we asked the data analysts which low level analytical tasks they used during their workflow, and how they approached these tasks, responses were consistent among the analysts with the exception of clustering; only four analysts reported to use clustering, while at least six analysts utilized the other remaining tasks.}

Given these insights, we selected a small number of appropriate tasks for our user study
encompassing eight of the ten exploration tasks described above:
{\sf f}, {\sf s}, {\sf r}, {\sf d}, {\sf a}, {\sf c}, {\sf co}, {\sf v}.
The other two---{\sf dv} and {\sf e}---finding derived values
and computing extrema, are important tasks in data analysis,
but existing tools (e.g., Excel) already provide adequate
capabilities for these tasks, and we did not expect \zv to 
provide additional benefits. 


\vspace{-2pt}
\subsection{User Study Methodology}
\vspace{-2pt}

The goal of our user study was to evaluate \zv with other tools,
on its ability to effectively support data exploration.

\paragraph{Participants.} 
We recruited 12 graduate students as participants with 
varying degrees of expertise in data analytics.
\papertext{In short, half of them used databases; eight of them 
used Matlab, R, Python or Java; eight of them used
spreadsheet software; and four of them used Tableau.
Data for other not as popular tools are not reported. 
}
\techreport{Table \ref{tab:toolsrep} depicts the participants' experience with different categories of tools.
\begin{table}[H]
\vspace{-10pt}
 \centering\scriptsize
  {\tt    
  \begin{tabular}{|l|l|} \hline
      \textbf{Tools} & \textbf{Count} \\ \hline
      Excel, Google spreadsheet, Google Charts  & 8 \\ \hline
      Tableau & 4 \\ \hline
      SQL, Databases & 6 \\ \hline
      Matlab,R,Python,Java & 8 \\ \hline
      Data mining tools such as weka, JNP & 2 \\ \hline
      Other tools like D3 & 2 \\ \hline
     \end{tabular}
  }
  \vspace{-10pt}\caption{Participants' prior experience with data analytic tools}
  \label{tab:toolsrep}
\vspace{-10pt}\end{table}
}

\paragraph{Baselines.}
For the purposes of our study, we explicitly wanted to
do a head-to-head qualitative and quantitative comparison with visual analytics tools,
and thus we developed a baseline tool to compare \zv against directly.
Further, via qualitative interviews, we compared \zv versus
against other types of tools, such as databases, data mining, and programming tools.
Our baseline tool was developed by replicating the visualization 
selection capabilities of visual analytics tools with a styling scheme identical to \zv to control for external factors.
The tool allowed users to specify the X-axis, Y-axis, dimensions, and filters.
The tool would then populate all visualizations meeting the specifications.


\paragraph{Dataset.}
We used a housing dataset from Zillow.com \cite{housing_data}, 
consisting of housing sales data for different cities, counties, and states from 2004-15, 
with over 245K rows, and 15 attributes. We selected this dataset since participants could relate to the dataset and understand the usefulness of the tasks.

% We designed the user study tasks with the case studies in Section~\ref{sec:intro} in mind, and we translated the case study tasks into tasks applicable to the real estate dataset. We prepared two sets of tasks for the baseline tool and \zv. The tasks differed only in the selection attributes so that the performance of the interfaces could be measured objectively. Section~\ref{sec:frontend} lists a few example queries that were used in the study.
\paragraph{Comparison Points.} 
There are no tools that offer the same functionalities as
\zv. Visual analytics tools do not offer the ability
to search for specific patterns, or issue complex visual exploration queries; 
data mining toolkits do not offer the ability to search for visual patterns 
and are instead tailored for general machine learning and prediction. 
\papertext{We decided to implement our baseline tool by replicating
the basic visualization specification capabilities of tools like Tableau,
augmented with additional filtering capabilities. 
The styling scheme was similar to \zv to control for external factors;
details can be found in \cite{techreport}.}\techreport{Since visual analytics tools are closer in spirit and functionality 
to \zv, we decided to implement a visual analytics tool as our baseline.
Thus, our baseline tool replicated the basic query specification and output visualization
capabilities of existing tools such as Tableau.  
We augmented the baseline tool with the ability to specify an arbitrary number of filters, allowing
users to use filters to drill-down on specific visualizations.
This baseline visualization tool was implemented with a styling scheme similar to \zv to control for external factors. 
As depicted in Figure \ref{fig:baseline}, the baseline allowed users to visualize data by allowing them to specify the x-axis, y-axis, category, and filters. The baseline tool would populate all the visualizations, which fit the user specifications, using an alpha-numeric sort order.} In addition to task-based comparisons with this baseline, we
also explicitly asked participants to compare \zv with existing data mining and visual analytics 
tools that they use in their workflow.

\paragraph{Tasks.}
We designed the user study tasks with the case studies 
from Section~\ref{sec:intro} in mind,
and translated them into the housing dataset. 
Further, we ensured that these tasks together evaluate 
eight of the exploration tasks described above---{\sf f}, {\sf s}, {\sf r}, {\sf d}, {\sf a}, {\sf c}, {\sf co}, 
and {\sf v}.
One task used in the user study is as follows: ``Find three cities in the state of NY where the Sold Price vs Year trend is very different from the state\textquotesingle s overall trend.'' This query required the participants to first retrieve the trend of NY ({\sf v}) and characterize its distribution ({\sf d}), then separately filter to retrieve the cities of NY ({\sf f}), compare the values to find a negative correlation ({\sf co}), sort the results ({\sf s}), and report the top three cities on the list.

\paragraph{Study Protocol.} 
The user study was conducted using a within-subjects study design~\cite{bordens2002research},
forming three phases.
First, participants described their previous experience with data 
analytics tools. 
Next, participants performed exploration tasks using 
\zv (Tool A) and the baseline tool (Tool B), with the orders 
randomized to reduce order effects.
Participants were provided a 15-minute tutorial-cum-practice session
per tool to get familiarized before performing the tasks.
Finally, participants completed a survey
that both measured their satisfaction levels and preferences,
along with open-ended questions on the strengths
and weaknesses of \zv and the baseline, when compared to 
other analytics tools they may have used.\techreport{ The average study session lasted for 75 minutes on average. 
Participants were paid ten dollars per hour for their participation.}
After the study, we reached out to participants with backgrounds
in data mining and programming, and asked if they could complete
a follow-up interview where they use their favorite analytics tool for performing
one of the tasks, via email. 

\paragraph{Metrics.} 
% We recorded how the participants used the tool, their answers for each task, the audio of discussions, and 
% the responses to the survey. 
Using data that we recorded, we collected the following metrics: 
completion time, accuracy, and the usability ratings 
and satisfaction level from the survey results. 
In addition, we also explicitly 
asked participants to compare \zv with tools that they use in their workflow.
For comparisons between \zv and general database and data mining tools
via follow-up interviews, 
we used the number of lines of code to evaluate the differences. 

\paragraph{Ground Truth.} 
Two expert data analysts prepared the ground truth 
for each the tasks in the form of ranked answers,
along with score cut-offs on a 0 to 5 scale (5 highest). 
Their inter-rater agreement, measured using Kendall's Tau coefficient, 
was 0.854. 
% Then, each expert independently rated the answers on their 
% ranked list on a 0 to 5 scale (5 highest). 
We took the average of the two scores to rate the participants' answers.

\techreport{
\begin{figure}
\vspace{-5pt}
\begin{center}
\fbox{\includegraphics[width=0.6\columnwidth]{figs/baseline.png}}
\end{center}
\vspace{-20pt}
\caption{The baseline interface implemented for the user study.}
\label{fig:baseline}
\vspace{-10pt}
\end{figure}
}

\vspace{-2pt}
\subsection{Key Findings}
\vspace{-2pt}

Three key findings emerged from the study and are described below.
We use $\mu$, $\sigma$, $\chi^2$ to denote average, standard deviation, 
and Chi-square test scores, respectively.

\paraem{Finding 1: \zv enabled over 50\% and 100\% faster task completion times than the baseline for the custom query builder and drag and drop interfaces, respectively.} 
%We timed the task completion time for all participants,
%and 
We found that the drag and drop interface
had the smallest, and most predictable completion time ($\mu=74s$, $\sigma=15.1$),
the custom query builder had a higher completion time and a higher variance ($\mu=115s$, $\sigma=51.6$),
while the baseline had a significantly higher completion time ($\mu=172.5s$, $\sigma=50.5$), more than twice the completion time of the drag and drop interface,
and almost 50\% higher than the custom query builder interface.
This is not surprising, given that the baseline tool requires more
manual exploration compared to the other two interfaces.
%We tested for statistical significance on the difference between the three interfaces 
Using 
a one-way between-subjects ANOVA,
followed by a post-hoc Tukey's test~\cite{tukey1949comparing},
we found that the
drag and drop interface and the custom query builder interface
had statistically significant
faster task completion times compared to the baseline interface,
with $p$ values of 0.0010 and 0.0069, respectively.
The difference between the drag and drop interface
and the custom query builder interface was not statistically significant,
with a $p$ value of $0.06$. Detailed statistics can be found in Table\ref{tab:turkeytest}.


% One-way between subject ANOVA~\cite{tukey1949comparing} on the completion time of the tasks revealed that the differences between the three interfaces were significant F(2, 33) = 16.02, p < 0.001. On further applying the post hoc Tukey's test\cite{tukey1949comparing} for comparing the pairwise task completion times among the three interfaces (Table \ref{tab:turkeytest}), we found that both the drag and drop interface and the custom query builder had significantly faster task completion times compared to the baseline tool (p < 0.01), whereas the difference between the drag and drop interface, and the custom query builder was not significantly different.  
\techreport{
\begin{table}[H]
 \centering \scriptsize
  {\tt    
  \scalebox{0.75}{
  \begin{tabular}{|l|l|l|l|} \hline
      \textbf{Treatments} & \textbf{Q statistic} & \textbf{p-value} & \textbf{inference} \\ \hline
	Drag and drop interface vs. Custom query builder & 3.3463 & 0.0605331 & insignificant \\ \hline
	Drag and drop interface vs. Baseline tool & 7.9701 & 0.0010053 & significant (p<0.01) \\ \hline
	Custom query builder vs. Baseline tool & 4.6238 & 0.0069276 & significant (p<0.01) \\ \hline    
     \end{tabular}
  }
  }
\vspace{-10pt}
\caption{Tukey's test on task completion time}
\label{tab:turkeytest}
\vspace{-10pt}
\end{table}
}

\begin{figure}
\begin{center}
\includegraphics[width=0.6\columnwidth]{figs/accuracyvstime.pdf}
\end{center}
\vspace{-25pt}
\caption{Accuracy over time results for zenvisage and baseline}
\label{fig:accuracyvstime}
\vspace{-20pt}
\end{figure}


\paraem{Finding 2: \zv helped retrieve 20\% and 35\% more accurate results than the baseline for drag and drop and custom query builder interfaces, respectively.} 
Comparing the participants' responses against the ground truth responses, 
we found that participants achieved the lowest accuracy with the baseline tool ($\mu=69.9\%$, $\sigma=13.3$). 
\techreport{Further, any tasks that required comparing multiple
pairs of visualizations or trends ended up having lower accuracy than those that looked
for a pattern, such as a peak or an increasing trend, in a single visualization.}
The low accuracy could be attributed to the fact that the participants selected suboptimal answers before browsing through the entire list of results for better answers. Conversely, \zv is able to
accept more fine-grained user input, and
rank output visualizations. With \zv,
participants were able to retrieve accurate answers
with less effort.
Between the two interfaces in \zv,
while the drag and drop interface had a faster task completion time,
it also had a lower accuracy ($\mu=85.3\%$, $\sigma=7.61$).
The custom query builder interface had the
highest accuracy ($\mu=96.3\%$, $\sigma=5.82$).
The accuracy was greater than the baseline by over 20\% (for drag and drop)
and over 35\% (for custom builder).
Finally, looking at both accuracy and task completion times together in Figure~\ref{fig:accuracyvstime}, we see that \zv \emph{helps in ``fast-forwarding to desired visualizations'' with high accuracy.} 


\paraem{Finding 3: The drag and drop interface and the custom query builder complemented each other.
The drag and drop interface was intuitive, while the custom builder was useful for complex queries.} 
The majority of participants (8/12) 
mentioned that the drag and drop 
and custom query builder interfaces complemented each other \techreport{in making \zv powerful}
when searching for specific insights.\techreport{ 25 percent (3/12) of the participants (all with backgrounds in machine learning and data mining) 
preferred using only the custom query builder interface, while just one participant (with no prior experience with query languages or programming languages) found only the drag and drop interface as useful.}
Participants stated that they would use drag and drop for exploration and simple pattern search and custom query builder for specific / complex queries. One stated: \textit{``When I know what I am looking for is exact, I want to use the query table. The other one [drag and drop] is for exploration when you are not so sure.'' (P9).} 
Participants liked the simplicity and intuitiveness of the drag and drop interface. 
One stated: \textit{``[The drawing feature] is very easy and intuitive, I can draw... and automatically get the results.''} (P2).
On a five-point Likert (5 is strongly agree), participants
found the drawing feature easy to use ($\mu=4.45$, $\sigma=0.674$). 
Despite the positive feedback, participants did identify limitations,
specifically, that the functionality was restricted to identifying trends
similar to a single hand-drawn trend.

The majority of the participants (11/12) 
stated that the custom query builder 
allowed them to search for complex insights that might be 
difficult to answer via drag and drop. 
When asked if the custom query builder was difficult to use compared to
the drag-and-drop interface, participants tended to agree ($\mu=3.73$, $\sigma=0.866$ on a five-point Likert scale where five is strongly agree).
At the same time, participants acknowledged 
the flexibility and the efficacy supported by the custom query builder interface. 
One participant explicitly stated why they 
preferred the custom query builder over the drag and drop interface: 
\textit{``When the query is very complicated, [the drag and drop] has its limitations, 
so I think I will use the query table most of the times unless I want to get a brief impression.''} (P6).
Another participant stated that the custom query builder interface \textit{``has more functionality and it lets me express what I want to do clearly more than the sketch''} (P4). This was consistent with other responses. 
Participants with a background in machine learning, 
data mining, and statistics (3/12) preferred
using the custom query builder over the drag and drop interface.

\paraem{Finding 4: \zv was more effective (4.27 vs. 2.67 on a five-point Likert scale)
than the baseline tool at visual data exploration, and would be
a valuable addition to the participants' analytics workflow.} 
In response to the survey question \emph{``I found the tool to be effective in visualizing the data I want to see''}, the participants rated \zv (the drag and drop interface and the custom query builder interface) higher ($\mu=4.27$, $\sigma=0.452$) than the baseline tool ($\mu=2.67$, $\sigma=0.890$) on a five-point Likert scale.
A participant experienced in Tableau commented: \textit{``In Tableau, there is no pattern searching. If I 
see some pattern in Tableau, such as a decreasing pattern, and I want to see if any other variable is 
decreasing in that month, I have to go one by one to find this trend. But here I can find this through the query table.''} (P10).

\paraem{Finding 5: \zv complements existing database and data mining systems, and programming languages.}
When explicitly asking participants about comparing \zv with the
tools they use on a regular basis for data analysis, 
all participants acknowledged that \zv adds %\zq and \zv adds 
value in data exploration not encompassed by their tools. 
\zq augmented with inputs from the sketching canvas proved to be extremely effective.
For example P8 stated: \emph{``you can just [edit] and draw to find out similar patterns. You\textquotesingle ll 
need to do a lot more through Matlab to do the same thing.''}
Another experienced participant mentioned the benefits of not needing to know much programming to accomplish certain tasks: \emph{``The obvious good thing is that you can do complicated queries, and you don\textquotesingle t have to write SQL queries... I can imagine a non-cs student [doing] this.''} (P9).
When asked about the specific tools they would use to solve the user study tasks,
all participants reported a programming language like Matlab or Python. 
This is despite half of the participants reporting using a relational database regularly,
and a smaller number of participants (2) reporting using a data mining tool regularly.
Additionally, multiple participants even with extensive programming experience
reported that \zv would take less time and fewer lines of code for certain data exploration tasks.
(Indeed, we found that all participants were able to complete the user study tasks in under 2 minutes.)
In follow-up email interviews, we asked a few participants to respond with code from their
favorite data analytics tool for the user study tasks.
Two participants responded --- one with Matlab code, one with Python code.
Both these code snippets were much longer than \zq:
as a concrete example, the participant accomplished the same task with 
38 lines of Python code compared to 4 lines of \zq.
While comparing code may not be fair, the roughly order of magnitude
difference demonstrates the power of \zv over existing systems.


\paraem{Finding 6: \zv can be improved.} While the participants looked forward to using custom query builder in their own workflow, a few of them were interested in directly exposing the commonly-used trends/patterns such as outliers, through the drag and drop interface. Some were interested in knowing how they could integrate custom functional primitives (we could not cover it in the tutorial due to time constraints). In order to improve the user experience, participants suggested adding instructions and guidance for new users as part of the interface. Participants also commented on the unrefined look and feel of the tool, as well as the lack of a diverse set of usability related features, such as bookmarking and search history, that are offered in existing systems.



\later{
\paraem{Finding 1: \zv enables faster and more accurate exploration than existing visualization tools.}
Since all of our tasks involved generating multiple visualizations
and comparing them to find desired ones, participants were not only able to complete the tasks
 {\em faster}---$\mu$=115s, $\sigma$=51.6 for 
\zv vs.~$\mu$=172.5s, $\sigma$=50.5 for the baseline---but also more 
{\em accurately}---$\mu$=96.3\%, $\sigma$=5.82 for \zv vs.~$\mu$=69.9\%, $\sigma$=13.3 for the baseline.
The baseline requires considerable manual exploration to complete
the same task, explaining the high task completion times; in addition, participants frequently compromised
by selecting suboptimal answers before browsing
the entire list of results for better ones, explaining the 
low accuracy.
On the other hand, \zv is able to 
automate the task of finding desired visualizations, considerably reducing manual
effort.
Also of note is the fact that the accuracy with \zv is close to 100\%---indicating
that a short 15 minute tutorial on \zq was enough to equip users with the knowledge they
needed to address the tasks---and that too, within 2 minutes (on average). 

When asked about using \zv vs.~the baseline in their current workflow, 
9 of the 12 participants stated that they would use \zv in their workflow, 
whereas only two participants stated that they would use our baseline tool ($\chi^2=8.22$, p<0.01). 
When the participants were asked how, 
one participant provided a specific scenario: \textit{``If I am doing my social science study, 
and I want to see some specific behavior among users, then I can use tool A [\zv] 
since I can find the trend I am looking for and easily see what users fit into the pattern.''} (P7). 
In response to the survey question \emph{``I found the tool to be effective in visualizing the data I want to see''}, 
the participants rated \zv higher ($\mu$=4.27, $\sigma$=0.452) than the baseline ($\mu$=2.67, $\sigma$=0.890) 
on a five-point Likert scale. A participant experienced in Tableau 
commented: \textit{``In Tableau, there is no pattern searching. If I see some pattern in Tableau, 
such as a decreasing pattern, and I want to see if any other variable is decreasing in that month, 
I have to go one by one to find this trend. But here I can find this through the query table.''} (P10). 

%we just need to say that all participants were able to successfully use a 15 min tutorial to write zql queries and receive accurate answers

\paraem{Finding 2: \zv complements existing database and data mining systems, and programming languages.}
When explicitly asking participants about comparing \zv with the
tools they use on a regular basis for data analysis, 
all participants acknowledged that \zv adds %\zq and \zv adds 
value in data exploration not encompassed by their tools. 
\zq augmented with inputs from the sketching canvas proved to be extremely effective.
For example P8 stated: \emph{``you can just [edit] and draw to find out similar patterns. You\textquotesingle ll 
need to do a lot more through Matlab to do the same thing.''}
Another experienced participant mentioned the benefits of not needing to know much programming to accomplish certain tasks: \emph{``The obvious good thing is that you can do complicated queries, and you don\textquotesingle t have to write SQL queries... I can imagine a non-cs student [doing] this.''} (P9).
When asked about the specific tools they would use to solve the user study tasks,
all participants reported a programming language like Matlab or Python. 
This is despite half of the participants reporting using a relational database regularly,
and a smaller number of participants (2) reporting using a data mining tool regularly.
Additionally, multiple participants even with extensive programming experience
reported that \zv would take less time and fewer lines of code for certain data exploration tasks.
(Indeed, we found that all participants were able to complete the user study tasks in under 2 minutes.)
In follow-up email interviews, we asked a few participants to respond with code from their
favorite data analytics tool for the user study tasks.
Two participants responded --- one with Matlab code, one with Python code.
Both these code snippets were much longer than \zq:
as a concrete example, the participant accomplished the same task with 
38 lines of Python code compared to 4 lines of \zq.
While comparing code may not be fair, the roughly order of magnitude
difference demonstrates the power of \zv over existing systems.
% While simply considering the number of lines of code 
% may not be a truly fair comparison, we argue that ZQL requiring 
% roughly only one tenth of the python code demonstrates the value of \zv, 
% and how it can complement existing database and data mining systems.

 % \john{Even those with considerable experience with programming languages such as Python and Matlab argued that \zv would take less time and fewer lines of code for certain data exploration tasks. Considering that all participants were able to complete the provided tasks under 2 minuets (as described in Finding 1) after a brief 15 minute tutorial, it reflects on the learnability of ZQL. Relatively simple queries in \zv can be difficult to reproduce in other languages. If a user wishes to identify trends which are similar to a specific graph, or locate trends which have been consistently decreasing, it would require the users substantial effort to accomplish such tasks. When we asked about the benefits of \zv over existing systems, P8 stated: \emph{``you can just [edit] and draw to find out similar patterns. You\textquotesingle ll need to do a lot more through Matlab to do the same thing.''} Another experienced participant mentioned the benefits of not needing to know programming languages to accomplish these tasks: \emph{``The obvious good thing is that you can do complicated queries, and you don\textquotesingle t have to write SQL queries... I can imagine a non-cs student [doing] this.''} (P9). We include a sample code written by a participant in their favorite language; the participants accomplished the same task with 38 lines of python code compared to 4 lines of instructions in \zv. While simply considering the number of lines of code may not be a truly fair comparison, we argue that ZQL requiring roughly only one tenth of the python code demonstrates the value of \zv, and how it can complement existing database and data mining systems. \papertext{Example code can be found in~\cite{techreport}.} \techreport{Example code can be found in the appendix \ref{sec:userstudy-appendix}.}}

\paraem{Finding 3: \zv can be improved.}  
\papertext{Participants outlined some areas for improvement: some requested drag-and-drop interactions 
to support additional operations, such as outlier finding; others wanted a more polished interface;
and some desired bookmarking and search history capabilities.}
%Others commented on how the interface could be more polished, and suggested that we add bookmarking and search history capabilities.}
\techreport{
 While the participants looked forward to using custom query builder in their own workflow, a few of them were interested in directly exposing the commonly-used trends/patterns such as outliers, through the drag and drop interface. Some were interested in knowing how they could integrate custom functional primitives (we could not cover it in the tutorial due to time constraints). In order to improve the user experience, participants suggested adding instructions and guidance for new users as part of the interface. Participants also commented on the unrefined look and feel of the tool, as well as the lack of a diverse set of usability related features, such as bookmarking and search history, that are offered in existing systems.
}
}

%\papertext{Participants also outlined some areas for improvement; details can be found in~\cite{techreport}.
%In brief, the participants requested drag-and-drop interactions to support additional operations, such as outlier finding. Others commented on how the interface could be more polished, and suggested that we add bookmarking and search history capabilities.}
%\john{\techreport{
%While the participants looked forward to using \zv in their own workflow, \zv is not without limitations. The algorithm for finding similar trends and patterns is abstracted to the backend, and participants wanted to learn about the algorithm behind the blackbox. ``I don\textquotesingle t know how the function is working behind the process... Knowing how this works is important'' (P1). They further wished to program their own similarity metrics for their datasets. It is unlikely that a single similarity metric will fit all users needs, and users asked for customizable similarity metrics. Another limitation of \zv is the lack of general features as a visual analytics tool. Existing tools such as Excel or Tableau allows users to directly edit data and generate resulting visualizations or apply statistical methods onto the results. These features are not offered with \zv. In order to improve the user experience, participants also suggested adding instructions and guidance for new users as part of the interface. Participants also commented on the unrefined look and feel of the tool, as well as the lack of a diverse set of usability related features, such as bookmarking and search history, that are offered in existing systems.
%}}


%In order to assess how \zv can aid data analysts in their workflow, we first identified the various analytical tasks commonly performed by data analysts, then designed a user study focused on visual data exploration tasks and how \zv compares to existing tools in this domain. 

%\john{There are no tools that offer the same functionalities as \zv. Existing visual analytics tools do not offer the ability to directly search for specific patterns, or issue complex visual exploration queries. Conversely, the current implementation of \zv is not capable of performing all tasks necessary for data analysts.} to evaluate how \zv can improve the current workflow of data analysts in searching for visual trends and patterns.}

% Following the taxonomy of low level analytical tasks by Amar et al. [cite], we identified four types of visual data exploration tasks that can be streamlined by the features offered by \zv. The four type of tasks are - characterizing distribution, finding anomalies, clustering, and correlating attributes. 
% In order to evaluate how the features of \zv can aid data analyst in these four types of tasks, we conducted a mixed methods study comparing \zv with a baseline tool. In addition, through the user study, we anticipated to a) examine and compare the usability of the drag and drop interface and the custom query builder interface of \zv; b) identify if, when, and how people would use \zv in their workflow; and c) receive general feedback for future improvements.

%can help in visualizing interesting patterns, trends, or insights from large datasets.
%focus on how it helps visual data exploration, make clear of limitations

%\john{We focused our user study tasks on three of the ten low level analytical tasks (finding anomalies, clustering, and correlating attributes) which have no straightforward solutions \cite{lee2006task}. In addition, existing tools already provide well defined functions for the other seven tasks (retrieving value, filtering, computing derived value, finding extremum, sorting, determining range, characterizing distribution). All seven analysts answered that they actively looked for correlation and anomalies in their datasets, and four analysts answered that they cluster data during their exploration stage. Six analysts used visualizations for these three tasks, with the exception of one analyst who used python libraries and customized code for his analysis. These three low level analytical tasks were most relevant to the potential improvements \zv offered to data analysts over existing tools, and we did not expect the features of \zv to offer significant improvements for the remaining seven tasks. With this in mind, we brainstormed realistic tasks using examples from the case studies in Section~\ref{sec:intro} as reference and translated the case study tasks into tasks applicable to the real estate dataset. We prepared three sets of tasks for the three interfaces (baseline, drag and drop, and custom query builder interfaces). The tasks differed only in the selection attributes so that the performance of the interfaces could be measured objectively. Section ~\ref{sec:frontend} lists a few example queries that were used in the study.}

%\papertext{The detailed responses can be found in our technical report~\cite{techreport}.} 
%\techreport{
%Table \ref{tab:tasks} shows the response for commonly used low level analytical tasks.}
%\techreport{
%\begin{table}[H]
%\vspace{-10pt}
 %\centering\scriptsize
 % {\tt    
  %\begin{tabular}{|l|l|} \hline
    %  \textbf{Tasks} & \textbf{Count} \\ \hline
      %Retrieve value & 7  \\ \hline
      %Filter & 7 \\ \hline
      %Compute derived value & 7 \\ \hline
      %Find extreme & 6 \\ \hline
      %Determine range & 7 \\ \hline
      %Characterize distribution & 6 \\ \hline
      %Find anomalies & 7 \\ \hline
      %Cluster & 4 \\ \hline
      %Correlate & 7 \\ \hline
     %\end{tabular}
  %}
  %\vspace{-10pt}\caption{Commonly used low level analytical tasks}
  %\label{tab:tasks}
%\vspace{-10pt}\end{table}
%}





==> userstudy.tex <==
%!TEX root=zenvisageql.tex

\section{User Study}
\label{sec:userstudy}
We conducted a mixed methods study~\cite{creswell2007designing} 
in order to assess the efficacy of \zv. 
We wanted to: 
a) examine and compare the usability of the drag and drop 
interface and the custom query builder interface of \zv; 
b) compare the performance and usefulness of \zv 
with existing tools;
\papertext{and}
c) identify if, when, and how people would use \zv in their workflow\techreport{;
and d) receive general feedback for future improvements}.

\subsection{User Study Methodology}
\paragraph{Participants.} We recruited 12 graduate students 
as participants with varying degrees of expertise in data analytics. 
\papertext{Details of their prior experience can be found in our 
technical report~\cite{techreport}.}
\techreport{Table \ref{tab:toolsrep} depicts the participants' experience with different categories of tools.
\begin{table}[H]
\vspace{-10pt}
 \centering\scriptsize
  {\tt    
  \begin{tabular}{|l|l|} \hline
      \textbf{Tools} & \textbf{Count} \\ \hline
      Excel, Google spreadsheet, Google Charts  & 8 \\ \hline
      Tableau & 4 \\ \hline
      SQL, Databases & 6 \\ \hline
      Matlab,R,Python,Java & 8 \\ \hline
      Data mining tools such as weka, JNP & 2 \\ \hline
      Other tools like D3 & 2 \\ \hline
     \end{tabular}
  }
  \vspace{-10pt}\caption{Participants' prior experience with data analytic tools}
  \label{tab:toolsrep}
\vspace{-10pt}\end{table}
}

\paragraph{Dataset.} 
We used a housing dataset from Zillow.com~\cite{housing_data} consisting of
housing sales data for different cities, counties, and states from 2004--15,
with over 245K rows, and 15 attributes.
\papertext{Since looking for housing is commonplace, the participants could relate to the dataset and understand the
usefulness of the tasks.}
\techreport{
We selected this dataset for two
reasons: 
First, housing data is often explored by data analysts using existing
visualization tools~\cite{elmqvist2008datameadow}. Second, looking for housing
is commonplace for graduate students while in school and upon
graduation; the participants could relate to the dataset and understand the
usefulness of the tasks.
}
  
\paragraph{Comparison Points.} 
There are no tools that offer the same functionalities as
\zv. Visual analytics tools do not offer the ability
to search for specific patterns, or issue complex visual exploration queries; 
data mining toolkits do not offer the ability to search for visual patterns 
and are instead tailored for general machine learning and prediction. 
\papertext{We decided to implement our baseline tool by replicating
the basic visualization specification capabilities of tools like Tableau,
augmented with additional filtering capabilities. 
The styling scheme was similar to \zv to control for external factors;
details can be found in \cite{techreport}.}\techreport{Since visual analytics tools are closer in spirit and functionality 
to \zv, we decided to implement a visual analytics tool as our baseline.
Thus, our baseline tool replicated the basic query specification and output visualization
capabilities of existing tools such as Tableau.  
We augmented the baseline tool with the ability to specify an arbitrary number of filters, allowing
users to use filters to drill-down on specific visualizations.
This baseline visualization tool was implemented with a styling scheme similar to \zv to control for external factors. 
As depicted in Figure \ref{fig:baseline}, the baseline allowed users to visualize data by allowing them to specify the x-axis, y-axis, category, and filters. The baseline tool would populate all the visualizations, which fit the user specifications, using an alpha-numeric sort order.} In addition to task-based comparisons with this baseline, we
also explicitly asked participants to compare \zv with existing data mining and visual analytics 
tools that they use in their workflow.
 
\paragraph{Study Protocol.} The user study was 
conducted using a within-subjects study design~\cite{bordens2002research}. 
The study consisted of three phases. 
In the first phase, participants described 
their previous experience with data analytics and visualization tools. 
In the second phase, participants performed visual analytics 
tasks using each of the tools. 
\techreport{\zv was introduced as Tool A and the baseline tool was introduced as Tool B.}
This phase began with a 15-minute tutorial that included an overview of the interface and two practice questions. 
The order of the baseline tool and the \zv interface was randomized to reduce order effects.
To compare the effectiveness of the drag and drop interface 
and the custom query builder interface of \zv, 
participants performed two separate sets of tasks on \zv, one for each component. Finally, in the third phase, participants completed a survey that measured 
their satisfaction levels and preferences, followed by open-ended interview questions\techreport{ assessing the strengths and weaknesses 
of the tools, and whether they would use the two tools in their workflow}. 
\techreport{
The average study session lasted for 75 minutes on average. 
Participants were paid ten dollars per hour for their participation.}

\paragraph{Tasks.}
We prepared three sets of tasks for the three interfaces (baseline, drag and
drop, and custom query builder interfaces). The tasks differed only in the
selection attributes so that the performance of the interfaces could be
measured objectively (Section~\ref{sec:frontend} lists a few example queries
that were used in the study \papertext{; others can be found
in the techreport~\cite{techreport}}).
\techreport{We carefully selected tasks which can surface during a
search for a house.
}
To demonstrate the efficacy of \zv, the tasks focused on
identifying patterns, trends or anomalies in housing data; these are
non-trivial tasks to complete with a large dataset with existing tools. 
\techreport{The tasks were targeted to test the core features of \zv and solicit responses from participants on how \zv could complement existing data analytics workflows.}

%The tasks that the participants performed on the two tools were designed to be similar in nature (differing only in selection attributes) so that we could compare the performance more objectively. The tasks focused on identifying visualizations with specific insights. Section~\ref{sec:frontend} lists a few example queries that were used in the study. 

\paragraph{Metrics.} 
We manually recorded how participants used the tool and their answers for each task. We further collected browser activity using screen capture software, system interaction logs, audio of discussions, and asked the participants to complete a survey. 
\techreport{Using this data, we collected the following metrics: task completion time, task accuracy, the number of visualizations browsed for each task, the number of edits made on the drawing panel and the query table, and the usability ratings and satisfaction level from the survey results.}

\paragraph{Ground Truth.} 
Two expert data analysts prepared the ground truth for each the tasks in the form of ranked answers. Their inter-rater agreement, measured using Kendall\textquotesingle s Tau rank correlation coefficient, was 0.854. 
% The experts further discussed and resolved the conflicting answers to produce a final single ranked list of answers for each task. 
Then, each expert independently rated the answers on their ranked list on a 0 to 5 scale (5 highest). We took the average of the two scores to rate the participants\textquotesingle~answers.

\techreport{
\begin{figure}
\vspace{-5pt}
\begin{center}
\fbox{\includegraphics[width=0.6\columnwidth]{figs/baseline.png}}
\end{center}
\vspace{-20pt}
\caption{The baseline interface implemented for the user study.}
\label{fig:baseline}
\vspace{-10pt}
\end{figure}
}


\subsection{Key Findings}
Six key findings emerged from the study.  We describe them below.
We use $\mu$, $\sigma$, $\chi^2$ to denote average, standard deviation, and Chi-square test scores, respectively.

\paraem{Finding 1: \zv enabled over 50\% and 100\% faster task completion times than the baseline for the custom query builder and drag and drop interfaces, respectively.} 
%We timed the task completion time for all participants,
%and 
We found that the drag and drop interface
had the smallest, and most predictable completion time ($\mu=74s$, $\sigma=15.1$),
the custom query builder had a higher completion time and a higher variance ($\mu=115s$, $\sigma=51.6$),
while the baseline had a significantly higher completion time ($\mu=172.5s$, $\sigma=50.5$), more than twice the completion time of the drag and drop interface,
and almost 50\% higher than the custom query builder interface.
This is not surprising, given that the baseline tool requires more
manual exploration compared to the other two interfaces.
%We tested for statistical significance on the difference between the three interfaces 
Using 
a one-way between-subjects ANOVA,
followed by a post-hoc Tukey's test~\cite{tukey1949comparing},
we found that the
drag and drop interface and the custom query builder interface
had statistically significant
faster task completion times compared to the baseline interface,
with $p$ values of 0.0010 and 0.0069, respectively.
The difference between the drag and drop interface
and the custom query builder interface was not statistically significant,
with a $p$ value of $0.06$.
\papertext{Detailed statistics can be found in ~\cite{techreport}.}


% One-way between subject ANOVA~\cite{tukey1949comparing} on the completion time of the tasks revealed that the differences between the three interfaces were significant F(2, 33) = 16.02, p < 0.001. On further applying the post hoc Tukey's test\cite{tukey1949comparing} for comparing the pairwise task completion times among the three interfaces (Table \ref{tab:turkeytest}), we found that both the drag and drop interface and the custom query builder had significantly faster task completion times compared to the baseline tool (p < 0.01), whereas the difference between the drag and drop interface, and the custom query builder was not significantly different.  
\techreport{
\begin{table}[H]
 \centering \scriptsize
  {\tt    
  \scalebox{0.75}{
  \begin{tabular}{|l|l|l|l|} \hline
      \textbf{Treatments} & \textbf{Q statistic} & \textbf{p-value} & \textbf{inference} \\ \hline
	Drag and drop interface vs. Custom query builder & 3.3463 & 0.0605331 & insignificant \\ \hline
	Drag and drop interface vs. Baseline tool & 7.9701 & 0.0010053 & significant (p<0.01) \\ \hline
	Custom query builder vs. Baseline tool & 4.6238 & 0.0069276 & significant (p<0.01) \\ \hline    
     \end{tabular}
  }
  }
\vspace{-10pt}
\caption{Tukey's test on task completion time}
\label{tab:turkeytest}
\vspace{-10pt}
\end{table}
}

\begin{figure}
\begin{center}
\includegraphics[width=0.6\columnwidth]{figs/accuracyvstime.pdf}
\end{center}
\vspace{-25pt}
\caption{Accuracy over time results for zenvisage and baseline}
\label{fig:accuracyvstime}
\vspace{-20pt}
\end{figure}


\paraem{Finding 2: \zv helped retrieve 20\% and 35\% more accurate results than the baseline for drag and drop and custom query builder interfaces, respectively.} 
Comparing the participants' responses against the ground truth responses, 
we found that participants achieved the lowest accuracy with the baseline tool ($\mu=69.9\%$, $\sigma=13.3$). 
\techreport{Further, any tasks that required comparing multiple
pairs of visualizations or trends ended up having lower accuracy than those that looked
for a pattern, such as a peak or an increasing trend, in a single visualization.}
The low accuracy could be attributed to the fact that the participants selected suboptimal answers before browsing through the entire list of results for better answers. Conversely, \zv is able to
accept more fine-grained user input, and
rank output visualizations. With \zv,
participants were able to retrieve accurate answers
with less effort.
Between the two interfaces in \zv,
while the drag and drop interface had a faster task completion time,
it also had a lower accuracy ($\mu=85.3\%$, $\sigma=7.61$).
The custom query builder interface had the
highest accuracy ($\mu=96.3\%$, $\sigma=5.82$).
The accuracy was greater than the baseline by over 20\% (for drag and drop)
and over 35\% (for custom builder).
Finally, looking at both accuracy and task completion times together in Figure~\ref{fig:accuracyvstime}, we see that \zv \emph{helps in ``fast-forwarding to desired visualizations'' with high accuracy.} 

% In the baseline, comparing multiple pairs of visualizations or trends revealed to be more difficult than looking for a visual property, such as a peak, or an increasing pattern, in a single visualization. on the other hand, since \zv returns a ranked list of filtered answers based on the user specification, which allowed the participants to browse through a smaller number of visualizations compared to the baseline tool. Among the two interfaces in \zv, participants completed the tasks faster ($\mu=74s$, $\sigma=15.1$) on the drag and drop interface, but at the price of accuracy ($\mu=85.3\%$, $\sigma=7.61$). Participants using the custom query builder had the highest accuracy ($\mu=96.3\%$, $\sigma=5.82$) while maintaining comparable speeds to the drag and drop interface ($\mu=115s$, $\sigma=51.6$). Finally, looking at both accuracy and task completion times together (as depicted in Figure~\ref{fig:accuracyvstime}), we can conclude that \zv \textbf{helps in fast-forwarding to desired visualizations with a high accuracy.}

% Figure \ref{fig:accuracyvstime} depicts the average accuracy over time results of each of the participants on each of the interfaces. \agp{move this later.} 

%\textbf{\zv helps retrieve accurate results}: We rated the participant's answers based on the expert's gold set answers. The ratings revealed that participants performed poorly with the baseline, with the lowest accuracy ($\mu=69.9\%$, $\sigma=13.3$) and longest task completion time. In the baseline, comparing multiple pairs of trends or graphs revealed to be more difficult than looking for a single trend such as a peak, or an increasing pattern. \zv, on other hand, returns a ranked list of results based on the user specification, which allowed the participants to browse through a smaller number of visualizations compared to the baseline tool. Among the two interfaces in \zv, participants completed the tasks fastest ($\mu=74s$, $\sigma=15.1$) on the drag and drop interface, but at the price of accuracy ($\mu=85.3\%$, $\sigma=7.61$). Participants using the custom query builder had the highest accuracy ($\mu=96.3\%$, $\sigma=5.82$) while maintaining comparable speeds to the drag and drop interface ($\mu=115s$, $\sigma=51.6$). \textbf{\zv, thus, helps in fast-forwarding to desired visualizations with a high accuracy}.


\paraem{Finding 3: The drag and drop interface and the custom query builder complemented each other.
The drag and drop interface was intuitive, while the custom builder was useful for complex queries.} 
The majority of participants (8/12) 
mentioned that the drag and drop 
and custom query builder interfaces complemented each other \techreport{in making \zv powerful}
when searching for specific insights.\techreport{ 25 percent (3/12) of the participants (all with backgrounds in machine learning and data mining) 
preferred using only the custom query builder interface, while just one participant (with no prior experience with query languages or programming languages) found only the drag and drop interface as useful.}
Participants stated that they would use drag and drop for exploration and simple pattern search and custom query builder for specific / complex queries. One stated: \textit{``When I know what I am looking for is exact, I want to use the query table. The other one [drag and drop] is for exploration when you are not so sure.'' (P9).} 
Participants liked the simplicity and intuitiveness of the drag and drop interface. 
One stated: \textit{``[The drawing feature] is very easy and intuitive, I can draw... and automatically get the results.''} (P2).
On a five-point Likert (5 is strongly agree), participants
found the drawing feature easy to use ($\mu=4.45$, $\sigma=0.674$). 
Despite the positive feedback, participants did identify limitations,
specifically, that the functionality was restricted to identifying trends
similar to a single hand-drawn trend.

The majority of the participants (11/12) 
stated that the custom query builder 
allowed them to search for complex insights that might be 
difficult to answer via drag and drop. 
When asked if the custom query builder was difficult to use compared to
the drag-and-drop interface, participants tended to agree ($\mu=3.73$, $\sigma=0.866$ on a five-point Likert scale where five is strongly agree).
At the same time, participants acknowledged 
the flexibility and the efficacy supported by the custom query builder interface. 
One participant explicitly stated why they 
preferred the custom query builder over the drag and drop interface: 
\textit{``When the query is very complicated, [the drag and drop] has its limitations, 
so I think I will use the query table most of the times unless I want to get a brief impression.''} (P6).
Another participant stated that the custom query builder interface \textit{``has more functionality and it lets me express what I want to do clearly more than the sketch''} (P4). This was consistent with other responses. 
Participants with a background in machine learning, 
data mining, and statistics (3/12) preferred
using the custom query builder over the drag and drop interface.

\paraem{Finding 4: \zv was more effective (4.27 vs. 2.67 on a five-point Likert scale)
than the baseline tool at visual data exploration, and would be
a valuable addition to the participants' analytics workflow.} 
In response to the survey question \emph{``I found the tool to be effective in visualizing the data I want to see''}, the participants rated \zv (the drag and drop interface and the custom query builder interface) higher ($\mu=4.27$, $\sigma=0.452$) than the baseline tool ($\mu=2.67$, $\sigma=0.890$) on a five-point Likert scale.
A participant experienced in Tableau commented: \textit{``In Tableau, there is no pattern searching. If I 
see some pattern in Tableau, such as a decreasing pattern, and I want to see if any other variable is 
decreasing in that month, I have to go one by one to find this trend. But here I can find this through the query table.''} (P10).

\paraem{Finding 5: \zv is a valuable addition to the participants' analytics workflow, and allows a quicker initial data exploration before performing complex analysis:}
When asked about using the two tools in their current workflow, 9 of the 12 participants stated that they would use \zv in their workflow, whereas two participants stated that they would use our baseline tool ($\chi^2=8.22$, p<0.01). When the participants were asked how they would use \zv in their workflow, one participant provided a specific scenario: \textit{``If I am doing my social science study, and I want to see some specific behavior among users, then I can use tool A [\zv] since I can find the trend I am looking for and easily see what users fit into the pattern.''} (P7). Other participants mentioned that they would use this tool for finding outliers during data cleaning, common patterns search, and initial understanding of data distributions before running a machine learning task. 
Participants could not articulate specific reasons for using the baseline tool. As one participant put it, \textit{``the existing solutions can already do what tool B [the baseline interface] can do.''} (P10).
Even those with considerable experience with programming languages such as Python and Matlab 
argued that \zv would take less time and fewer lines of code for basic data exploration tasks. 
Participants (2/12) who had considerable experience with data mining libraries were asked a follow-up 
question to write code for a task similar to Table 11 in their favorite language;
this task took them multiple orders of magnitudes more time and lines of code compared to \zq. 
\papertext{Example code can be found in~\cite{techreport}.} \techreport{Example code can be found in the appendix \ref{sec:userstudy-appendix}.} 



% \textbf{\zv is novel with real world applications}: All the participants described \zv as a novel tool and mentioned that they have not seen the declarative pattern searching functionality in any other tool.

\paraem{Finding 6: \zv can be improved.}  
\papertext{Participants also outlined some areas for improvement; details can be found in~\cite{techreport}.
In brief, the participants requested drag-and-drop interactions to support additional operations, such as outlier finding.
Others commented on how the interface could be more polished, and suggested that we add bookmarking and search history capabilities.}
\techreport{
 While the participants looked forward to using custom query builder in their own workflow, a few of them were interested in directly exposing the commonly-used trends/patterns such as outliers, through the drag and drop interface. Some were interested in knowing how they could integrate custom functional primitives (we could not cover it in the tutorial due to time constraints). In order to improve the user experience, participants suggested adding instructions and guidance for new users as part of the interface. Participants also commented on the unrefined look and feel of the tool, as well as the lack of a diverse set of usability related features, such as bookmarking and search history, that are offered in existing systems.
}




